Stable Autoregressive Speech Generation with Low-Frame-Rate High-Dimensional Continuous Tokens

Balancing sequence length, representational capacity, and long-horizon stability is a central problem in autoregressive (AR) speech and audio generation. Representations with higher frame rates or greater capacity can preserve more signal detail, but they also make streaming generation more vulnerable to distribution drift and AR error accumulation. Conversely, shorter and more compressed representations simplify AR modeling, but their limited bandwidth may discard important components and constrain the upper bound of reconstruction fidelity and generation quality. We ask whether a low-frame-rate, high-dimensional, high-bandwidth continuous representation can be co-designed with a streaming generation framework to support robust high-fidelity reconstruction, strong single-token predictability, and superior long-horizon stability. We decompose this goal into two coupled problems: what geometric and statistical properties a high-dimensional representation space should have, and how an AR continuous-token generator should be structured to resist error accumulation. Accordingly, we propose Locodec, a locally encoded codec that shapes its representation space to improve the interpolatability of a lower-dimensional core manifold and the identifiability of the native high-dimensional coordinates, thereby improving the predictability of high-dimensional high-bandwidth tokens. We also propose MP-ELD, a single-token AR flow-matching framework that uses multi-path information routing and residual classifier-free guidance to mitigate error accumulation. Experiments with 8-Hz, 768-dimensional tokens show that our design preserves reconstruction quality, improves single-token predictability, achieves competitive WER, and maintains stable long-form synthesis, without using external SSL/ASR models, pretrained text language models, or post-training stages.

==> sections_old/DRF.tex <==
\section{High-Dimensional Direction-only Rectified Flow}
\label{sec:DRF}

We now revisit a flow matching bridge from a different perspective: in high-dimensional token spaces, the bridge state $x_t$ is not only a point along a transport path, but also a carrier of \emph{progress-identifiability} cues that the model can exploit when predicting the flow. Under high-dimensional concentration, such cues---most notably shell-related statistics such as $\|x_t\|_2$ and source--target mixture ratios---become sharply regular functions of $t$ under the training bridge, and therefore provide strong shortcuts for inferring \emph{where the current state lies on the bridge} and \emph{how much target information it already contains}. This is useful during training, but it also creates a failure mode at inference: if the learned sampler causes these state statistics to deviate from their training-time schedule, then the model is queried on states whose \emph{identifiability proxies} no longer match the nominal progress $t$, leading to train--test mismatch and stronger exposure bias. Standard velocity-prediction-based rectified flow is particularly vulnerable to this issue, because directional errors in the predicted velocity induce systematic step-size shrinkage, which in turn distorts the radius-related statistics of intermediate states. Moreover, most practical flow models also take a time embedding as an auxiliary input, making bridge progress jointly identifiable from both the explicit time signal and the implicit state statistics. These two sources are perfectly aligned during training, but can become inconsistent at inference once the trajectory drifts away from the training bridge, potentially creating conflicting progress cues for the model. This observation suggests a different design principle: rather than asking the model to implicitly handle both the bridge-specific identifiability statistics and the residual geometric information needed for transport, we should let the model learn only the part that is not already determined by the bridge schedule---namely, the \emph{direction field}---and explicitly restore the identifiable state statistics at inference to match their training-time reference values. Based on this view, we propose \textbf{direction-only rectified flow (DRF)}, which removes time embedding, treats $\|x_t\|_2$ as the unique source of bridge progress identifiability, and enforces a reference radius schedule during sampling so that training and inference remain aligned in the high-dimensional regime.

\subsection{State Statistics as Progress-Identifiability Proxies}
\label{subsec:ref_identifiability}

We begin by formalizing the notion of \emph{progress-identifiability}. In a flow bridge, progress-identifiability refers to how strongly the current state $x_t$ reveals the bridge progress that is relevant for prediction. In high dimensions, this progress is typically not inferred from fine-grained sample-specific details, but from coarse state statistics that become sharply concentrated under the training bridge. We refer to such statistics as \emph{progress-identifiability proxies}. For the standard rectified-flow (RF) bridge
\begin{equation}
x_t=(1-t)x_0+tx_1,\qquad t\in[0,1],
\label{eq:bridge_RF}
\end{equation}
two proxies are especially natural:
\begin{itemize}
    \item \textbf{Bridge-location proxy.} This proxy indicates \emph{where the current state lies on the bridge}. Since shell-like high-dimensional distributions are most naturally organized by radius, we use the expected radius
    \begin{equation}
    \rho(t)
    \;\triangleq\;
    \sqrt{\mathbb E\big[\|x_t\|_2^2\big]}
    \label{eq:rho_def_full}
    \end{equation}
    as the corresponding reference schedule. Here $\rho(t)$ is a \emph{statistical} bridge-location schedule rather than a sample-wise exact identity.

    \item \textbf{Source--target balance proxy.} This proxy indicates \emph{how much target information the current state already contains relative to the source}. A natural quantity is the source--target signal-to-noise ratio (SNR). Since the source contribution is itself random, we define its \emph{mean} schedule by
    \begin{equation}
    \overline{\mathrm{SNR}}(t)
    \;\triangleq\;
    \mathbb E\!\left[
    \log
    \frac{t^2\|x_1\|_2^2}{(1-t)^2\|x_0\|_2^2}
    \right].
    \label{eq:snr_mean_def_full}
    \end{equation}
    This quantity measures, on average, how target-dominant the bridge state is at time $t$.
\end{itemize}

These proxies are especially important in high dimensions because they become highly regular under concentration. Expanding the bridge norm gives
\begin{equation}
\|x_t\|_2^2
=
(1-t)^2\|x_0\|_2^2+t^2\|x_1\|_2^2+2(1-t)t\langle x_0,x_1\rangle.
\label{eq:norm_expand_full}
\end{equation}
When $x_0$ and $x_1$ are sampled independently from concentrated high-dimensional distributions with bounded norms, the cross term is negligible relative to the shell energies, so
\begin{equation}
\|x_t\|_2^2
\approx
(1-t)^2\|x_0\|_2^2+t^2\|x_1\|_2^2.
\label{eq:norm_concentrated_full}
\end{equation}
If in addition both endpoint norms are sharply concentrated, and without loss of generality we assume
\begin{equation}
\mathbb E[\|x_0\|_2^2]=\mathbb E[\|x_1\|_2^2]=N,
\end{equation}
then the bridge-location proxy becomes
\begin{equation}
\rho(t)^2
=
\mathbb E[\|x_t\|_2^2]
\approx
(1-t)^2\mathbb E[\|x_0\|_2^2]+t^2\mathbb E[\|x_1\|_2^2]
=
N\big((1-t)^2+t^2\big).
\label{eq:rho_mean_full_general}
\end{equation}
Likewise, the source--target balance proxy becomes
\begin{equation}
\overline{\mathrm{SNR}}(t)
\approx
\log\frac{t^2\mathbb E[\|x_1\|_2^2]}{(1-t)^2\,\mathbb E[\|x_0\|_2^2]}
=
2\log\frac{t}{1-t}.
\label{eq:snr_mean_concentrated_full_general}
\end{equation}

Therefore, under a high-dimensional RF bridge, the main progress-identifiability proxies become sharply regular functions of time. This has two consequences. On the one hand, such regularity makes them easy for the model to exploit: bridge progress and source--target balance can often be inferred from simple state statistics rather than from the full fine-grained geometry of $x_t$. On the other hand, this also makes them a potential source of train--test mismatch: once inference trajectories deviate from the training bridge, these same proxies may no longer agree with the nominal time index $t$, and the model may be queried on states whose apparent bridge progress is internally inconsistent.

\subsection{Under-stepping in $v$-Prediction Loss: Step-Size Underestimation under Angular Errors}
\label{subsec:rf_vpred}

The analysis above suggests that, in high dimensions, reliable flow inference should preserve the progress-identifiability proxies induced by the training bridge. We next show that standard velocity-prediction-based rectified flow has a systematic tendency to do the opposite: even when the predicted direction is only slightly mismatched with the oracle transport direction, the commonly used $\ell_2$ regression objective already favors a \emph{smaller-than-intended} velocity magnitude. As iterative inference accumulates such shrinkage over multiple steps, the resulting trajectory can deviate from the training bridge in exactly the state statistics that the model is most likely to rely on.

Standard RF trains a network $\hat v(x_t,t,c)$ by regressing the oracle velocity
\begin{equation}
v^\star = x_1 - x_0
\end{equation}
with an $\ell_2$ loss. To isolate the geometry of this objective, decompose the prediction into a unit direction and a nonnegative magnitude:
\begin{equation}
\hat v \;=\; \hat s\,\hat r,
\qquad
\hat r\in\mathbb{S}^{N-1}(1),\ \hat s\ge 0,
\end{equation}
and similarly write the oracle transport as
\begin{equation}
v^\star \;=\; s^\star r^\star,
\qquad
r^\star=\mathrm{Norm}_1(v^\star)\in\mathbb{S}^{N-1}(1),\ 
s^\star=\|v^\star\|_2.
\end{equation}
Let $\theta=\angle(\hat r,r^\star)$ denote the angular mismatch between the predicted and oracle directions, so that
\begin{equation}
\langle \hat r,r^\star\rangle=\cos\theta.
\end{equation}
Conditioned on a fixed predicted direction $\hat r$, the $\ell_2$ regression objective becomes
\begin{align}
\|\hat v - v^\star\|_2^2
&=\|\hat s\hat r - s^\star r^\star\|_2^2 \nonumber\\
&=\hat s^2 + (s^\star)^2 - 2\hat s s^\star \langle \hat r,r^\star\rangle \nonumber\\
&=\hat s^2 + (s^\star)^2 - 2\hat s s^\star \cos\theta.
\label{eq:vpred_quadratic}
\end{align}
This is a convex quadratic in $\hat s$, whose minimizer is
\begin{equation}
\hat s_{\mathrm{opt}} \;=\; s^\star \cos\theta.
\label{eq:vpred_shrinkage}
\end{equation}
Therefore, whenever the predicted direction is not perfectly aligned with the oracle direction, the optimal predicted magnitude is multiplicatively shrunk by $\cos\theta$. Equivalently, the component of the optimal prediction along the oracle transport direction is
\begin{equation}
\langle \hat v, r^\star\rangle
=
\hat s_{\mathrm{opt}}\langle \hat r,r^\star\rangle
=
s^\star \cos^2\theta,
\end{equation}
which is strictly smaller than the intended transport magnitude unless $\theta=0$.

This geometric shrinkage directly translates into \emph{under-stepping} during iterative inference: each update moves less than intended along the bridge, and the accumulated effect biases the trajectory toward states with systematically distorted bridge statistics. In our setting, the most important distortion is radial. Since the bridge-location proxy in high dimensions is strongly tied to $\|x_t\|_2$, under-stepping makes the realized state norm lag behind the nominal bridge progress specified by $t$. As a result, the model is evaluated on states whose radius suggests one stage of the bridge while the explicit time input suggests another. This creates a particularly undesirable form of exposure bias: the model is no longer asked to extrapolate only from slightly imperfect states, but from states whose most salient progress-identifiability cues have become internally inconsistent.

This issue is especially consequential in high-dimensional token spaces. As discussed in Sec.~\ref{sec:analysis_thin_shell}, both standard VAE-style latents and our spherical tokens are concentrated near a thin shell or a fixed-radius hypersphere. The tokenizer decoder is therefore trained primarily on on-shell states and can be brittle to off-shell inputs. Under-stepping pushes inference trajectories toward exactly such atypical regions. Consequently, the resulting error is amplified twice: first in the generative model, through the mismatch of progress-identifiability proxies, and then in the tokenizer decoder, through off-shell decoding.

\subsection{A Direction-only Variant of Rectified Flow}
\label{subsec:DRF}

The analysis above suggests a simple principle: in high-dimensional flow matching, the model should not be asked to regress bridge-specific statistics whose typical values are already determined by the bridge schedule and can be restored explicitly at inference. Instead, the model should learn only the residual information that is not specified by those statistics, namely, the \emph{transport direction}. Based on this view, we propose \textbf{direction-only rectified flow (DRF)}. Instead of predicting the full velocity vector $x_1-x_0$, DRF predicts only the \emph{unit transport ray}
\begin{equation}
r^\star = \mathrm{Norm}_1(x_1-x_0)\in\mathbb{S}^{N-1}(1),
\end{equation}
and is trained with the cosine loss
\begin{equation}
L_{\mathrm{DRF}}
=
1-\cos\big(\hat r(x_t,c),\,r^\star\big),
\end{equation}
where $\hat r(x_t,c)$ denotes the predicted direction field. We further sample the source $x_0$ on the same hypersphere as the spherical tokenizer target $x_1$, i.e.,
\begin{equation}
\|x_0\|_2=\|x_1\|_2=\sqrt{N},
\end{equation}
so that the bridge-location proxy is governed exactly by shell geometry rather than by a Gaussian thin-shell approximation.

At inference, we use a time schedule $0=t_0<t_1<\cdots<t_K=1$ as a \emph{reference index} for the bridge statistics, but do not ask the model to predict a velocity magnitude. Instead, we query the direction predictor at $t_k$
\begin{equation}
\hat r_{t_k}=\hat r(x_{t_k},c)\in\mathbb{S}^{N-1}(1),
\end{equation}
and update the state by
\begin{equation}
x_{t_{k+1}} = x_{t_k} + \Delta_{t_k}\,\hat r_{t_k},
\label{eq:DRF_update}
\end{equation}
where the scalar step size $\Delta_{t_k}$ is chosen so that the next state matches the reference bridge-location schedule:
\begin{equation}
\|x_{t_{k+1}}\|_2 = \rho(t_{k+1}).
\label{eq:radius_lock}
\end{equation}
In this way, the model is responsible only for the transport direction, while the coarse bridge-location statistics are explicitly aligned with their training-time reference values throughout sampling.

Substituting Eq.~\eqref{eq:DRF_update} into Eq.~\eqref{eq:radius_lock} yields
\begin{align}
\|x_{t_k}+\Delta_{t_k}\hat r_{t_k}\|_2^2
&=\|x_{t_k}\|_2^2+\Delta_{t_k}^2+2\Delta_{t_k}\langle x_{t_k},\hat r_{t_k}\rangle \nonumber\\
&=\rho(t_{k+1})^2,
\end{align}
that is,
\begin{equation}
\Delta_{t_k}^2 + 2\langle x_{t_k},\hat r_{t_k}\rangle\,\Delta_{t_k}
+ \big(\|x_{t_k}\|_2^2-\rho(t_{k+1})^2\big)=0.
\label{eq:delta_quadratic}
\end{equation}
Let
\begin{equation}
c_k=\langle x_{t_k},\hat r_{t_k}\rangle,
\qquad
\Delta\rho_k^2 = \rho(t_{k+1})^2-\rho(t_k)^2.
\end{equation}
Under radius-locking, $\|x_{t_k}\|_2=\rho(t_k)$, so the two roots are
\begin{equation}
\Delta_{t_k} = -c_k \pm \sqrt{c_k^2+\Delta\rho_k^2}.
\label{eq:DRF_two_roots}
\end{equation}

For the standard RF bridge with shell-matched endpoints, the reference radius schedule
\begin{equation}
\rho(t)^2 = N\big((1-t)^2+t^2\big)
\end{equation}
is non-monotone and reaches its minimum at $t=0.5$. We therefore distinguish two phases:
\begin{itemize}
    \item \textbf{Expansion phase} ($t\in(0.5,1]$): here $\Delta\rho_k^2>0$, and the valid radius-locking solution is
    \begin{equation}
    \Delta_{t_k} = -c_k + \sqrt{c_k^2+\Delta\rho_k^2}.
    \end{equation}
    This is the unique forward step along the predicted ray that lands on the target-radius hypersphere.

    \item \textbf{Contraction phase} ($t\in[0,0.5]$): here $\Delta\rho_k^2<0$, and the quadratic may have no real solution when the predicted ray does not intersect the smaller target-radius hypersphere. When $c_k^2+\Delta\rho_k^2>0$
    In this case, exact ray-based radius locking is geometrically impossible, and we use an Euler-style step along the predicted direction using the typical RF transport magnitude under shell-matched high-dimensional endpoints,
    \begin{equation}
    \bar x_{t_{k+1}}
    =
    x_{t_k}
    +
    \sqrt{2N}(t_{k+1}-t_k)\,\hat r_{t_k},
    \end{equation}
    where $\sqrt{2N}$ is motivated by the high-dimensional approximation
    \begin{equation}
    \|x_1-x_0\|_2
    \approx
    \sqrt{\|x_0\|_2^2+\|x_1\|_2^2}
    =
    \sqrt{2N}.
    \end{equation}
    We then retract the intermediate state back to the reference shell:
    \begin{equation}
    x_{t_{k+1}} = \mathrm{Norm}_{\rho(t_{k+1})}(\bar x_{t_{k+1}}).
    \end{equation}
\end{itemize}

\subsection{The Role of Time Embedding: Anti-ambiguity or Identifiability Shortcut?}
\label{subsec:time_emb_role}

Many continuous generative models provide the network with an explicit time embedding or an equivalent step-dependent signalm and here we ask what functional role such a signal may play in bridge learning. Our working hypothesis is that time embedding serves as a readily usable \emph{progress-identifiability cue}: it provides direct information about the nominal bridge progress, and may therefore help the model infer both bridge location and the source--target balance typically associated with that progress. This role is most natural in lower-dimensional bridges, where coarse state statistics can remain ambiguous across time. In such a regime, different values of $t$ may induce overlapping norms or similar source--target balance, so an explicit time signal can help reduce \emph{cross-time ambiguity}. To quantify this effect, we analyze how much ambiguity remains in the bridge state statistics under the standard RF bridge
\begin{equation}
x_t=(1-t)x_0+tx_1,\qquad x_0\sim\mathcal N(0,I_N),
\label{eq:rf_bridge_gaussian_source}
\end{equation}
while taking $x_1$ to be a spherical target token from our tokenizer, so that $\|x_1\|_2^2=N$ is fixed. We consider two coarse progress-identifiability proxies: bridge location as measured by $\|x_t\|_2$, and source--target balance as measured by an energy-based SNR.

\paragraph{\textbf{Location ambiguity.}}
Under \eqref{eq:rf_bridge_gaussian_source},
\begin{equation}
x_t \sim \mathcal N(tx_1,\,(1-t)^2I_N),
\end{equation}
so the squared norm $Y_t=\|x_t\|_2^2$ follows a noncentral chi-square law. Its mean and variance are
\begin{align}
\mathbb E[Y_t]
&=
\|tx_1\|_2^2 + N(1-t)^2
=
t^2\|x_1\|_2^2 + N(1-t)^2
\nonumber\\
&=
N\big((1-t)^2+t^2\big),
\label{eq:location_mean}
\\
\mathrm{Var}(Y_t)
&=
2N(1-t)^4 + 4(1-t)^2\|tx_1\|_2^2
\nonumber\\
&=
2N(1-t)^4 + 4N(1-t)^2t^2.
\label{eq:location_var}
\end{align}
Thus, while the nominal bridge-location schedule follows the familiar symmetric radius curve, the realized bridge location still has nonzero spread at each fixed $t$. In low dimensions, this spread can make the distributions of $\|x_t\|_2^2$ overlap across different time points, so radius alone does not uniquely identify bridge location.

\paragraph{\textbf{SNR ambiguity.}}
To quantify source--target balance, define the random energy-based SNR
\begin{equation}
\mathrm{SNR}_t
\;\triangleq\;
\log\frac{t^2\|x_1\|_2^2}{(1-t)^2\|x_0\|_2^2}.
\label{eq:snr_random}
\end{equation}
Since $\|x_1\|_2^2=N$ is fixed and $\|x_0\|_2^2\sim\chi^2_N$,
\begin{equation}
\mathrm{SNR}_t
=
2\log\frac{t}{1-t} + \log N - \log\|x_0\|_2^2.
\label{eq:snr_expand}
\end{equation}
Let $U\sim\chi^2_N$. Since
\begin{equation}
U\sim\mathrm{Gamma}\!\left(\frac{N}{2},2\right),
\end{equation}
its logarithmic moments satisfy
\begin{equation}
\mathbb E[\log U]
=
\psi\!\left(\frac{N}{2}\right)+\log 2,
\qquad
\mathrm{Var}(\log U)
=
\psi_1\!\left(\frac{N}{2}\right),
\end{equation}
where $\psi$ and $\psi_1$ are the digamma and trigamma functions. Applying this to \eqref{eq:snr_expand} gives
\begin{align}
\mathbb E[\mathrm{SNR}_t]
&=
2\log\frac{t}{1-t}
+
\log N
-
\psi\!\left(\frac{N}{2}\right)-\log 2,
\label{eq:snr_mean_exact}
\\
\mathrm{Var}(\mathrm{SNR}_t)
&=
\psi_1\!\left(\frac{N}{2}\right).
\label{eq:snr_var_exact}
\end{align}
Using the standard asymptotics
\begin{equation}
\psi\!\left(\frac{N}{2}\right)
=
\log\frac{N}{2}-\frac{1}{N}+O(N^{-2}),
\qquad
\psi_1\!\left(\frac{N}{2}\right)
=
\frac{2}{N}+O(N^{-2}),
\end{equation}
we obtain
\begin{align}
\mathbb E[\mathrm{SNR}_t]
&=
2\log\frac{t}{1-t}+O(N^{-1}),
\label{eq:snr_mean_asymp}
\\
\mathrm{Std}(\mathrm{SNR}_t)
&=
\sqrt{\psi_1(N/2)}
=
\sqrt{\frac{2}{N}}+O(N^{-3/2}).
\label{eq:snr_std_asymp}
\end{align}
Thus, even at a fixed nominal time $t$, the realized source--target balance still has nonzero spread, although this spread shrinks as dimension grows.

To express this spread on the time axis, let
\begin{equation}
g(t)=2\log\frac{t}{1-t}
\end{equation}
denote the mean SNR schedule. Its derivative is
\begin{equation}
g'(t)=\frac{2}{t(1-t)}.
\label{eq:snr_schedule_derivative}
\end{equation}
A first-order conversion of SNR fluctuation into an effective time ambiguity gives
\begin{equation}
\delta_N^{\mathrm{snr}}(t)
\;\approx\;
\frac{\mathrm{Std}(\mathrm{SNR}_t)}{|g'(t)|}
=
\frac{t(1-t)}{2}\sqrt{\psi_1\!\left(\frac{N}{2}\right)}
\;\approx\;
\frac{t(1-t)}{\sqrt{2N}}.
\label{eq:snr_time_ambiguity}
\end{equation}
In low dimensions, this local interval can remain non-negligible, meaning that the same nominal $t$ still corresponds to a range of realized source--target balances. Therefore, even when time embedding is provided, it does not uniquely determine the actual SNR carried by an individual bridge state; low-dimensional bridges retain substantial \emph{within-time ambiguity}.

The picture changes qualitatively in the high-dimensional regime. As $N$ grows, the ambiguities above shrink rapidly: the relative spread of $\|x_t\|_2^2$ vanishes under Eq.~\eqref{eq:location_var}, and Eq.~\eqref{eq:snr_std_asymp} shows that the SNR fluctuation at fixed $t$ decreases as $O(N^{-1/2})$. Consequently, the bridge state statistics become sharply concentrated around their nominal schedules, so an explicit time embedding can make bridge progress and source--target regime almost directly recoverable from the nominal time label. A natural question is: what happens if explicit time conditioning is removed in this regime? In this case, the most easy-to-obtain identifiability proxy is the state norm $\|x_t\|_2$. However, under the RF bridge, the radius schedule $\rho(t)$ remains non-monotone,
\begin{equation}
\rho(t)=\rho(1-t),
\end{equation}
so the state norm alone cannot distinguish the two sides of the bridge. Removing time embedding therefore reintroduces a residual \emph{symmetric ambiguity}: from radius alone, a state may be compatible with both $t$ and $1-t$. While this weakens direct progress identifiability, it may also discourage the model from relying too heavily on easy progress proxies and instead encourage it to use the internal structure of $x_t$. This issue is especially important near the bridge center, i.e., around $t=0.5$, where the mean SNR is zero and source and target information are maximally mixed. In this regime, a small misestimation of source--target balance can directly affect which components are treated as already target-like and which are still treated as source-dominated. At the same time, this is precisely where the symmetric ambiguity induced by removing time embedding is most meaningful. In lower dimensions, the bridge center already has a substantial intrinsic ambiguity: Eq.~\eqref{eq:snr_time_ambiguity} shows that even the nominally central state corresponds to a non-negligible local interval of realized SNRs. In the high-dimensional setting without time embedding, the ambiguity takes a different form---a symmetric $t$ versus $1-t$ ambiguity induced by the non-monotone radius schedule---but near the bridge center the two become closely related. If $t=0.5+\epsilon$ with small $\epsilon$, then its symmetric counterpart $1-t=0.5-\epsilon$ lies in the same central neighborhood. Since
\begin{equation}
g(0.5)=0,
\qquad
g'(0.5)=\frac{2}{0.5(1-0.5)}=8,
\end{equation}
the first-order Taylor expansion of $g(t)=2\log\frac{t}{1-t}$ around $t=0.5$ yields
\begin{equation}
g(0.5+\epsilon)=8\epsilon+O(\epsilon^2),
\qquad
g(0.5-\epsilon)=-8\epsilon+O(\epsilon^2).
\label{eq:snr_center_linear}
\end{equation}
Thus, in the most mixed part of the bridge, symmetric ambiguity effectively restores a form of uncertainty about source--target dominance: a coarse progress cue alone no longer suffices to determine which side should be regarded as slightly dominant.

From this viewpoint, removing time embedding in the high-dimensional setting can be interpreted as a way to suppress identifiability shortcut reliance while partially restoring, in a structured form, the ambiguity that lower-dimensional bridges naturally possess. This does not remove bridge guidance from inference, since the schedule is still imposed externally through radius locking; rather, it changes where progress-related information is explicitly available to the model. Instead of reading off source--target regime from a highly informative time label, the model is pushed toward inferring it from the realized state itself. We hypothesize that this is a more robust inductive bias under inference mismatch: once the sampled trajectory deviates from the ideal training bridge, the actual source--target balance carried by $x_t$ may no longer agree with the nominal time index. In that case, a predictor trained to estimate balance from $x_t$ itself should be less prone to overconfident errors than one strongly anchored to an explicit time signal. For this reason, in our default high-dimensional setting we remove time embedding.

==> sections_old/DRF_old.tex <==
\section{A Two-Phase Direction-only Flow Matching Framework}
\label{sec:spoon_flow}

We propose a two-stage flow-matching framework for conditional token generation on $\mathbb{S}^{N-1}(R)$. The central idea is to decompose the overall transport into two stages with complementary roles, so that each stage can be modeled and sampled in a way that is well matched to the spherical token geometry. This staged construction yields a stable conditional sampling procedure and avoids failure modes that can arise when a single flow-matching formulation is used across the entire time horizon. Moreover, using the aforementioned thin-shell concentration property, we perform \emph{direction-only} velocity field modeling in which the actual speed is unnecessary throughout training and inference.

This section is organized as follows. We begin by analyzing why standard rectified flow with $v$-prediction can underestimate effective step sizes under angular errors, which is particularly harmful in hyperspherical token spaces. We then present spherical flow matching as a natural on-shell baseline and discuss its robustness to radial drift as well as its potential conditioning-collapse failure mode. Next, we introduce Outward Ray Flow (ORF), which predicts only a unit transport direction and enforces a dimension-stable inference step-size schedule via \emph{radius locking}, and we highlight the ill-defined ``contraction regime problem'' that motivates a two-phase design. Finally, we propose \textbf{Spoon Flow}, a two-phase spherical transport that uses SFM with \emph{radian locking inference} in the early-time regime and ORF with \emph{radius locking inference} in the late-time expansion regime, combining the strengths of both frameworks in different time intervals.

\subsection{Rectified Flow with $v$-Prediction: Step-Size Underestimation under Angular Errors}
\label{subsec:rf_vpred}

We first recall a standard rectified-flow (RF) training setup. Let $x_1\in\mathbb{S}^{N-1}(R)$ denote a target token and let $x_0$ be a source sample. A linear bridge is defined by
\begin{equation}
x_t = (1-t)x_0 + t x_1,\qquad t\in[0,1],
\end{equation}
with the corresponding constant transport vector
\begin{equation}
v^\star = x_1 - x_0.
\end{equation}
Standard RF trains a network $\hat v(x_t,t,c)$ (optionally conditioned on $c$) by minimizing an $\ell_2$ regression loss $\|\hat v - v^\star\|_2^2$.

\paragraph{$v$-pred magnitude shrinkage under directional mismatch.}
We analyze a purely geometric property of $\ell_2$ regression: if the predicted direction is mismatched with the target direction, then the optimal predicted magnitude is reduced. Decompose the prediction into a unit direction and a scalar magnitude:
\begin{equation}
\hat v \;=\; \hat s\,\hat r,\qquad \hat r\in\mathbb{S}^{N-1}(1),\ \hat s\ge 0,
\end{equation}
and similarly write the ground-truth transport as
\begin{equation}
v^\star \;=\; s^\star r^\star,\qquad r^\star=\mathrm{Norm}_1(v^\star)\in\mathbb{S}^{N-1}(1),\ s^\star=\|v^\star\|_2.
\end{equation}
Let $\theta=\angle(\hat r,r^\star)$ denote the angular mismatch, so that $\langle \hat r,r^\star\rangle=\cos\theta$.
Conditioned on a fixed direction $\hat r$, the $\ell_2$ objective is a convex quadratic in $\hat s$:
\begin{align}
\|\hat v - v^\star\|_2^2
&=\|\hat s\hat r - s^\star r^\star\|_2^2 \nonumber\\
&=\hat s^2 + (s^\star)^2 - 2\hat s s^\star \langle \hat r,r^\star\rangle \nonumber\\
&=\hat s^2 + (s^\star)^2 - 2\hat s s^\star \cos\theta.
\label{eq:vpred_quadratic}
\end{align}
Minimizing \eqref{eq:vpred_quadratic} over $\hat s$ yields
\begin{equation}
\hat s_{\mathrm{opt}} \;=\; s^\star \cos\theta,
\label{eq:vpred_shrinkage}
\end{equation}
i.e., the optimal magnitude is scaled by the cosine of the directional mismatch. Equivalently, the component of $\hat v$ along the true transport direction satisfies
\begin{equation}
\langle \hat v, r^\star\rangle
=
\hat s_{\mathrm{opt}}\langle \hat r,r^\star\rangle
=
s^\star \cos^2\theta.
\end{equation}

\paragraph{Implication for iterative sampling.}
In iterative integration, this shrinkage translates into smaller-than-intended step sizes and can accumulate over multiple steps, yielding a biased trajectory that fails to reach the intended radius. In high-dimensional token spaces, such radius drift is particularly harmful because the decoder (no matter standard VAEs or out spherical token) is trained on a thin shell or a hypersphere and is sensitive to off-shell samples. Moreover, step size shrinkage may also make intermediate output statistics (e.g., $\|x_t\|_2$) biased from their training-time counterparts, further leads to training-inference mismatch.

\subsection{Spherical Flow Matching on the Token Sphere}
\label{subsec:sfm_baseline}

Spherical Flow Matching (SFM) is a special case of Riemannian Flow Matching \cite{chen2023flow} in which the state is constrained to evolve on a hypersphere. This makes SFM a natural choice for hyperspherical token generation, and has been investigated in recent works \cite{kumar2026learning}.

\subsubsection{SFM Definition}

\paragraph{Slerp bridge on $\mathbb{S}^{N-1}(R)$.}
Given two endpoints $x_a,x_b\in\mathbb{S}^{N-1}(R)$, let
\begin{equation}
\omega \;=\; \arccos\!\Big(\frac{\langle x_a,x_b\rangle}{R^2}\Big)\in[0,\pi]
\end{equation}
denote their geodesic angle. The spherical linear interpolation (slerp) defines a constant-speed geodesic curve
\begin{equation}
x_t \;=\; \mathrm{slerp}(x_a,x_b;t)
\;=\;
\frac{\sin((1-t)\omega)}{\sin\omega}\,x_a
+
\frac{\sin(t\omega)}{\sin\omega}\,x_b,
\qquad t\in[0,1],
\label{eq:slerp_bridge}
\end{equation}
which satisfies $\|x_t\|_2=R$ for all $t$. SFM trains a tangent vector field $\hat v(x_t,t,c)\in T_{x_t}$ by regressing the constant-speed geodesic velocity along the slerp bridge between endpoints $x_a,x_b\in\mathbb{S}^{N-1}(R)$. Using the Riemannian logarithm map on the sphere, the target velocity can be written as
\begin{equation}
v_t^\star
\;=\;
\|\mathrm{Log}_{x_a}(x_b)\|_2\cdot \mathrm{Norm}_1\!\big(\mathrm{Log}_{x_t}(x_b)\big),
\label{eq:sfm_v_target}
\end{equation}
where $\|\mathrm{Log}_{x_a}(x_b)\|_2$ is the total geodesic arc-length from $x_a$ to $x_b$, and $\mathrm{Norm}_1(\cdot)$ normalizes a nonzero vector to unit $\ell_2$ norm. By construction, $\|v_t^\star\|_2=\|\mathrm{Log}_{x_a}(x_b)\|_2$ is \emph{constant in $t$}.

\subsubsection{Conditioning Collapse via Decoder-induced Basins and a Self-bootstrapping Shortcut}
\label{sec:sfm_shortcut}

We empirically observe that applying SFM to the aforementioned tokenizer can suffer from \emph{conditioning collapse}, where the conditional generative model may easily ignores the conditioning signal $c$ due to training dynamics. We argue that this failure mode is primarily cased by an interaction between (i) the \emph{basin structure} induced by the tokenizer/decoder training objective and (ii) the fact that SFM trajectories remain on the same hyperspherical shell as valid tokens.

\paragraph{Decoder-induced basins on the token sphere.}
Let $D:\mathbb{S}^{N-1}(R)\to\mathcal{X}$ denote the tokenizer decoder and let $d_\phi(\cdot,\cdot)$ be the reconstruction/perceptual metric used to define output similarity. For a target token $x_1\in\mathbb{S}^{N-1}(R)$, define its \emph{basin} on the token sphere by
\begin{equation}
\mathcal{B}_\epsilon(x_1)
\;\triangleq\;
\Big\{z\in\mathbb{S}^{N-1}(R):\ d_\phi\big(D(z),D(x_1)\big)\le \epsilon\Big\}.
\label{eq:basin_def}
\end{equation}
The tokenizer is trained with dimension-aware geodesic perturbations (Sec.~\ref{sec:noise_inject}) so that decoding is stable within a controlled angular neighborhood around each training token. In particular, for typical perturbation angles $\theta$ in the training phase, the reconstruction objective encourages
\begin{equation}
D\!\big(\mathrm{Exp}_{x_1}(R\theta u)\big)\approx D(x_1)
\quad\Rightarrow\quad
\mathrm{Exp}_{x_1}(R\theta u)\in \mathcal{B}_\epsilon(x_1)
\ \text{for many }u\in T_{x_1}\mathbb{S}^{N-1}(R),
\label{eq:basin_contains_cap}
\end{equation}
i.e., each $x_1$ is surrounded by a nontrivial basin on the sphere. Importantly, the tokenizer is also trained to avoid \emph{representation collapse} (e.g., degenerate embeddings with vanishing variance or rank), so distinct tokens are encouraged to remain semantically separable. Consequently, basins corresponding to different targets are expected to be largely disjoint:
\begin{equation}
\mathcal{B}_\epsilon(x_1)\cap \mathcal{B}_\epsilon(x_1') \approx \emptyset
\qquad \text{for }x_1\neq x_1',
\label{eq:basin_separation}
\end{equation}
since otherwise distinct tokens would decode to indistinguishable outputs, contradicting the tokenizer objective.

\paragraph{Posterior sharpening and self-bootstrapping on-shell.}
Consider SFM with endpoint $x_b=x_1$ and intermediate states $x_t\in\mathbb{S}^{N-1}(R)$ along the slerp bridge. Because the entire trajectory stays on the same shell as valid tokens, it can enter the basin $\mathcal{B}_\epsilon(x_1)$ for a non-negligible range of times $t$ (often well before $t\to 1$). Once $x_t\in\mathcal{B}_\epsilon(x_1)$, the endpoint becomes effectively determined by $x_t$:
\begin{equation}
x_t\in\mathcal{B}_\epsilon(x_1)
\ \stackrel{\eqref{eq:basin_separation}}{\Longrightarrow}\
\mathbb{P}(X_1=x_1\mid X_t=x_t,t)\approx 1,
\label{eq:posterior_sharpening}
\end{equation}
i.e., the conditional uncertainty over the endpoint collapses (``posterior sharpening''). In this regime, the optimal regression target for the velocity field satisfies
\begin{equation}
\mathbb{E}\big[v_t^\star \mid X_t=x_t,t,c\big]
\;\approx\;
\mathbb{E}\big[v_t^\star \mid X_t=x_t,t\big],
\label{eq:cond_redundant}
\end{equation}
so the conditioning signal $c$ becomes nearly redundant for minimizing the SFM loss. This creates a \emph{self-bootstrapping shortcut}: the model can reduce training error by learning a mapping from $x_t$ to a velocity that points toward the basin center, without using $c$. 

\paragraph{Training--inference dynamics and error accumulation.}
The shortcut in \eqref{eq:cond_redundant} is particularly harmful because the same network parameters are shared across all times. Once the model learns to ignore $c$ on a subset of times (typically large $t$ where basin membership is common), the resulting representation and attention pathways tend to generalize to smaller $t$ as well. However, for small $t$ the state is farther from any basin center and the conditional ambiguity is higher, so a $c$-agnostic predictor incurs large directional errors. Equivalently, the learned predictor approaches $\mathbb{E}[v_t^\star\mid x_t,t]$ on large $t$, and parameter sharing biases it toward the same $c$-agnostic conditional expectation on small $t$, where $\mathbb{E}[v_t^\star\mid x_t,t]$ is a poor surrogate for $\mathbb{E}[v_t^\star\mid x_t,t,c]$.

At inference time, these small-$t$ errors are amplified: early-time deviations move the trajectory toward an incorrect basin, after which the on-shell dynamics further reinforce the wrong endpoint (since basin membership again sharpens the effective posterior). This creates a feedback loop in which (i) large-$t$ training encourages a $c$-agnostic shortcut, (ii) the shortcut induces large errors at small $t$, and (iii) the resulting trajectory drift makes later-time updates increasingly consistent with the wrong basin, further weakening conditional dependence or even generating completely collapsed outputs.

\paragraph{Why this shortcut is specific to on-shell spherical trajectories.}
The above mechanism relies on the trajectory remaining on the token shell where decoder basins are defined. In contrast, Euclidean linear bridges typically traverse off-shell regions where $D(\cdot)$ is not trained to be stable and where basin membership is less likely, so the posterior sharpening effect in \eqref{eq:posterior_sharpening} is weaker. Thus, the same tokenizer design that promotes well-separated, stable basins on the sphere (to avoid representational collapse) can inadvertently make on-shell SFM training more prone to conditioning collapse.

\subsection{Outward Ray Flow (ORF): Direction-Only Transport with Explicit Radius Control}
\label{subsec:orf}

We now introduce Outward Ray Flow (ORF), a direction-only transport scheme with explicitly controls on the radius of intermediate outputs during inference. The key idea is to predict only a unit \emph{ray} (bearing) and to recover the step size by enforcing a prescribed \emph{radius schedule}.

\subsubsection{Inner-to-Outer Bridge and Direction-only Supervision}
\label{sec:orf_bridge}

We term our method \textbf{Outward Ray Flow (ORF)} because it exploits a simple geometric identifiability property of \emph{inner-to-outer} linear mappings: when the source lies on an inner sphere ($a<1$) and the target lies on the outer token sphere, the endpoint on the outer sphere is uniquely determined by an outward ray from the source. Unlike high-dimensional SFM which requires the thin-shell concentration property for direction-only modeling, such property naturally supports direction-only parameterization in a linear bridge.

\paragraph{Definition.}
Let the source distribution be uniform on an \emph{inner} sphere:
\begin{equation}
x_0 \sim \mathrm{Unif}\big(\mathbb{S}^{N-1}(aR)\big),\qquad a\in(0,1),
\end{equation}
and let $x_1\in\mathbb{S}^{N-1}(R)$ be the target. We use the linear bridge
\begin{equation}
x_t=(1-t)x_0+t x_1,\qquad t\in[0,1],
\label{eq:orf_lerp_bridge}
\end{equation}
with constant transport vector $v^\star=x_1-x_0$. ORF trains a network to predict the \emph{unit transport ray}
\begin{equation}
r^\star = \mathrm{Norm}_1(x_1-x_0)\in\mathbb{S}^{N-1}(1),
\end{equation}
using a angular loss on the estimated and target rays
\begin{equation}
L_{\mathrm{ORF}} = 1-\cos\big(\hat r(x_t,t,c),\,r^\star\big).
\end{equation}

\paragraph{Uniqueness of the outer-sphere intersection.}
Consider the ray starting at $x_0$ in direction $r\in\mathbb{S}^{N-1}(1)$:
\begin{equation}
\ell(\Delta)=x_0+\Delta r,\qquad \Delta\ge 0.
\end{equation}
The intersection(s) with the outer sphere satisfy $\|\ell(\Delta)\|_2=R$, i.e.,
\begin{equation}
\|x_0+\Delta r\|_2^2 = a^2R^2 + \Delta^2 + 2\Delta\langle x_0,r\rangle = R^2.
\label{eq:ray_sphere_intersection}
\end{equation}
When $a<1$ and we restrict to the \emph{outward} branch $\Delta\ge 0$, the ray yields a unique physically valid intersection on $\mathbb{S}^{N-1}(R)$ (the first hit of the outer sphere along the outward direction). This makes it meaningful to learn only the ray direction.

\paragraph{Why the standard thin-shell RF setting is ambiguous.}
In the standard RF setup, the source is typically sampled from an isotropic Gaussian,
\begin{equation}
x_0 \sim \mathcal N(0,I_N),
\end{equation}
which concentrates on a thin shell of radius $\|x_0\|_2\approx \sqrt{N}$ in high dimensions. Likewise, in common latent-variable tokenizers (e.g., VAEs with an isotropic Gaussian prior), both the target and intermediate states also concentrate on a thin shell (up to a scale factor), e.g.,
\begin{equation}
x_1 \approx \sigma\sqrt{N}\cdot u,\qquad u\sim \mathrm{Unif}(\mathbb S^{N-1}(1)).
\end{equation}
As a consequence, the RF transport direction $r^\star \propto (x_1-x_0)$ is not guaranteed to be \emph{outward} with respect to the shell: depending on the relative radii and the random orientation, the velocity can point from a point on (or near) the shell toward the interior (i.e., it can have a negative radial component with respect to $x_0$). In this regime, a direction-only parameterization becomes ill-posed: knowing only a unit direction $r$ from a point $x_0$ on a thin shell does not uniquely identify the intended endpoint $x_1$ on (approximately) the same shell, because the line $x_0+\Delta r$ intersects the shell at (typically) two locations and the physically correct choice depends on the (unknown) step size/magnitude. 

\subsubsection{Dimension-stable Radius Schedule and Contraction/Expansion Phases}
\label{sec:orf_radius_schedule}

A central ingredient of ORF is a deterministic radius schedule $\rho(t)$ that approximates $\|x_t\|_2$ in high dimensions. Expanding \eqref{eq:orf_lerp_bridge} and using the thin-shell concentration property gives
\begin{align}
\|x_t\|_2^2
&=\|(1-t)x_0+t x_1\|_2^2 \nonumber\\
&=(1-t)^2\|x_0\|_2^2+t^2\|x_1\|_2^2+2t(1-t)\langle x_0,x_1\rangle\\
&\approx R^2\big(a^2(1-t)^2+t^2\big)\;\triangleq\;\rho(t)^2.
\label{eq:xt_norm_exact}
\end{align}
The schedule $\rho(t)$ is \emph{non-monotone}: it first shrinks and then expands. It is easy to see that the minimum-radius time is
\begin{equation}
t_{\min}=\frac{a^2}{1+a^2},
\label{eq:tmin}
\end{equation}
so we call $t\in[0,t_{\min}]$ the \emph{contraction phase} and $t\in[t_{\min},1]$ the \emph{expansion phase}.

\subsubsection{Radius Locking Inference for ORF}
\label{sec:orf_step}

Unlike standard RF or SFM inference-phase samplers, which typically rely on a pre-specified step-size schedule schedule on the constant-speed velocity field to advance the state, ORF does \emph{not} assume an explicit step-size schedule. Instead, ORF uses a time schedule $t_0<t_1<\cdots<t_K$ together with the \emph{radius schedule $\rho(t)$} (Sec.~\ref{sec:orf_radius_schedule}) to \emph{dynamically compute} the step size at each iteration. Concretely, at step $k$ we choose the scalar step size $\Delta_{t_k}$ so that the updated state lands exactly on the target radius prescribed by $\rho(t_{k+1})$. This systematically mitigates the step-size underestimation problem in standard $v$-prediction RF framework.

Let $x_{t_k}$ denote the current state at time $t_k$ and let $\hat r_{t_k}=\hat r(x_{t_k},t_k,c)\in\mathbb{S}^{N-1}(1)$ be the predicted ray. We update
\begin{equation}
x_{t_{k+1}} = x_{t_k} + \Delta_{t_k}\,\hat r_{t_k},
\label{eq:orf_update}
\end{equation}
and enforce the radius-locking constraint
\begin{equation}
\|x_{t_{k+1}}\|_2 = \rho(t_{k+1}).
\label{eq:radius_lock}
\end{equation}
Squaring \eqref{eq:radius_lock} and expanding yields a quadratic equation in $\Delta_{t_k}$:
\begin{align}
\|x_{t_k}+\Delta_{t_k}\hat r_{t_k}\|_2^2
&=\|x_{t_k}\|_2^2+\Delta_{t_k}^2+2\Delta_{t_k}\langle x_{t_k},\hat r_{t_k}\rangle \nonumber\\
&=\rho(t_{k+1})^2,
\end{align}
i.e.,
\begin{equation}
\Delta_{t_k}^2 + 2\langle x_{t_k},\hat r_{t_k}\rangle\,\Delta_{t_k}
+ \big(\|x_{t_k}\|_2^2-\rho(t_{k+1})^2\big)=0.
\label{eq:delta_quadratic}
\end{equation}

Let $c_k=\langle x_{t_k},\hat r_{t_k}\rangle$ and define the target radius increment
\begin{equation}
\Delta\rho_k^2 \;=\; \rho(t_{k+1})^2-\rho(t_k)^2.
\end{equation}
since $\|x_{t_k}\|_2=\rho(t_k)$ under the radius schedule, we obtain the two roots of \eqref{eq:delta_quadratic}
\begin{equation}
\Delta_{t_k} = -c_k \pm \sqrt{c_k^2+\Delta\rho_k^2}.
\label{eq:orf_two_roots}
\end{equation}

\subsubsection{Ill-defined Contraction Regime and Training-Inference Mismatch}
\label{sec:orf_ill_defined}

During the expansion phase, $c_k^2+\Delta\rho_k^2$ is always positive and the valid root becomes $\Delta_{t_k} = -c_k + \sqrt{c_k^2+\Delta\rho_k^2}$. However, the contraction phase of the radius schedule is intrinsically problematic for ray-based radius locking: $c_k^2+\Delta\rho_k^2$ is not guaranteed to be nonnegative, and the resulting fallback introduces a biased update that is not reflected in the training distribution:
\begin{enumerate}
\item \textbf{Feasible contraction ($c_k^2+\Delta\rho_k^2\ge 0$).}
There exist two real roots, both having the same sign. The physically consistent update is the negative root (moving against the radial component of $\hat r_{t_k}$):
\begin{equation}
\Delta_{t_k} = -c_k - \sqrt{c_k^2+\Delta\rho_k^2}.
\end{equation}

\item \textbf{Infeasible contraction ($c_k^2+\Delta\rho_k^2<0$).}
No real step size can reach the target smaller radius along the straight-ray update
$x_{t_{k+1}}=x_{t_k}+\Delta_{t_k}\hat r_{t_k}$.
Geometrically, along a fixed ray direction $\hat r_{t_k}$ the \emph{minimal achievable radius} is attained at
\begin{equation}
\Delta_{t_k}^{\min}=-c_k,\qquad c_k=\langle x_{t_k},\hat r_{t_k}\rangle,
\end{equation}
which yields the closest point to the origin on the ray,
\begin{equation}
x_{t_{k+1}}^\ast = x_{t_k}+\Delta_{t_k}^{\min}\hat r_{t_k},
\qquad
\langle x_{t_{k+1}}^\ast,\hat r_{t_k}\rangle=0.
\end{equation}
When $c_k^2+\Delta\rho_k^2<0$, the target radius $\rho(t_{k+1})$ is smaller than $\|x_{t_{k+1}}^\ast\|_2$, hence the radius-locking constraint is infeasible along the ray and a \emph{retraction} operator is required to map $x_{t_{k+1}}^\ast$ to the target radius. A natural idea is to retract $x_{t_{k+1}}^\ast$ to the target radius by moving along some auxiliary direction $q_{t_k}\in\mathbb{S}^{N-1}(1)$ (e.g., a correction direction). This would take the form
\begin{equation}
x_{t_{k+1}} = x_{t_{k+1}}^\ast + \lambda_{t_k}\,q_{t_k},
\qquad
\|x_{t_{k+1}}\|_2=\rho(t_{k+1}).
\label{eq:orf_aux_retract_form}
\end{equation}
However, \eqref{eq:orf_aux_retract_form} is itself not always solvable for the same reason as \eqref{eq:delta_quadratic}. Therefore, replacing the ray update by an auxiliary direction does not theoretically eliminate infeasibility; it merely shifts the feasibility condition to a different direction. To define a universally feasible retraction operator for \emph{all} nonzero $x_{t_{k+1}}^\ast$, we can simply take the radial normalization operator:
\begin{equation}
R^{\mathrm{ORF}}_{\rho'}(x_{t_{k+1}})
=
\rho(t_{k+1})\mathrm{Norm}_1(x_{t_{k+1}}^\ast).
\label{eq:orf_radial_retract}
\end{equation}
This mapping is always well-defined and enforces $\|x_{t_{k+1}}\|_2=\rho(t_{k+1})$ by construction. Crucially, in the infeasible contraction case the retraction direction defined by the radial normalization operator is \emph{necessarily orthogonal} to the predicted ray. Indeed, by definition of $x_{t_{k+1}}^\ast$ we have $\langle x_{t_{k+1}}^\ast,\hat r_{t_k}\rangle=0$, hence
\begin{equation}
\left\langle \frac{x_{t_{k+1}}^\ast}{\|x_{t_{k+1}}^\ast\|_2},\ \hat r_{t_k}\right\rangle = 0,
\qquad\Rightarrow\qquad
\angle\!\left(\frac{x_{t_{k+1}}^\ast}{\|x_{t_{k+1}}^\ast\|_2},\hat r_{t_k}\right)=\frac{\pi}{2}.
\label{eq:orf_retract_orthogonal}
\end{equation}
That is, whenever the radius-locking equation is infeasible and we fall back to the closest point $x_{t_{k+1}}^\ast$ followed by radial normalization, the retraction introduces an update component that is \emph{maximally misaligned} with the model-predicted ray. This geometric mismatch is intrinsic to the infeasible contraction regime: it does not depend on the particular choice of model or training objective, but follows directly from the ray geometry and the requirement to hit a smaller target radius.

This issue is particularly severe in settings where a single network predicts rays for multiple inputs $\{\hat r_{t_k}\}_{k=0}^{K-1}$: within the same forward pass, some inputs may satisfy $c_k^2+\Delta\rho_k^2\ge 0$ (unbiased, exact radius-locking), while others satisfy $c_k^2+\Delta\rho_k^2<0$ (biased, retracted update). This creates a sharp training--inference mismatch: during training, the model is supervised on oracle bridge states $x_{t_k}$ constructed from the ground-truth pair $(x_0,x_1)$, so every $x_{t_k}$ lies exactly on the intended bridge distribution. At inference time, however, the sampler produces states that are a mixture of (i) exact updates and (ii) biased retracted updates, and the latter can move the trajectory off the oracle bridge in a time-dependent manner. Since later predictions $\hat r_{t_{k'}}$ are conditioned on these perturbed states, the mismatch compounds across steps and can be strongly amplified in the subsequent expansion phase.
\end{enumerate}

\subsection{Analysis of Possible Radius Locking Operators}
\label{subsec:radius_locking_analysis}

We now analyze several possible inference operators for direction-only sampling under a standard RF bridge, with the goal of understanding which operator is most suitable in the contraction and expansion regimes. The analysis is purely geometric and is intended to separate \emph{bridge geometry} from \emph{prediction error}. In particular, we study two questions:
\begin{enumerate}[leftmargin=2.0em,label=(\roman*)]
\item under oracle states and oracle directions, whether a given operator exactly reaches the oracle next state;
\item under oracle states but imperfect predicted directions, how far the resulting update deviates from the oracle next state.
\end{enumerate}

Throughout this subsection, we consider the standard RF bridge
\begin{equation}
x_t=(1-t)x_0+t x_1,
\qquad
t\in[0,1],
\label{eq:rf_bridge_analysis}
\end{equation}
with
\begin{equation}
\|x_0\|_2=\|x_1\|_2=R,
\qquad
R=\sqrt N,
\end{equation}
and use the high-dimensional concentration approximation
\begin{equation}
\langle x_0,x_1\rangle \approx 0.
\label{eq:rf_orth_approx}
\end{equation}
Under this approximation, the oracle velocity is the constant vector
\begin{equation}
v^\star = x_1-x_0,
\qquad
L\triangleq \|v^\star\|_2 \approx \sqrt2\,R,
\qquad
r^\star \triangleq \frac{v^\star}{\|v^\star\|_2}.
\label{eq:oracle_velocity_analysis}
\end{equation}
For a time step $h>0$, the oracle next state is
\begin{equation}
x_{t+h}^\star = x_t + hL r^\star.
\label{eq:oracle_next_state_analysis}
\end{equation}

\subsubsection{Oracle Radius Schedule and the Contraction/Expansion Split}
Under Eq.~\eqref{eq:rf_orth_approx}, the bridge radius is
\begin{equation}
r_t \triangleq \|x_t\|_2
\approx
R\sqrt{(1-t)^2+t^2}.
\label{eq:rt_analysis}
\end{equation}
The minimum radius occurs at
\begin{equation}
t_{\min}=\frac12.
\label{eq:tmin_standard_rf}
\end{equation}
Thus the interval $t\in[0,\frac12]$ is the \emph{contraction regime}, and $t\in[\frac12,1]$ is the \emph{expansion regime}.

A useful geometric quantity is the signed radial component of the oracle direction at time $t$:
\begin{equation}
c_t \triangleq \langle x_t,r^\star\rangle.
\label{eq:ct_def_analysis}
\end{equation}
Using Eqs.~\eqref{eq:rf_bridge_analysis} and \eqref{eq:oracle_velocity_analysis}, we obtain
\begin{align}
\langle x_t,v^\star\rangle
&=
\langle (1-t)x_0+t x_1,\ x_1-x_0\rangle \nonumber\\
&\approx
(1-t)(0-R^2)+t(R^2-0)
=
(2t-1)R^2,
\end{align}
hence
\begin{equation}
\boxed{
c_t
=
\langle x_t,r^\star\rangle
\approx
\frac{(2t-1)R}{\sqrt2}.
}
\label{eq:ct_analysis}
\end{equation}
Therefore, $c_t<0$ in the contraction regime and $c_t>0$ in the expansion regime.

\subsubsection{Oracle Exactness of Different Inference Operators}

We first verify that under oracle states and oracle directions, all natural operators considered below exactly recover the oracle next state.

\paragraph{(A) Standard Euler step with fixed oracle norm.}
Consider
\begin{equation}
x_{t+h}^{\mathrm{E}} = x_t + hL r^\star.
\end{equation}
By Eq.~\eqref{eq:oracle_next_state_analysis}, this is exactly the oracle update.

\paragraph{(B) Euler step followed by normalization to the target radius.}
Let
\begin{equation}
\tilde x_{t+h}=x_t+hLr^\star=x_{t+h}^\star,
\end{equation}
and define
\begin{equation}
x_{t+h}^{\mathrm{EN}}
=
r_{t+h}\frac{\tilde x_{t+h}}{\|\tilde x_{t+h}\|_2}.
\end{equation}
Since $\|\tilde x_{t+h}\|_2=\|x_{t+h}^\star\|_2=r_{t+h}$, the normalization does nothing and
\begin{equation}
x_{t+h}^{\mathrm{EN}}=x_{t+h}^\star.
\end{equation}

\paragraph{(C) Standard radius locking.}
Consider the update
\begin{equation}
x_{t+h}^{\mathrm{RL}}=x_t+\Delta r^\star,
\label{eq:radius_lock_oracle_update}
\end{equation}
with $\Delta$ chosen so that
\begin{equation}
\|x_{t+h}^{\mathrm{RL}}\|_2=r_{t+h}.
\label{eq:radius_lock_oracle_constraint}
\end{equation}
Since $\Delta=hL$ produces the oracle next state and the oracle next state already has radius $r_{t+h}$, Eq.~\eqref{eq:radius_lock_oracle_update} with $\Delta=hL$ satisfies Eq.~\eqref{eq:radius_lock_oracle_constraint}. Therefore, in the oracle case, standard radius locking also reaches the oracle next state exactly whenever the corresponding root is selected.

\paragraph{Implication.}
The above shows that the differences among these operators do not appear at the level of oracle consistency. They appear only when the predicted direction is imperfect.

\subsubsection{A General Parameterization of Direction Errors}
We now analyze the one-step error under oracle $x_t$ but imperfect predicted direction. Let $\hat r$ denote the predicted unit direction, and define its angular error with respect to the oracle direction by
\begin{equation}
\angle(\hat r,r^\star)=\theta,
\qquad
\theta\in[0,\pi].
\end{equation}
We do \emph{not} assume $\theta$ is small.

To fully characterize the effect of direction error on radius evolution, we must also specify how the prediction error is oriented relative to the current state $x_t$. Write
\begin{equation}
x_t^\perp \triangleq x_t-\langle x_t,r^\star\rangle r^\star
=
x_t-c_t r^\star.
\end{equation}
When $x_t^\perp\neq 0$, define
\begin{equation}
u_t \triangleq \frac{x_t^\perp}{\|x_t^\perp\|_2},
\end{equation}
and let $w$ be any unit vector such that
\begin{equation}
w\perp r^\star,\qquad w\perp u_t,\qquad \|w\|_2=1.
\end{equation}
Then any unit prediction direction with angular error $\theta$ can be written as
\begin{equation}
\boxed{
\hat r = \cos\theta\, r^\star + \sin\theta\big(\cos\varphi\,u_t+\sin\varphi\,w\big),
}
\label{eq:hatr_decomposition}
\end{equation}
for some $\varphi\in[0,2\pi)$. Here:
\begin{itemize}
\item $\theta$ controls the angle to the oracle direction;
\item $\varphi$ controls how the error is oriented relative to the current state's radial direction.
\end{itemize}

A key simplification in the standard RF setting is that $\|x_t^\perp\|_2$ is constant in $t$. Indeed,
\begin{equation}
\|x_t^\perp\|_2^2 = \|x_t\|_2^2-c_t^2.
\end{equation}
Using Eq.~\eqref{eq:rt_analysis} and Eq.~\eqref{eq:ct_analysis},
\begin{align}
\|x_t^\perp\|_2^2
&\approx
R^2\big((1-t)^2+t^2\big)-\frac{(2t-1)^2R^2}{2}\nonumber\\
&=
R^2\left(1-2t+2t^2-\left(2t^2-2t+\frac12\right)\right)
=
\frac{R^2}{2},
\end{align}
hence
\begin{equation}
\boxed{
\|x_t^\perp\|_2 = \frac{R}{\sqrt2}.
}
\label{eq:xt_perp_norm}
\end{equation}

Substituting Eq.~\eqref{eq:hatr_decomposition} into $\langle x_t,\hat r\rangle$ yields
\begin{equation}
\langle x_t,\hat r\rangle
=
c_t\cos\theta+\|x_t^\perp\|_2\sin\theta\cos\varphi,
\end{equation}
which, using Eqs.~\eqref{eq:ct_analysis} and \eqref{eq:xt_perp_norm}, becomes
\begin{equation}
\boxed{
\langle x_t,\hat r\rangle
=
\frac{R}{\sqrt2}\Big[(2t-1)\cos\theta+\sin\theta\cos\varphi\Big].
}
\label{eq:xt_hatr_inner}
\end{equation}

Equation~\eqref{eq:xt_hatr_inner} will be the central quantity in all subsequent comparisons.

\subsubsection{Method A: Standard Euler Step with Fixed Oracle Velocity Norm}

Consider the update
\begin{equation}
x_{t+h}^{\mathrm{E}} = x_t + hL\hat r.
\label{eq:euler_update_analysis}
\end{equation}

\paragraph{Deviation from the oracle next state.}
The one-step error is
\begin{equation}
e_{\mathrm E}
=
x_{t+h}^{\mathrm{E}}-x_{t+h}^\star
=
hL(\hat r-r^\star).
\end{equation}
Since $\angle(\hat r,r^\star)=\theta$,
\begin{equation}
\|\hat r-r^\star\|_2^2 = 2(1-\cos\theta),
\end{equation}
hence
\begin{equation}
\boxed{
\|e_{\mathrm E}\|_2
=
hL\sqrt{2(1-\cos\theta)}
=
2hL\sin\frac{\theta}{2}.
}
\label{eq:euler_error_exact}
\end{equation}
Using $L\approx \sqrt2 R$,
\begin{equation}
\boxed{
\|e_{\mathrm E}\|_2
=
2\sqrt2\,hR\sin\frac{\theta}{2}.
}
\label{eq:euler_error_exact_R}
\end{equation}

\paragraph{Radius error.}
The updated radius satisfies
\begin{align}
\|x_t+hL\hat r\|_2^2
&=
r_t^2 + 2hL\langle x_t,\hat r\rangle + h^2L^2.
\end{align}
Using Eq.~\eqref{eq:xt_hatr_inner} and $L=\sqrt2 R$,
\begin{equation}
\boxed{
\|x_t+hL\hat r\|_2^2
=
r_t^2
+
2hR^2\Big[(2t-1)\cos\theta+\sin\theta\cos\varphi\Big]
+
2h^2R^2.
}
\label{eq:euler_radius}
\end{equation}
By contrast, the oracle target radius is
\begin{equation}
r_{t+h}^2
=
r_t^2 + 2h(2t-1)R^2 + 2h^2R^2.
\end{equation}
Subtracting gives
\begin{equation}
\boxed{
\|x_t+hL\hat r\|_2^2-r_{t+h}^2
=
2hR^2\Big[(2t-1)(\cos\theta-1)+\sin\theta\cos\varphi\Big].
}
\label{eq:euler_radius_error}
\end{equation}

\paragraph{Interpretation.}
Equation~\eqref{eq:euler_radius_error} already reveals the asymmetry between contraction and expansion:
\begin{itemize}
\item \textbf{Contraction regime} $(t<1/2)$: since $(2t-1)<0$, the term $(2t-1)(\cos\theta-1)$ is nonnegative. Thus directional error \emph{reduces} contraction in a systematic way. Standard Euler therefore tends to shrink \emph{less} than the oracle trajectory, and may even fail to shrink at all if the second term is sufficiently positive.
\item \textbf{Expansion regime} $(t>1/2)$: now $(2t-1)>0$, so the same term is nonpositive. Thus directional error systematically weakens expansion, which is the direct analogue of under-reaching in the expansion regime.
\end{itemize}

\subsubsection{Method B: Euler Step Followed by Normalization to the Target Radius}

Consider the update
\begin{equation}
\tilde x_{t+h}=x_t+hL\hat r,
\qquad
x_{t+h}^{\mathrm{EN}}
=
r_{t+h}\frac{\tilde x_{t+h}}{\|\tilde x_{t+h}\|_2}.
\label{eq:euler_normalize_update}
\end{equation}
This operator removes all radius error after the Euler step and preserves only the angular discrepancy on the target shell.

\paragraph{Exact shell-angle error formula.}
Since both $x_{t+h}^{\mathrm{EN}}$ and $x_{t+h}^\star$ lie on the sphere of radius $r_{t+h}$, their Euclidean deviation is
\begin{equation}
\|x_{t+h}^{\mathrm{EN}}-x_{t+h}^\star\|_2
=
2r_{t+h}\sin\frac{\psi_{\mathrm{EN}}}{2},
\label{eq:EN_shell_error}
\end{equation}
where
\begin{equation}
\psi_{\mathrm{EN}} \triangleq \angle(\tilde x_{t+h},x_{t+h}^\star).
\end{equation}
Thus the exact error is determined by
\begin{equation}
\cos\psi_{\mathrm{EN}}
=
\frac{\langle \tilde x_{t+h},x_{t+h}^\star\rangle}{\|\tilde x_{t+h}\|_2\,r_{t+h}}.
\end{equation}

\paragraph{Exact numerator.}
Expanding
\begin{equation}
\tilde x_{t+h}=x_t+hL\hat r,
\qquad
x_{t+h}^\star=x_t+hLr^\star,
\end{equation}
gives
\begin{align}
\langle \tilde x_{t+h},x_{t+h}^\star\rangle
&=
r_t^2 + hL\langle x_t,\hat r\rangle + hL\langle x_t,r^\star\rangle + h^2L^2\langle \hat r,r^\star\rangle.
\end{align}
Using Eqs.~\eqref{eq:xt_hatr_inner} and \eqref{eq:ct_analysis}, together with $L=\sqrt2R$ and $\langle \hat r,r^\star\rangle=\cos\theta$, we obtain
\begin{equation}
\boxed{
\langle \tilde x_{t+h},x_{t+h}^\star\rangle
=
r_t^2
+
hR^2\Big[(2t-1)(1+\cos\theta)+\sin\theta\cos\varphi\Big]
+
2h^2R^2\cos\theta.
}
\label{eq:EN_numerator}
\end{equation}

\paragraph{Exact denominator.}
From Eq.~\eqref{eq:euler_radius},
\begin{equation}
\|\tilde x_{t+h}\|_2^2
=
r_t^2
+
2hR^2\Big[(2t-1)\cos\theta+\sin\theta\cos\varphi\Big]
+
2h^2R^2.
\label{eq:EN_denominator_tilde}
\end{equation}
Therefore,
\begin{equation}
\boxed{
\cos\psi_{\mathrm{EN}}
=
\frac{
r_t^2
+
hR^2\Big[(2t-1)(1+\cos\theta)+\sin\theta\cos\varphi\Big]
+
2h^2R^2\cos\theta
}{
\sqrt{
r_t^2
+
2hR^2\Big[(2t-1)\cos\theta+\sin\theta\cos\varphi\Big]
+
2h^2R^2
}
\cdot r_{t+h}
}.
}
\label{eq:EN_cos_exact}
\end{equation}

\paragraph{Interpretation.}
This operator removes the radius error in Eq.~\eqref{eq:euler_radius_error} exactly at every step. Therefore, compared with raw Euler, its remaining deviation from the oracle next state is \emph{purely angular on the target shell}. In the contraction regime, where directional error tends to reduce shrinkage, this correction is especially valuable: it prevents the trajectory from drifting away from the theoretical shell schedule even when the direction error is large.

\subsubsection{Method C: Standard Radius Locking in the Expansion Regime}

Consider the update
\begin{equation}
x_{t+h}^{\mathrm{RL}} = x_t+\Delta \hat r,
\label{eq:RL_update_analysis}
\end{equation}
where $\Delta$ is chosen so that
\begin{equation}
\|x_t+\Delta\hat r\|_2 = r_{t+h}.
\label{eq:RL_constraint_analysis}
\end{equation}
Squaring and solving gives
\begin{equation}
\Delta^2 + 2\langle x_t,\hat r\rangle \Delta + (r_t^2-r_{t+h}^2)=0.
\end{equation}
Using Eq.~\eqref{eq:xt_hatr_inner}, let
\begin{equation}
b \triangleq \langle x_t,\hat r\rangle
=
\frac{R}{\sqrt2}\Big[(2t-1)\cos\theta+\sin\theta\cos\varphi\Big].
\label{eq:b_def_analysis}
\end{equation}
Then the expansion-regime root is
\begin{equation}
\boxed{
\Delta
=
-b+\sqrt{b^2+r_{t+h}^2-r_t^2}
=
-b+\sqrt{b^2+2h(2t-1)R^2+2h^2R^2}.
}
\label{eq:RL_delta_exact}
\end{equation}

\paragraph{Exact one-step error.}
The deviation from the oracle next state is
\begin{equation}
e_{\mathrm{RL}}
=
x_{t+h}^{\mathrm{RL}}-x_{t+h}^\star
=
\Delta \hat r - hLr^\star.
\end{equation}
Hence
\begin{equation}
\|e_{\mathrm{RL}}\|_2^2
=
\Delta^2 + h^2L^2 - 2\Delta hL\cos\theta.
\end{equation}
Using $L=\sqrt2R$ gives
\begin{equation}
\boxed{
\|e_{\mathrm{RL}}\|_2^2
=
\Delta^2 + 2h^2R^2 - 2\sqrt2\,hR\,\Delta\cos\theta.
}
\label{eq:RL_error_exact}
\end{equation}

\paragraph{Interpretation.}
Standard radius locking enforces the target shell \emph{without} adding an extra radial projection after the step. Instead, it adjusts the step length along the current predicted direction. In the expansion regime, this is geometrically natural: the target shell is reachable along the predicted direction, and the operator preserves the model's directional decision while correcting only the step magnitude.

\subsubsection{Method D: Retraction-Based Radius Locking in the Contraction Regime}

In the contraction regime, the target radius decreases. If Eq.~\eqref{eq:RL_constraint_analysis} has no real solution, one may consider the following fallback:
\begin{enumerate}[leftmargin=2.0em,label=(\arabic*)]
\item move along the predicted direction to the smallest radius attainable on that ray;
\item normalize that point to the target radius.
\end{enumerate}

\paragraph{Smallest attainable radius along the predicted ray.}
Along the ray
\begin{equation}
x_t+\Delta\hat r,
\end{equation}
the squared radius is
\begin{equation}
f(\Delta)=r_t^2+2b\Delta+\Delta^2.
\end{equation}
This is minimized at
\begin{equation}
\Delta_{\min}=-b,
\end{equation}
and the minimum attainable squared radius is
\begin{equation}
f_{\min}=r_t^2-b^2.
\label{eq:fmin_analysis}
\end{equation}
Thus contraction along $\hat r$ is feasible iff
\begin{equation}
r_{t+h}^2 \ge r_t^2-b^2,
\end{equation}
equivalently
\begin{equation}
b^2 \ge r_t^2-r_{t+h}^2.
\label{eq:contraction_feasible_analysis}
\end{equation}

\paragraph{Retraction fallback.}
When Eq.~\eqref{eq:contraction_feasible_analysis} fails, define
\begin{equation}
x^\flat = x_t-b\hat r
\end{equation}
and retract to the target shell by
\begin{equation}
x_{t+h}^{\mathrm{RET}}
=
r_{t+h}\frac{x^\flat}{\|x^\flat\|_2}.
\label{eq:RET_update}
\end{equation}

\paragraph{Geometric issue.}
By construction,
\begin{equation}
\langle x^\flat,\hat r\rangle = 0.
\end{equation}
Thus once the ray reaches its minimum-radius point, the subsequent normalization in Eq.~\eqref{eq:RET_update} necessarily moves in a direction orthogonal to the predicted direction. Therefore, when contraction becomes infeasible, retraction-based radius locking introduces a correction that is geometrically misaligned with the model's own update direction. This is exactly the instability mechanism identified earlier in the ORF contraction analysis.

\subsubsection{Comparison Under Large Direction Errors}

The above formulas are exact and do not rely on small-angle approximations. This is essential in the contraction regime, where the model's direction error may remain large during training. We summarize the implications as follows.

\paragraph{Raw Euler step.}
Its exact one-step deviation from the oracle next state is given by Eq.~\eqref{eq:euler_error_exact_R}, while its shell mismatch is given by Eq.~\eqref{eq:euler_radius_error}. In the contraction regime, directional error systematically weakens shrinkage. Therefore, under large angle errors, raw Euler steps can drift substantially away from the intended shell schedule.

\paragraph{Euler + normalize to target radius.}
This operator removes the shell mismatch exactly at each step, so the remaining error is the angular shell error in Eq.~\eqref{eq:EN_shell_error}, with exact shell-angle cosine given by Eq.~\eqref{eq:EN_cos_exact}. In particular, even when the direction error is large, the trajectory remains on the intended radius schedule. Hence this operator is the most natural shell-tracking correction in the contraction regime.

\paragraph{Standard radius locking.}
In the expansion regime, the shell is naturally reachable along the predicted direction, and the exact step length is given by Eq.~\eqref{eq:RL_delta_exact}. The corresponding error with respect to the oracle next state is given by Eq.~\eqref{eq:RL_error_exact}. Since this operator preserves the predicted direction and adjusts only the step length, it is geometrically better aligned with the intended ORF-style expansion dynamics than Euler + normalize.

\paragraph{Retraction-based radius locking in contraction.}
Although oracle-consistent in the feasible case, it becomes geometrically problematic exactly in the regime where contraction is hard: when no feasible contraction exists along the predicted direction, the fallback retraction introduces an update component orthogonal to the predicted direction. This makes it the least attractive operator among the contraction-phase candidates.

\subsubsection{Practical Conclusion}

The exact formulas above suggest the following inference strategy for a standard-RF-trained model with a phase split at $t=1/2$:
\begin{itemize}
\item \textbf{Contraction regime} ($t\in[0,1/2]$):
use a fixed-norm Euler step with $\|v_t\|=\sqrt2 R$, followed by normalization to the target radius $r_{t+h}$ at each step.
This operator exactly matches the oracle update under oracle directions, and under large direction errors it enforces the correct shell schedule without introducing a retraction orthogonal to the model's prediction.

\item \textbf{Expansion regime} ($t\in[1/2,1]$):
use standard radius locking.
This operator also matches the oracle update under oracle directions, and in the non-contraction regime it is the most geometrically faithful way to enforce the target shell while preserving the predicted direction.
\end{itemize}

Taken together, this analysis suggests a simple hybrid rule: \emph{Euler + per-step shell normalization in the contraction regime, and standard radius locking in the expansion regime}. This combination preserves oracle exactness, avoids the geometric pathology of retraction-based contraction, and keeps the trajectory on the intended radius schedule even when contraction-phase direction errors are large.

\subsection{Relaxing Time-Induced Target-Identifiability via Source-Radius Randomization}
\label{subsec:radius_randomization_identifiability}

In the previous subsection, we analyzed several inference operators under a standard RF bridge and showed that radius locking resolves the train--inference mismatch associated with \emph{progress-identifiability}: by explicitly enforcing the target radius schedule, the sampler keeps the generated trajectory on the intended shell even when directional prediction errors are present. However, this does \emph{not} resolve a second and more subtle issue in high-dimensional bridge design, namely that the \emph{target-identifiability} of the bridge state can remain too tightly coupled to time. In this subsection, we formalize this issue and introduce a simple training-time remedy: \emph{source-radius randomization}.

Our central idea is to preserve the standard RF bridge and the test-time fixed-radius initialization, but to inject a controlled amount of training-time variability into the source norm $\|x_0\|_2$. This weakens the deterministic coupling between time and source--target SNR, thereby reducing the model's incentive to infer ``how much target information should already be present'' directly from time (or from the radius, which itself is tightly tied to time under locking). We further motivate a \emph{negatively biased} center-SNR distribution at $t=\frac12$, based on the fact that under imperfect directional prediction, contraction-phase inference with shell projection reaches $t=\frac12$ with an \emph{effective} target SNR that is strictly smaller than the theoretical value $0$.

\subsubsection{Progress-Identifiability and Target-Identifiability}

We first formalize the two notions that are relevant here.

\paragraph{Progress-identifiability.}
A bridge exhibits high \emph{progress-identifiability} if the current state strongly reveals where it lies on the bridge. Under shell-like high-dimensional geometry, the most natural progress statistic is the bridge radius
\begin{equation}
\rho(t) \triangleq \sqrt{\mathbb E[\|x_t\|_2^2]}.
\label{eq:progress_ident_def}
\end{equation}
When $\|x_t\|_2$ concentrates sharply around $\rho(t)$ and $\rho(t)$ is itself a nearly deterministic function of $t$, the current radius becomes an almost perfect progress indicator.

\paragraph{Target-identifiability.}
A bridge exhibits high \emph{target-identifiability} if the current state strongly reveals how much target information it already contains. A natural proxy is the source--target signal-to-noise ratio (SNR) of the bridge state. Under a linear bridge
\begin{equation}
x_t=(1-t)x_0+t x_1,
\label{eq:linear_bridge_snr_ident}
\end{equation}
we define the state-level source--target SNR by
\begin{equation}
\mathrm{SNR}_x(t)
\triangleq
\log\frac{t^2\|x_1\|_2^2}{(1-t)^2\|x_0\|_2^2}.
\label{eq:snr_x_ident}
\end{equation}
This quantity characterizes the relative strength of the target and source contributions in the bridge state.

\subsubsection{Why Time-Induced Identifiability Is Weak in Low Dimensions but Strong in High Dimensions}

The key issue is not merely that $\rho(t)$ and $\mathrm{SNR}_x(t)$ depend on time, but that in high dimensions they can become \emph{too sharply determined} by time.

\paragraph{Low-dimensional RF.}
In standard low-dimensional RF settings, the source is often sampled from a Gaussian,
\begin{equation}
x_0\sim\mathcal N(0,I_d),
\end{equation}
with modest latent dimension $d$ (e.g., $d\le 16$). Then
\begin{equation}
\|x_0\|_2^2\sim \chi_d^2,
\end{equation}
so the source norm exhibits substantial relative fluctuation. As a result, even at a fixed $t$, the bridge radius and the bridge-state SNR remain statistically noisy. In particular, at $t=\frac12$,
\begin{equation}
\mathrm{SNR}_x\!\left(\frac12\right)
=
\log\frac{\|x_1\|_2^2}{\|x_0\|_2^2},
\end{equation}
which is non-degenerate because $\|x_0\|_2$ fluctuates substantially in low dimensions. Consequently, the model cannot reliably infer from $t$ alone how much target information should already be present in the current state.

\paragraph{High-dimensional fixed-shell RF.}
By contrast, in our high-dimensional token setting we use
\begin{equation}
\|x_0\|_2=\|x_1\|_2=R,\qquad R=\sqrt N,
\end{equation}
so Eq.~\eqref{eq:snr_x_ident} reduces to
\begin{equation}
\boxed{
\mathrm{SNR}_x(t)=2\log\frac{t}{1-t}.
}
\label{eq:snr_deterministic_highd}
\end{equation}
Likewise, under the standard RF bridge and the concentration approximation $\langle x_0,x_1\rangle\approx 0$, the radius is
\begin{equation}
\|x_t\|_2
\approx
R\sqrt{(1-t)^2+t^2},
\label{eq:radius_deterministic_highd}
\end{equation}
which is also a deterministic function of $t$.

Thus, in the high-dimensional fixed-shell setting, both progress-identifiability and target-identifiability are strongly tied to time:
\begin{itemize}
\item $\|x_t\|_2$ almost perfectly reveals progress;
\item progress almost perfectly reveals the \emph{theoretical} source--target SNR.
\end{itemize}
This creates a shortcut: the model can learn to infer from time (or equivalently, from the shell radius) how much target information \emph{should} be present, rather than genuinely inferring how much target information is \emph{actually} present in the current state.

\paragraph{Why this is problematic at inference.}
At inference, directional prediction errors perturb the state away from the oracle bridge even when the radius schedule is perfectly enforced. In particular, in the contraction regime, the generated state can remain \emph{more source-dominated} than the theoretical bridge state associated with that same time. If the model has learned to trust the theoretical time--SNR relation too strongly, it may interpret source-biased residual structure or even accumulated error as target evidence, thereby amplifying error over steps. In other words, radius locking resolves the progress mismatch, but it does not by itself resolve the shortcut that ties \emph{target-identifiability} too tightly to time.

\subsubsection{Training-Time Source-Radius Randomization}

To weaken the deterministic time--SNR shortcut without changing the test-time bridge geometry, we randomize the source radius during training.

\paragraph{Definition.}
We sample
\begin{equation}
x_0 = \rho_0\,u,
\qquad
u\sim \mathrm{Unif}(\mathbb S^{N-1}(1)),
\label{eq:x0_radius_randomized}
\end{equation}
where $\rho_0$ is a scalar random variable with controlled support and mean, while keeping the target fixed on the token shell:
\begin{equation}
x_1\in \mathbb S^{N-1}(R).
\end{equation}
At inference time, however, we still start from the fixed shell
\begin{equation}
x_0^{\mathrm{test}}\sim \mathrm{Unif}(\mathbb S^{N-1}(R)),
\end{equation}
so the test-time geometry remains unchanged and compatible with the shell-based locking operators.

\paragraph{Effect on state-level SNR.}
Under Eq.~\eqref{eq:linear_bridge_snr_ident}, the state-level SNR becomes
\begin{equation}
\mathrm{SNR}_x(t;\rho_0)
=
\log\frac{t^2R^2}{(1-t)^2\rho_0^2}
=
2\log\frac{t}{1-t}
+
2\log\frac{R}{\rho_0}.
\label{eq:snr_radius_randomized}
\end{equation}
Thus the deterministic schedule in Eq.~\eqref{eq:snr_deterministic_highd} is replaced by a random offset:
\begin{equation}
\boxed{
\mathrm{SNR}_x(t;\rho_0)
=
\mathrm{SNR}_{\mathrm{det}}(t)+\varepsilon_{\mathrm{snr}},
\qquad
\varepsilon_{\mathrm{snr}}=2\log\frac{R}{\rho_0}.
}
\label{eq:snr_random_offset}
\end{equation}
This directly weakens the model's ability to infer the current target-information level from time alone.

\paragraph{Design goal.}
The purpose of source-radius randomization is not to create a train--test mismatch in the undesirable sense. Rather, it is a deliberate \emph{coverage expansion} mechanism, analogous in spirit to noise augmentation or dropout: during training, we enlarge the family of states that correspond to a given nominal time, so that the model cannot overfit to a brittle time-induced target-identifiability shortcut and must instead rely more on the actual content of $x_t$.

\subsubsection{Calibrating the Center SNR Variance by Low-Dimensional RF}

A natural design question is how large the randomization of $\rho_0$ should be. Instead of treating this as a purely heuristic hyperparameter, we propose calibrating it using a low-dimensional RF reference.

\paragraph{Low-dimensional reference variance at $t=\frac12$.}
Suppose in a low-dimensional RF system the source is Gaussian,
\begin{equation}
x_0^{\mathrm{low}}\sim\mathcal N(0,I_d),
\end{equation}
and the target has typical norm $\|x_1^{\mathrm{low}}\|_2^2\approx d$. Then at $t=\frac12$,
\begin{equation}
\mathrm{SNR}_x^{\mathrm{low}}\!\left(\frac12\right)
\approx
\log\frac{d}{\|x_0^{\mathrm{low}}\|_2^2}.
\end{equation}
Since $\|x_0^{\mathrm{low}}\|_2^2\sim \chi_d^2$, we obtain
\begin{equation}
\boxed{
\mathrm{Var}\!\left[\mathrm{SNR}_x^{\mathrm{low}}\!\left(\frac12\right)\right]
=
\mathrm{Var}[\log \chi_d^2]
=
\psi_1(d/2),
}
\label{eq:lowd_var_target}
\end{equation}
where $\psi_1$ is the trigamma function.

\paragraph{High-dimensional randomized-shell variance at $t=\frac12$.}
Under Eq.~\eqref{eq:snr_radius_randomized},
\begin{equation}
\mathrm{SNR}_x\!\left(\frac12;\rho_0\right)
=
2\log\frac{R}{\rho_0},
\end{equation}
so
\begin{equation}
\boxed{
\mathrm{Var}\!\left[\mathrm{SNR}_x\!\left(\frac12\right)\right]
=
4\,\mathrm{Var}[\log \rho_0].
}
\label{eq:highd_center_var}
\end{equation}
This suggests a simple calibration principle:
\begin{equation}
\boxed{
4\,\mathrm{Var}[\log \rho_0]
\approx
\psi_1(d_{\mathrm{eff}}/2),
}
\label{eq:variance_alignment}
\end{equation}
where $d_{\mathrm{eff}}$ is an \emph{effective low dimension}. In practice, however, we do not force an exact match to a preselected low-dimensional system. Instead, we first choose a practically acceptable source-radius range, compute the resulting center-SNR variance, and then interpret that variance in terms of the corresponding effective low dimension.

\subsubsection{Why the Center SNR Should Be Biased Toward Negative Values}

The center region $t=\frac12$ is special: under the theoretical bridge, it is exactly the source--target balance point, so Eq.~\eqref{eq:snr_deterministic_highd} gives
\begin{equation}
\mathrm{SNR}_{\mathrm{det}}\!\left(\frac12\right)=0.
\end{equation}
However, under practical inference with directional errors in the contraction regime, the actual state that reaches $t=\frac12$ is \emph{not} balanced in this way. We now formalize this point.

\paragraph{A geometric proxy for effective SNR sign.}
Let $v^\star=x_1-x_0$ and $r^\star=v^\star/\|v^\star\|_2$ as before. For any state $z$ on the midpoint shell $\|z\|_2=R/\sqrt2$, define
\begin{equation}
\Delta(z)\triangleq \langle z,x_1\rangle-\langle z,x_0\rangle.
\label{eq:delta_z_def}
\end{equation}
Since $x_1-x_0=v^\star$, we have
\begin{equation}
\Delta(z)=\langle z,v^\star\rangle = \|v^\star\|_2\,\langle z,r^\star\rangle.
\label{eq:delta_z_rstar}
\end{equation}
Thus:
\begin{itemize}
\item $\Delta(z)>0$ means $z$ is target-dominant (effective SNR $>0$);
\item $\Delta(z)=0$ means balanced (effective SNR $=0$);
\item $\Delta(z)<0$ means source-dominant (effective SNR $<0$).
\end{itemize}

For the oracle midpoint $x_{1/2}^\star=\frac12(x_0+x_1)$, we have
\begin{equation}
\langle x_{1/2}^\star,r^\star\rangle = 0,
\end{equation}
so its effective SNR is exactly zero.

\paragraph{Contraction-phase inference with fixed-norm Euler + shell projection.}
Now consider contraction-phase inference using the operator analyzed in Sec.~\ref{subsec:radius_locking_analysis}:
\begin{equation}
\tilde x_{t+h}=x_t+hL\hat r,
\qquad
x_{t+h}
=
r_{t+h}\frac{\tilde x_{t+h}}{\|\tilde x_{t+h}\|_2},
\label{eq:contraction_update_recalled}
\end{equation}
where $L=\|v^\star\|_2\approx \sqrt2 R$ and $\hat r$ is the predicted unit direction. Suppose
\begin{equation}
\angle(\hat r,r^\star)=\theta_t,
\qquad
0<\theta_t<\frac{\pi}{2},
\end{equation}
so that $\langle \hat r,r^\star\rangle=\cos\theta_t<1$.

Before projection,
\begin{equation}
\langle \tilde x_{t+h},r^\star\rangle
=
\langle x_t,r^\star\rangle + hL\cos\theta_t,
\end{equation}
whereas the oracle increment would be
\begin{equation}
\langle x_{t+h}^\star,r^\star\rangle
=
\langle x_t,r^\star\rangle + hL.
\end{equation}
Hence
\begin{equation}
\langle \tilde x_{t+h},r^\star\rangle
<
\langle x_{t+h}^\star,r^\star\rangle
\qquad\text{whenever }\theta_t>0.
\label{eq:preproj_progress_less}
\end{equation}

After projection,
\begin{equation}
x_{t+h}
=
\gamma_t \tilde x_{t+h},
\qquad
\gamma_t=\frac{r_{t+h}}{\|\tilde x_{t+h}\|_2}.
\end{equation}
In the contraction regime, directional error weakens contraction, so $\|\tilde x_{t+h}\|_2>r_{t+h}$ and therefore
\begin{equation}
0<\gamma_t<1.
\end{equation}
Thus
\begin{equation}
\langle x_{t+h},r^\star\rangle
=
\gamma_t\langle \tilde x_{t+h},r^\star\rangle
<
\langle \tilde x_{t+h},r^\star\rangle
<
\langle x_{t+h}^\star,r^\star\rangle.
\label{eq:projected_progress_less}
\end{equation}

Starting from
\begin{equation}
\langle x_0,r^\star\rangle = -\frac{R}{\sqrt2}<0,
\end{equation}
and iterating Eq.~\eqref{eq:projected_progress_less} over the entire contraction regime up to $t=\frac12$, we obtain
\begin{equation}
\boxed{
\langle x_{1/2}^{\mathrm{inf}},r^\star\rangle < 0
}
\label{eq:midpoint_negative_progress}
\end{equation}
whenever the contraction-phase predictor is not oracle-perfect. By Eq.~\eqref{eq:delta_z_rstar}, this implies
\begin{equation}
\boxed{
\Delta(x_{1/2}^{\mathrm{inf}})<0,
}
\qquad\Longleftrightarrow\qquad
\boxed{
\mathrm{SNR}_{\mathrm{eff}}(x_{1/2}^{\mathrm{inf}})<0.
}
\label{eq:midpoint_negative_snr}
\end{equation}

\paragraph{Interpretation.}
Equation~\eqref{eq:midpoint_negative_snr} shows that under realistic contraction-phase inference, the actual center state is generically \emph{more source-dominant} than the theoretical bridge midpoint. Therefore, a training distribution in which $t=\frac12$ corresponds almost deterministically to SNR $=0$ is actually \emph{misaligned} with the states the model will encounter at inference. This motivates not only adding variance to the center-SNR distribution, but also biasing that distribution so that negative SNR values occur with high probability.

\subsubsection{Choice of Source-Radius Distribution}

We next describe a simple bounded single-parameter family that implements the above idea.

\paragraph{Bounded Beta family.}
We define
\begin{equation}
\rho_0 = L + (U-L)Y,
\qquad
Y\sim \mathrm{Beta}(\alpha,1),
\qquad
\alpha>1,
\label{eq:beta_radius_family}
\end{equation}
where $L$ is a fixed lower bound and $U$ is chosen so that
\begin{equation}
\mathbb E[\rho_0]=R.
\label{eq:radius_mean_constraint}
\end{equation}
Since
\begin{equation}
\mathbb E[Y]=\frac{\alpha}{\alpha+1},
\end{equation}
Eq.~\eqref{eq:radius_mean_constraint} gives
\begin{equation}
L+(U-L)\frac{\alpha}{\alpha+1}=R,
\end{equation}
hence
\begin{equation}
\boxed{
U=\frac{(\alpha+1)R-L}{\alpha}.
}
\label{eq:U_from_alpha_L}
\end{equation}

If we parameterize the lower bound by
\begin{equation}
L=\lambda R,\qquad 0<\lambda<1,
\end{equation}
then
\begin{equation}
\boxed{
\frac{U}{R}=\frac{\alpha+1-\lambda}{\alpha}
=
1+\frac{1-\lambda}{\alpha}.
}
\label{eq:U_over_R}
\end{equation}

\paragraph{Why fix the lower bound.}
Fixing a lower bound such as $L=0.8R$ serves two purposes. First, it keeps the source-radius randomization within a moderate and controllable range. Second, it prevents $\|x_0\|_2$ from becoming too small, which would make
\begin{equation}
v^\star=x_1-x_0
\end{equation}
nearly determined by $x_1$ alone and thereby shift the training dynamics toward a degenerate $x$-prediction-like regime rather than a proper transport-direction regime.

\paragraph{Why use $\mathrm{Beta}(\alpha,1)$.}
The choice $\mathrm{Beta}(\alpha,1)$ has three practical advantages:
\begin{enumerate}[leftmargin=2.0em,label=(\roman*)]
\item it is a single-parameter family, so $\alpha$ can be tuned by a simple grid search;
\item for $\alpha>1$, it places more mass near the upper end of the interval, thereby increasing the probability that $\rho_0>R$ and thus that the center SNR is negative;
\item together with Eq.~\eqref{eq:U_from_alpha_L}, it allows the mean radius to remain fixed at $R$ without introducing additional free parameters.
\end{enumerate}

\paragraph{Design summary.}
We therefore adopt the following logic:
\begin{itemize}
\item fix a moderate lower bound $L=\lambda R$ (e.g., $\lambda=0.8$);
\item choose $\alpha>1$ as the primary hyperparameter;
\item set the upper bound $U$ by Eq.~\eqref{eq:U_from_alpha_L};
\item train with $x_0=\rho_0 u$, where $\rho_0$ is sampled from Eq.~\eqref{eq:beta_radius_family}.
\end{itemize}
This yields a bounded source-radius distribution with mean $R$, increased center-SNR variance, and a higher probability of negative SNR at $t=\frac12$, which better matches the practical inference behavior induced by contraction-phase directional errors.

\paragraph{Overall conclusion.}
Source-radius randomization weakens the deterministic time--SNR shortcut of high-dimensional fixed-shell RF while preserving the shell geometry used at test time. By calibrating the center-SNR variance to a low-dimensional RF reference and biasing the center SNR toward negative values, the resulting training distribution better matches the effective source-dominant center states encountered under realistic inference. In this sense, the proposed randomization acts not as an undesirable train--test mismatch, but as a robustness-oriented expansion of the training state distribution that directly targets time-induced exposure bias.

\subsection{Time Sampling, Time Embeddings, and the Role of Nominal versus Actual Progress}
\label{subsec:time_sampling_time_emb}

The analyses in the previous subsections suggest that, once inference is changed from standard RF Euler sampling to a direction-only, locked-step procedure, two design choices that are often treated as routine in standard RF---the \emph{time sampling distribution} during training and the use of \emph{explicit time embeddings}---must be re-examined jointly. The key reason is that both choices are closely tied to how the model acquires and uses \emph{progress information}. In particular, under standard RF with a fixed-shell source and target, the nominal bridge time $t$ simultaneously determines (i) the expected geometric progress along the bridge and (ii) the expected source--target information balance in $x_t$. If the model has access to explicit time embeddings, then this nominal progress information becomes available through a shortcut channel that may dominate over the actual information contained in $x_t$. This issue is further affected by the training-time sampling density over $t$, especially in the small-$t$ regime where the prediction problem is intrinsically harder.

We therefore revisit these two ingredients together. We first analyze why the standard logit-normal time sampling schedule is well matched to \emph{standard} $v$-prediction RF with standard Euler inference, but may become suboptimal once inference uses fixed step norms or radius locking. We then discuss what information the model actually needs in an RF bridge, and argue that for RF-like time-independent direction targets, explicit time embeddings are not only unnecessary in principle, but can also become a nominal-progress shortcut that interferes with the intended robustness of the model. This viewpoint also changes how one should think about source-radius randomization: if the primary source of the over-strong time--SNR binding is the explicit time channel, then removing time embeddings may already address the issue at its root, potentially reducing or eliminating the need for additional radius perturbation of $x_0$.

\subsubsection{Why Logit-Normal Time Sampling Is Reasonable in Standard RF}

We begin with the standard RF setting with $v$-prediction and standard Euler inference. Recall that under the standard RF bridge
\begin{equation}
x_t=(1-t)x_0+t x_1,
\qquad
v^\star=x_1-x_0,
\label{eq:rf_bridge_time_sampling}
\end{equation}
the bridge state contains very little target information when $t$ is close to $0$. As a result, the posterior $p(x_1\mid x_t)$ is broad in the small-$t$ regime, making the direction of $v^\star$ intrinsically harder to infer from $x_t$. In contrast, at larger $t$, the target contribution is stronger and the posterior narrows, so the model can more easily identify the correct transport direction. This asymmetry is routinely observed in practice through lower training loss at larger $t$ than at smaller $t$.

Under standard full-vector $v$-prediction, this directional difficulty is coupled to magnitude shrinkage. If the predicted direction deviates from the oracle direction by angle $\theta$, then the optimal predicted magnitude under the $\ell_2$ objective is
\begin{equation}
\hat s_{\mathrm{opt}}=s^\star\cos\theta,
\end{equation}
so larger angular errors lead automatically to smaller predicted step magnitudes. Therefore, in the small-$t$ regime where the direction error is typically larger, standard $v$-prediction naturally produces smaller effective Euler updates. While this under-stepping is undesirable from the perspective of exact bridge simulation, it has a stabilizing side effect: it prevents the earliest and most uncertain updates from moving too far away from the source. In other words, under standard RF with standard Euler inference, the model's intrinsic uncertainty at small $t$ is partially converted into conservative step sizes.

This observation explains why the commonly used logit-normal $t$-sampling distribution can work well in standard RF. Logit-normal sampling places most probability mass away from the endpoints $t=0$ and $t=1$, and especially under-samples the small-$t$ region. In a standard $v$-prediction setting, this is not necessarily harmful: the under-sampled small-$t$ region is also the regime in which the model would naturally take very small steps at inference time due to under-stepping. Thus, the training deficiency near $t=0$ is partly compensated by conservative inference dynamics. Moreover, classifier-free guidance (CFG) often has an effective norm-amplification effect through vector extrapolation, so some of the early under-stepping can be partially compensated later in the trajectory when predictions are already more accurate. This leads to a self-consistent picture:
\begin{itemize}
\item small-$t$ prediction is difficult and receives relatively little training budget;
\item the corresponding Euler steps are naturally short because of under-stepping;
\item mid-to-late trajectory predictions are more accurate and can absorb part of the missing progress;
\item CFG further amplifies later updates, providing an implicit partial correction.
\end{itemize}
Therefore, in the \emph{standard} RF setting, logit-normal time sampling is not merely an arbitrary convenience; it is implicitly compatible with the conservative early-time behavior induced by standard $v$-prediction.

\subsubsection{Why This Logic Changes under Fixed-Norm Locking Inference}

The above rationale no longer applies once inference is changed from standard Euler updates with predicted vector norms to direction-only updates with \emph{fixed} step norm (in the contraction regime) or \emph{radius locking} (in the expansion regime). In our current formulation, the contraction regime uses fixed-norm Euler updates with prescribed norm $\|v_t\|\approx \sqrt2R$, followed by projection to the target shell, while the expansion regime uses radius locking. In such a setting, the model no longer has the freedom to respond to large uncertainty by shrinking the step norm. Hence the stabilizing side effect of standard under-stepping disappears.

This creates a new mismatch if training still uses the same logit-normal time sampling schedule. The small-$t$ regime remains intrinsically harder, but it is still under-sampled during training; meanwhile, inference in that regime now enforces a significantly larger effective step than standard $v$-prediction would have produced. As a result, the earliest updates become both \emph{poorly learned} and \emph{geometrically consequential}. This is precisely the opposite of the standard RF situation, where the earliest updates are poorly learned but also naturally small.

Consequently, once fixed-norm locking is introduced, the rationale for logit-normal $t$-sampling weakens substantially. The model is now required to make accurate directional decisions in precisely the regime where the posterior is broadest and where standard RF would otherwise have relied on under-stepping to avoid catastrophic early errors. This suggests that training should allocate \emph{more} budget to small $t$, not less. A natural alternative is to use a training-time distribution that biases sampling toward early times, for example a Beta family such as
\begin{equation}
t \sim \mathrm{Beta}(1,\tau),
\qquad \tau>1,
\end{equation}
which places more mass near $t=0$ while still covering the full interval. Such a change aligns training with the new inference requirement: if the contraction phase uses fixed step norms and therefore cannot avoid taking nontrivial steps, then the directional predictor must be trained more aggressively in the small-$t$ regime.

The same logic applies to the inference time grid itself. If fixed-norm Euler updates are used in the contraction phase, then a uniform time grid produces unnecessarily large early steps exactly where the directional uncertainty is largest. A more suitable strategy is therefore to use a non-uniform inference grid that is denser near $t=0$ and coarser at larger $t$, e.g.,
\begin{equation}
t_k = \left(\frac{k}{K}\right)^\gamma,
\qquad \gamma>1,
\end{equation}
so that the earliest steps are shortened while later, easier regions can be traversed more aggressively. In summary, once inference uses fixed norm or shell-locking operators, both training-time $t$-sampling and inference-time discretization should be re-designed to allocate \emph{more resolution to small $t$}, not less.

\subsubsection{Nominal Progress versus Actual Progress}

The above discussion about time sampling is tightly connected to a deeper issue: \emph{what kind of progress information the model actually uses}. In RF-like bridges, one can distinguish two notions of progress:
\begin{enumerate}[leftmargin=2.0em,label=(\roman*)]
\item \textbf{Nominal time progress:} where the state lies along the bridge according to the external time variable $t$;
\item \textbf{Actual information progress:} how much target information is actually present in the current state $x_t$.
\end{enumerate}
In the standard RF bridge with fixed source and target norms, these two notions are strongly coupled in expectation: the bridge radius and the source--target signal-to-noise ratio (SNR) are both nearly deterministic functions of $t$ in high dimensions. This creates the possibility of a time-induced shortcut: instead of inferring target information from the actual content of $x_t$, the model may simply use nominal time as a lookup variable that tells it how much target information \emph{should} be present.

At first glance, one may think that this shortcut is harmless or even necessary, because the bridge radius $\|x_t\|$ is symmetric around $t=1/2$, so a given norm does not uniquely identify whether the model is in the contraction or expansion phase. However, this ambiguity exists only at the level of the scalar radius. The model does not observe merely $\|x_t\|$; it observes the full high-dimensional vector $x_t$. In many signal restoration problems, including denoising models for audio and images, the model can recover the clean target without being explicitly told the input SNR or the noise type. What matters is not a scalar global progress label, but whether the input representation itself contains enough structure for the model to identify which components belong to the clean target.

The same reasoning applies here. If the model can identify which components of $x_t$ correspond to the target $x_1$, then it can in principle infer the actual target-information level directly from $x_t$ itself. Put differently, if the model is capable of recovering $x_1$ (or the direction toward it), then the actual source--target balance is already encoded in the input. This suggests that explicit time may not be needed to determine where the model is on the bridge in any operational sense. The model does not necessarily need to know the exact scalar value of $t$; it needs to know \emph{which bridge it is on} and \emph{what target-relevant information is currently present in the observed state}.

\subsubsection{Why Explicit Time Embeddings Become a Shortcut in RF-like Bridges}

The above distinction becomes especially important because explicit time embeddings provide a direct nominal-progress signal. When such a signal is available, optimization tends to use it as the cheapest route to disambiguate the current bridge phase and to infer the expected target-information level. This is a general form of shortcut behavior: if the same information can be obtained either from a difficult mapping of $x_t$ or from an explicit low-dimensional side channel, the model tends to rely on the side channel.

In our setting, this shortcut is especially problematic because the nominal time variable does not merely indicate where the model is on the bridge; it also implicitly specifies what the bridge statistics \emph{should} be. Hence the model may learn to use time embeddings not only to identify the current phase, but also to decide how much target-like structure should be extracted from $x_t$. This is exactly the mechanism underlying the time-induced SNR shortcut discussed earlier.

A useful way to think about this is through a residual-prediction perspective. In many architectures with strong residual pathways, the model output can be viewed informally as a correction added to the input. If the network can identify target-like structure in $x_t$, then a simple optimization route is to learn a residual that subtracts or reweights the target component in a way that aligns with the desired transport direction. Under this view, the relevant problem is not to ``estimate $t$'' explicitly, but to determine \emph{how target-like the current input is}. If time embeddings are present, the model can use them to decide how aggressively it should interpret parts of $x_t$ as belonging to $x_1$. If time embeddings are removed, the model is forced to base this decision on the actual content of $x_t$.

This observation also explains why explicit time embeddings are bridge-dependent. In bridges such as SFM or VP-style trigonometric paths, the oracle velocity field itself is explicitly time-dependent, so time embeddings are naturally useful and often necessary. In contrast, under standard RF and ORF-like bridges, the target direction $x_1-x_0$ is time-independent. In such settings, explicit time embeddings are not needed to define the oracle direction field; their main role is to supply nominal progress information. If this nominal information becomes a shortcut, then removing time embeddings may improve train--inference alignment rather than harm it.

\subsubsection{Empirical Motivation from Time-Independent versus Time-Dependent Bridges}

This interpretation is consistent with our empirical observations in earlier experiments. In ORF-like settings, where the target direction is time-independent, removing explicit time embeddings had essentially no effect on the training loss or prediction quality, and the norm of the time-embedding pathway did not show systematic variation across time. In contrast, in SFM-like settings where the target vector field is explicitly time-dependent, the time-embedding pathway became significantly more active, especially at larger $t$. This suggests that the model uses time embeddings when they are functionally necessary for describing the target field, but does not benefit from them in the same way when the target direction is inherently time-independent.

This difference is highly relevant here. Since our current formulation is based on an RF-like bridge with direction-only prediction of a time-independent target direction, the model should in principle be able to infer the relevant transport information directly from $x_t$. If so, explicit time embeddings are not only unnecessary, but may also reintroduce exactly the nominal-progress shortcut that we seek to suppress.

\subsubsection{Implication for Source-Radius Randomization}

The above joint analysis also changes how one should interpret source-radius randomization. Earlier, one may be tempted to randomize the source radius $\|x_0\|$ during training in order to break the near-deterministic relation between $t$ and the source--target SNR of $x_t$. This can indeed increase the variance of the actual target-information level at a fixed nominal time and thereby weaken the time-induced shortcut.

However, if explicit time embeddings are removed, then the main route by which the model could directly exploit the nominal time--SNR relation is already suppressed. In that case, the model must infer target-information progress primarily from the actual observed state $x_t$, not from an explicit time side channel. This substantially reduces the need to artificially perturb the source radius for the sole purpose of destroying the time--SNR binding. In other words, if the root problem is that the model overuses explicit nominal time information, then removing explicit time embeddings may address this issue more directly than source-radius randomization.

This does not mean that source-radius randomization is always useless. It may still serve as a robustness augmentation or as a way to further enlarge the range of target-information patterns seen during training. But it is no longer required as the primary mechanism for defeating the time-induced SNR shortcut. Once explicit time embeddings are removed, the necessity of such perturbation becomes an empirical question rather than a conceptual requirement.

\subsubsection{Practical Conclusion}

Taken together, the above reasoning suggests the following design principle for RF-like direction-only bridges with fixed-norm or radius-locking inference:
\begin{enumerate}[leftmargin=2.0em,label=(\roman*)]
\item \textbf{Revisit time sampling when inference no longer under-steps automatically.}
In standard RF, logit-normal time sampling is compatible with the conservative early-time behavior induced by standard $v$-prediction. Once inference uses fixed step norms, this compatibility disappears. Therefore, small-$t$ regions should receive \emph{more} training coverage and \emph{finer} inference discretization.

\item \textbf{Distinguish nominal time from actual information progress.}
The model does not need a scalar phase label if the full state $x_t$ already contains enough structure to infer target-relevant information. In RF-like bridges, actual information progress can in principle be inferred directly from $x_t$.

\item \textbf{Remove explicit time embeddings by default in RF-like time-independent bridges.}
Since the oracle target direction is time-independent, explicit time embeddings are not functionally necessary for defining the prediction target. Their main effect is to provide nominal progress information, which can become a shortcut. Removing them forces the model to rely on the actual observed content of $x_t$.

\item \textbf{Re-evaluate the need for source-radius perturbation after removing time embeddings.}
If the primary source of the time-induced SNR shortcut is the explicit time channel, then removing time embeddings may already resolve most of the issue, making source-radius perturbation optional rather than mandatory.
\end{enumerate}

Therefore, in our current formulation, we adopt the following default view: for RF-like bridges with time-independent direction targets, explicit time embeddings should be removed by default, training-time $t$ sampling should allocate more mass to the small-$t$ regime than standard logit-normal schedules, and inference should use a non-uniform time grid with finer resolution near $t=0$. Under this view, source-radius randomization becomes an optional robustness augmentation rather than a necessary ingredient for suppressing time-induced shortcuts.

==> sections_old/REF.tex <==
\section{A High-Dimensional Bridge Design Framework for Direction-only Flow Matching}
\label{sec:REF}

We now revisit continuous flow matching from the viewpoint of \emph{learnability-aware bridge design} in high-dimensional token spaces. Our starting point is that, in such spaces, a bridge does more than define a transport path between a source and a target. It also determines what information an intermediate state $x_t$ carries about (i) \emph{where it lies on the bridge}, (ii) \emph{how much target information it already contains}, and---crucially for learning---(iii) how these state statistics relate to \emph{what the model is asked to predict}. In a direction-only framework, the model does not regress the bridge state itself, but rather the \emph{direction field} associated with it. Therefore, what matters for learnability is not only the geometry of the bridge states, but the \emph{joint structure} of the model input $x_t$ and the oracle target direction field $v_t^\star$.

This perspective differs slightly from standard bridge design discussions that focus primarily on transport geometry. In our setting, we are equally concerned with \emph{training dynamics}: what shortcuts the model can exploit, what information the model can reliably infer from $x_t$, and whether the learned rule remains stable once the inference trajectory deviates from the ideal training bridge. This learnability view is consistent with the rest of our framework: in the tokenizer, we shape the token space so that local neighborhoods are traversable and decodable; in the AR generator, we route conditioning and residual guidance so that the model learns stable functional roles rather than brittle overlaps. Here, on the flow side, we similarly seek a bridge whose state statistics and target statistics are jointly easy to learn and robust at inference.

This section is organized as follows. We first introduce two high-dimensional notions---\emph{progress-identifiability} and \emph{target-identifiability}---as state-level proxies that affect learnability under a general bridge, and use them to compare standard RF, standard VP, and spherical flow matching (SFM) in high dimensions. We then show that high-dimensional concentration creates a tension: identifiability can help learning, but if it becomes too rigidly tied to time, it also induces shortcut solutions. We next revisit the under-stepping pathology of standard $v$-prediction from a \emph{bridge-agnostic} perspective, and explain how under-stepping and time-induced shortcuts together create train--inference mismatch. This motivates direction-only inference with \emph{radius locking}, which explicitly stabilizes the inference geometry. Once a nontrivial progress schedule is introduced, however, the bridge-state statistics and the direction-field statistics become coupled through that schedule. We therefore redesign the source--target mixing geometry directly under the chosen progress schedule, analyze why standard RF- and VP-style mixings become problematic, and derive a closed-form bridge under linear radius expansion whose bridge-state SNR and direction-field SNR retain a simple, smooth, VP-like relation while recovering the standard VP bridge as the limiting case $a\to 1$.

\subsection{State statistics as learnability proxies in high dimensions}
\label{subsec:ref_identifiability_full}

Consider a general bridge
\begin{equation}
x_t=\alpha(t)x_0+\beta(t)x_1,\qquad t\in[0,1],
\label{eq:bridge_general_full}
\end{equation}
with boundary conditions
\begin{equation}
\alpha(0)=1,\ \beta(0)=0,\qquad
\alpha(1)=0,\ \beta(1)=1.
\label{eq:bridge_bc_general_full}
\end{equation}
We assume that the target token lies on the token sphere
\begin{equation}
x_1\in\mathbb S^{N-1}(R),\qquad R=\sqrt N,
\label{eq:x1_sphere_full}
\end{equation}
and for now we only assume that the source distribution is \emph{concentrated} in high dimensions, without imposing any inner-shell radius parameterization yet. The inner-shell / radius-expansion setting will be introduced later only after discussing inference stability and the need for a monotone progress schedule.

In high dimensions, an intermediate state $x_t$ can carry two particularly important types of information that directly affect how easy it is for a model to learn the flow.

\paragraph{Progress-identifiability.}
We define the \emph{progress-identifiability} of a bridge as how well the current state reveals \emph{where it lies on the bridge}. Since shell-like high-dimensional distributions are most naturally organized by radius, we define the bridge progress schedule by the expected radius
\begin{equation}
\rho(t)
\;\triangleq\;
\sqrt{\mathbb E\big[\|x_t\|_2^2\big]}.
\label{eq:rho_def_full}
\end{equation}
Thus $\rho(t)$ is a \emph{statistical} radius schedule rather than a sample-wise exact identity. From a learning viewpoint, progress-identifiability reflects how strongly a state statistic such as radius acts as a cue for bridge progress.

\paragraph{Target-identifiability.}
We define the \emph{target-identifiability} of a bridge as how well the current state reveals \emph{how much target information it already contains}. A natural proxy is a source--target signal-to-noise ratio (SNR). Since the source contribution can itself be random, we define the \emph{mean} target-information schedule by
\begin{equation}
\overline{\mathrm{SNR}}(t)
\;\triangleq\;
\mathbb E\!\left[
\log
\frac{\beta(t)^2\|x_1\|_2^2}{\alpha(t)^2\|x_0\|_2^2}
\right].
\label{eq:snr_mean_def_full}
\end{equation}
This quantity measures the expected amount of target information contained in the bridge state. From a learnability viewpoint, it reflects how strongly the bridge state reveals the source--target balance that the model should act upon.

\paragraph{High-dimensional concentration.}
To understand why these notions matter especially in high dimensions, expand the bridge norm:
\begin{equation}
\|x_t\|_2^2
=
\alpha(t)^2\|x_0\|_2^2+\beta(t)^2\|x_1\|_2^2+2\alpha(t)\beta(t)\langle x_0,x_1\rangle.
\label{eq:norm_expand_full}
\end{equation}
When $x_0$ and $x_1$ are sampled independently from concentrated high-dimensional distributions with bounded norms, the cross term is negligible relative to the shell energies, so
\begin{equation}
\|x_t\|_2^2
\approx
\alpha(t)^2\|x_0\|_2^2+\beta(t)^2\|x_1\|_2^2.
\label{eq:norm_concentrated_full}
\end{equation}
If in addition both endpoint norms are sharply concentrated, then
\begin{equation}
\rho(t)^2
=
\mathbb E[\|x_t\|_2^2]
\approx
\alpha(t)^2\mathbb E[\|x_0\|_2^2]+\beta(t)^2R^2.
\label{eq:rho_mean_full_general}
\end{equation}
Likewise,
\begin{equation}
\overline{\mathrm{SNR}}(t)
\approx
\log\frac{\beta(t)^2R^2}{\alpha(t)^2\,\mathbb E[\|x_0\|_2^2]}.
\label{eq:snr_mean_concentrated_full_general}
\end{equation}
Hence, in high dimensions, both the \emph{mean progress-identifiability} and the \emph{mean target-identifiability} can become sharply regular functions of time.

\paragraph{Why the variances matter for learnability.}
The mean schedules in Eqs.~\eqref{eq:rho_mean_full_general}--\eqref{eq:snr_mean_concentrated_full_general} are not the whole story. Their conditional variances,
\begin{equation}
\mathrm{Var}\!\big(\|x_t\|_2^2\mid t\big),
\qquad
\mathrm{Var}\!\big(\mathrm{SNR}(x_t)\mid t\big),
\label{eq:ident_variances_full}
\end{equation}
determine how rigidly progress-identifiability and target-identifiability are tied to time. In low-dimensional spaces these variances are naturally larger, so time does not sharply determine the bridge statistics. In high-dimensional spaces they can become unusually small, making both progress and target-information levels appear almost deterministic given $t$. This can help learning by reducing ambiguity, but it can also make training dynamics vulnerable to shortcuts: the model may learn to interpret states primarily through the \emph{expected} bridge statistics associated with time rather than through the actual content of the state.

In this sense, identifiability is useful but not sufficient. Good bridge design should make state statistics informative enough to support learning, while avoiding an overly rigid time-to-statistics coupling that encourages shortcut solutions. This tension will be central to the design of REF.

\subsection{Three canonical bridges under high-dimensional concentration}
\label{subsec:ref_canonical_bridges}

The above notions provide a unified way to compare several standard bridge constructions from the viewpoint of learnability-relevant state statistics.

\paragraph{Standard RF.}
For the standard rectified-flow interpolation
\begin{equation}
x_t=(1-t)x_0+t x_1,
\end{equation}
we have
\begin{equation}
\alpha(t)=1-t,\qquad \beta(t)=t.
\end{equation}
Under the high-dimensional approximation $\langle x_0,x_1\rangle\approx 0$ and assuming both endpoints have comparable concentrated norm $\approx R$, the mean progress schedule satisfies
\begin{equation}
\rho_{\mathrm{RF}}(t)^2
\approx
R^2\big((1-t)^2+t^2\big),
\end{equation}
which is minimized near $t=\frac12$. Thus standard RF exhibits a \emph{contraction--expansion} behavior in expected radius. Its mean bridge-state SNR is
\begin{equation}
\overline{\mathrm{SNR}}_{\mathrm{RF}}(t)
\approx
\log\frac{t^2}{(1-t)^2}
=
2\log\frac{t}{1-t}.
\end{equation}
Hence target-identifiability is monotone, but progress-identifiability is non-monotone in radius.

\paragraph{Standard VP.}
For the standard VP-style trigonometric bridge
\begin{equation}
x_t=\cos\!\Big(\frac{\pi t}{2}\Big)x_0+\sin\!\Big(\frac{\pi t}{2}\Big)x_1,
\end{equation}
we have
\begin{equation}
\alpha(t)=\cos\!\Big(\frac{\pi t}{2}\Big),\qquad
\beta(t)=\sin\!\Big(\frac{\pi t}{2}\Big).
\end{equation}
Again under $\langle x_0,x_1\rangle\approx 0$ and comparable endpoint norms $\approx R$, the mean progress schedule becomes
\begin{equation}
\rho_{\mathrm{VP}}(t)^2
\approx
R^2\Big(\cos^2\!\Big(\frac{\pi t}{2}\Big)+\sin^2\!\Big(\frac{\pi t}{2}\Big)\Big)
=
R^2,
\end{equation}
so the expected radius is approximately constant. Its mean bridge-state SNR is
\begin{equation}
\overline{\mathrm{SNR}}_{\mathrm{VP}}(t)
\approx
2\log\tan\!\Big(\frac{\pi t}{2}\Big),
\end{equation}
which is monotone and symmetric in the usual VP sense.

\paragraph{Spherical flow matching (SFM).}
For spherical flow matching, the bridge follows the spherical geodesic (slerp) between normalized endpoints. Writing
\begin{equation}
\vartheta=\angle(x_0,x_1)=\arccos\!\Big(\frac{\langle x_0,x_1\rangle}{\|x_0\|_2\|x_1\|_2}\Big),
\end{equation}
the slerp bridge can be written as
\begin{equation}
x_t
=
\frac{\sin((1-t)\vartheta)}{\sin\vartheta}\,x_0
+
\frac{\sin(t\vartheta)}{\sin\vartheta}\,x_1.
\label{eq:sfm_slerp_full}
\end{equation}
In high dimensions, if $x_0$ and $x_1$ are independent concentrated directions, then
\begin{equation}
\frac{\langle x_0,x_1\rangle}{\|x_0\|_2\|x_1\|_2}
\approx 0,
\qquad
\vartheta\approx \frac{\pi}{2},
\end{equation}
with fluctuations shrinking as dimension grows. Therefore
\begin{equation}
\frac{\sin((1-t)\vartheta)}{\sin\vartheta}
\approx
\cos\!\Big(\frac{\pi t}{2}\Big),
\qquad
\frac{\sin(t\vartheta)}{\sin\vartheta}
\approx
\sin\!\Big(\frac{\pi t}{2}\Big),
\end{equation}
and the SFM bridge reduces to the standard VP bridge up to vanishing high-dimensional error:
\begin{equation}
x_t^{\mathrm{SFM}}
\approx
\cos\!\Big(\frac{\pi t}{2}\Big)x_0+\sin\!\Big(\frac{\pi t}{2}\Big)x_1.
\end{equation}
Consequently, under the same high-dimensional approximation,
\begin{equation}
\rho_{\mathrm{SFM}}(t)\approx R,
\qquad
\overline{\mathrm{SNR}}_{\mathrm{SFM}}(t)\approx 2\log\tan\!\Big(\frac{\pi t}{2}\Big).
\end{equation}

\paragraph{Implication for learnability.}
This comparison highlights two points. First, in high dimensions, standard RF naturally induces a non-monotone radius schedule, whereas standard VP and SFM both induce approximately constant-radius progress. Second, SFM provides an additional geometric justification for using a VP-like formulation in high dimensions: because typical pairs of high-dimensional directions are nearly orthogonal, the spherical geodesic bridge itself collapses to the VP bridge in the high-dimensional limit. This perspective is useful because it shows that VP-like state statistics are not merely algebraically convenient; they also arise as the high-dimensional limit of spherical transport between generic endpoint directions.

\subsection{Two high-dimensional failure modes: under-stepping and time-induced shortcuts}
\label{subsec:ref_failure_modes}

The previous discussion characterizes what information the bridge state carries. We now turn to two failure modes that arise when these statistics interact with the training dynamics of direction or velocity prediction.

\subsubsection{Bridge-agnostic under-stepping of standard $v$-prediction}
\label{subsec:ref_vpred_full}

Let the oracle transport field under a given bridge be $v_t^\star$, and let the model predict a vector $\hat v_t$. Write
\begin{equation}
v_t^\star=s^\star r^\star,\qquad
\hat v_t=\hat s\,\hat r,
\end{equation}
where $r^\star,\hat r\in\mathbb S^{N-1}(1)$ and $s^\star,\hat s\ge 0$. Let
\begin{equation}
\cos\theta=\langle \hat r,r^\star\rangle
\end{equation}
denote the directional mismatch. Then the $\ell_2$ regression loss is
\begin{align}
\|\hat v_t-v_t^\star\|_2^2
&=
\|\hat s\hat r-s^\star r^\star\|_2^2 \nonumber\\
&=
\hat s^2+(s^\star)^2-2\hat s s^\star\cos\theta.
\label{eq:vpred_quad_full}
\end{align}
Minimizing Eq.~\eqref{eq:vpred_quad_full} over $\hat s$ gives
\begin{equation}
\hat s_{\mathrm{opt}}=s^\star\cos\theta.
\label{eq:vpred_understep_full}
\end{equation}
Thus any directional error systematically shrinks the optimal predicted magnitude. This is a purely geometric property of full-vector regression and does not depend on the particular bridge family. We refer to the resulting effect as \emph{under-stepping}.

From a learnability viewpoint, the key issue is that under-stepping is not just a local regression bias. It alters the actual trajectory seen at inference time. In high dimensions, where progress-identifiability and target-identifiability can be sharply tied to time, this means that the actual inference state no longer matches the bridge statistics the model was trained on. If the downstream decoder is also trained on a narrow shell or spherical latent distribution, this mismatch becomes even more consequential.

\subsubsection{Time-induced identifiability shortcuts and exposure bias}
\label{subsec:ref_time_shortcut_full}

High-dimensional concentration creates a second pathology beyond under-stepping. Even if the bridge is statistically well designed during training, the strong coupling between time, progress-identifiability, and target-identifiability can itself induce shortcut solutions.

During training, oracle bridge states satisfy the mean schedules
\begin{equation}
\rho(t)=\sqrt{\mathbb E[\|x_t\|_2^2]},
\qquad
\overline{\mathrm{SNR}}(t)=\mathbb E[\mathrm{SNR}(x_t)],
\end{equation}
with small conditional variances in Eq.~\eqref{eq:ident_variances_full}. In this regime, a model can reduce training loss by learning shortcuts of the following form:
\begin{itemize}
\item infer bridge progress from explicit time $t$ or simple proxies such as $\|x_t\|_2$;
\item infer the expected target-information level from $t$;
\item interpret the current state according to the theoretical bridge statistics associated with that time.
\end{itemize}
In high dimensions, this shortcut can be especially strong because both progress-identifiability and target-identifiability are often close to deterministic functions of time.

At inference, however, prediction errors perturb the actual state away from the oracle bridge manifold. The \emph{actual} progress-identifiability and target-identifiability of the generated state may therefore differ from the \emph{theoretical} values implied by its time index. If the model relies too strongly on these low-variance time-induced statistics, it may interpret irrelevant or erroneous structures in the generated $x_t$ as if they were the correct target signal for that time, thereby amplifying error over steps.

This creates a high-dimensional form of exposure bias that is distinct from, but complementary to, under-stepping: under-stepping perturbs the trajectory geometry itself, while time-induced shortcut learning perturbs how the model \emph{interprets} off-bridge states once such errors arise.

\paragraph{A unified view.}
These two pathologies have a common consequence: they break the alignment between the \emph{nominal bridge semantics} seen during training and the \emph{actual state semantics} encountered at inference. Under-stepping changes where the trajectory goes; time-induced shortcuts change how the model interprets states once the trajectory deviates. This motivates a design in which (i) inference geometry is explicitly stabilized, and (ii) the bridge is designed not only for transport geometry but for the joint learnability of the input state and the target direction field.

\subsection{Stabilizing inference geometry by direction-only prediction and radius locking}
\label{subsec:ref_radius_locking_full}

The first design principle of REF is to separate \emph{direction learning} from \emph{step-length control}. Once a mean progress schedule $\rho(t)$ is specified, a direction-only model can recover step lengths geometrically.

Let the model predict a unit direction field
\begin{equation}
\hat r(x_t,t,c)\in\mathbb S^{N-1}(1).
\end{equation}
At inference step $k$, given the current state $x_{t_k}$, we update
\begin{equation}
x_{t_{k+1}}=x_{t_k}+\Delta_k \hat r_k,
\qquad
\hat r_k=\hat r(x_{t_k},t_k,c),
\end{equation}
and enforce the radius-locking constraint
\begin{equation}
\|x_{t_{k+1}}\|_2=\rho(t_{k+1}).
\label{eq:radius_lock_constraint_full}
\end{equation}
Expanding Eq.~\eqref{eq:radius_lock_constraint_full} yields
\begin{equation}
\Delta_k^2+2\langle x_{t_k},\hat r_k\rangle\Delta_k+\big(\|x_{t_k}\|_2^2-\rho(t_{k+1})^2\big)=0,
\end{equation}
whose positive root is
\begin{equation}
\Delta_k=
-\langle x_{t_k},\hat r_k\rangle
+
\sqrt{
\langle x_{t_k},\hat r_k\rangle^2
+
\rho(t_{k+1})^2-\|x_{t_k}\|_2^2 }.
\label{eq:radius_lock_solution_full}
\end{equation}
Thus the model predicts only direction, while the step length is recovered from the progress schedule.

This directly eliminates the bridge-agnostic under-stepping pathology of full-vector regression: the model is no longer asked to learn magnitude, and inference is explicitly constrained to follow the prescribed progress schedule. In the high-dimensional spherical-token regime, this is especially appealing because it keeps inference states close to the shell geometry on which the tokenizer decoder is typically trained.

\subsection{Why a monotone progress schedule is needed}
\label{subsec:ref_linear_progress_full}

The previous subsection assumes that the progress schedule $\rho(t)$ is itself suitable for radius locking. This is not true for all bridges. In particular, for standard RF bridges, the induced mean radius schedule first contracts and then expands. This creates a contraction phase in which the radius-locking equation can become infeasible or geometrically awkward, requiring retraction operators that are misaligned with the predicted direction.

To avoid this pathology, we require the mean progress schedule to be monotone. Moreover, if progress-identifiability is to remain stable across time, it is desirable that the expected bridge progress be distributed more uniformly over time. This motivates the canonical linear mean radius schedule
\begin{equation}
\rho(t)=R\big(a+(1-a)t\big),\qquad t\in[0,1],
\label{eq:rho_linear_full}
\end{equation}
with $a\in(0,1)$. Here $a$ should be interpreted as the \emph{source-shell ratio} induced by the radius-expansion design: the trajectory starts from a typical inner shell of radius $aR$ and expands monotonically to the token sphere of radius $R$. Eq.~\eqref{eq:rho_linear_full} has three useful properties:
\begin{enumerate}[leftmargin=2.0em,label=(\roman*)]
\item it is strictly monotone;
\item it has constant growth rate, since $\rho'(t)=R(1-a)$;
\item it makes uniform sampling in $t$ exactly equivalent to uniform sampling in expected radius.
\end{enumerate}
Thus linear time parameterization becomes the canonical schedule induced by the bridge itself.

At this point the question is no longer only how to choose a progress schedule. Once $\rho(t)$ is fixed, we must also ask whether the \emph{source--target mixing geometry} remains learnable under that schedule.

\subsection{State-target joint learnability under a prescribed progress schedule}
\label{subsec:ref_dual_snr_setup}

The second design principle of REF is that bridge geometry should be redesigned under the chosen progress schedule from the viewpoint of \emph{joint learnability}. In a direction-only setting, the model sees the bridge state $x_t$ but is trained against the oracle direction field $v_t^\star$. Therefore, under any given progress schedule, two source--target balances matter simultaneously:
\begin{itemize}
\item the balance visible in the model input $x_t$;
\item the balance present in the training target $v_t^\star$.
\end{itemize}
Good bridge design should make both of them well behaved.

To make this explicit, write the bridge in the general form
\begin{equation}
x_t=\alpha(t)x_0+\beta(t)x_1,
\end{equation}
and define the oracle direction field by differentiation:
\begin{equation}
v_t^\star = \frac{d x_t}{dt}
=
\alpha'(t)x_0+\beta'(t)x_1.
\label{eq:vt_general_full}
\end{equation}
The model takes $x_t$ as input and predicts the direction of $v_t^\star$, so two source--target balances matter simultaneously.

\paragraph{Bridge-state SNR.}
Under the concentrated-shell approximation $\|x_0\|_2\approx aR$ and $\|x_1\|_2=R$, the bridge-state SNR is
\begin{equation}
\mathrm{SNR}_x(t)
\;\triangleq\;
\log\frac{\beta(t)^2R^2}{\alpha(t)^2 a^2R^2}
=
\log\frac{\beta(t)^2}{a^2\alpha(t)^2}.
\label{eq:snr_x_general_full}
\end{equation}
This quantity describes what source--target information is visible in the model input $x_t$.

\paragraph{Direction-field SNR.}
Likewise, the direction-field SNR is
\begin{equation}
\mathrm{SNR}_{\mathrm{dir}}(t)
\;\triangleq\;
\log\frac{\beta'(t)^2R^2}{\alpha'(t)^2 a^2R^2}
=
\log\frac{\beta'(t)^2}{a^2\alpha'(t)^2}.
\label{eq:snr_dir_general_full}
\end{equation}
This quantity describes what source--target directional balance appears in the training target $v_t^\star$.

These two SNRs play different roles: $\mathrm{SNR}_x(t)$ describes what the model \emph{sees}, while $\mathrm{SNR}_{\mathrm{dir}}(t)$ describes what the model is asked to \emph{predict}. For direction-only learning, both matter, and what ultimately affects learnability is their \emph{joint relation}.

\subsection{What happens to RF-/VP-style mixing under linear progress schedules?}
\label{subsec:ref_standard_bridges_under_linear_progress}

We now examine what happens if we preserve the linear progress schedule in Eq.~\eqref{eq:rho_linear_full} and attach a familiar RF- or VP-style mixing pattern on top of it.

A convenient common parameterization is
\begin{equation}
\beta(t)=\frac{\rho(t)}{R}\sqrt{q(t)},
\qquad
\alpha(t)=\frac{\rho(t)}{aR}\sqrt{1-q(t)},
\label{eq:alpha_beta_q_full}
\end{equation}
where $q(t)$ is the source--target mixing schedule.

\paragraph{RF-style mixing.}
Choosing
\begin{equation}
q(t)=t
\label{eq:q_rf_full}
\end{equation}
gives
\begin{equation}
\beta(t)=g(t)\sqrt{t},
\qquad
\alpha(t)=\frac{g(t)}{a}\sqrt{1-t},
\qquad
g(t)=a+(1-a)t.
\label{eq:ab_rf_linearrho_full}
\end{equation}
Hence the bridge state is
\begin{equation}
x_t
=
\frac{g(t)}{a}\sqrt{1-t}\,x_0
+
g(t)\sqrt{t}\,x_1.
\label{eq:xt_rf_linearrho_full}
\end{equation}
Differentiating gives
\begin{equation}
\beta'(t)
=
(1-a)\sqrt{t}
+
\frac{g(t)}{2\sqrt{t}}
=
\frac{a+3(1-a)t}{2\sqrt{t}},
\label{eq:beta_prime_rf_linearrho_full}
\end{equation}
and
\begin{equation}
\alpha'(t)
=
\frac{1}{a}
\left[
(1-a)\sqrt{1-t}
-
\frac{g(t)}{2\sqrt{1-t}}
\right]
=
\frac{(2-3a)-3(1-a)t}{2a\sqrt{1-t}}.
\label{eq:alpha_prime_rf_linearrho_full}
\end{equation}
Thus the oracle direction field is
\begin{equation}
v_t^\star
=
\frac{(2-3a)-3(1-a)t}{2a\sqrt{1-t}}\,x_0
+
\frac{a+3(1-a)t}{2\sqrt{t}}\,x_1.
\label{eq:vt_rf_linearrho_full}
\end{equation}
The bridge-state SNR is
\begin{equation}
\mathrm{SNR}_x(t)=\log\frac{t}{1-t},
\label{eq:snr_x_rf_linearrho_full}
\end{equation}
while the direction-field SNR becomes
\begin{equation}
\mathrm{SNR}_{\mathrm{dir}}(t)
=
\log\frac{\beta'(t)^2}{a^2\alpha'(t)^2}
=
2\log \left|
\frac{a+3(1-a)t}{(2-3a)-3(1-a)t}
\right|
+
\log\frac{1-t}{t}.
\label{eq:snr_dir_rf_linearrho_full}
\end{equation}
Even though the bridge-state SNR remains monotone, the direction-field SNR is no longer RF-like: the source coefficient $\alpha'(t)$ can cross zero inside $(0,1)$, producing an internal singularity in $\mathrm{SNR}_{\mathrm{dir}}(t)$.

\paragraph{VP-style mixing.}
Choosing
\begin{equation}
q(t)=\sin^2\!\Big(\frac{\pi t}{2}\Big)
\label{eq:q_vp_full}
\end{equation}
gives
\begin{equation}
\beta(t)=g(t)\sin\!\Big(\frac{\pi t}{2}\Big),
\qquad
\alpha(t)=\frac{g(t)}{a}\cos\!\Big(\frac{\pi t}{2}\Big).
\label{eq:ab_vp_linearrho_full}
\end{equation}
Thus
\begin{equation}
x_t
=
\frac{g(t)}{a}\cos\!\Big(\frac{\pi t}{2}\Big)x_0
+
g(t)\sin\!\Big(\frac{\pi t}{2}\Big)x_1.
\label{eq:xt_vp_linearrho_full}
\end{equation}
Differentiating gives
\begin{equation}
\beta'(t)
=
(1-a)\sin\!\Big(\frac{\pi t}{2}\Big)
+
\frac{\pi}{2}g(t)\cos\!\Big(\frac{\pi t}{2}\Big),
\label{eq:beta_prime_vp_linearrho_full}
\end{equation}
and
\begin{equation}
\alpha'(t)
=
\frac{1}{a}
\left[
(1-a)\cos\!\Big(\frac{\pi t}{2}\Big)
-
\frac{\pi}{2}g(t)\sin\!\Big(\frac{\pi t}{2}\Big)
\right].
\label{eq:alpha_prime_vp_linearrho_full}
\end{equation}
Hence the oracle direction field is
\begin{equation}
v_t^\star
=
\frac{1}{a}
\left[
(1-a)\cos\!\Big(\frac{\pi t}{2}\Big)
-
\frac{\pi}{2}g(t)\sin\!\Big(\frac{\pi t}{2}\Big)
\right]x_0
+
\left[
(1-a)\sin\!\Big(\frac{\pi t}{2}\Big)
+
\frac{\pi}{2}g(t)\cos\!\Big(\frac{\pi t}{2}\Big)
\right]x_1.
\label{eq:vt_vp_linearrho_full}
\end{equation}
The bridge-state SNR is
\begin{equation}
\mathrm{SNR}_x(t)
=
2\log\tan\!\Big(\frac{\pi t}{2}\Big),
\label{eq:snr_x_vp_linearrho_full}
\end{equation}
while the direction-field SNR becomes
\begin{equation}
\mathrm{SNR}_{\mathrm{dir}}(t)
=
2\log
\left|
\frac{
(1-a)\sin\!\big(\frac{\pi t}{2}\big)
+
\frac{\pi}{2}g(t)\cos\!\big(\frac{\pi t}{2}\big)
}{
(1-a)\cos\!\big(\frac{\pi t}{2}\big)
-
\frac{\pi}{2}g(t)\sin\!\big(\frac{\pi t}{2}\big)
}
\right|.
\label{eq:snr_dir_vp_linearrho_full}
\end{equation}
Again, once the linear progress scaling is introduced, the bridge-state SNR remains simple, but the direction-field SNR is reshaped by the additional $g'(t)$-dependent terms and can develop internal sign changes of the source coefficient.

\paragraph{Implication for learnability.}
The key point is that once a nontrivial progress schedule $\rho(t)$ is imposed, the bridge-state SNR and the direction-field SNR are both altered by that schedule. Hence preserving a familiar state-level source--target schedule is not enough: what matters is whether the \emph{joint relation} between $\mathrm{SNR}_x(t)$ and $\mathrm{SNR}_{\mathrm{dir}}(t)$ still retains the good qualitative properties of the original bridges, such as monotonicity, smooth source--target transition, and the absence of internal singularities. In particular, the standard VP bridge provides a useful benchmark: in the limiting case $a=1$ (so $\rho(t)\equiv R$), one recovers
\begin{equation}
\alpha(t)=\cos\!\Big(\frac{\pi t}{2}\Big),\qquad
\beta(t)=\sin\!\Big(\frac{\pi t}{2}\Big),
\end{equation}
for which the bridge-state SNR and direction-field SNR satisfy the exact relation
\begin{equation}
\mathrm{SNR}_{\mathrm{dir}}(t)=-\mathrm{SNR}_x(t).
\end{equation}
Combined with the high-dimensional SFM discussion above, this also means that VP-like structure is not merely algebraically convenient: it is the natural high-dimensional limit of spherical geodesic transport between generic endpoint directions. Under radius expansion ($a<1$), this exact identity is no longer generally achievable, but it remains a natural benchmark to approximate.

\subsection{Closed-form bridge design under linear radius expansion}
\label{subsec:ref_closed_form_bridge}

We now derive a closed-form bridge under the linear radius schedule that preserves a simple, monotone, VP-like relation between the bridge-state SNR and the direction-field SNR, while reducing to the standard VP bridge in the limit $a\to 1$.

\subsubsection{Angle parameterization}
Under the shell constraint
\begin{equation}
a^2\alpha(t)^2+\beta(t)^2=\frac{\rho(t)^2}{R^2}=g(t)^2,
\qquad
g(t)\triangleq a+(1-a)t,
\end{equation}
a natural parameterization is
\begin{equation}
\beta(t)=g(t)\sin\phi(t),
\qquad
\alpha(t)=\frac{g(t)}{a}\cos\phi(t),
\label{eq:angle_param_full}
\end{equation}
for some monotone angle function $\phi(t)$ satisfying the boundary conditions
\begin{equation}
\phi(0)=0,\qquad \phi(1)=\frac{\pi}{2}.
\label{eq:phi_bc_full}
\end{equation}
Under this parameterization, the bridge state is
\begin{equation}
x_t
=
\frac{g(t)}{a}\cos\phi(t)\,x_0
+
g(t)\sin\phi(t)\,x_1.
\label{eq:xt_angle_full}
\end{equation}
The corresponding bridge-state SNR is
\begin{equation}
\mathrm{SNR}_x(t)
=
\log\frac{\beta(t)^2}{a^2\alpha(t)^2}
=
2\log\tan\phi(t).
\label{eq:snr_x_phi_full}
\end{equation}

Differentiating Eq.~\eqref{eq:xt_angle_full}, the oracle direction field is
\begin{equation}
v_t^\star=\alpha'(t)x_0+\beta'(t)x_1,
\label{eq:vt_angle_general_full}
\end{equation}
with
\begin{equation}
\beta'(t)=g'(t)\sin\phi(t)+g(t)\phi'(t)\cos\phi(t),
\label{eq:beta_prime_angle_full}
\end{equation}
and
\begin{equation}
\alpha'(t)=\frac{1}{a}
\Big(
g'(t)\cos\phi(t)-g(t)\phi'(t)\sin\phi(t)
\Big).
\label{eq:alpha_prime_angle_full}
\end{equation}
Hence
\begin{equation}
v_t^\star
=
\frac{g'(t)\cos\phi(t)-g(t)\phi'(t)\sin\phi(t)}{a}\,x_0
+
\Big(
g'(t)\sin\phi(t)+g(t)\phi'(t)\cos\phi(t)
\Big)x_1.
\label{eq:vt_angle_expanded_full}
\end{equation}
The direction-field SNR is therefore
\begin{equation}
\mathrm{SNR}_{\mathrm{dir}}(t)
=
\log\frac{\beta'(t)^2}{a^2\alpha'(t)^2}.
\label{eq:snr_dir_angle_general_full}
\end{equation}

\subsubsection{A solvable VP-like benchmark relation}
To obtain a closed-form bridge, we introduce an auxiliary benchmark angle $\Theta(t)$ and impose the ratio condition
\begin{equation}
\frac{\beta'(t)}{-a\alpha'(t)}
=
\cot\Theta(t).
\label{eq:ratio_theta_full}
\end{equation}
This reproduces the standard VP relation when $a=1$ and $\Theta(t)=\frac{\pi t}{2}$, but under radius expansion it should be viewed as a \emph{benchmark relation} rather than an exact self-duality constraint.

Substituting Eqs.~\eqref{eq:beta_prime_angle_full}--\eqref{eq:alpha_prime_angle_full} into Eq.~\eqref{eq:ratio_theta_full}, we obtain
\begin{equation}
\frac{g'(t)\sin\phi(t)+g(t)\phi'(t)\cos\phi(t)}
{-g'(t)\cos\phi(t)+g(t)\phi'(t)\sin\phi(t)}
=
\cot\Theta(t).
\label{eq:ratio_theta_substituted_full}
\end{equation}
Rearranging,
\begin{equation}
g(t)\phi'(t)\big(\cos\phi(t)-\cot\Theta(t)\sin\phi(t)\big)
=
-g'(t)\big(\sin\phi(t)+\cot\Theta(t)\cos\phi(t)\big).
\end{equation}
Using
\begin{equation}
\sin\phi+\cot\Theta\cos\phi
=
\frac{\cos(\phi-\Theta)}{\sin\Theta},
\qquad
\cos\phi-\cot\Theta\sin\phi
=
\frac{\sin(\Theta-\phi)}{\sin\Theta},
\end{equation}
we obtain
\begin{equation}
\phi'(t)
=
\frac{g'(t)}{g(t)}\cot\big(\phi(t)-\Theta(t)\big).
\label{eq:phi_ode_theta_full}
\end{equation}
Define
\begin{equation}
u(t)\triangleq \phi(t)-\Theta(t).
\end{equation}
Then Eq.~\eqref{eq:phi_ode_theta_full} becomes
\begin{equation}
u'(t)+\Theta'(t)=\frac{g'(t)}{g(t)}\cot u(t).
\label{eq:u_ode_general_full}
\end{equation}

To obtain a closed-form solution, we consider the solvable case where the offset $u(t)$ is constant:
\begin{equation}
u(t)\equiv u_0.
\end{equation}
Then Eq.~\eqref{eq:u_ode_general_full} reduces to
\begin{equation}
\Theta'(t)=\frac{g'(t)}{g(t)}\cot u_0.
\end{equation}
Integrating,
\begin{equation}
\Theta(t)=\cot u_0\,\log g(t)+C.
\label{eq:theta_log_full}
\end{equation}
Now impose the bridge boundary conditions through $\phi(t)=\Theta(t)+u_0$:
\begin{equation}
\phi(0)=0,\qquad \phi(1)=\frac{\pi}{2}.
\end{equation}
Since $g(1)=1$, Eq.~\eqref{eq:theta_log_full} gives
\begin{equation}
\phi(1)=C+u_0=\frac{\pi}{2},
\qquad\Longrightarrow\qquad
C=\frac{\pi}{2}-u_0.
\end{equation}
Using $g(0)=a$ and $\phi(0)=0$ yields
\begin{equation}
0
=
\cot u_0\,\log a+\frac{\pi}{2},
\end{equation}
so
\begin{equation}
\cot u_0=-\frac{\pi}{2\log a}.
\end{equation}
Substituting back into $\phi(t)=\Theta(t)+u_0$, we obtain the closed-form solution
\begin{equation}
\boxed{
\phi(t)
=
\frac{\pi}{2}
-
\frac{\pi}{2\log a}\log\big(a+(1-a)t\big).
}
\label{eq:phi_closed_form_full}
\end{equation}
It is immediate to verify
\begin{equation}
\phi(0)=
\frac{\pi}{2}
-
\frac{\pi}{2\log a}\log a
=0,
\qquad
\phi(1)=
\frac{\pi}{2}
-
\frac{\pi}{2\log a}\log 1
=
\frac{\pi}{2}.
\end{equation}

Substituting Eq.~\eqref{eq:phi_closed_form_full} into Eq.~\eqref{eq:angle_param_full}, we obtain the final closed-form bridge:
\begin{equation}
\boxed{
\beta(t)=\big(a+(1-a)t\big)\sin\phi(t),
\qquad
\alpha(t)=\frac{a+(1-a)t}{a}\cos\phi(t),
}
\label{eq:alpha_beta_closed_form_full}
\end{equation}
with $\phi(t)$ given by Eq.~\eqref{eq:phi_closed_form_full}.

\subsubsection{Expanded bridge state and direction field}
Using Eqs.~\eqref{eq:phi_closed_form_full} and \eqref{eq:alpha_beta_closed_form_full}, the bridge state can be written explicitly as
\begin{equation}
x_t
=
\frac{a+(1-a)t}{a}\cos\phi(t)\,x_0
+
\big(a+(1-a)t\big)\sin\phi(t)\,x_1.
\label{eq:xt_closed_form_full}
\end{equation}
Differentiating Eq.~\eqref{eq:phi_closed_form_full}, we have
\begin{equation}
\phi'(t)
=
-\frac{\pi}{2\log a}\cdot
\frac{1-a}{a+(1-a)t}.
\label{eq:phi_prime_closed_form_full}
\end{equation}
Since $a\in(0,1)$ implies $\log a<0$, we have $\phi'(t)>0$.

Substituting Eq.~\eqref{eq:phi_prime_closed_form_full} into Eqs.~\eqref{eq:beta_prime_angle_full} and \eqref{eq:alpha_prime_angle_full}, we obtain
\begin{equation}
\beta'(t)
=
(1-a)\sin\phi(t)
-
\frac{\pi(1-a)}{2\log a}\cos\phi(t),
\label{eq:beta_prime_closed_form_full}
\end{equation}
and
\begin{equation}
\alpha'(t)
=
\frac{1-a}{a}
\left(
\cos\phi(t)
+
\frac{\pi}{2\log a}\sin\phi(t)
\right).
\label{eq:alpha_prime_closed_form_full}
\end{equation}
Hence the oracle direction field is
\begin{equation}
v_t^\star
=
\frac{1-a}{a}
\left(
\cos\phi(t)
+
\frac{\pi}{2\log a}\sin\phi(t)
\right)x_0
+
\left(
(1-a)\sin\phi(t)
-
\frac{\pi(1-a)}{2\log a}\cos\phi(t)
\right)x_1.
\label{eq:vt_closed_form_full}
\end{equation}

\subsubsection{Bridge-state and direction-field SNR under the closed-form bridge}
For the closed-form bridge in Eqs.~\eqref{eq:phi_closed_form_full}--\eqref{eq:alpha_beta_closed_form_full}, the bridge-state SNR is
\begin{equation}
\boxed{
\mathrm{SNR}_x(t)=2\log\tan\phi(t).
}
\label{eq:snr_x_closed_form_full}
\end{equation}
The corresponding direction-field SNR is
\begin{equation}
\boxed{
\mathrm{SNR}_{\mathrm{dir}}(t)
=
2\log
\left|
\frac{
(1-a)\sin\phi(t)-\frac{\pi(1-a)}{2\log a}\cos\phi(t)
}{
(1-a)\cos\phi(t)+\frac{\pi(1-a)}{2\log a}\sin\phi(t)
}
\right|.
}
\label{eq:snr_dir_closed_form_full}
\end{equation}
This relation is no longer the exact self-duality
\(
\mathrm{SNR}_{\mathrm{dir}}=-\mathrm{SNR}_x
\)
unless $a=1$, which is precisely the standard VP limit. However, the closed-form bridge preserves the key qualitative structure we seek:
\begin{itemize}
\item the bridge-state SNR remains monotone;
\item the direction-field SNR is induced by a closed-form, nonsingular coefficient schedule;
\item the construction reduces continuously to the standard VP bridge as $a\to 1$;
\item the bridge-state and direction-field balances remain jointly controlled by a single interpretable parameter $a$.
\end{itemize}

\paragraph{Numerical illustration on a coarse time grid.}
To make the above schedules more concrete, Table~\ref{tab:ref_snr_grid} reports representative values of $\mathrm{SNR}_x(t)$ and $\mathrm{SNR}_{\mathrm{dir}}(t)$ on a coarse grid
\(
t\in\{0.1,0.3,0.5,0.7,0.9\}
\)
for several typical transition centers
\(
\tau\in\{0.50,0.45,0.40,0.35\}
\),
where
\(
a=\big(\frac{\tau}{1-\tau}\big)^2
\).
For $\tau=0.5$ we have $a=1$, i.e., the standard VP limit, and thus
\(
\mathrm{SNR}_{\mathrm{dir}}(t)=-\mathrm{SNR}_x(t)
\).
For $\tau<0.5$, the bridge enters the radius-expansion regime.

\begin{table}[t]
\centering
\small
\caption{Representative bridge-state and direction-field SNR values (natural-log scale) under the closed-form bridge on a coarse time grid. Here $\tau$ denotes the bridge-state transition center and $a=\left(\frac{\tau}{1-\tau}\right)^2$. Values are rounded to two decimals.}
\label{tab:ref_snr_grid}
\begin{tabular}{c c c c c c c c}
\toprule
$\tau$ & $a$ & quantity & $t=0.1$ & $t=0.3$ & $t=0.5$ & $t=0.7$ & $t=0.9$ \\
\midrule
0.50 & 1.000 &
$\mathrm{SNR}_x$ & -3.69 & -1.69 & 0.00 & 1.69 & 3.69 \\
     &       &
$\mathrm{SNR}_{\mathrm{dir}}$ & 3.69 & 1.69 & 0.00 & -1.69 & -3.69 \\
\midrule
0.45 & 0.669 &
$\mathrm{SNR}_x$ & -3.33 & -1.47 & 0.11 & 1.72 & 3.83 \\
     &       &
$\mathrm{SNR}_{\mathrm{dir}}$ & 4.06 & 1.87 & -0.14 & -2.09 & -4.68 \\
\midrule
0.40 & 0.444 &
$\mathrm{SNR}_x$ & -3.02 & -1.29 & 0.22 & 1.79 & 4.00 \\
     &       &
$\mathrm{SNR}_{\mathrm{dir}}$ & 4.35 & 2.01 & -0.31 & -2.48 & -5.34 \\
\midrule
0.35 & 0.290 &
$\mathrm{SNR}_x$ & -2.77 & -1.15 & 0.33 & 1.90 & 4.20 \\
     &       &
$\mathrm{SNR}_{\mathrm{dir}}$ & 4.54 & 2.10 & -0.47 & -2.85 & -5.92 \\
\bottomrule
\end{tabular}
\end{table}

Several qualitative patterns are visible. First, $\mathrm{SNR}_x(t)$ remains smooth and monotone for all tested $\tau$, and its zero-crossing shifts earlier as $\tau$ decreases. Second, $\mathrm{SNR}_{\mathrm{dir}}(t)$ also remains smooth and nonsingular, but deviates systematically from the exact VP self-duality once $a<1$: early times become more target-leaning in the direction field, while later times become more source-suppressed. Third, as $\tau$ decreases (equivalently, as radius expansion becomes stronger), this asymmetry increases gradually rather than abruptly, which is consistent with the intended role of $a$ as a continuous geometric control parameter.

Thus the goal here is not exact duality for all $a<1$, but rather a smooth VP-like extension that remains geometrically compatible with linear radius expansion.

\subsubsection{Choosing $a$ by the shared transition center}
The source radius ratio $a$ now plays a direct geometric role: it controls the transition structure of the bridge.

A particularly useful quantity is the bridge-state balance point, defined by
\begin{equation}
\mathrm{SNR}_x(t)=0
\quad\Longleftrightarrow\quad
\phi(t)=\frac{\pi}{4}.
\end{equation}
Substituting Eq.~\eqref{eq:phi_closed_form_full}, this gives
\begin{equation}
a+(1-a)t=\sqrt a,
\end{equation}
hence the bridge-state transition center is
\begin{equation}
\boxed{
t_0(a)=\frac{\sqrt a-a}{1-a}
=
\frac{\sqrt a}{1+\sqrt a}.
}
\label{eq:t0_of_a_full}
\end{equation}
Conversely, if one wishes this transition center to occur at a prescribed location $\tau$, then
\begin{equation}
\boxed{
a
=
\left(
\frac{\tau}{1-\tau}
\right)^2.
}
\label{eq:a_from_tau_full}
\end{equation}
Since $a\in(0,1)$ in the expanding-shell regime, Eq.~\eqref{eq:t0_of_a_full} immediately implies
\begin{equation}
t_0(a)<\frac12.
\end{equation}
In other words, under radius expansion, the bridge-state source--target balance always occurs before the midpoint of the trajectory. Equivalently, throughout the early half of the bridge, the bridge state remains source-dominated while the trajectory is still expanding toward the target shell. This is a useful structural property of the expanding-shell geometry itself.

Eq.~\eqref{eq:a_from_tau_full} therefore provides a simple theory-guided way to choose $a$: instead of treating it as a purely heuristic shell parameter, we interpret it as the parameter that sets where the bridge state becomes source--target balanced. Some representative values are:
\begin{equation}
\tau=0.5 \;\Longrightarrow\; a=1
\quad\text{(the standard VP limit),}
\end{equation}
\begin{equation}
\tau=0.45 \;\Longrightarrow\; a=\left(\frac{9}{11}\right)^2\approx 0.669,
\end{equation}
\begin{equation}
\tau=0.4 \;\Longrightarrow\; a=\left(\frac{2}{3}\right)^2=\frac49\approx 0.444,
\end{equation}
\begin{equation}
\tau=0.35 \;\Longrightarrow\; a=\left(\frac{7}{13}\right)^2\approx 0.290.
\end{equation}
Thus larger $a$ shifts the bridge-state transition center toward later times and recovers a bridge closer to the standard VP limit; smaller $a$ shifts the transition earlier and emphasizes stronger source-dominated phases before the state reaches balance.

\paragraph{Discussion.}
The parameterization in Eq.~\eqref{eq:a_from_tau_full} does not eliminate the need for empirical validation, but it turns the search over $a$ into a search over a semantically meaningful quantity---the bridge-state transition center $\tau$. In practice, this yields a much more principled exploration strategy than unconstrained grid search over bridge coefficients. We therefore use $\tau$ as the primary control variable in our experiments and include the limiting case $a=1$ as the standard-VP benchmark configuration.

\subsection{Source-Shell Randomization for Time-Induced Shortcut Mitigation}
\label{subsec:ref_source_shell_randomization}

The discussion above identifies a potential high-dimensional training pathology that is conceptually distinct from under-stepping. In low-dimensional standard bridges, even when $t$ is fixed, the bridge state norm $\|x_t\|_2$ still exhibits nontrivial variability due to the finite-dimensional geometry of the source and target. As a result, the current state does not map too rigidly to a single nominal progress level or a single nominal source--target balance. In high dimensions, however, concentration makes this mapping much sharper: for a fixed time index $t$, the bridge state norm and related bridge statistics can become almost deterministic. This creates a strong \emph{time-induced shortcut}: the model can infer progress and expected source--target balance too directly from time or norm proxies, and this shortcut can dominate the training dynamics. Importantly, our goal here is \emph{not} to eliminate the general fact that large-$t$ states contain more target information---that is an intrinsic property of any bridge. Rather, the goal is to prevent such rigid time-induced statistics from excessively biasing the training dynamics of the \emph{small-$t$ regime}, where condition-dependent prediction should remain important.

To mitigate this effect while preserving the geometric interpretation of REF, we introduce a \emph{source-shell randomization} strategy: instead of using a single deterministic source-shell ratio $a$ for all training samples, we perturb the source radius slightly across samples. This increases the ambiguity of $\|x_t\|_2$ at fixed $t$ without adding arbitrary noise directly to $x_t$. Compared with a noisy bridge construction $x_t+\varepsilon$, this has two advantages. First, it preserves the bridge-family interpretation: each training sample still lies on a valid bridge from an inner shell to the target shell, rather than on an externally corrupted bridge state. Second, it allows us to increase the conditional variance of $\|x_t\|_2$ while keeping the \emph{mean progress schedule} conceptually unchanged, so that the perturbation targets the time-induced shortcut more directly.

A key question is then how large this source-shell perturbation should be. Our design principle is to calibrate the induced high-dimensional ambiguity to the \emph{natural ambiguity level of a low-dimensional standard bridge}. This is motivated by the empirical observation that standard RF/VP-style bridges do not appear to suffer from the same severe time-induced shortcut pathology in the low-dimensional token regime, even when substantial token information mixing is present. We therefore take the low-dimensional regime as a reference and seek a perturbation strength that restores, in high dimensions, a comparable degree of norm-induced progress ambiguity.

\paragraph{Time aliasing interval under a mean progress schedule.}
We first formalize what we mean by \emph{progress ambiguity}. Let
\begin{equation}
\rho(t)=R\big(a+(1-a)t\big),\qquad R=\sqrt N,
\end{equation}
be the canonical mean progress schedule used by REF. Since $\rho(\cdot)$ is strictly monotone, any radius interval can be mapped back to a corresponding interval on the time axis. For a fixed nominal time $t$, let
\begin{equation}
m_t \triangleq \mathbb E[\|x_t\|_2],
\qquad
s_t \triangleq \mathrm{Std}(\|x_t\|_2).
\end{equation}
We define the $k$-$\sigma$ \emph{time aliasing interval} induced by the norm variability at time $t$ as
\begin{equation}
I_t^{(k)}
\triangleq
\left[
\rho^{-1}(m_t-k s_t),
\;
\rho^{-1}(m_t+k s_t)
\right]\cap[0,1].
\end{equation}
Its width
\begin{equation}
W_t^{(k)}
\triangleq
\mathrm{length}(I_t^{(k)})
\end{equation}
serves as our proxy for time-induced ambiguity: it measures how wide a time interval on the canonical progress schedule is ``covered'' by the radius uncertainty at fixed nominal time $t$. In particular, if concentration is so strong that $s_t\approx 0$, then $W_t^{(k)}\approx 0$ and the current state norm reveals an almost unique bridge progress. Conversely, larger $W_t^{(k)}$ means that the same nominal time corresponds to a broader range of effective progress values.

Because $\rho(t)$ is linear,
\begin{equation}
\rho^{-1}(r)=\frac{r/R-a}{1-a},
\end{equation}
so the aliasing width reduces to
\begin{equation}
W_t^{(k)}=\frac{2k\,s_t}{R(1-a)}.
\label{eq:alias_width_raw}
\end{equation}
It is convenient to work with the normalized radius
\begin{equation}
\tilde r_t\triangleq \frac{\|x_t\|_2}{R},
\end{equation}
for which
\begin{equation}
W_t^{(k)}=\frac{2k\,\mathrm{Std}(\tilde r_t)}{1-a}.
\label{eq:alias_width_normalized}
\end{equation}
Thus, under our linear progress schedule, the time aliasing width is equivalent to the normalized radius standard deviation.

\paragraph{Low-dimensional reference ambiguity.}
We next derive a reference ambiguity level from a low-dimensional standard bridge. Let the reference dimension be $d$ (e.g., $d\in\{4,8,16\}$). We use the standard VP bridge with a Gaussian source:
\begin{equation}
x_t=\alpha_t x_0+\beta_t x_1,
\qquad
\alpha_t=\cos\!\Big(\frac{\pi t}{2}\Big),
\quad
\beta_t=\sin\!\Big(\frac{\pi t}{2}\Big),
\end{equation}
where
\begin{equation}
x_0\sim \mathcal N(0,I_d),
\qquad
\|x_1\|_2^2=d.
\end{equation}
The bridge norm expands as
\begin{equation}
\|x_t\|_2^2
=
\alpha_t^2\|x_0\|_2^2+\beta_t^2\|x_1\|_2^2+2\alpha_t\beta_t\langle x_0,x_1\rangle.
\end{equation}
A fully precise calibration could retain both stochastic contributions:
\begin{itemize}
\item the source-norm fluctuation through $\|x_0\|_2^2$,
\item the angular fluctuation through $\langle x_0,x_1\rangle$.
\end{itemize}
Indeed,
\begin{equation}
\|x_0\|_2^2\sim\chi_d^2,
\qquad
\mathbb E[\|x_0\|_2^2]=d,
\qquad
\mathrm{Var}(\|x_0\|_2^2)=2d,
\end{equation}
and
\begin{equation}
\mathrm{Var}(\langle x_0,x_1\rangle)=d
\end{equation}
when $\|x_1\|_2^2=d$. Moreover, the covariance between these two terms is zero by vanishing Gaussian third moments. Hence
\begin{equation}
\mathrm{Var}(\|x_t\|_2^2)
=
2d\,\alpha_t^4+4d\,\alpha_t^2\beta_t^2.
\end{equation}
Using a delta approximation around $\mathbb E[\|x_t\|_2^2]=d$, this gives
\begin{equation}
\mathrm{Std}(\|x_t\|_2)
\approx
\alpha_t\sqrt{\frac12\alpha_t^2+\beta_t^2}.
\end{equation}

However, our purpose here is not to exactly replicate every low-dimensional fluctuation mechanism. Rather, we seek a \emph{simple and interpretable} calibration rule for the amount of source-shell randomization needed to break the excessive rigidity of high-dimensional norm statistics. For this purpose, we make two deliberate approximations.

\paragraph{Approximation 1: source-norm fluctuation as the dominant low-dimensional reference effect.}
We treat the fluctuation of $\|x_0\|_2^2$ as the principal low-dimensional source of progress ambiguity and ignore the angular term in the calibration formula. This is a natural approximation because (i) the source norm is precisely the quantity we wish to randomize in high dimensions; (ii) in standard Gaussian-source bridges, the source norm is the most direct mechanism by which the bridge progress becomes non-rigid; and (iii) retaining only this term yields a much cleaner closed-form calibration while preserving the correct qualitative dependence on $t$ and $d$. Under this approximation,
\begin{equation}
\mathrm{Var}(\|x_t\|_2^2)\approx 2d\,\alpha_t^4.
\end{equation}
Applying the same delta approximation gives
\begin{equation}
\mathrm{Std}(\|x_t\|_2)
\approx
\frac{1}{2\sqrt d}\sqrt{2d\,\alpha_t^4}
=
\frac{\alpha_t^2}{\sqrt2}.
\end{equation}
Normalizing by the reference radius $\sqrt d$, we obtain
\begin{equation}
\mathrm{Std}\!\Big(\frac{\|x_t\|_2}{\sqrt d}\Big)
\approx
\frac{\alpha_t^2}{\sqrt{2d}}
=
\frac{\cos^2(\pi t/2)}{\sqrt{2d}}.
\end{equation}
Therefore, the low-dimensional reference aliasing width becomes
\begin{equation}
W_{t,\mathrm{ref}}^{(k)}
\approx
\frac{2k}{1-a}\cdot \frac{\cos^2(\pi t/2)}{\sqrt{2d}}.
\label{eq:alias_width_ref}
\end{equation}

\paragraph{High-dimensional source-shell randomization.}
We now introduce a randomized source-shell ratio
\begin{equation}
A,\qquad \mathbb E[A]=a,\qquad \mathrm{Std}(A)=\sigma_A,
\end{equation}
and use $A$ in place of the fixed shell ratio $a$ during training. At the level of the normalized mean progress schedule, this induces
\begin{equation}
\tilde \rho_A(t)=A+(1-A)t=t+(1-t)A.
\end{equation}
Hence, for fixed $t$,
\begin{equation}
\mathrm{Std}(\tilde \rho_A(t))=(1-t)\sigma_A.
\end{equation}
This is the main ambiguity injection effect we seek.

One could also retain the intrinsic angular fluctuation of high-dimensional random directions, since even in high dimensions the directions are only \emph{approximately} orthogonal. If
\begin{equation}
x_0=AR\,u_0,\qquad x_1=R\,u_1,
\end{equation}
with independent random directions $u_0,u_1\in\mathbb S^{N-1}(1)$, then
\begin{equation}
\mathrm{Var}(\langle u_0,u_1\rangle)\approx \frac{1}{N}.
\end{equation}
This gives a small intrinsic contribution to the high-dimensional norm variance. For a fully precise calibration, one could add this baseline term and fit the total high-dimensional aliasing width to the low-dimensional target. However, we intentionally do \emph{not} include this term in the main calibration rule. This is our second simplifying approximation.

\paragraph{Approximation 2: intrinsic high-dimensional angular variance as a negligible baseline.}
In the high-dimensional regime of interest, the angular fluctuation scales as $N^{-1/2}$ in normalized radius, and is therefore much smaller than the ambiguity level we wish to inject by design. Since our goal is to obtain a simple formula for a \emph{controllable} source-shell perturbation strength, we treat the intrinsic angular variance as a small baseline effect and calibrate $\sigma_A$ using only the dominant shell-randomization term. This keeps the resulting formula clean and practical, while still matching the intended geometry.

Under this approximation,
\begin{equation}
W_{t,\mathrm{high}}^{(k)}
\approx
\frac{2k(1-t)\sigma_A}{1-a}.
\label{eq:alias_width_high}
\end{equation}

\paragraph{Matching the low-dimensional ambiguity profile.}
We now choose $\sigma_A$ so that the high-dimensional aliasing width in Eq.~\eqref{eq:alias_width_high} approximates the low-dimensional reference width in Eq.~\eqref{eq:alias_width_ref}. Since Eq.~\eqref{eq:alias_width_high} is proportional to $(1-t)$ while Eq.~\eqref{eq:alias_width_ref} is proportional to $\cos^2(\pi t/2)$, an exact match over the full interval is impossible with a single scalar $\sigma_A$. This is expected: the randomized source-shell mechanism and the low-dimensional Gaussian-source mechanism induce similar but not identical $t$-dependence. Since our aim is to reproduce the \emph{overall level and trend} of low-dimensional ambiguity rather than every detail of its shape, the natural choice is to match the two curves in an $L^2$ sense over the full time interval.

With a uniform weight $w(t)=1$, we minimize
\begin{equation}
\int_0^1
\left(
(1-t)\sigma_A
-
\frac{\cos^2(\pi t/2)}{\sqrt{2d}}
\right)^2dt.
\end{equation}
This is a one-dimensional least-squares problem with a closed-form solution:
\begin{equation}
\sigma_A^\star
=
\frac{
\int_0^1 (1-t)\,\frac{\cos^2(\pi t/2)}{\sqrt{2d}}\,dt
}{
\int_0^1 (1-t)^2\,dt
}.
\end{equation}
The denominator is
\begin{equation}
\int_0^1 (1-t)^2\,dt=\frac13.
\end{equation}
For the numerator, using
\begin{equation}
\cos^2\Big(\frac{\pi t}{2}\Big)=\frac{1+\cos(\pi t)}{2},
\end{equation}
we obtain
\begin{align}
\int_0^1 (1-t)\cos^2\Big(\frac{\pi t}{2}\Big)\,dt
&=
\frac12\int_0^1 (1-t)\,dt
+
\frac12\int_0^1 (1-t)\cos(\pi t)\,dt \\
&=
\frac14+\frac{1}{\pi^2}.
\end{align}
Hence
\begin{equation}
\boxed{
\sigma_A^\star
=
\frac{3}{\sqrt{2d}}
\left(
\frac14+\frac{1}{\pi^2}
\right)
\approx
\frac{0.53}{\sqrt d}.
}
\label{eq:sigmaA_closed_form}
\end{equation}

\paragraph{Interpretation.}
Eq.~\eqref{eq:sigmaA_closed_form} provides a simple and interpretable calibration rule: the source-shell randomization strength should scale as $d^{-1/2}$, where $d$ is the reference low-dimensional token dimension whose ambiguity profile we wish to emulate. This matches the intuition that lower-dimensional token spaces naturally exhibit larger relative progress ambiguity, while high-dimensional spaces exhibit much less. In practice, we may additionally introduce a user-controlled scale factor
\begin{equation}
\lambda_{\mathrm{amb}}\in[0,1]
\end{equation}
to interpolate between no randomization and the full calibrated ambiguity level:
\begin{equation}
\sigma_A^{\mathrm{calib}}
=
\lambda_{\mathrm{amb}}
\cdot
\frac{3}{\sqrt{2d_{\mathrm{ref}}}}
\left(
\frac14+\frac{1}{\pi^2}
\right)
\approx
\lambda_{\mathrm{amb}}\frac{0.53}{\sqrt{d_{\mathrm{ref}}}}.
\label{eq:sigmaA_calib}
\end{equation}

\paragraph{Why the perturbation must be bounded.}
While increasing $\sigma_A$ increases time aliasing width and weakens the time-induced shortcut, it cannot be made arbitrarily large. If the randomized shell ratio $A$ exceeds 1 with non-negligible probability, then the training bridge is no longer an \emph{expanding-shell} bridge from an inner shell to the target shell; instead, some source samples start outside the target sphere. This would break the intended geometric interpretation of REF and introduce training trajectories that are qualitatively different from the ones used at inference, where the canonical schedule remains expanding from radius $aR$ to radius $R$.

To preserve the expanding-shell regime with high probability, we impose a simple $k$-$\sigma$ feasibility constraint:
\begin{equation}
a+k\sigma_A \le 1,
\end{equation}
where typically $k\in\{3,5\}$. Equivalently,
\begin{equation}
\sigma_A \le \frac{1-a}{k}.
\label{eq:sigmaA_max}
\end{equation}
This can be viewed as a high-probability upper bound ensuring that the randomized source shell remains inside the target shell.

Combining the low-dimensional calibration rule with the expanding-shell feasibility constraint, we use the final source-shell randomization strength
\begin{equation}
\boxed{
\sigma_A
=
\min\!\left(
\sigma_A^{\mathrm{calib}},
\frac{1-a}{k}
\right),
\qquad
\sigma_A^{\mathrm{calib}}
\approx
\lambda_{\mathrm{amb}}\frac{0.53}{\sqrt{d_{\mathrm{ref}}}}.
}
\label{eq:sigmaA_final}
\end{equation}

\paragraph{Summary.}
The above construction gives a geometry-preserving way to weaken the high-dimensional time-induced shortcut. Rather than adding arbitrary noise to bridge states, we randomize the source-shell ratio so that fixed-time radius statistics induce a controlled nonzero aliasing width on the canonical progress schedule. The perturbation strength is calibrated by matching the resulting aliasing profile to the natural ambiguity level of a low-dimensional Gaussian-source VP bridge, while a $k$-$\sigma$ upper bound ensures that the randomized bridges remain in the expanding-shell regime. In this way, source-shell randomization restores part of the progress ambiguity naturally present in low dimensions, without sacrificing the geometric interpretation and inference stability of REF.

\subsection{Explicit time embeddings in high dimensions}
\label{subsec:ref_time_emb_full}

The above analysis also changes how explicit time embeddings should be interpreted.

In low-dimensional or non-concentrated settings, progress-identifiability and target-identifiability are weak and noisy, so explicit time conditioning acts primarily as an anti-ambiguity signal. In the high-dimensional setting considered here, however, the situation is different: under the linear mean-radius design, progress-identifiability is already strongly encoded in the bridge state itself through $\|x_t\|_2$, while the source--target relation is further constrained by the closed-form bridge geometry. Explicit time can therefore become a shortcut that reveals not only where the state lies on the bridge, but also what bridge statistics the model should \emph{expect} it to have.

This suggests that, in high-dimensional bridges, explicit time embeddings may act less like pure disambiguation signals and more like optimization shortcuts that encourage the model to interpret the state according to a theoretical bridge schedule rather than according to its actual content. In our experiments, we therefore also study the effect of removing explicit time embeddings. Importantly, this does not eliminate progress information altogether: under the linear mean-radius design, progress-identifiability is already carried implicitly by the bridge state itself. Rather, removing explicit time embeddings suppresses the most direct shortcut channel and forces the model to infer progress from the state content instead of from an explicit lookup variable.

\subsection{Radius Expansion Flow (REF)}
\label{subsec:ref_final_full}

Putting the above together, our high-dimensional \textbf{Radius Expansion Flow (REF)} framework consists of four ingredients:
\begin{enumerate}[leftmargin=2.0em,label=(\roman*)]
\item \textbf{Direction-only training:}
the model predicts only transport direction, avoiding the under-stepping pathology of full-vector regression.

\item \textbf{A monotone linear mean progress schedule:}
we use the canonical mean radius schedule
\begin{equation}
\rho(t)=R\big(a+(1-a)t\big),
\end{equation}
which yields stable and uniform progress-identifiability and supports globally feasible radius locking.

\item \textbf{A closed-form bridge under linear radius expansion:}
instead of prescribing only a state-level source--target schedule, we redesign the source--target mixing geometry directly under the imposed progress schedule. The resulting bridge has a closed-form state and direction field, remains smooth and nonsingular in the expanding-shell regime, and recovers the standard VP bridge in the limit $a\to 1$.

\item \textbf{A semantically interpretable bridge parameterization:}
the source radius ratio $a$ is chosen through the bridge-state transition center
\begin{equation}
t_0(a)=\frac{\sqrt a}{1+\sqrt a},
\end{equation}
or equivalently
\begin{equation}
a=\left(\frac{\tau}{1-\tau}\right)^2,\qquad \tau\in(0,1/2],
\end{equation}
so that bridge design can be performed by selecting the desired location of the source--target balance point, with $\tau=0.5$ corresponding to the standard VP limit.
\end{enumerate}

In this way, REF is not merely a hand-crafted bridge. It is a high-dimensional bridge-design framework guided by three coupled goals: informative but not brittle state statistics, stable inference geometry, and good joint learnability of the bridge input and the oracle direction field. The resulting framework jointly targets stable radius-locked inference, interpretable source--target transition control, and improved train--inference alignment in high-dimensional token spaces.

==> sections_old/REF_old.tex <==
\section{A Direction-only Flow-Matching Framework with Radius-Locking Inference}
\label{sec:REF}

We propose a direction-only flow-matching framework for conditional token generation in high-dimensional continuous spaces. The central idea is to decouple \emph{direction} and \emph{step length}: instead of training the model to regress a full velocity vector---thereby jointly learning both its direction and magnitude---we train it to predict only the transport \emph{direction}, and recover the step length at inference time from geometric constraints induced by the bridge. This is motivated by a systematic pathology of standard $v$-prediction under angular errors, which becomes particularly harmful in high dimensions.

This section is organized as follows. We begin by analyzing why standard rectified flow with $v$-prediction can underestimate effective step sizes under angular errors, which is particularly harmful in hyperspherical token spaces. We then present a direction-only modeling framework to address the under-stepping issue, where the inference step size is recovered via a \emph{radius schedule} where ``radius'' corresponds to $\|x_t\|$. We then highlight the ``contraction regime problem'' in standard rectified-flow (RF) bridge where radius-locking inference can be ill-defined, which motivates an variant of the variance-preserving (VP) bridge, which we refer to as the \textbf{radius expansion flow (REF)}, that enables \emph{monotically increasing radius schedule} that systematically bypasses the issue in RF bridge.

\subsection{Rectified Flow with $v$-Prediction: Step-Size Underestimation under Angular Errors}
\label{subsec:rf_vpred}

We first recall a standard rectified-flow (RF) training setup. Let $x_1\in\mathbb{S}^{N-1}(R)$ denote a target token and let $x_0$ be a source sample. A linear bridge is defined by
\begin{equation}
x_t = (1-t)x_0 + t x_1,\qquad t\in[0,1],
\end{equation}
with the corresponding constant transport vector
\begin{equation}
v^\star = x_1 - x_0.
\end{equation}
Standard RF trains a network $\hat v(x_t,t,c)$ (optionally conditioned on $c$) by minimizing an $\ell_2$ regression loss $\|\hat v - v^\star\|_2^2$.

\paragraph{$v$-pred magnitude shrinkage under directional mismatch.}
We analyze a purely geometric property of $\ell_2$ regression: if the predicted direction is mismatched with the target direction, then the optimal predicted magnitude is reduced. Decompose the prediction into a unit direction and a scalar magnitude:
\begin{equation}
\hat v \;=\; \hat s\,\hat r,\qquad \hat r\in\mathbb{S}^{N-1}(1),\ \hat s\ge 0,
\end{equation}
and similarly write the ground-truth transport as
\begin{equation}
v^\star \;=\; s^\star r^\star,\qquad r^\star=\mathrm{Norm}_1(v^\star)\in\mathbb{S}^{N-1}(1),\ s^\star=\|v^\star\|_2.
\end{equation}
Let $\theta=\angle(\hat r,r^\star)$ denote the angular mismatch, so that $\langle \hat r,r^\star\rangle=\cos\theta$.
Conditioned on a fixed direction $\hat r$, the $\ell_2$ objective is a convex quadratic in $\hat s$:
\begin{align}
\|\hat v - v^\star\|_2^2
&=\|\hat s\hat r - s^\star r^\star\|_2^2 \nonumber\\
&=\hat s^2 + (s^\star)^2 - 2\hat s s^\star \langle \hat r,r^\star\rangle \nonumber\\
&=\hat s^2 + (s^\star)^2 - 2\hat s s^\star \cos\theta.
\label{eq:vpred_quadratic_ref}
\end{align}
Minimizing \eqref{eq:vpred_quadratic_ref} over $\hat s$ yields
\begin{equation}
\hat s_{\mathrm{opt}} \;=\; s^\star \cos\theta,
\label{eq:vpred_shrinkage_ref}
\end{equation}
i.e., the optimal magnitude is scaled by the cosine of the directional mismatch. Equivalently, the component of $\hat v$ along the true transport direction satisfies
\begin{equation}
\langle \hat v, r^\star\rangle
=
\hat s_{\mathrm{opt}}\langle \hat r,r^\star\rangle
=
s^\star \cos^2\theta.
\end{equation}

\paragraph{Implication for iterative sampling.}
In iterative integration, this shrinkage translates into smaller-than-intended step sizes and can accumulate over multiple steps, yielding a biased trajectory that fails to reach the intended radius. In high-dimensional token spaces, such radius drift is particularly harmful because the decoder (no matter standard VAEs or our spherical tokenizer) is trained on a thin shell or a hypersphere and is sensitive to off-shell samples. Moreover, step size shrinkage may also make intermediate output statistics (e.g., $\|x_t\|_2$) biased from their training-time counterparts, further leads to training-inference mismatch.

\subsection{Direction-only Modeling and Radius-Locking Inference}
\label{subsec:rf_radius_locking}

The above analysis immediately suggests a natural question: if jointly predicting direction and magnitude causes systematic under-stepping, can we instead \emph{predict only the direction} and recover the step length by other means at inference time? A natural candidate is to exploit bridge-induced statistics. We start from the standard RF bridge and show that in high dimensions, the norm of the intermediate state is already almost determined by time. Consider the standard rectified-flow bridge
\begin{equation}
x_t=(1-t)x_0+t x_1,\qquad t\in[0,1],
\label{eq:rf_standard_bridge}
\end{equation}
where the source is sampled from an isotropic Gaussian,
\begin{equation}
x_0 \sim \mathcal N(0,I_N),
\end{equation}
and the target token lies on the token sphere
\begin{equation}
x_1\in\mathbb{S}^{N-1}(R),\qquad R=\sqrt N.
\end{equation}
By high-dimensional thin-shell concentration, $\|x_0\|_2\approx R$ with high probability, and for a random source/target pair we also have $\langle x_0,x_1\rangle\approx 0$ relative to $R^2$. Expanding \eqref{eq:rf_standard_bridge} yields
\begin{align}
\|x_t\|_2^2
&=\|(1-t)x_0+t x_1\|_2^2 \nonumber\\
&=(1-t)^2\|x_0\|_2^2+t^2\|x_1\|_2^2+2t(1-t)\langle x_0,x_1\rangle \nonumber\\
&\approx R^2\big((1-t)^2+t^2\big)\;\triangleq\;\rho_{\mathrm{RF}}(t)^2.
\label{eq:rf_rho_schedule}
\end{align}
Thus, in high dimensions the radius $\|x_t\|_2$ is already highly concentrated around a deterministic time-dependent schedule
\begin{equation}
\rho_{\mathrm{RF}}(t)=R\sqrt{(1-t)^2+t^2}.
\end{equation}

This observation suggests that the step length need not be learned by the model under high-dimensional approximations: if the model predicts the local transport direction, then the desired radius at the next time is already specified by the bridge. We therefore consider a \emph{direction-only} predictor
\begin{equation}
\hat r(x_t,t,c)\in\mathbb S^{N-1}(1),
\end{equation}
trained to match the oracle velocity direction
\begin{equation}
r_t^\star=\mathrm{Norm}_1(v^\star)=\mathrm{Norm}_1(x_1-x_0).
\end{equation}
At inference time, instead of asking the model to provide the full velocity magnitude, we recover the step size from the target radius schedule. Let $x_{t_k}$ denote the current state and let $\hat r_{t_k}=\hat r(x_{t_k},t_k,c)$ be the predicted direction. We update
\begin{equation}
x_{t_{k+1}} = x_{t_k} + \Delta_{t_k}\,\hat r_{t_k},
\label{eq:rf_radius_lock_update}
\end{equation}
and enforce the \emph{radius-locking} constraint
\begin{equation}
\|x_{t_{k+1}}\|_2 = \rho_{\mathrm{RF}}(t_{k+1}).
\label{eq:rf_radius_lock_constraint}
\end{equation}
Expanding \eqref{eq:rf_radius_lock_constraint} yields
\begin{equation}
\Delta_{t_k}^2 + 2\langle x_{t_k},\hat r_{t_k}\rangle\,\Delta_{t_k}
+ \big(\|x_{t_k}\|_2^2-\rho_{\mathrm{RF}}(t_{k+1})^2\big)=0.
\label{eq:rf_radius_lock_quad}
\end{equation}
Thus the step size is recovered from a scalar quadratic equation rather than regressed by the network. 

However, it is easy to notice that the schedule $\rho_{\mathrm{RF}}(t)$ is \emph{non-monotone}: it first shrinks and then expands and the minimum-radius time (transition point) is $t_{\min}=\frac{1}{2}$. We call $t\in[0,t_{\min}]$ the \emph{contraction phase} and $t\in[t_{\min},1]$ the \emph{expansion phase}. During the expansion phase, the target radius always increases, so the quadratic \eqref{eq:rf_radius_lock_quad} always admits a valid positive root. Writing
\begin{equation}
c_k=\langle x_{t_k},\hat r_{t_k}\rangle,
\qquad
\Delta\rho_k^2=\rho_{\mathrm{RF}}(t_{k+1})^2-\rho_{\mathrm{RF}}(t_k)^2,
\end{equation}
we obtain
\begin{equation}
\Delta_{t_k}=-c_k+\sqrt{c_k^2+\Delta\rho_k^2}.
\label{eq:rf_radius_lock_positive_root}
\end{equation}
Hence the expansion phase is always well-defined. In the contraction phase, however, we have $\Delta\rho_k^2<0$ and the discriminant $c_k^2+\Delta\rho_k^2$ may become negative. Geometrically, along a fixed direction $\hat r_{t_k}$ the \emph{minimal achievable radius} is attained at
\begin{equation}
\Delta_{t_k}^{\min}=-c_k,
\end{equation}
which yields the closest point to the origin on the ray,
\begin{equation}
x_{t_{k+1}}^\ast = x_{t_k}+\Delta_{t_k}^{\min}\hat r_{t_k}.
\end{equation}
When $c_k^2+\Delta\rho_k^2<0$, the target radius $\rho_{\mathrm{RF}}(t_{k+1})$ is smaller than $\|x_{t_{k+1}}^\ast\|_2$, hence the radius-locking constraint is infeasible along the direction and a \emph{retraction} operator is required to map $x_{t_{k+1}}^\ast$ to the target radius. To define a universally feasible retraction operator for any $x_{t_{k+1}}^\ast$, we can simply take the radial normalization operator:
\begin{equation}
R_{\rho'}(x_{t_{k+1}})
=
\rho_{\mathrm{RF}}(t_{k+1})\mathrm{Norm}_1(x_{t_{k+1}}^\ast).
\label{eq:rf_radial_retract}
\end{equation}
This mapping is always well-defined and enforces $\|x_{t_{k+1}}\|_2=\rho_{\mathrm{RF}}(t_{k+1})$ by construction. Crucially, the radial normalization operator is \emph{necessarily orthogonal} to the predicted direction. Indeed, by definition of $x_{t_{k+1}}^\ast$ we have $\langle x_{t_{k+1}}^\ast,\hat r_{t_k}\rangle=0$, hence
\begin{equation}
\left\langle \frac{x_{t_{k+1}}^\ast}{\|x_{t_{k+1}}^\ast\|_2},\ \hat r_{t_k}\right\rangle = 0,
\qquad\Rightarrow\qquad
\angle\!\left(\frac{x_{t_{k+1}}^\ast}{\|x_{t_{k+1}}^\ast\|_2},\hat r_{t_k}\right)=\frac{\pi}{2}.
\label{eq:rf_retract_orthogonal}
\end{equation}
That is, whenever the radius-locking equation is infeasible and we fall back to the closest point $x_{t_{k+1}}^\ast$ followed by radial normalization, the retraction introduces an update component that is \emph{maximally misaligned} with the model-predicted direction. This geometric mismatch is intrinsic to the infeasible contraction regime: it does not depend on the particular choice of model or training objective, but follows directly from the geometry and the requirement to hit a smaller target radius. This issue is particularly severe in settings where a single network predicts directions for multiple inputs (e.g., a NAR model): within the same forward pass, some inputs may satisfy $c_k^2+\Delta\rho_k^2\ge 0$ (unbiased, exact radius-locking), while others satisfy $c_k^2+\Delta\rho_k^2<0$ (biased, retracted update). This creates a sharp training--inference mismatch: during training, the model is supervised on oracle bridge states constructed from the ground-truth source-target pairs, so every intermediate input lies exactly on the intended bridge distribution. At inference time, however, the sampler produces states that are a mixture of (i) exact updates and (ii) biased retracted updates, and the latter can move the trajectory off the oracle bridge in a time-dependent manner. Since later-step predictions $\hat r_{t_{k'}}$ are conditioned on these perturbed states, the mismatch compounds across steps and can be strongly amplified in the subsequent expansion phase.

\subsection{Radius Expansion Flow}
\label{subsec:ref}

The above analysis suggests a natural next question: can we construct a bridge whose radius is \emph{monotone throughout the entire trajectory}, so that the radius-locking inference is always well-defined? We show that by constructing an \emph{inner-to-outer} flow with a \emph{variance-preserving} bridge, such constraint can be easily satisfied. We refer to this construction as \textbf{radius expansion flow (REF)}, as it ensures a monotonically expanding radius schedule.

We now assume that the source $x_0$ is sampled on a sphere of radius $aR,\,a\in\mathbb R^+$ instead of an isotropic Gaussian, as it provides exact fixed-norm property without the need of high-dimensional approximation. Consider the bridge
\begin{equation}
x_t=\alpha(t)x_0+\beta(t)x_1,\qquad t\in[0,1],
\label{eq:general_alpha_beta_bridge}
\end{equation}
with boundary conditions
\begin{equation}
\alpha(0)=1,\quad \beta(0)=0,\qquad
\alpha(1)=0,\quad \beta(1)=1.
\label{eq:alpha_beta_boundary}
\end{equation}
Expanding the squared norm gives
\begin{equation}
\|x_t\|_2^2
=
\alpha(t)^2\|x_0\|_2^2+\beta(t)^2\|x_1\|_2^2+2\alpha(t)\beta(t)\langle x_0,x_1\rangle.
\label{eq:general_bridge_norm_exact}
\end{equation}
Under the same high-dimensional concentration approximation $\langle x_0,x_1\rangle\approx 0$, this becomes
\begin{equation}
\|x_t\|_2^2
\approx
R^2\big(a^2\alpha(t)^2+\beta(t)^2\big),
\label{eq:general_bridge_norm_approx}
\end{equation}
Hence a sufficient condition for monotone radius is that the scalar function
\begin{equation}
a^2\alpha(t)^2+\beta(t)^2
\end{equation}
be monotonic. A particularly natural choice is the variance-preserving (VP) parameterization \cite{}
\begin{equation}
\alpha(t)=\cos\theta(t),\qquad \beta(t)=\sin\theta(t), \qquad \theta(t)=\frac{\pi}{2}t.
\label{eq:vp_alpha_beta}
\end{equation}
Substituting \eqref{eq:vp_alpha_beta} into \eqref{eq:general_bridge_norm_approx} yields
\begin{equation}
\|x_t\|_2^2
\approx
R^2\big(a^2\cos^2\theta(t)+\sin^2\theta(t)\big).
\label{eq:vp_bridge_norm}
\end{equation}
Differentiating with respect to $\theta$ gives
\begin{equation}
\frac{d}{d\theta}\Big(a^2\cos^2\theta+\sin^2\theta\Big)
=
2(1-a^2)\sin\theta\cos\theta.
\end{equation}
Therefore, for any $a\in(0,1)$, the radius is \emph{monotone increasing} throughout the entire bridge, and for $a=1$ the radius is \emph{constant} throughout the entire bridge (corresponds to the standard VP bridge with isotropic Gaussian source distribution). This immediately removes the contraction-phase pathology of standard RF. The radius schedule thus becomes
\begin{equation}
\rho_{\mathrm{REF}}(t)
=
R\sqrt{a^2\cos^2\!\Big(\frac{\pi t}{2}\Big)+\sin^2\!\Big(\frac{\pi t}{2}\Big)}.
\label{eq:ref_rho_schedule}
\end{equation}

We determine an $R$-agnostic choice of $a$ by balancing two competing desiderata. First, the source should retain sufficient randomness: if $a$ is too small, the source energy becomes weak and the bridge is dominated by the deterministic radius-growth schedule rather than by the source variation itself. A natural scale for this source randomness is the source norm squared $
\|x_0\|_2^2 = a^2R^2$. Second, the bridge should exhibit a sufficiently strong observable radius change for radius locking to be informative and stable. A natural scale for this is the total radius-squared growth budget $\|x_1\|_2^2-\|x_0\|_2^2 = R^2(1-a^2)$. When $a\to 1$, the source is nearly on the data shell and the dynamic range of radius locking collapses; when $a\to 0$, the radius-growth budget is maximal but the source contribution becomes too weak. To obtain a dimension- and model-independent canonical choice, we balance these two scales:
\begin{equation}
a^2R^2 = R^2(1-a^2).
\end{equation}
Solving gives
\begin{equation}
\boxed{
a=\frac{1}{\sqrt2}.
}
\label{eq:a_ref}
\end{equation}
This choice makes the source-energy scale and the radius-growth budget equal in squared-energy units, yielding a simple symmetry between source randomness and observable geometric progress.

The overall training and inference procedure of REF is summarized in Algorithm~\ref{alg:ref}.

\begin{algorithm}[!ht]
\caption{Radius Expansion Flow (REF): training and inference}
\label{alg:ref}
\DontPrintSemicolon
\KwIn{Token dimension $N$, conditioning $c$, $R=\sqrt N$, inner ratio $a=1/\sqrt2$, time schedule $\theta(t)=\frac{\pi}{2}t$, radius schedule $\rho_{\mathrm{REF}}(t)=R\sqrt{a^2\cos^2\theta(t)+\sin^2\theta(t)}$}
\KwOut{final token $x_{t=1}\in\mathbb{S}^{N-1}(R)$}

\BlankLine
\textbf{Training}\;
\Indp
Sample target token $x_1\in\mathbb{S}^{N-1}(R)$\;
Sample source $x_0\sim \mathrm{Unif}(\mathbb{S}^{N-1}(R))$\;
Sample $t\sim\mathrm{Unif}(0,1)$ and construct bridge state
\[
x_t=\cos\theta(t)\,x_0+\sin\theta(t)\,x_1
\]
\;
Construct oracle direction
\[
r_t^\star
=
\mathrm{Norm}_1\!\Big(\cos\theta(t)\,x_1-\sin\theta(t)\,x_0\Big)
\]
\;
Predict $\hat r_t=\mathrm{Norm}_1(\hat r(x_t,t,c))$\;
Backpropagate by minimizing
\[
L_{\mathrm{REF}} = 1-\cos(\hat r_t,r_t^\star)
\]
\;
\Indm

\BlankLine
\textbf{Inference}\;
\Indp
Sample $x_{t_0}\sim \mathrm{Unif}(\mathbb{S}^{N-1}(R))$\;
Choose a time grid $0=t_0<t_1<\cdots<t_K=1$\;
\For{$k\leftarrow 0$ \KwTo $K-1$}{
  Predict unconditional and conditional directions
  \[
  \hat r_{\varnothing}\leftarrow \hat r(x_{t_k},t_k,\varnothing),\qquad
  \hat r_c\leftarrow \hat r(x_{t_k},t_k,c)
  \]
  \;
  Apply CFG and normalize:
  \[
  \hat r_{\mathrm{cfg}}
  \leftarrow
  \mathrm{Norm}_1\!\big(
  \hat r_{\varnothing}
  +
  w_{\mathrm{cfg}}(\hat r_c-\hat r_{\varnothing})
  \big)
  \]
  \;
  Compute $\Delta_{t_k}$ by radius locking:
  \[
  \Delta_{t_k}
  =
  -\langle x_{t_k},\hat r_{\mathrm{cfg}}\rangle
  +
  \sqrt{
  \langle x_{t_k},\hat r_{\mathrm{cfg}}\rangle^2
  +
  \rho_{\mathrm{REF}}(t_{k+1})^2-\|x_{t_k}\|_2^2
  }
  \]
  \;
  Update
  \[
  x_{t_{k+1}} = x_{t_k} + \Delta_{t_k}\hat r_{\mathrm{cfg}}
  \]
  \;
}
\Return{$x_{t=1}$}\;
\Indm
\end{algorithm}

\subsection{Discussion: Connecting REF with Standard VP-bridge and Spherical Flow Matching}

Note that if we set $a=1$ in REF, we have $\|x_t\|_2^2
\approx
R^2\big(\cos^2\theta(t)+\sin^2\theta(t)\big)=R^2$ and the radius schedule becomes constant on the token sphere. It is easy to see that $a=1$ corresponds to the standard VP bridge with isotropic Gaussian $x_0$ under high-dimensional approximations, and such constant-radius schedule can be connected to \emph{spherical flow matching (SFM)} \cite{chen2023flow} where the entire bridge lies strictly on the geodesic curve between source and target. Here we identify the core difference between a \emph{constant} radius schedule and a \emph{monotonic increasing} radius schedule by three factors: the \emph{$t$-identifiability}, the \emph{locking-inference feasibility}, and the \emph{self-boostrapping shortcut}.

\subsubsection{$t$-identifiability}

Generative models typically rely on \emph{time embeddings} to identify the location of the current input on the bridge. As we discussed in Sec.~\ref{subsec:rf_vpred}, the misalignment between $\|x_t\|$ and $t$ may cause training-inference mismatch and may hurt inference-phase performance even if the training is smooth and stable. When $\|x_t\|$ is (statistically) uniquely determined by $t$, the location of $x_t$ on the bridge can be directly inferred from $\|x_t\|$, which means that the \emph{$t$-identifiability} of $x_t$ under such radius schedule is adequately high so that the time embedding only serves as an auxiliary information that helps the optimization process of the model, instead of being the only information source of the location of $x_t$. However, for standard VP bridge or SFM where $\|x_t\|$ remains constant across the bridge, the time embedding becomes the only identifier to locate the current $x_t$ on the bridge. In this case, the core statistical property of $x_t$ with respect to $t$ becomes the signal-to-noise ratio (SNR) between the source and the target, which is implicit (compared to $\|x_t\|$) and can be ambiguous when $x_t$ locates on different source-target bridges. This makes the generative model relies more on the time embedding instead of statistical properties of $x_t$ to perform velocity/direction field estimation, which can be systematically harder.

\subsubsection{Locking-inference Feasibility}

Here we derive a \emph{radian-locking} inference scheme for direction-only SFM modeling and show its potential drawbacks.

Given two endpoints $x_a,x_b\in\mathbb{S}^{N-1}(R)$, let
\begin{equation}
\omega \;=\; \arccos\!\Big(\frac{\langle x_a,x_b\rangle}{R^2}\Big)\in[0,\pi]
\end{equation}
denote their geodesic angle. The spherical linear interpolation (slerp) defines a constant-speed geodesic curve
\begin{equation}
x_t \;=\; \mathrm{slerp}(x_a,x_b;t)
\;=\;
\frac{\sin((1-t)\omega)}{\sin\omega}\,x_a
+
\frac{\sin(t\omega)}{\sin\omega}\,x_b,
\qquad t\in[0,1],
\label{eq:slerp_bridge}
\end{equation}
which satisfies $\|x_t\|_2=R$ for all $t$. With direction-only modeling, SFM predicts a tangent direction field $\hat v(x_t,t,c)\in T_{x_t}$ using the Riemannian logarithm map on the sphere
\begin{equation}
v_t^\star
\;=\;
\mathrm{Norm}_1\!\big(\mathrm{Log}_{x_t}(x_b)\big).
\label{eq:sfm_v_target}
\end{equation}
We define the total geodesic arc length of the bridge by the endpoint angle
\begin{equation}
\omega \;\triangleq\; \angle(x_a,x_b),
\end{equation}
which satisfies (under high-dimensional approximations)
\begin{equation}
\cos\omega
=
\frac{\langle x_a,\bar x_b\rangle}{\|x_a\|_2\,\|\bar x_b\|_2}
=
\frac{\langle x_a,x_b\rangle}{\|x_a\|_2\,\|x_b\|_2}
\approx
0,\qquad \omega\approx \frac \pi2.
\end{equation}
Thus the endpoint is almost always $\pi/2$ away from the start point, which enables us to design a radian-locking inference scheme that constrains the angle between intermediate states and the start point during inference. Specifically, let $0=t_0<t_1<\cdots<t_{K_1}=1$ be the SFM phase time grid and prescribe a radian schedule $\alpha_k=\alpha(t_k)=\frac{\pi t_k}{2}$. At step $k$, the model predicts a unit tangent direction
$\hat u_k \in T_{x_k}\mathbb{S}^{N-1}(R)$, and we choose an angular step $\eta_k\ge 0$ along $\hat u_k$ and update by the exponential map on $\mathbb{S}^{N-1}(R)$:
\begin{equation}
x_{k+1}=x_k(\eta_k,\,\hat u_k)
\triangleq
\mathrm{Exp}_{x_k}\!\big(R\eta_k\,\hat u_k\big)
=
\cos\eta_k\,x_k+\sin\eta_k\,R\hat u_k,
\label{eq:sfm_exp_update_eta}
\end{equation}
where $\eta_k$ is an \emph{angular} step (radians) and the corresponding arc-length is $R\eta_k$.
Radian locking enforces the progress constraint
\begin{equation}
\angle\big(x_k(\eta_k,\,\hat u_k),x_0\big)=\alpha_{k+1}
\quad\Longleftrightarrow\quad
\frac{\langle x_k(\eta_k,\,\hat u_k),x_0\rangle}{R^2}=\cos\alpha_{k+1}.
\label{eq:sfm_angle_lock_constraint}
\end{equation}
Define the scalars
\begin{equation}
A_k=\frac{\langle x_k,x_0\rangle}{R^2}=\cos\alpha_k,
\qquad
B_k=\frac{\langle \hat u_k,x_0\rangle}{R}.
\end{equation}
Substituting \eqref{eq:sfm_exp_update_eta} into \eqref{eq:sfm_angle_lock_constraint} yields a 1D trigonometric equation for $\eta_k$:
\begin{equation}
A_k\cos\eta_k + B_k\sin\eta_k = \cos\alpha_{k+1}.
\label{eq:sfm_eta_equation}
\end{equation}
Let $R_k=\sqrt{A_k^2+B_k^2}$, $\phi_k=\mathrm{atan2}(B_k,A_k)$ and $\gamma_k=\arccos(\frac{\cos\alpha_{k+1}}{R_k})$. Since
$A_k\cos\eta + B_k\sin\eta = R_k\cos(\eta-\phi_k)$, the two solution branches of \eqref{eq:sfm_eta_equation} are
\begin{equation}
\eta_k^{(\pm)}=\phi_k \pm \gamma_k.
\label{eq:sfm_two_branches}
\end{equation}

Eq.~\eqref{eq:sfm_eta_equation} is feasible iff $
|\cos\alpha_{k+1}|\le R_k$. Similar to Eq.~\ref{eq:rf_radial_retract}, a retraction operation is still required in this case, which leads to the same training-inference mismatch problem discussed in Sec.~\ref{subsec:rf_radius_locking}. Moreover, such radian-locking scheme is designed based on \emph{relative statistics} (i.e., angle between $x_k$ and the start point) instead of \emph{absolute statistics} (i.e., $\|x_t\|$), which also suffers from the $t$-identifiability problem as a same $x_k$ can still correspond to different $t$ locations on bridges of different start and end points.

\subsubsection{Self-boostrapping Shortcut}

We empirically observe that applying SFM to the aforementioned spherical tokenizer can suffer from \emph{conditioning collapse}, where the conditional generative model may easily ignores the conditioning signal $c$ due to training dynamics. We argue that this failure mode is primarily cased by an interaction between (i) the \emph{basin structure} induced by the tokenizer/decoder training objective and (ii) the fact that SFM trajectories remain on the same hyperspherical shell as valid tokens.

\paragraph{Decoder-induced basins on the token sphere.}
Let $D:\mathbb{S}^{N-1}(R)\to\mathcal{X}$ denote the tokenizer decoder and let $d_\phi(\cdot,\cdot)$ be the reconstruction/perceptual metric used to define output similarity. For a target token $x_1\in\mathbb{S}^{N-1}(R)$, define its \emph{basin} on the token sphere by
\begin{equation}
\mathcal{B}_\epsilon(x_1)
\;\triangleq\;
\Big\{z\in\mathbb{S}^{N-1}(R):\ d_\phi\big(D(z),D(x_1)\big)\le \epsilon\Big\}.
\label{eq:basin_def}
\end{equation}
The tokenizer is trained with dimension-aware geodesic perturbations (Sec.~\ref{sec:noise_inject}) so that decoding is stable within a controlled angular neighborhood around each training token. In particular, for typical perturbation angles $\theta$ in the training phase, the reconstruction objective encourages
\begin{equation}
D\!\big(\mathrm{Exp}_{x_1}(R\theta u)\big)\approx D(x_1)
\quad\Rightarrow\quad
\mathrm{Exp}_{x_1}(R\theta u)\in \mathcal{B}_\epsilon(x_1)
\ \text{for many }u\in T_{x_1}\mathbb{S}^{N-1}(R),
\label{eq:basin_contains_cap}
\end{equation}
i.e., each $x_1$ is surrounded by a nontrivial basin on the sphere. Importantly, the tokenizer is also trained to avoid \emph{representation collapse} (e.g., degenerate embeddings with vanishing variance or rank), so distinct tokens are encouraged to remain semantically separable. Consequently, basins corresponding to different targets are expected to be largely disjoint:
\begin{equation}
\mathcal{B}_\epsilon(x_1)\cap \mathcal{B}_\epsilon(x_1') \approx \emptyset
\qquad \text{for }x_1\neq x_1',
\label{eq:basin_separation}
\end{equation}
since otherwise distinct tokens would decode to indistinguishable outputs, contradicting the tokenizer objective.

\paragraph{Posterior sharpening and self-bootstrapping on-shell.}
Consider SFM with endpoint $x_b=x_1$ and intermediate states $x_t\in\mathbb{S}^{N-1}(R)$ along the slerp bridge. Because the entire trajectory stays on the same shell as valid tokens, it can enter the basin $\mathcal{B}_\epsilon(x_1)$ for a non-negligible range of times $t$ (often well before $t\to 1$). Once $x_t\in\mathcal{B}_\epsilon(x_1)$, the endpoint becomes effectively determined by $x_t$:
\begin{equation}
x_t\in\mathcal{B}_\epsilon(x_1)
\ \stackrel{\eqref{eq:basin_separation}}{\Longrightarrow}\
\mathbb{P}(X_1=x_1\mid X_t=x_t,t)\approx 1,
\label{eq:posterior_sharpening}
\end{equation}
i.e., the conditional uncertainty over the endpoint collapses (``posterior sharpening''). In this regime, the optimal regression target for the velocity field satisfies
\begin{equation}
\mathbb{E}\big[v_t^\star \mid X_t=x_t,t,c\big]
\;\approx\;
\mathbb{E}\big[v_t^\star \mid X_t=x_t,t\big],
\label{eq:cond_redundant}
\end{equation}
so the conditioning signal $c$ becomes nearly redundant for minimizing the SFM loss. This creates a \emph{self-bootstrapping shortcut}: the model can reduce training error by learning a mapping from $x_t$ to a velocity that points toward the basin center, without using $c$. 

\paragraph{Training--inference dynamics and error accumulation.}
The shortcut in \eqref{eq:cond_redundant} is particularly harmful because the same network parameters are shared across all times. Once the model learns to ignore $c$ on a subset of times (typically large $t$ where basin membership is common), the resulting representation and attention pathways tend to generalize to smaller $t$ as well. However, for small $t$ the state is farther from any basin center and the conditional ambiguity is higher, so a $c$-agnostic predictor incurs large directional errors. Equivalently, the learned predictor approaches $\mathbb{E}[v_t^\star\mid x_t,t]$ on large $t$, and parameter sharing biases it toward the same $c$-agnostic conditional expectation on small $t$, where $\mathbb{E}[v_t^\star\mid x_t,t]$ is a poor surrogate for $\mathbb{E}[v_t^\star\mid x_t,t,c]$.

At inference time, these small-$t$ errors are amplified: early-time deviations move the trajectory toward an incorrect basin, after which the on-shell dynamics further reinforce the wrong endpoint (since basin membership again sharpens the effective posterior). This creates a feedback loop in which (i) large-$t$ training encourages a $c$-agnostic shortcut, (ii) the shortcut induces large errors at small $t$, and (iii) the resulting trajectory drift makes later-time updates increasingly consistent with the wrong basin, further weakening conditional dependence or even generating completely collapsed outputs.

\paragraph{Why this shortcut is specific to on-shell spherical trajectories.}
The above mechanism relies on the trajectory remaining on the token shell where decoder basins are defined. In contrast, Euclidean linear bridges typically traverse off-shell regions where $D(\cdot)$ is not trained to be stable and where basin membership is less likely, so the posterior sharpening effect in \eqref{eq:posterior_sharpening} is weaker. Thus, the same tokenizer design that promotes well-separated, stable basins on the sphere (to avoid representational collapse) can inadvertently make on-shell SFM training more prone to conditioning collapse.


==> sections_old/SFM.tex <==
\section{Generative Modeling on the Hierarchical Sphere}
\label{sec:generation}

With the tokenizer of Sec.~\ref{sec:tokenizer}, each token is no longer an unconstrained Euclidean vector, but a point on a fixed-radius sphere endowed with a predefined group-wise energy hierarchy. This changes the geometry of continuous generation in a fundamental way. The source state should be interpreted as a random-like spherical state whose group energies are approximately equalized, while the target state is a structured token on a product-of-spheres manifold with non-uniform group energies. A suitable generative bridge should therefore be geometrically compatible with the sphere, should preserve the distinction between random-like and structured states, and should avoid introducing training shortcuts through easily exploitable progress statistics.

This section develops the corresponding generation framework. We first analyze a general flow-matching bridge from the perspective of \emph{progress identifiability}, and show that in high-dimensional continuous tokens many low-order statistics become almost deterministic functions of the bridge progress. This creates a characteristic source of training--inference mismatch, especially in non-autoregressive multi-token prediction. We then motivate the use of spherical flow matching (SFM), whose bridge follows geodesics on the sphere and removes the strongest radial progress proxy. Next, we show that under the group-energy hierarchy introduced in Sec.~\ref{sec:tokenizer}, the SFM bridge admits a coarse-to-fine interpretation through group-wise signal-to-noise evolution. Finally, we present the practical training and inference rules used in our generator: group-structured \textit{x}-prediction, manifold-preserving classifier-free guidance in \textit{x}-space, and a weighted loss whose form is directly derived from the single-step error of spherical DDIM-style inference.

\subsection{Progress Identifiability in High-Dimensional Continuous Bridges}
\label{subsec:gen_progress_identifiability}

We begin from a generic continuous bridge between a source token $x_0$ and a target token $x_1$. For clarity, we first write the bridge in the affine form
\begin{equation}
x_t = a_t x_0 + b_t x_1,
\qquad
t\in[0,1],
\label{eq:general_affine_bridge}
\end{equation}
where the scalar coefficients satisfy the endpoint conditions
\begin{equation}
a_0=1,\ b_0=0,
\qquad
a_1=0,\ b_1=1.
\end{equation}
Standard rectified flow (RF) corresponds to
\begin{equation}
a_t = 1-t,
\qquad
b_t = t.
\end{equation}
Even before committing to a particular bridge, \eqref{eq:general_affine_bridge} already reveals a general phenomenon: in high dimension, many low-order statistics of $x_t$ become almost deterministic functions of the bridge coefficients $(a_t,b_t)$, and therefore almost deterministic functions of $t$ itself.

We refer to such low-order statistics as \emph{progress-identifiability proxies}, because they allow the model to infer where the current state lies on the bridge and how much source/target information it contains.

\paragraph{Global norm.}
Assume that $x_0$ and $x_1$ are high-dimensional vectors with concentrated norms and negligible cross inner product, i.e.
\begin{equation}
\|x_0\|_2^2 \approx N,
\qquad
\|x_1\|_2^2 \approx N,
\qquad
\langle x_0,x_1\rangle \approx 0.
\label{eq:high_dim_endpoint_assumptions}
\end{equation}
Then
\begin{align}
\|x_t\|_2^2
&=
a_t^2\|x_0\|_2^2+b_t^2\|x_1\|_2^2+2a_tb_t\langle x_0,x_1\rangle
\nonumber\\
&\approx
N(a_t^2+b_t^2).
\label{eq:norm_xt_general}
\end{align}
Thus the global norm is almost fully determined by $(a_t,b_t)$.

\paragraph{Alignment with source and target.}
Under the same assumptions,
\begin{align}
\langle x_t,x_1\rangle
&=
a_t\langle x_0,x_1\rangle+b_t\|x_1\|_2^2
\approx
b_t N,
\\
\langle x_t,x_0\rangle
&=
a_t\|x_0\|_2^2+b_t\langle x_1,x_0\rangle
\approx
a_t N.
\end{align}
Combining with \eqref{eq:norm_xt_general}, we obtain
\begin{align}
\cos(x_t,x_1)
&=
\frac{\langle x_t,x_1\rangle}{\|x_t\|_2\|x_1\|_2}
\approx
\frac{b_t}{\sqrt{a_t^2+b_t^2}},
\label{eq:cos_xt_x1_general}
\\
\cos(x_t,x_0)
&\approx
\frac{a_t}{\sqrt{a_t^2+b_t^2}}.
\label{eq:cos_xt_x0_general}
\end{align}
Again, these are almost deterministic functions of the bridge coefficients.

\paragraph{Signal-to-noise ratio.}
If one interprets the source contribution $a_t x_0$ as the noise component and the target contribution $b_t x_1$ as the signal component, then the energy-based SNR is
\begin{equation}
\mathrm{SNR}(t)
=
\frac{b_t^2\|x_1\|_2^2}{a_t^2\|x_0\|_2^2}
\approx
\frac{b_t^2}{a_t^2}.
\label{eq:snr_general_bridge}
\end{equation}
Thus the source--target information ratio is likewise almost a deterministic function of $t$.

\paragraph{Implication.}
In high-dimensional continuous token spaces, the bridge state $x_t$ often carries cheap and highly reliable statistical cues about its own bridge progress. If the model is additionally given an explicit time embedding, then the bridge progress becomes even more identifiable. This is not necessarily beneficial. During training, the bridge state is constructed from the ground-truth target, so the nominal progress $t$ and all progress-identifiability proxies are perfectly matched. During inference, however, the generated state after one or more imperfect updates need not preserve the same statistical relations. Even a small prediction bias can move the state to a region whose norm, source--target ratio, or angular relation no longer matches the nominal progress index. The model is then queried on states whose apparent progress differs from the time label with which they are paired.

This mismatch is especially consequential in non-autoregressive multi-token prediction. During training, all tokens in the predicted set are generated from the same clean bridge construction, hence their progress statistics are jointly consistent. During inference, different tokens may accumulate different amounts of error, so their effective denoising progress may drift apart. The larger the predicted token set, the more severe this cross-token inconsistency can become.

\subsection{Why Spherical Flow Matching}
\label{subsec:gen_why_sfm}

The analysis above suggests two design principles:
\begin{enumerate}[leftmargin=2em,label=(\roman*)]
\item the bridge should be as geometrically consistent as possible with the token space itself;
\item the bridge should avoid introducing unnecessary progress-identifiability proxies.
\end{enumerate}
Both points favor a spherical bridge over an affine Euclidean one.

\paragraph{The sphere is the native geometry of the token space.}
The target token $x_1$ lies on $\mathbb S^{N-1}(\sqrt N)$ and, by construction, also satisfies a product-of-spheres group structure. The source state $x_0$ is chosen as a random spherical vector on the same ambient sphere:
\begin{equation}
x_0 \sim \mathrm{Unif}\big(\mathbb S^{N-1}(\sqrt N)\big).
\end{equation}
Since both endpoints lie on the sphere, the most natural bridge between them is the spherical geodesic.

\paragraph{Spherical flow matching bridge.}
Let
\begin{equation}
\Omega = \angle(x_0,x_1)
=
\arccos\!\left(\frac{\langle x_0,x_1\rangle}{N}\right).
\end{equation}
The spherical geodesic interpolation, or \emph{slerp}, is
\begin{equation}
x_t
=
\operatorname{slerp}(x_0,x_1,t)
=
\frac{\sin((1-t)\Omega)}{\sin\Omega}x_0
+
\frac{\sin(t\Omega)}{\sin\Omega}x_1.
\label{eq:sfm_bridge_exact}
\end{equation}
We refer to generation based on this bridge as \textbf{spherical flow matching (SFM)}.

\paragraph{SFM as a high-dimensional VP path.}
In high dimension, two independent random spherical vectors are almost orthogonal:
\begin{equation}
\Omega \approx \frac{\pi}{2}.
\end{equation}
Substituting this into \eqref{eq:sfm_bridge_exact} yields
\begin{equation}
x_t
\approx
\cos\!\left(\frac{\pi}{2}t\right)x_0
+
\sin\!\left(\frac{\pi}{2}t\right)x_1.
\label{eq:sfm_bridge_vp_like}
\end{equation}
This is exactly the form of a variance-preserving trigonometric path. Therefore, in the high-dimensional regime relevant here, SFM can be understood as the spherical-geometric realization of a VP-style denoising bridge.

\paragraph{SFM removes the strongest global progress proxy.}
Unlike affine Euclidean bridges, the SFM bridge remains on the sphere:
\begin{equation}
\|x_t\|_2 = \sqrt N
\qquad
\text{for all } t.
\label{eq:sfm_global_norm_constant}
\end{equation}
Hence the most direct progress proxy, namely the global norm, is completely eliminated. This is an important reduction in shortcut identifiability.

\paragraph{RF induces a more complicated cross-group norm geometry.}
In an affine bridge such as RF,
\begin{equation}
x_t = (1-t)x_0 + tx_1,
\end{equation}
the global norm follows a quadratic profile
\begin{equation}
\|x_t\|_2^2 \approx N\big((1-t)^2+t^2\big),
\end{equation}
which decreases and then increases with a minimum near $t=1/2$. The same behavior appears group-wise:
\begin{equation}
\|x_{t,g}\|_2^2
\approx
(1-t)^2\|x_{0,g}\|_2^2+t^2\|x_{1,g}\|_2^2.
\end{equation}
Since $\|x_{1,g}\|_2^2=r_g^2$ is group-dependent, the minima of the different group norms occur at different effective locations and induce a nontrivial cross-group alignment signature. This creates additional progress-related statistics that must remain consistent at inference.

By contrast, SFM locks the global norm and replaces the quadratic cross-group profile with a monotone interpolation of group energies, as shown below.

\subsection{Group-Wise Energy Evolution Under the SFM Bridge}
\label{subsec:gen_groupwise_snr}

The main structural role of the group-energy hierarchy appears when we examine how each group's energy evolves along the SFM bridge.

Write the SFM bridge in the coefficient form
\begin{equation}
x_t = a_t x_0 + b_t x_1,
\qquad
a_t = \frac{\sin((1-t)\Omega)}{\sin\Omega},
\quad
b_t = \frac{\sin(t\Omega)}{\sin\Omega}.
\label{eq:sfm_coeffs}
\end{equation}
At the group level,
\begin{equation}
x_{t,g} = a_t x_{0,g} + b_t x_{1,g}.
\end{equation}
Expanding the group norm gives
\begin{align}
\|x_{t,g}\|_2^2
&=
a_t^2\|x_{0,g}\|_2^2
+
b_t^2\|x_{1,g}\|_2^2
+
2a_tb_t\langle x_{0,g},x_{1,g}\rangle.
\end{align}
In high dimension, with random spherical source and structured target, we have
\begin{equation}
\|x_{0,g}\|_2^2 \approx H,
\qquad
\|x_{1,g}\|_2^2 = r_g^2,
\qquad
\langle x_{0,g},x_{1,g}\rangle \approx 0,
\end{equation}
hence
\begin{equation}
\boxed{
\|x_{t,g}\|_2^2
\approx
a_t^2 H + b_t^2 r_g^2.
}
\label{eq:group_norm_sfm}
\end{equation}

Several consequences follow immediately.

\paragraph{Monotone group-energy evolution.}
Since $a_t$ decreases from $1$ to $0$ and $b_t$ increases from $0$ to $1$, each group energy evolves monotonically between its random-state value $H$ and its target value $r_g^2$:
\begin{equation}
\|x_{t,g}\|_2^2
\approx
\begin{cases}
\text{increasing in } t, & r_g^2>H,\\[3pt]
\text{decreasing in } t, & r_g^2<H.
\end{cases}
\end{equation}
Thus there is no group-wise ``minimum norm time'' analogous to the affine bridge.

\paragraph{Group-wise SNR.}
The target-to-source SNR inside group $g$ is
\begin{equation}
\mathrm{SNR}_g(t)
=
\frac{b_t^2\|x_{1,g}\|_2^2}{a_t^2\|x_{0,g}\|_2^2}
\approx
\frac{b_t^2 r_g^2}{a_t^2 H}.
\label{eq:group_snr_general}
\end{equation}
Taking logarithms,
\begin{equation}
\log \mathrm{SNR}_g(t)
\approx
2\log\frac{b_t}{a_t} + \log\frac{r_g^2}{H}.
\label{eq:group_snr_log}
\end{equation}
Therefore the time dependence is shared across groups through $b_t/a_t$, while the hierarchy contributes a group-specific constant offset through $\log(r_g^2/H)$.

A useful milestone is the time at which a group's signal and noise energies are equal, i.e.
\begin{equation}
\mathrm{SNR}_g(t_g^\star)=1.
\end{equation}
From \eqref{eq:group_snr_general},
\begin{equation}
\frac{b_{t_g^\star}}{a_{t_g^\star}}
=
\sqrt{\frac{H}{r_g^2}}.
\label{eq:snr1_condition}
\end{equation}
Hence groups with larger $r_g$ reach unit SNR earlier. Since the group energies are ordered as
\begin{equation}
r_1 > r_2 > \cdots > r_G,
\end{equation}
their SNRs become signal-dominant in the same order.

This gives the SFM bridge a direct \emph{coarse-to-fine denoising interpretation}: the highest-energy groups become target-dominant first, followed by progressively lower-energy groups. Because the tokenizer has already been encouraged to place reconstruction-critical content into the more stable high-energy groups, this denoising order mirrors the progression typically observed in continuous signal denoising, where coarse or low-frequency structure is recovered earlier than fine detail.

\subsection{Prediction Target: Why We Predict the Endpoint}
\label{subsec:gen_xpred}

The geometry above suggests that the target state itself is the most natural prediction object.

Recall that the endpoint $x_1$ lies on the product manifold
\begin{equation}
x_{1,g}\in \mathbb S^{H-1}(r_g),
\qquad
g=1,\dots,G.
\label{eq:x1_product_sphere}
\end{equation}
Thus, once the group energies are fixed, the only free variables are the \emph{group-wise directions}. The generative model therefore need not predict an arbitrary Euclidean vector field; it suffices to predict the endpoint directions on each group sphere.

Concretely, the network outputs
\begin{equation}
\hat h = [\hat h_1,\dots,\hat h_G],
\qquad
\hat h_g\in\mathbb R^H,
\end{equation}
which are converted into a valid endpoint prediction by
\begin{equation}
\hat x_{1,g}
=
r_g\frac{\hat h_g}{\|\hat h_g\|_2+\varepsilon}.
\label{eq:xpred_group_param}
\end{equation}
This guarantees
\begin{equation}
\hat x_{1,g}\in \mathbb S^{H-1}(r_g),
\qquad
\hat x_1 \in \mathbb S^{N-1}(\sqrt N).
\end{equation}
The model therefore predicts directly on the same manifold as the true target.

This endpoint prediction formulation is particularly attractive in the present setting. The target manifold is simple and explicit, whereas the instantaneous velocity field depends on both the source and the current bridge state. Predicting the endpoint keeps the prediction target aligned with the geometry that the tokenizer itself defines.

\subsection{Spherical DDIM-Style Inference from Endpoint Prediction}
\label{subsec:gen_spherical_ddim}

Given a current state $x_{t_i}$ and an endpoint prediction $\hat x_1$, inference proceeds by moving along the geodesic from $x_{t_i}$ toward $\hat x_1$. Let the time grid satisfy
\begin{equation}
0=t_0<t_1<\cdots<t_K=1.
\end{equation}
We define
\begin{equation}
\alpha_i
=
\frac{t_{i+1}-t_i}{1-t_i},
\label{eq:alpha_ddim_sphere}
\end{equation}
and update the state by
\begin{equation}
x_{t_{i+1}}
=
\operatorname{slerp}(x_{t_i},\hat x_1,\alpha_i).
\label{eq:spherical_ddim_update}
\end{equation}
This is the spherical analogue of a DDIM-style deterministic update.

The formula \eqref{eq:spherical_ddim_update} has a simple interpretation. At time $t_i$, the fraction of the remaining bridge that should be traversed in one step is exactly
\begin{equation}
\frac{t_{i+1}-t_i}{1-t_i},
\end{equation}
and \eqref{eq:spherical_ddim_update} moves by precisely that fraction along the geodesic from the current state to the predicted endpoint.

\paragraph{Relation to spherical velocity transport.}
The same update can be viewed as the exponential-map integration of a spherical velocity field induced by endpoint prediction. Thus, although our model predicts the endpoint rather than a tangent vector directly, the inference rule remains fully compatible with geodesic transport on the sphere.

\subsection{Manifold-Preserving CFG in Endpoint Space}
\label{subsec:gen_cfg}

Classifier-free guidance (CFG) is also performed in endpoint space. Since both the conditional and unconditional predictions lie on the same product manifold, the guidance operation should preserve the group energies.

Let $\hat x_1^{(u)}$ and $\hat x_1^{(c)}$ denote the unconditional and conditional endpoint predictions, respectively. For each group $g$, both
\begin{equation}
\hat x_{1,g}^{(u)},\ \hat x_{1,g}^{(c)} \in \mathbb S^{H-1}(r_g).
\end{equation}
We define the guided endpoint group by spherical extrapolation on the group sphere:
\begin{equation}
\hat x_{1,g}^{\mathrm{cfg}}
=
\operatorname{slerp}\!\left(
\hat x_{1,g}^{(u)},
\hat x_{1,g}^{(c)},
\lambda
\right),
\label{eq:cfg_group_slerp}
\end{equation}
where $\lambda\ge 1$ is the guidance scale. Since the operation is performed on $\mathbb S^{H-1}(r_g)$, the group energy is preserved:
\begin{equation}
\|\hat x_{1,g}^{\mathrm{cfg}}\|_2 = r_g.
\end{equation}
Stacking all groups yields a guided endpoint prediction
\begin{equation}
\hat x_1^{\mathrm{cfg}}
=
[\hat x_{1,1}^{\mathrm{cfg}},\dots,\hat x_{1,G}^{\mathrm{cfg}}]
\in
\mathbb S^{N-1}(\sqrt N)
\end{equation}
that remains on the same product manifold as the training targets.

This manifold-preserving CFG is important for training--inference consistency. The generator is trained to predict endpoints with the predefined group-energy hierarchy. If guidance were to alter the group energies arbitrarily, the resulting endpoint would leave the target manifold and create a mismatch between training geometry and inference geometry. Group-wise spherical extrapolation avoids this issue.

\subsection{Training Loss from Single-Step Slerp Error}
\label{subsec:gen_loss}

We now derive the training loss corresponding to the spherical DDIM-style inference rule \eqref{eq:spherical_ddim_update}.

At a training time $t$, let the current bridge state be $x_t$, the true endpoint be $x_1$, and the model prediction be $\hat x_1$. The ideal next state at $t' = t+\Delta t$ is
\begin{equation}
x_{t'}^\star
=
\operatorname{slerp}(x_t,x_1,\alpha),
\qquad
\alpha=\frac{\Delta t}{1-t},
\end{equation}
while the actual one-step prediction is
\begin{equation}
\hat x_{t'}
=
\operatorname{slerp}(x_t,\hat x_1,\alpha).
\end{equation}
We seek a loss that directly controls the one-step inference error
\begin{equation}
d_{\mathbb S}(\hat x_{t'},x_{t'}^\star),
\end{equation}
where $d_{\mathbb S}$ denotes the geodesic distance on $\mathbb S^{N-1}(\sqrt N)$.

\paragraph{First-order sensitivity of slerp to endpoint error.}
For a fixed starting point $x_t$, geodesic interpolation scales small endpoint perturbations linearly with the interpolation fraction. Specifically, when $\hat x_1$ is close to $x_1$,
\begin{equation}
d_{\mathbb S}\!\big(
\operatorname{slerp}(x_t,\hat x_1,\alpha),
\operatorname{slerp}(x_t,x_1,\alpha)
\big)
\approx
\alpha\, d_{\mathbb S}(\hat x_1,x_1).
\label{eq:slerp_error_scaling}
\end{equation}
Therefore the one-step state error is minimized, to first order, by minimizing
\begin{equation}
\alpha^2\, d_{\mathbb S}(\hat x_1,x_1)^2.
\end{equation}
Since the step size $\Delta t$ is an inference-schedule constant, the essential time dependence is
\begin{equation}
\boxed{
L_{\mathrm{step}}
\propto
\frac{1}{(1-t)^2}
d_{\mathbb S}(\hat x_1,x_1)^2.
}
\label{eq:step_error_geodesic_loss}
\end{equation}

\paragraph{Geodesic and cosine forms.}
On the sphere of radius $\sqrt N$,
\begin{equation}
d_{\mathbb S}(\hat x_1,x_1)
=
\sqrt N\,
\arccos\!\left(\frac{\langle \hat x_1,x_1\rangle}{N}\right).
\end{equation}
Hence the exact geodesic form of the loss is
\begin{equation}
L_{\mathrm{geo}}
=
\frac{N}{(1-t)^2}
\arccos^2\!\left(\frac{\langle \hat x_1,x_1\rangle}{N}\right).
\label{eq:exact_geo_loss}
\end{equation}
For small endpoint errors, we may use the approximation
\begin{equation}
d_{\mathbb S}(\hat x_1,x_1)^2
\approx
\|\hat x_1-x_1\|_2^2
=
2N\big(1-\cos(\hat x_1,x_1)\big),
\end{equation}
which yields the surrogate losses
\begin{align}
L_{\mathrm{mse}}
&=
\frac{1}{(1-t)^2}\|\hat x_1-x_1\|_2^2,
\label{eq:mse_weighted_loss}
\\
L_{\mathrm{cos}}
&=
\frac{1}{(1-t)^2}\big(1-\cos(\hat x_1,x_1)\big).
\label{eq:cos_weighted_loss}
\end{align}
In practice, these weighted endpoint losses are stable and geometrically well aligned with the spherical inference rule.

\paragraph{Interpretation.}
The factor $(1-t)^{-2}$ is not inherited from an Euclidean velocity formulation; in the present framework it has a direct geometric meaning. It is precisely the first-order amplification factor with which endpoint prediction error translates into one-step error under spherical DDIM-style interpolation.

\subsection{Summary}
\label{subsec:gen_summary}

The generation framework introduced in this section is defined by four coupled design choices:
\begin{enumerate}[leftmargin=2em,label=(\arabic*)]
\item \textbf{Spherical flow matching (SFM):}
generation follows the geodesic bridge between a random spherical source and a structured hierarchical target token.

\item \textbf{Endpoint prediction on the product manifold:}
the model predicts the target token directly in group-wise directional form, using the fixed group energies defined by the tokenizer.

\item \textbf{Spherical DDIM-style inference:}
sampling proceeds by geodesic interpolation from the current state toward the predicted endpoint, with progress fraction $\alpha=(t_{i+1}-t_i)/(1-t_i)$.

\item \textbf{Manifold-preserving guidance and loss:}
CFG is performed by per-group spherical extrapolation, and training uses a weighted endpoint loss derived from the single-step spherical interpolation error.
\end{enumerate}

Together, these ingredients yield a generation procedure that is geometrically aligned with the tokenizer, reduces progress-identifiability shortcuts relative to affine Euclidean bridges, and induces an explicit coarse-to-fine denoising order through the group-wise signal-to-noise evolution of the hierarchical sphere.

==> sections_old/baton_flow.tex <==
\subsection{Baton Flow: Product-Manifold Switching-Code Generation and High-Dimensional ORF Transport}
\label{subsec:baton_flow}

We propose \textbf{Baton Flow}, a two-stage framework for conditional token generation that separates \emph{switching-state construction} from \emph{final high-dimensional transport}. The name is chosen by analogy to the final handoff in a 4$\times$100 relay: the penultimate runner exits the curve and delivers the baton in a well-positioned, forward-moving state, after which the anchor runner takes over on the straight and sprints to the finish. In our setting, phase I generates a target-dominant \emph{switching code} in the tokenizer's low-dimensional spherical core-token space, and phase II takes over in the full token space using ORF, whose geometry is particularly well matched to the final outward transport to the target.

The bridge construction is defined on the tokenizer's product manifold rather than on an unconstrained full-vector space. In particular, the source token, target token, and switching token are all interpreted blockwise through their core and residual parts. The core part and the residual part each follow the same RF mean-radius geometry as in the original high-dimensional derivation, but with dimensions $d$ and $N-d$, respectively. The phase-I target is defined by projecting the core part of the RF switching point back to the corresponding core-token sphere, while phase II starts from a full-token proxy whose core part is copied directly from the perturbed switching code and whose residual part is predicted by the tokenizer's residual predictor.

The resulting framework has three components: (i) an RF SNR-balance switching point that defines where the handoff should occur; (ii) a low-dimensional spherical phase-I generator that predicts the core switching token associated with that point; and (iii) a high-dimensional ORF phase that starts from a full-token proxy constructed from the perturbed core switching token and completes the final transport to the target token.

\subsubsection{Product-Manifold RF Source and SNR-Balance Switching Point}
\label{sec:baton_boundary}

Let
\begin{equation}
x_0 = [\, x_0^{\mathrm c};\, x_0^{\mathrm r} \,],
\qquad
x_1 = [\, x_1^{\mathrm c};\, x_1^{\mathrm r} \,],
\end{equation}
where the source token is sampled from the inner product manifold
\begin{equation}
x_0^{\mathrm c}\sim \mathrm{Unif}\big(\mathbb S^{d-1}(a\sqrt d)\big),
\qquad
x_0^{\mathrm r}\sim \mathrm{Unif}\big(\mathbb S^{N-d-1}(a\sqrt{N-d})\big),
\label{eq:baton_x0_product}
\end{equation}
and the target token lies on the outer product manifold
\begin{equation}
x_1^{\mathrm c}\in \mathbb S^{d-1}(\sqrt d),
\qquad
x_1^{\mathrm r}\in \mathbb S^{N-d-1}(\sqrt{N-d}).
\label{eq:baton_x1_product}
\end{equation}
Consequently,
\begin{equation}
\|x_0\|_2 = a\sqrt N,
\qquad
\|x_1\|_2=\sqrt N.
\end{equation}

We use the ambient RF bridge
\begin{equation}
x_t=(1-t)x_0+t x_1,
\label{eq:baton_rf_bridge}
\end{equation}
with the same SNR proxy
\begin{equation}
\mathrm{SNR}(t)
\;\triangleq\;
\log\frac{t\|x_1\|_2}{(1-t)\|x_0\|_2}
=
\log\frac{t}{a(1-t)}.
\label{eq:baton_snr}
\end{equation}
The equal-contribution time is
\begin{equation}
t_{\mathrm{eq}}
=
\frac{a}{1+a}.
\label{eq:baton_teq}
\end{equation}
We define the corresponding RF mixture point
\begin{equation}
x_{t_{\mathrm{eq}}}
=
(1-t_{\mathrm{eq}})x_0+t_{\mathrm{eq}}x_1
\label{eq:baton_xteq}
\end{equation}
as the canonical \emph{switching point}. As before, we use
\begin{equation}
a=\sqrt2-1,
\label{eq:baton_a}
\end{equation}
so that the switching point is aligned with the end of the non-expanding interval in the original RF radius geometry.

\paragraph{Blockwise mean-radius geometry.}
Because the source and target tokens are sampled on a product manifold, the same RF mean-radius analysis applies blockwise. For the core part,
\begin{equation}
x_t^{\mathrm c}=(1-t)x_0^{\mathrm c}+t x_1^{\mathrm c},
\end{equation}
and therefore
\begin{equation}
\|x_t^{\mathrm c}\|_2^2
=
a^2(1-t)^2 d+t^2 d+2t(1-t)\langle x_0^{\mathrm c},x_1^{\mathrm c}\rangle.
\label{eq:core_radius_raw}
\end{equation}
Since $\langle x_0^{\mathrm c},x_1^{\mathrm c}\rangle$ has mean zero under independent spherical sampling,
\begin{equation}
\mathbb E\|x_t^{\mathrm c}\|_2^2
=
d\big(a^2(1-t)^2+t^2\big).
\label{eq:core_radius_mean}
\end{equation}
Likewise, for the residual part,
\begin{equation}
\mathbb E\|x_t^{\mathrm r}\|_2^2
=
(N-d)\big(a^2(1-t)^2+t^2\big).
\label{eq:res_radius_mean}
\end{equation}
Thus the full ambient norm still satisfies
\begin{equation}
\mathbb E\|x_t\|_2^2
=
N\big(a^2(1-t)^2+t^2\big),
\label{eq:full_radius_mean}
\end{equation}
while the core and residual blocks follow the same radius law at their own dimensions. In particular, at $t=t_{\mathrm{eq}}$ with $a=\sqrt2-1$,
\begin{equation}
\mathbb E\|x_{t_{\mathrm{eq}}}^{\mathrm c}\|_2^2 = a^2 d,
\qquad
\mathbb E\|x_{t_{\mathrm{eq}}}^{\mathrm r}\|_2^2 = a^2 (N-d).
\label{eq:switching_mean_shells}
\end{equation}
Hence the switching point returns in expectation to the inner-shell scale, now blockwise on the product manifold.

\subsubsection{Phase I: Low-Dimensional Core Switching Token Generation}
\label{sec:baton_phase1}

Phase I only models the switching token in the core-token space. For the source core token and switching-point core token, we define
\begin{equation}
x_0^{\mathrm c}\in\mathbb S^{d-1}(a\sqrt d),
\qquad
x_{t_{\mathrm{eq}}}^{\mathrm c,\,\mathrm{raw}}
=
(1-t_{\mathrm{eq}})x_0^{\mathrm c}+t_{\mathrm{eq}}x_1^{\mathrm c}.
\end{equation}
Since $x_{t_{\mathrm{eq}}}^{\mathrm c,\,\mathrm{raw}}$ lies on the desired inner shell only in the mean-radius sense, we project it back to the corresponding core sphere:
\begin{equation}
\bar x_{t_{\mathrm{eq}}}^{\mathrm c}
=
\mathrm{Norm}_{a\sqrt d}\!\big(x_{t_{\mathrm{eq}}}^{\mathrm c,\,\mathrm{raw}}\big)
\in \mathbb S^{d-1}(a\sqrt d).
\label{eq:projected_core_switch}
\end{equation}
This is the phase-I target.

\paragraph{Low-dimensional spherical transport.}
We use spherical flow matching in the inner-shell core-token space. Concretely, we define the slerp bridge
\begin{equation}
x_t^{\mathrm{sfm}}
=
\mathrm{slerp}(x_0^{\mathrm c},\bar x_{t_{\mathrm{eq}}}^{\mathrm c};t),
\qquad t\in[0,1],
\label{eq:baton_lowd_slerp}
\end{equation}
and train a tangent vector field to predict the corresponding spherical transport direction. Since this phase operates entirely in the fixed-radius core-token space, the generated quantity is a \emph{core switching token} rather than a full high-dimensional token. We denote the resulting phase-I generator by
\begin{equation}
\hat x_{t_{\mathrm{eq}}}^{\mathrm c} = G_{\mathrm{c}}(x_0^{\mathrm c},c),
\label{eq:baton_phase1_generator}
\end{equation}
where $c$ denotes the conditioning signal.

\paragraph{Why the projected core token is the phase-I target.}
The role of phase I is to prepare a semantically accurate and generation-friendly handoff state for ORF. The projected switching core token $\bar x_{t_{\mathrm{eq}}}^{\mathrm c}$ is the natural target for this purpose for two reasons. First, it is constructed from the same RF switching semantics as the full-token bridge, but projected back to the legitimate core-token sphere exactly as in the original Spoon-style geometric design. Second, the tokenizer explicitly trains the core token under spherical perturbations and low-dimensional reconstruction, so this is the token subspace that is directly shaped to be generative and robust.

\subsubsection{Tokenizer-Consistent Core-Token Perturbation}
\label{sec:baton_phase1_noise}

A central question is how the ORF phase should be trained with respect to uncertainty in the phase-I output. Training ORF directly from the unperturbed switching code would make the second stage overly reliant on a nearly oracle handoff state. We therefore perturb the projected switching core token in the same low-dimensional spherical space and with the same perturbation rule used during tokenizer training.

Given the oracle projected switching core token $\bar x_{t_{\mathrm{eq}}}^{\mathrm c}$, we sample a unit tangent direction
\begin{equation}
u \in T_{\bar x_{t_{\mathrm{eq}}}^{\mathrm c}}\mathbb S^{d-1}(a\sqrt d),
\qquad \|u\|_2=1,
\qquad \langle u,\bar x_{t_{\mathrm{eq}}}^{\mathrm c}\rangle=0,
\end{equation}
and define the perturbed core token by geodesic rotation
\begin{equation}
\tilde x_{t_{\mathrm{eq}}}^{\mathrm c}
=
\mathrm{Exp}_{\bar x_{t_{\mathrm{eq}}}^{\mathrm c}}(a\sqrt d\,\theta u)
=
\cos(\theta)\,\bar x_{t_{\mathrm{eq}}}^{\mathrm c} + a\sqrt d\,\sin(\theta)\,u.
\label{eq:baton_core_noise}
\end{equation}
We use the same low-dimensional angular sampling rule as in the tokenizer:
\begin{equation}
\theta
=
\theta_{\max}^{(d)}\cdot \mathrm{Beta}(1,2),
\qquad
\theta_{\max}^{(d)}=\arccos\!\Big(\frac{3}{\sqrt d}\Big).
\label{eq:baton_theta}
\end{equation}

This yields a handoff uncertainty model that is tokenizer-consistent by construction. The same spherical neighborhood is explicitly seen by the tokenizer through the low-dimensional reconstruction path, so the residual predictor is trained on exactly the type of perturbation that Baton Flow later uses at the phase boundary.

\subsubsection{Residual-Predicted Handoff State for ORF}
\label{sec:baton_phase2_start}

We construct a full-token switching-state proxy by directly copying the perturbed core token and predicting only the residual token through the tokenizer residual predictor:
\begin{equation}
x_{\mathrm{sw}}^{\mathrm r}
=
\mathrm{Norm}_{a\sqrt{N-d}}\!\big(Q(\tilde x_{t_{\mathrm{eq}}}^{\mathrm c})\big)
\in
\mathbb S^{N-d-1}(a\sqrt{N-d}),
\label{eq:baton_residual_pred}
\end{equation}
and
\begin{equation}
x_{\mathrm{sw}}
=
[\, \tilde x_{t_{\mathrm{eq}}}^{\mathrm c};\; x_{\mathrm{sw}}^{\mathrm r} \,].
\label{eq:baton_xsw}
\end{equation}
We interpret $x_{\mathrm{sw}}$ as a \emph{product-manifold switching-state proxy} for the oracle RF switching point $x_{t_{\mathrm{eq}}}$. This interpretation is supported by the tokenizer training objective: the residual predictor $Q$ is trained from the core token to the residual token under both clean and perturbed low-dimensional inputs, and the residual commitment loss explicitly aligns the predicted residual with the original residual token.

At inference time, the same construction is applied using the phase-I prediction $\hat x_{t_{\mathrm{eq}}}^{\mathrm c}$ in place of the oracle projected switching core token:
\begin{equation}
\hat x_{\mathrm{sw}}^{\mathrm r}
=
\mathrm{Norm}_{a\sqrt{N-d}}\!\big(Q(\hat x_{t_{\mathrm{eq}}}^{\mathrm c})\big),
\qquad
\hat x_{\mathrm{sw}}
=
[\, \hat x_{t_{\mathrm{eq}}}^{\mathrm c};\; \hat x_{\mathrm{sw}}^{\mathrm r} \,].
\label{eq:baton_xsw_infer}
\end{equation}

\subsubsection{Phase II: Product-Manifold ORF Transport}
\label{sec:baton_phase2}

The second stage uses the same ORF formulation as in Sec.~\ref{subsec:orf}, but with product-manifold source and target tokens. Given the switching-state proxy $x_{\mathrm{sw}}$ and the target token $x_1$, we define the ORF bridge
\begin{equation}
x_s^{\mathrm{orf}}=(1-s)x_{\mathrm{sw}}+s x_1,
\qquad s\in[0,1],
\label{eq:baton_orf_bridge}
\end{equation}
with target ray
\begin{equation}
r^\star=\mathrm{Norm}_1(x_1-x_{\mathrm{sw}}).
\label{eq:baton_orf_ray}
\end{equation}
The ORF model predicts only the unit transport direction, and inference uses the same radius-locking rule as in Sec.~\ref{sec:orf_step}. Since $x_{\mathrm{sw}}$ is constructed to live on the same inner product-manifold scale as the expected switching point, the second stage preserves the original interpretation of ORF as the target-dominant expansion phase of the RF bridge, while allowing the actual start state to be a lower-information, more realistic handoff proxy rather than the oracle switching point itself.

\paragraph{Blockwise mean-radius geometry of phase II.}
Because both $x_{\mathrm{sw}}$ and $x_1$ are product-manifold tokens, the same mean-radius analysis applies blockwise in phase II. Writing
\begin{equation}
x_s^{\mathrm{orf}}
=
[\, x_s^{\mathrm c};\, x_s^{\mathrm r} \,],
\qquad
x_s^{\mathrm c}=(1-s)x_{\mathrm{sw}}^{\mathrm c}+s x_1^{\mathrm c},
\qquad
x_s^{\mathrm r}=(1-s)x_{\mathrm{sw}}^{\mathrm r}+s x_1^{\mathrm r},
\end{equation}
we obtain
\begin{equation}
\mathbb E\|x_s^{\mathrm c}\|_2^2
=
d\big(a^2(1-s)^2+s^2\big),
\qquad
\mathbb E\|x_s^{\mathrm r}\|_2^2
=
(N-d)\big(a^2(1-s)^2+s^2\big),
\end{equation}
hence
\begin{equation}
\mathbb E\|x_s^{\mathrm{orf}}\|_2^2
=
N\big(a^2(1-s)^2+s^2\big).
\label{eq:baton_orf_radius_mean}
\end{equation}
Thus the original ORF mean-radius schedule is recovered exactly at the level of blockwise mean geometry.

\subsubsection{Training and Inference Procedure}
\label{sec:baton_training}

The full training procedure is summarized as follows.

\paragraph{Phase I training.}
For each sampled pair $(x_0,x_1)$ on the source and target product manifolds, compute the RF switching point $x_{t_{\mathrm{eq}}}$ by Eq.~\eqref{eq:baton_xteq}, extract its core block, and project it to the corresponding inner-shell core sphere by Eq.~\eqref{eq:projected_core_switch}. Train the low-dimensional spherical generator to model $\bar x_{t_{\mathrm{eq}}}^{\mathrm c}$ from $x_0^{\mathrm c}$.

\paragraph{Phase II training.}
For the same pair $(x_0,x_1)$, perturb the projected switching core token by Eqs.~\eqref{eq:baton_core_noise}--\eqref{eq:baton_theta}, predict the residual token through Eq.~\eqref{eq:baton_residual_pred}, and form the full switching-state proxy by Eq.~\eqref{eq:baton_xsw}. Train ORF on the bridge from $x_{\mathrm{sw}}$ to $x_1$.

\paragraph{Inference.}
We first sample a source token $x_0$ from the inner product manifold and extract its core token $x_0^{\mathrm c}$. Phase I generates a switching core token $\hat x_{t_{\mathrm{eq}}}^{\mathrm c}=G_{\mathrm{c}}(x_0^{\mathrm c},c)$, which is combined with the predicted residual token through Eq.~\eqref{eq:baton_xsw_infer} to form a full handoff state $\hat x_{\mathrm{sw}}$. Phase II then applies ORF sampling from $\hat x_{\mathrm{sw}}$ to obtain the final token $x_1$.

\paragraph{Interpretation.}
Baton Flow assigns distinct geometric roles to the two stages. Phase I runs in the low-dimensional spherical core-token space and predicts a projected switching token associated with the RF SNR-balance point. Phase II takes over in the full product-manifold token space, where the core token is copied directly and the residual token is predicted from it, and then performs the final outward transport with ORF. In the 4$\times$100 relay analogy, phase I is the runner exiting the curve and delivering the baton in a well-positioned, target-dominant state; phase II is the anchor leg that receives the baton and runs the straight sprint to the finish.

==> sections_old/generator.tex <==
```latex
\subsection{Training-time State Perturbation for Covering Rollout-induced Off-trajectory States}
\label{subsec:state_perturbation_rollout}

The discussion above suggests that, in high-dimensional continuous-token generation, a substantial part of the train--test mismatch may not come from the endpoint distribution itself, but from the fact that \emph{inference states are produced by iterative rollout rather than by the oracle bridge construction}. Even if the bridge family is fixed during training, the states seen at test time are generated by recursively applying an approximate vector field, whereas the training states are sampled exactly from the bridge defined by $(x_0,x_1)$. As a result, inference-time states generally do not follow the same conditional distribution as training-time bridge states at the same nominal $t$. This motivates a natural question: \emph{if one wishes to enlarge the behavior-stable basin of the model without explicit rollout training, how should one perturb the training-time state $x_t$ so that the perturbed training distribution better covers the states encountered during inference?}

A common heuristic in standard flow matching is to add isotropic Gaussian perturbation directly to $x_t$ while keeping the target velocity defined by the clean $(x_0,x_1)$ pair. Here we provide a more explicit motivation for this practice and derive a principled time-dependent perturbation schedule from the statistics of rollout error. The resulting design does not rely on a particular solver step size at training time and applies broadly to high-dimensional continuous-token settings.

\paragraph{Ideal bridge states versus rollout states.}
Let $x_t^\star$ denote the ideal bridge state at time $t$ under the training construction. For concreteness, one may think of the standard RF bridge
\begin{equation}
x_t^\star = (1-t)x_0 + t x_1,
\label{eq:ideal_bridge_state}
\end{equation}
although the argument below only requires the existence of a smooth target vector field $v^\star(x,t)$ such that the ideal trajectory solves
\begin{equation}
\frac{d}{dt}x_t^\star = v^\star(x_t^\star,t).
\label{eq:ideal_ode}
\end{equation}
At inference time, however, the model uses an approximate vector field
\begin{equation}
\hat v(x,t) = v^\star(x,t) + \varepsilon(x,t),
\label{eq:approx_field}
\end{equation}
where $\varepsilon$ is the prediction error, and rollout is performed by numerical integration. Under an Euler step with step size $h_k=t_{k+1}-t_k$,
\begin{equation}
x_{k+1} = x_k + h_k \hat v(x_k,t_k).
\label{eq:euler_rollout}
\end{equation}
Therefore, the inference-time state distribution at a given nominal time $t$ is generally not the same as the oracle bridge distribution $p_{\mathrm{train}}(x_t^\star\mid t)$.

To study this mismatch, define the rollout error
\begin{equation}
e_k \triangleq x_k - x_{t_k}^\star.
\label{eq:error_def_discrete}
\end{equation}
Subtracting the first-order Taylor expansion of the ideal solution from the Euler update yields a discrete error recursion. Since the ideal trajectory satisfies
\begin{equation}
x_{t_{k+1}}^\star
=
x_{t_k}^\star + h_k v^\star(x_{t_k}^\star,t_k) + O(h_k^2),
\label{eq:ideal_taylor}
\end{equation}
we have
\begin{align}
e_{k+1}
&=
x_{k+1}-x_{t_{k+1}}^\star
\nonumber\\
&=
x_k + h_k \hat v(x_k,t_k)
-
\Big(x_{t_k}^\star + h_k v^\star(x_{t_k}^\star,t_k) + O(h_k^2)\Big)
\nonumber\\
&=
e_k
+
h_k\Big(\hat v(x_k,t_k)-v^\star(x_{t_k}^\star,t_k)\Big)
+
O(h_k^2).
\label{eq:error_recursion_prelin}
\end{align}
Using $\hat v=v^\star+\varepsilon$ and linearizing $v^\star(x_k,t_k)$ around $x_{t_k}^\star$ gives
\begin{equation}
v^\star(x_k,t_k)
=
v^\star(x_{t_k}^\star,t_k)
+
J_k e_k
+
O(\|e_k\|^2),
\qquad
J_k \triangleq \nabla_x v^\star(x_{t_k}^\star,t_k),
\label{eq:v_linearization}
\end{equation}
so the first-order error dynamics become
\begin{equation}
e_{k+1}
\approx
(I+h_k J_k)e_k + h_k \varepsilon_k,
\qquad
\varepsilon_k \triangleq \varepsilon(x_{t_k}^\star,t_k).
\label{eq:error_recursion_linearized}
\end{equation}
Equation~\eqref{eq:error_recursion_linearized} makes the source of train--test mismatch explicit: the rollout error at the next step is the sum of (i) propagated past error and (ii) newly injected prediction error.

\paragraph{Continuous-time approximation and covariance dynamics.}
When the step size is small, the discrete recursion above can be approximated by a linear stochastic differential equation. Writing $e_t$ for the continuous-time rollout error and modeling the accumulated local prediction noise as a diffusion term yields
\begin{equation}
de_t = J_t e_t\,dt + B_t\,dW_t,
\label{eq:error_sde}
\end{equation}
where $W_t$ is a standard Wiener process and
\begin{equation}
Q_t \triangleq B_t B_t^\top
\end{equation}
is the instantaneous covariance of injected model error. Let
\begin{equation}
\Sigma_e(t) \triangleq \mathrm{Cov}(e_t).
\end{equation}
Assuming for simplicity that $\mathbb E[e_t]=0$, we can derive the covariance dynamics by applying It\^{o}'s formula to the matrix process $e_t e_t^\top$:
\begin{equation}
d(e_t e_t^\top)
=
(de_t)e_t^\top + e_t(de_t)^\top + (de_t)(de_t)^\top.
\label{eq:ito_outer}
\end{equation}
Substituting Eq.~\eqref{eq:error_sde} into Eq.~\eqref{eq:ito_outer} and using the It\^{o} identity $dW_t dW_t^\top = I\,dt$ gives
\begin{equation}
\frac{d}{dt}\Sigma_e(t)
=
J_t \Sigma_e(t) + \Sigma_e(t) J_t^\top + Q_t.
\label{eq:lyapunov_cov}
\end{equation}
This is the continuous-time Lyapunov differential equation governing the train--test state mismatch.

Equation~\eqref{eq:lyapunov_cov} has a simple interpretation. The term
\begin{equation}
J_t \Sigma_e(t) + \Sigma_e(t) J_t^\top
\end{equation}
describes how previously accumulated error is transformed by the local flow geometry. Importantly, this term does not merely ``propagate'' error: depending on the sign structure of the local Jacobian, it can either \emph{amplify} or \emph{contract} existing deviation. The term
\begin{equation}
Q_t
\end{equation}
is the new prediction-error covariance injected at time $t$. Thus the instantaneous mismatch is determined by the competition between \emph{error injection} and \emph{error contraction/expansion}.

\paragraph{A one-dimensional intuition.}
The mechanism is especially transparent in one dimension. If
\begin{equation}
de_t = a_t e_t\,dt + b_t\,dW_t,
\end{equation}
then the variance $s_t=\mathrm{Var}(e_t)$ satisfies
\begin{equation}
\frac{d}{dt}s_t = 2a_t s_t + b_t^2.
\label{eq:1d_lyapunov}
\end{equation}
If $a_t>0$, existing error is amplified; if $a_t<0$, existing error is contracted; and $b_t^2$ always injects new variance. Therefore, a ``variance hump'' is entirely natural: the mismatch can grow in the middle of the trajectory when uncertainty injection remains substantial and enough error has accumulated, and then shrink again near the end if the dynamics become locally contractive and the injected noise decreases. In high dimensions, Eq.~\eqref{eq:lyapunov_cov} can be understood approximately as a superposition of such one-dimensional behaviors along local principal directions of the Jacobian and covariance.

\paragraph{Why the mismatch can peak in the middle.}
The covariance equation above provides a distribution-level explanation for a common empirical observation: inference trajectories often appear close to the training bridge near the start and near the end, but deviate more in the middle. In our setting, this has a natural interpretation:
\begin{itemize}
\item \textbf{Early stage:} although the model uncertainty can be large, the state remains close to the source/noise manifold, and moderate prediction error may still produce states that look statistically similar to valid source-side bridge states.
\item \textbf{Middle stage:} source and target information are strongly mixed, posterior ambiguity is large, historical rollout error has already accumulated, and the trajectory is not yet strongly attracted to the target manifold.
\item \textbf{Late stage:} the injected prediction-error covariance $Q_t$ tends to decrease because the target becomes easier to infer, while the local flow may become contractive toward the target manifold, causing previously accumulated mismatch to shrink.
\end{itemize}
Therefore, from the perspective of \emph{state-distribution mismatch}, a middle-peaked perturbation schedule is more natural than a schedule that is monotone in either $t$ or $1-t$.

\paragraph{A more principled proxy for the perturbation schedule.}
The ideal training perturbation would sample directly from the rollout error distribution,
\begin{equation}
\delta x_t \sim \mathcal N(0,\Sigma_e(t)),
\label{eq:ideal_state_perturb}
\end{equation}
but $\Sigma_e(t)$ is unavailable in practice. Nevertheless, Eq.~\eqref{eq:lyapunov_cov} suggests a more principled approximation than directly using the variance of the bridge itself. In particular, the instantaneous injection term $Q_t$ is more naturally related to \emph{prediction uncertainty} than to the unconditional variance of $x_t$. For an approximately optimal predictor, the irreducible part of the error is tied to the conditional posterior covariance of the target. Thus, in $v$-prediction form one expects
\begin{equation}
Q_t \;\propto\; \mathbb E\!\left[\mathrm{Cov}\big(v^\star \mid x_t,t,c\big)\right],
\label{eq:Qt_v}
\end{equation}
and in an $x$-prediction parameterization,
\begin{equation}
Q_t \;\propto\; \frac{1}{(1-t)^2}\,
\mathbb E\!\left[\mathrm{Cov}\big(x_1 \mid x_t,t,c\big)\right].
\label{eq:Qt_x}
\end{equation}
Although these quantities are not directly computable either, they strongly suggest that the effective mismatch covariance should peak in the regime where posterior ambiguity is largest, rather than monotonically near the start or the end.

\paragraph{State-transition representation.}
The covariance dynamics also admit the integral solution
\begin{equation}
\Sigma_e(t)
=
\Phi(t,0)\Sigma_e(0)\Phi(t,0)^\top
+
\int_0^t \Phi(t,s)\,Q_s\,\Phi(t,s)^\top ds,
\label{eq:sigma_integral}
\end{equation}
where $\Phi(t,s)$ is the state-transition matrix associated with $J_t$:
\begin{equation}
\frac{\partial}{\partial t}\Phi(t,s)=J_t\Phi(t,s),\qquad \Phi(s,s)=I.
\end{equation}
If the initial mismatch is zero, i.e.\ $\Sigma_e(0)=0$, then
\begin{equation}
\Sigma_e(t)
=
\int_0^t \Phi(t,s)\,Q_s\,\Phi(t,s)^\top ds.
\label{eq:sigma_integral_zero_init}
\end{equation}
Equation~\eqref{eq:sigma_integral_zero_init} makes the structure particularly clear: mismatch at time $t$ is the accumulation of all previously injected error covariances, transported by the local linearized flow. This is why the rollout mismatch is fundamentally a \emph{distribution-level} phenomenon and cannot be fully characterized by the bridge variance alone.

\paragraph{A simple isotropic approximation.}
To obtain a practical perturbation rule without explicit rollout, we approximate $\Sigma_e(t)$ by an isotropic covariance whose total magnitude follows the middle-peaked behavior implied by the analysis above. Since our tokens live at norm scale $\|x_t\|_2=\Theta(\sqrt N)$, the perturbation should also be calibrated at the \emph{same global scale} if it is meant to model a fixed relative geometric deviation in a high-dimensional latent space. Therefore, the perturbation norm should scale like $\sqrt N$, rather than remain $O(1)$. A simple no-extra-hyperparameter approximation is
\begin{equation}
\tilde x_t
=
x_t + \epsilon_t,
\qquad
\epsilon_t \sim \mathcal N\!\big(0,\; t^2(1-t)^2\, I_N\big).
\label{eq:state_perturb_final}
\end{equation}
This construction has three useful properties:
\begin{itemize}
\item \textbf{Middle-peaked time dependence:} the perturbation vanishes at $t=0$ and $t=1$ and reaches its maximum at $t=0.5$, matching the expected shape of rollout mismatch.
\item \textbf{Dimension-aware scaling:} since
\begin{equation}
\mathbb E\|\epsilon_t\|_2 = t(1-t)\sqrt{N},
\end{equation}
the perturbation norm scales as $\sqrt N$, which is consistent with the $\sqrt N$ norm scale of high-dimensional tokens.
\item \textbf{No extra scale hyperparameter:} the amplitude is fully determined by the time-dependent mismatch ansatz and the ambient dimensionality.
\end{itemize}

\paragraph{Interpretation.}
Equation~\eqref{eq:state_perturb_final} should be understood as a \emph{trace-matched isotropic approximation} to the unknown rollout covariance $\Sigma_e(t)$: instead of perturbing the endpoint $x_1$ and reconstructing a new bridge state from the perturbed endpoint, we directly perturb the oracle bridge state itself in a way that more closely matches the local geometry of Euler rollout error. The target remains the clean $x_1$, so the model is explicitly trained to recover the clean endpoint from states that are slightly off the ideal bridge, which is precisely the situation encountered during iterative inference.

In summary, if one believes that high-dimensional bridge statistics are overly tightly coupled to the nominal time index $t$, and that iterative inference therefore produces states that drift away from the thin training bridge distribution, then training-time state perturbation provides a principled way to thicken the state distribution without explicit rollout. The covariance analysis above suggests that such perturbation should not be tied merely to endpoint noise or to a monotone function of $t$, but should instead reflect the statistics of rollout mismatch itself. Under a linearized error model, this naturally leads to a middle-peaked perturbation schedule and to the isotropic approximation in Eq.~\eqref{eq:state_perturb_final}.
```

==> sections_old/introduction_old.tex <==
\section{Introduction}

Token-based generation has become a practical route to scalable synthesis across modalities, as tokenization compresses high-resolution or high-sampling-rate signals into compact sequences, enabling generative modeling at scales where direct modeling in the raw signal space is computationally prohibitive \cite{rombach2022high, peebles2023scalable, ma2024sit, esser2024scaling}. In this paradigm, a tokenizer maps a signal (e.g., an image or an audio segment) into a sequence of tokens, and a generative model learns to sample tokens under conditions such as class labels or text. \emph{Low token rates} are attractive for efficiency, while \emph{high-dimensional continuous tokens} are attractive for fidelity: with fewer tokens, each token must carry more information, and increasing token dimensionality is a direct way to preserve fine details under aggressive downsampling. However, this regime also exposes a central tension: while high-dimensional tokens can improve reconstruction, their distributions can be substantially more complex and harder to model generatively, making reliable sampling challenging \cite{lai2025toward, yao2025reconstruction, ning2026spectrum}. Besides recent works on joint training the tokenizer with the generator \cite{heek2026unified, duggal2026end}, a more common workaround is to leverage large-scale self-supervised learning (SSL) representations as high-dimensional tokens, by directly using pretrained SSL embeddings \cite{zheng2025diffusion, tong2026scaling}, adding auxiliary SSL losses during tokenizer training \cite{chen2025masked}, or using pretrained SSL models to regularize a reconstruction tokenizer \cite{yao2025reconstruction, leng2025repa, page2026boosting}. While this strategy can yield token spaces that are easier to model than standard tokenizers, it introduces several practical and methodological limitations. First, SSL pretraining is resource-intensive, and the amenability of SSL embedding spaces to generative modeling can vary substantially across SSL objectives and model families; identifying a suitable SSL recipe often requires additional large-scale experimentation beyond the downstream generative training itself \cite{yao2025reconstruction, zheng2025diffusion, page2026boosting}. Second, many domains do not enjoy the same ecosystem as vision, where multiple strong pretrained SSL backbones are readily available: in less-studied modalities or specialized domains, one may have no appropriate pretrained SSL model to reuse, and the available data may not support training a competitive SSL model from scratch. Third, once an SSL embedding space is fixed, it is typically difficult to modify or fine-tune it for a specific tokenization budget; as a result, the token rate and token dimensionality are effectively inherited from the SSL model design, limiting customization and making it hard to adapt the representation to different compute--quality trade-offs. Fourth, SSL-based tokenization pipelines are often evaluated primarily with distributional metrics such as (r)FID, while omitting reference-based, signal-level reconstruction fidelity \cite{zheng2025diffusion, tong2026scaling, duggal2026end}; this is problematic for fidelity-preserving uses of tokens such as editing and inpainting, where signal-level faithfulness matters. Importantly, using SSL as an auxiliary signal does not fully resolve these issues, as it still depends on the availability and suitability of pretrained SSL models and inherits the limited controllability of the SSL representation geometry. Moreover, existing ``reconstruction-first, SSL-regularized'' tokenizers still do not consistently translate improved reconstruction metrics into commensurate gains in generative quality when the token dimensionality becomes high \cite{yao2025reconstruction, page2026boosting}, suggesting that high-dimensional token generation requires mechanisms beyond SSL-based regularization.

Beyond tokenization, the dominant practice for continuous token generation is to adopt standard flow matching framework with a velocity-prediction loss \cite{lipman2022flow, liu2022flow}. However, this seemingly natural choice hides a systematic inference pathology: when the model is trained to regress a velocity vector (thereby implicitly predicting both its direction and magnitude), any directional error in the predicted vector induces a systematic shrinkage of its optimal magnitude, biasing the update toward smaller inference step sizes independent of architectural choices. We refer to this effect as \emph{under-stepping}. Moreover, this issue becomes particularly consequential in the high-dimensional token regime. A basic fact of high-dimensional probability is that if $x\sim\mathcal N(0,I_N)$, then $\|x\|$ concentrates sharply around $\sqrt{N}$: most probability mass lies in a thin annulus near a hypersphere of radius $\sqrt{N}$. Since standard VAE-style Gaussian priors encourage token distributions to match such high-dimensional Gaussians, the tokenizer decoder is effectively trained on tokens whose norms stay close to this typical radius, and it may be brittle to off-shell inputs that it rarely observes. Under-stepping during flow inference produces exactly such off-shell states: the trajectory fails to reach the typical radius, yielding tokens with systematically smaller norms than those seen during tokenizer training. Moreover, if the generative model itself relies on such $\|x\|$-related information when predicting the velocity vector, a mismatched $\|x\|$ caused by under-stepping will further bias the velocity prediction at next step, creates stronger exposure bias. Consequently, generation errors are amplified twice in such high-dimensional regime: first by exaggerating the exposure bias in the prediction of the generative model, and then by pushing samples into regions where the tokenizer decoder is out-of-distribution.

In addition, even with a well-shaped token space and a stable sampler, practical conditional generation can remain fragile under \emph{AR distribution shift} or \emph{AR exposure bias} \cite{schmidt2019generalization}. AR generators are trained with teacher forcing but are deployed in a free-running mode, so small prediction errors can accumulate and progressively corrupt the context used for subsequent predictions. This effect is often amplified by classifier-free guidance (CFG), whose extrapolation can push predictions away from the model's typical continuation dynamics. In an AR setting, such guided deviations not only affect the current prediction, but also alter the future conditioning context, so any mismatch between the guided update and the model's typical in-domain continuation can compound over time. As a result, guidance can improve condition adherence while increasing the risk of long-horizon drift, where errors accumulate into noticeable artifacts or attribute instability. Recent works have extensively studied this issue and various training and inference-phase methods have been proposed \cite{chen2024diffusion, huang2025self, cui2025self, liu2025rolling, yuan2026helios}.

Taken together, the above analysis suggests a concrete goal: \textbf{how to design low-rate, high-dimensional tokenizers and generators in a principled way, such that the overall system remains robust and effective across modalities and across AR/NAR generation paradigms?} Concretely, we seek (i) a reconstruction-faithful yet generative-friendly tokenizer, whose token space is regular and traversable for generation while preserving reference-based reconstruction fidelity; (ii) a stable high-dimensional generation framework that avoids systematic inference pathologies such as under-stepping and prevents trajectories from drifting into regions that are out-of-distribution for the tokenizer decoder; and (iii) a conditional generation model that remains robust under AR distribution shift and CFG, so that condition adherence can be improved without inducing long-horizon drift or compounding inconsistencies.

We argue that achieving these goals hinges on four ingredients:
\begin{enumerate}[leftmargin=2.0em,label=(\roman*)]
\item \textbf{Geometry shaping without SSL.}
We hypothesize that the main benefit of SSL embeddings for high-dimensional generation lies in the \emph{geometry} they induce in representation space. This suggests that generation-friendly geometry can be induced without SSL by explicitly shaping the token space with geometry-aware constraints and perturbations under a reconstruction-only regime.

\item \textbf{Decoder robustness to generator-typical inconsistencies.}
We hypothesize that reconstruction quality under generation is limited not only by clean-token fidelity, but also by how the decoder responds to \emph{structured inconsistencies} that arise from imperfect token generation. Tokenization should therefore be trained to decode a controlled neighborhood around each token, so that small generation errors do not immediately amplify into large reconstruction artifacts.

\item \textbf{Inference with stable step lengths, coupled to token geometry.}
We hypothesize that stable high-dimensional sampling requires an inference mechanism whose effective step lengths remain well-behaved at test time (avoiding systematic under-stepping), and that this mechanism should be \emph{geometrically coupled} to the tokenizer's token space so that inference trajectories stay within the decoder's typical region.
\end{enumerate}

These ingredients directly motivate three corresponding contributions of this paper:
\begin{enumerate}[leftmargin=2.0em,label=(\arabic*)]
\item \textbf{Spherical tokenization with geometry-aware training.}
We propose a reconstruction-first, SSL-free tokenizer that produces fixed-norm spherical tokens and is trained with geometry-respecting perturbations and constraints to induce a regular, traversable token space while explicitly targeting reference-based reconstruction fidelity.

\item \textbf{Direction-only Rectified Flow (DRF): direction-only flow matching with geometric step recovery.}
Based on the properties of high-dimensional fixed-norm spherical tokens, we propose \textbf{direction-only rectified flow (DRF)}, a modified rectified flow framework that only predicts the direction of the velocity and recovers step lengths at inference time via geometric constraints, yielding more stable training and sampling in high-dimensional token spaces.

\item \textbf{Multi-path residual classifier-free guidance for stable conditional generation.}
We introduce a minimalist autoregressive model design with routed conditioning and a residual multi-path CFG formulation. By anchoring guidance on stable continuation paths and separately scaling role-specific guidance components, the proposed guidance mitigates error accumulation under autoregressive distribution shift and provides an interpretable trade-off between condition adherence and sample fidelity.
\end{enumerate}

We evaluate the proposed framework on label-to-image generation on ImageNet-1k \cite{deng2009imagenet} using \textbf{f32d512 (8\texttimes 8\texttimes 512D)} continuous tokens, and on text-to-speech generation on Seed-TTS \cite{anastassiou2024seed} using \textbf{6\texttimes 512D} tokens. We report both reference-based reconstruction fidelity and generative performance, and provide ablations that isolate the effects of spherical tokenization, REF, and routed residual guidance. 

The rest of the paper is organized as follows. Section~\ref{sec:tokenizer} introduces the core idea of spherical tokenization, describes how we enforce low-dimensional manifold constraints, and presents a minimalist architectural design paradigm. Section~\ref{sec:DRF} analyzes why standard rectified flow can fail in high-dimensional settings, and presents our modifications to flow matching that enable direction-only training with geometry-based, adaptive step-size inference. Section~\ref{sec:models} describes a multi-path conditioning AR generative model design, which assigns different functional roles to different conditioning signals and applies multi-path CFG to balance condition adherence, sample fidelity, and distribution drift. Section~\ref{sec:experiments} presents experimental results and further discussions.

==> sections_old/models.tex <==
\section{Information-routed AR Generator with Multi-path CFG}
\label{sec:models}

\label{sec:generative_model_design}
\begin{figure}[!ht]
    \centering
    \includegraphics[width=1.0\textwidth]{figs/generative_model.pdf}
    \caption{Caption generative model}
    \label{fig:generative_model}
\end{figure}

In this section, we study exposure bias and the resulting distribution drift in autoregressive (AR) generative models. In the aforementioned sections, we have removed the radial degree of freedom from tokens and modeled only their directions, enforced causal token mixing in the tokenizer encoder via axis-mixing constraints to prevent future information leakage, and stabilized inference magnitudes through DRF with radius-locking. This raises a natural question: are these geometric and solver-level stabilizations sufficient to eliminate AR exposure bias and distribution drift? By extensive experiments on an AR text-to-speech (TTS) task, we find that they are not. While the above design choices substantially mitigate error accumulation, AR generation can still exhibit progressive degradation over long horizons. This suggests that token geometry and solver stability, although necessary, are not the whole story: additional factors can still induce mismatch and compounding errors in AR sampling.

Empirically, we hypothesize that a core remaining source of AR error accumulation is \emph{information pathway conflict under CFG}. Specifically, conditioning signals with similar functionality may appear in multiple CFG paths but be combined inconsistently across paths; the resulting conflicts are then fed back through the AR loop and manifest as gradual drift of the corresponding attributes. We illustrate this phenomenon in the AR-TTS setting: in practice, AR-TTS degradation often emerges as drift in \emph{acoustic attributes}---e.g., spectral distortion, gradually drifting loudness, or changing speaking rate---whereas \emph{content consistency} is typically much more stable. This asymmetry suggests that acoustic-state drift, rather than semantic inconsistency, is the dominant mode of error accumulation. We attribute it to partially overlapping or redundant acoustic cues across CFG paths that can become mutually inconsistent under guidance, thereby inducing slow but systematic drift when iterated autoregressively.

Motivated by this hypothesis, we propose an explicit \emph{information-pathway decoupling} design for modality-agnostic AR generation and guidance. Concretely, we route conditioning into functionally distinct channels and apply CFG as structured residual corrections, so that each guidance component targets a specific role rather than implicitly entangling overlapping information across paths.

\subsection{ELD: A Conditional Autoregressive Generation Framework}
\label{sec:eld_baseline}

We start from the \textbf{ELD} (Encoder--LM--Decoder) framework, which is a common recipe for in-context conditional AR generation \cite{lee2023sequential, ruhe2024rolling, jia2025ditar, yin2025slow, jiang2025diffrhythm}: given a human-specified control signal $c$ (e.g., text, labels, or reference inputs) and a token prefix, ELD first \emph{integrates} them into a step-wise conditioning signal, and then uses a decoder to predict the next tokens. Here we assume a single-token prediction scheme for simplicity, and the block-AR framework where the decoder predicts a set of tokens follows the same logic.

\paragraph{Problem setup.}
Let $x_{1:L}=(x_1,\dots,x_L)$ denote the token sequence, where ground-truth tokens are used for teacher forcing training and model-generated tokens are used for inference. At step $t$, the goal is to model the conditional next-token distribution $p(x_{t+1}\mid x_{1:t},\,c)$. ELD aggregates the control signal $c$ and the prefix $x_{1:t}$ into a \emph{step-wise} control signal $c'_t$ (or a sequence $\{c'_j\}$ aligned to token positions), and the decoder predicts $x_{t+1}$ conditioned on the fixed-length time-dependent condition $c'_t$:
\begin{equation}
p(x_{t+1}\mid x_{1:t},c)\ \equiv\ p(x_{t+1}\mid c'_t).
\end{equation}

\paragraph{Model components.}
ELD constructs $c'_t$ using an encoder, a sequence modeling module (LM), and a flow-matching decoder predictor.

\textbf{Encoder.}
A token encoder $E$ maps a (clean) token to a hidden representation, which serves as a token adaptor mapped to a hidden space aligned for better sequential modeling with the control signal:
\begin{equation}
h_{t} = E(x_{t}),\qquad h\in\mathbb{R}^{d}.
\end{equation}

\textbf{LM.}
The control signal $c$ is embed as a sequence $\phi(c)$ in the same hidden space and form an in-context sequence by concatenation:
\begin{equation}
s_t = [\,\phi(c)\,;\, h_{1:t}\,].
\end{equation}
An autoregressive LM produces step-wise conditioning vectors
\begin{equation}
c'_{1:t} = \mathrm{LM}(s_t),\qquad c'_j\in\mathbb{R}^{d},
\end{equation}
and we use $c'_t$ as the control signal for predicting $x_{t+1}$.

\textbf{Decoder.}
Given $c'_t$ and a noisy intermediate token at step $t+1$ constructed by any bridge, the decoder $D$ predicts the target velocity field by modeling $p(x_{t+1}\mid c'_t)$. Additional flow time $\tau$ and its time embedding is also fed to the model.

\paragraph{Noisy teacher forcing.}
To mitigate exposure bias, during training the ground-truth prefix tokens are typically perturbed with a small noise before feeding them to the encoder. This simulates mild inference-time distribution drifts while staying within a semantics-preserving neighborhood and is a standard technique \cite{ning2023input, chen2024diffusion}.

\paragraph{CFG efficiency.}
At inference time, CFG is applied only at the decoder level, while the encoder and LM are evaluated once to produce $c'_t$. This is computationally cheaper than settings where the LM/backbone must participate in CFG (e.g., non-autoregressive models or streaming diffusion-style backbones such as Transfusion), since CFG does not require multiple forward passes through the encoder/LM.

\subsection{MP-ELD: Information Routing and Multi-path CFG}
\label{sec:mpeld}

In practice, we find that the ELD framework can be fragile when CFG (with stronger guidance weight) is applied in decoder. Empirically, this failure mode is closely tied to two design ambiguities: (i) what information the step-wise control signal $c'_t$ is expected to preserve and how it should be used/amplified by the decoder, and (ii) how to define the ``conditional'' and ``unconditional'' paths in CFG for the decoder. In particular, a fully null unconditional path can be problematic in this setting, as it provides no local continuation anchor and may yield a high-variance early-time velocity field and makes the training extremely ill-posed. Based on these observations, we introduce \textbf{Multi-path ELD (MP-ELD)}, a modification of ELD that makes the roles of conditioning signals explicit. The core idea is \emph{information routing}: we construct multiple conditioning paths that intentionally receive different information, so that each path naturally specializes to a different role. We further combine these paths using \emph{multi-path CFG} \cite{liu2022compositional} with \emph{time-varying CFG weights}, and enforce a residual, non-overlapping structure among conditioning signals via an orthogonalization transform.

\paragraph{Multi-path conditioning.}
At step $t$, MP-ELD constructs three step-wise conditioning vectors:
\begin{itemize}
\item \textbf{Local-continuity conditioning} $c^{\mathrm{lc}}_t$: a local continuation anchor derived from current token responsible for local continuity constraint.
\item \textbf{Self-consistency conditioning} $c^{\mathrm{sc}}_t$: an in-context summary of modality-internal, in-context evolution over the prefix mainly responsible for capturing long-horizon stability and self attribute consistency.
\item \textbf{Alignment-consistency conditioning} $c^{\mathrm{ac}}_t$: a condition-aware signal mainly responsible for aligning cross-modality or external control information.
\end{itemize}
All three are represented in a shared $d$-dimensional conditioning space.

\paragraph{Information modeling paths.}
We implement the three conditioning sources using three lightweight token encoders and two LMs:
\begin{itemize}
\item A \emph{local encoder} $E_{\mathrm{lc}}$ produces the local-continuity signal from current token:
\begin{equation}
c^{\mathrm{lc}}_t = E_{\mathrm{lc}}(\tilde x_{t})\in\mathbb{R}^{d}.
\end{equation}
This can be viewed as an ``in-context, unconditional local continuation'' path.
\item A \emph{self-consistency encoder} $E_{\mathrm{sc}}$ and a \emph{self-consistency LM} $\mathrm{LM}_{\mathrm{sc}}$ produce the self-consistency signal from the history tokens:
\begin{equation}
h^{\mathrm{sc}}_{t}=E_{\mathrm{sc}}(\tilde x_{t}),\qquad
c^{\mathrm{sc}}_{1:t}=\mathrm{LM}_{\mathrm{sc}}(h^{\mathrm{sc}}_{1:t}),\qquad
c^{\mathrm{sc}}_t\in\mathbb{R}^d.
\end{equation}
This can be viewed as an ``in-context, unconditional global continuation'' path.
\item An \emph{alignment-consistency encoder} $E_{\mathrm{ac}}$ and an \emph{alignment-consistency LM} $\mathrm{LM}_{\mathrm{ac}}$ produce the alignment signal by integrating the external condition with the history tokens:
\begin{equation}
h^{\mathrm{ac}}_{t} = E_{\mathrm{ac}}(\tilde x_{t}),\qquad
c^{\mathrm{ac}}_{1:t} = \mathrm{LM}_{\mathrm{ac}}\big([\phi(c);\, h^{\mathrm{ac}}_{1:t}]\big),\qquad
c^{\mathrm{ac}}_t\in\mathbb{R}^{d}.
\end{equation}
This can be viewed as an ``instruct-based, conditional global continuation'' path.
\end{itemize}
Intuitively, such paths can be viewed as the following roles in the TTS task:
\begin{itemize}
    \item $c^{\mathrm{lc}}_t$ encourages smooth local continuation of short-range acoustic attributes (e.g., pitch/phase/energy) and preventing abrupt discontinuities.
    \item $c^{\mathrm{sc}}_t$ captures slowly-varying acoustic attributes that should remain stable over an utterance (e.g., timbre, overall energy profile, and accent/style).
    \item $c^{\mathrm{ac}}_t$ indicates ``where we are'' in the conditioned content and thus what should be generated next (e.g., which part of the text should be spoken at the current step).
\end{itemize}
Similar roles can also be defined for other modalities (e.g., video).

For tasks that require explicit duration/stop detection (e.g., TTS or video generation), we augment the alignment-consistency LM with an additional scalar head, analogous to predicting an EoS token in text generation. Concretely, in addition to the step-wise alignment vector $c^{\mathrm{ac}}_t$, the alignment-consistency LM outputs a scalar $\pi_t\in[0,1]$ that represents the probability of \emph{continuing} generation at the next step. During training, we supervise $\pi_t$ with a binary cross-entropy loss against the ground-truth stop label/sequence length, and at inference time we terminate decoding when $\pi_t$ falls below 0.5.

\paragraph{Orthogonal residual conditioning.}
To encourage a residual, non-overlapping decomposition of conditioning information, we orthogonalize the three condition vectors via a Gram--Schmidt transform and normalize each component to a fixed radius:
\begin{align}
\bar c^{\mathrm{lc}}_t &= \mathrm{Norm}_{\sqrt{d}}(c^{\mathrm{lc}}_t), \\
\bar c^{\mathrm{sc}}_t &= \mathrm{Norm}_{\sqrt{d}}\!\Big(c^{\mathrm{sc}}_t - \frac{\langle c^{\mathrm{sc}}_t,\bar c^{\mathrm{lc}}_t\rangle}{\|\bar c^{\mathrm{lc}}_t\|^2}\,\bar c^{\mathrm{lc}}_t\Big), \\
\bar c^{\mathrm{ac}}_t &= \mathrm{Norm}_{\sqrt{d}}\!\Big(c^{\mathrm{ac}}_t - \frac{\langle c^{\mathrm{ac}}_t,\bar c^{\mathrm{lc}}_t\rangle}{\|\bar c^{\mathrm{lc}}_t\|^2}\,\bar c^{\mathrm{lc}}_t
- \frac{\langle c^{\mathrm{ac}}_t,\bar c^{\mathrm{sc}}_t\rangle}{\|\bar c^{\mathrm{sc}}_t\|^2}\,\bar c^{\mathrm{sc}}_t\Big),
\end{align}
Intuitively, this orthogonalization operation ensures that each condition vector only encodes \emph{residual information} that other condition vectors do not contain. This allows us to define the full-path condition as the \emph{summation} of the orthogonalized components instead of the \emph{concatenation} of the original vectors, which also controls the overall vector dimension and the related model dimensions and complexities when $d$ is large.

\paragraph{Multi-path residual CFG.}
To support guidance with multiple conditioning paths, we apply CFG dropout to the \emph{nonlocal} branches only: during training we randomly drop $\bar c^{\mathrm{sc}}_t$ and $\bar c^{\mathrm{ac}}_t$ by setting them to zero, while always keeping the local-continuity anchor $\bar c^{\mathrm{lc}}_t$ present.
This preserves the decoder an always-stable local continuation signal throughout training. Since the full-path condition is formed by summation, dropping
$\bar c^{\mathrm{sc}}_t$ or $\bar c^{\mathrm{ac}}_t$ leads to the same final vector norm, and the decoder cannot reliably infer which signal is missing from the summed vector alone. We therefore additionally provide a lightweight \emph{condition presence embedding} $e(\delta^{\mathrm{sc}}_t,\delta^{\mathrm{ca}}_t)$, where $\delta^{(\cdot)}_t\in\{0,1\}$, to the decoder to disambiguate which nonlocal paths are present. At inference time, we combine multiple conditioning paths by linearly combining the decoder outputs. By default we use three paths:
\begin{itemize}
\item $P$: local-continuity only, $(\bar c^{\mathrm{lc}}_t,0,0)$, $\delta^{\mathrm{sc}}_t=0$, $\delta^{\mathrm{ca}}_t=0$;
\item $PS$: local-continuity + self-consistency, $(\bar c^{\mathrm{lc}}_t,\bar c^{\mathrm{sc}}_t,0)$, $\delta^{\mathrm{sc}}_t=1$, $\delta^{\mathrm{ca}}_t=0$;
\item $PSC$: local-continuity + self-consistency + condition-alignment, $(\bar c^{\mathrm{lc}}_t,\bar c^{\mathrm{sc}}_t,\bar c^{\mathrm{ac}}_t)$, $\delta^{\mathrm{sc}}_t=1$, $\delta^{\mathrm{ca}}_t=1$.
\end{itemize}
Following the residual decomposition of the three conditioning paths, we perform \emph{multi-path residual CFG}:
\begin{equation}
v_t
=
v_t^{P}
+
\lambda_{\mathrm{sc}}\big(v_t^{PS}-v_t^{P}\big)
+
\lambda_{\mathrm{ac}}\big(v_t^{PSC}-v_t^{PS}\big),
\label{eq:multipath_cfg_mpeld}
\end{equation}
where $(v_t^{PS}-v_t^{P})$ is the self-consistency residual relative to the local-continuity path, and $(v_t^{PSC}-v_t^{PS})$ is the alignment residual relative to the self-consistent path. When $\lambda_{\mathrm{sc}}=\lambda_{\mathrm{ac}}=1$, the inference falls back to the ``no CFG'' mode where $v_t=v_t^{PSC}$, which matches the common configuration in standard two-path CFG.

\paragraph{Time-dependent CFG guidance.}
We empirically find that extrapolating the self-consistency residual $(v_t^{PS}-v_t^{P})$ (i.e., $\lambda_{\mathrm{sc}}>1$) is a key ingredient for improving in-context / in-domain consistency (e.g., speaker-timbre consistency in TTS), but it is also the primary cause of distribution drift and long-horizon error accumulation. In contrast, extrapolating the alignment residual $(v_t^{PSC}-v_t^{PS})$ (i.e., $\lambda_{\mathrm{ac}}>1$) is important for strengthening conditional controllability, and we do not observe comparable drift induced by this term. We further hypothesize that the extrapolation instability of the self-consistency residual is mainly caused by an unreliable estimate of $v_t^{P}$ in the small-$t$ regime, where the decoder tends to rely more on conditioning signals than on $x_t$ itself due to the broader self-bootstrapping shortcut posterior $p(x_1 \mid x_t)$ (Sec.~\ref{sec:sfm_shortcut}). As the $P$ path only contains local continuation information, which is far less sufficient than the $PS$ path for a reliable estimate of $v_t$ at small $t$, the ``base point'' $v_t^{P}$ on which the self-consistency extrapolation applies is typically less reliable, and extrapolation from it can easily produce off-manifold intermediate states whose errors may be further amplified at larger $t$ due to the same mechanism in the self-bootstrapping shortcut. On the other hand, since we design the alignment residual to be based on $v_t^{PS}$ instead of $v_t^{P}$, extrapolation along $(v_t^{PSC}-v_t^{PS})$ is typically stable across all $t$.

Motivated by the hypothesis above, we use a time-dependent self-consistency guidance weight $\lambda_{\mathrm{sc}}(t)$ to avoid extrapolating from an unreliable base in the early-time regime. Concretely, we start from $\lambda_{\mathrm{sc}}(0)=1$ (no extrapolation) and gradually increase to a predefined maximum $\lambda_{\mathrm{sc}}$:
\begin{equation}
\lambda_{\mathrm{sc}}(t)
\;=\;
1 + \big(\lambda_{\mathrm{sc}}-1\big)\,s(t),
\qquad
s(0)=0,\ s(1)=1,
\label{eq:lambda_sc_schedule}
\end{equation}
where $s(t)$ is a non-decreasing schedule, e.g., $s(t)=t^\tau$. We keep $\lambda_{\mathrm{ac}}$ constant by default.

==> sections_old/orf.tex <==
\section{Outward Ray Flow}
\label{sec:ORF}

We introduce \textbf{Outward Ray Flow (ORF)}, a flow-matching style generation method tailored to the high-dimensional spherical tokens described above. Different from the problem formulation of the standard rectified flow method, ORF defines the source distribution as an \emph{inner-sphere} of the token's underlying sphere, and learns only the \emph{direction (ray)} of the \emph{inner-to-outer} transport field. During inference, the step size for each ODE integration step is controlled by a well-defined \emph{radial progress} instead of a fixed, predefined step size progress.

ORF leverages a core structural property: in high dimensions, linear interpolation between two nearly orthogonal vectors yields a radius that is (approximately) a deterministic function of time. ORF therefore learns only the \emph{direction} (ray) of the transport field during training, while the step size is explicitly calculated by a \emph{radial schedule} during inference.

\subsection{Inner-to-Outer Spherical Transport}
With the target state of $x_1 \in \mathbb{S}^{N-1}(R)$, we sample the source state from an \emph{inner} sphere of radius $aR$:
\begin{align}
x_0 \sim \mathrm{Unif}\big(\mathbb{S}^{N-1}(aR)\big),\quad a\in(0,1)
\label{eq:x0_inner_sphere}
\end{align}
We use the standard linear bridge to define the intermediate states, and we also use the standard velocity field definition in rectified flow to define the \emph{transport ray} $r^\star$:
\begin{align}
x_t &= (1-t)x_0 + t x_1,\quad t\in[0,1] \\
v^\star &= \frac{d x_t}{dt} = x_1 - x_0,\quad r^\star = \frac{v^\star}{\|v^\star\|_2}
\label{eq:bridge_and_ray}
\end{align}
This \emph{inner-to-outer} setup yields a well-defined outward geometry: for any $x_0\in \mathbb{S}^{N-1}(aR)$ and any direction $r\in\mathbb{S}^{N-1}(1)$, the ray $\{x_0+\lambda r:\lambda\ge 0\}$ intersects the outer sphere $\mathbb{S}^{N-1}(R)$ at a unique point (i.e., at a unique $\lambda>0$).

\subsection{Time Sampling Schedule and the Choice of $a$}

A common time sampling schedule in modern diffusion and flow-matching models is the \textit{logit-normal} distribution~\cite{}:
\begin{align}
z \sim \mathcal{N}(m,s),\quad t = \sigma(z)=\frac{1}{1+e^{-z}}
\label{eq:logit_normal_t}
\end{align}
where $\sigma(m)$ is the median of $t$ due to the monotonicity of $\sigma(\cdot)$. We measure the relative contribution of the two endpoints in the linear bridge by the (log) signal-to-noise ratio
\begin{align}
\mathrm{SNR}(t)
\;\triangleq\;
\log\frac{\|t x_1\|_2}{\|(1-t)x_0\|_2}
\;=\;
\log\frac{t}{a(1-t)}
\label{eq:snr}
\end{align}
The equal-contribution point is given by $\mathrm{SNR}(t^\star)=0$, yielding
\begin{align}
t^\star=\frac{a}{1+a}
\end{align}
Intuitively, this point corresponds to the most ambiguous intermediate states, where neither endpoint dominates the mixture. We thus center the time sampling distribution at $t^\star$ by setting the logit-normal median $\sigma(m)=t^\star$, i.e.,
\begin{align}
m=\mathrm{logit}(t^\star)=\log\frac{t^\star}{1-t^\star}=\log a
\end{align}
We next motivate a principled choice $a$. With Eq.~\eqref{eq:cosine_gaussian}, i.e., $\langle x_0,x_1\rangle \approx 0$, the squared norm of the bridge concentrates around
\begin{align}
\|x_t\|_2^2
&=
\|(1-t)x_0+t x_1\|_2^2
\nonumber\\
&\approx
(1-t)^2\|x_0\|_2^2+t^2\|x_1\|_2^2
=
R^2\!\left(a^2(1-t)^2+t^2\right)
\label{eq:xt_norm_approx}
\end{align}
This implies a characteristic \emph{radial contraction--expansion} behavior: starting from $\|x_0\|_2=aR$, the radius may initially decrease (contract) before increasing (expand) toward $R$. It is easy to see that the radius is minimized at $t_{\min}=\frac{a^2}{1+a^2}$, and we refer to $[0,t_{\min}]$ as the \emph{contraction phase}. Intuitively, during this phase the state is pushed further toward the origin, which is undesirable for conditional generation since states closer to the origin tend to be less informative about the target endpoint and make the conditional transport more challenging. While it is easy to see that the equal-contribution point $t^\star$ always occurs \emph{no earlier than} the contraction endpoint:
\begin{align}
\Delta(a)\triangleq t^\star-t_{\min}
=
\frac{a}{1+a}-\frac{a^2}{1+a^2}
=
\frac{a(1-a)}{(1+a)(1+a^2)}
>0,\quad \forall a\in(0,1)
\end{align}
a larger $\Delta(a)$ is still typically beneficial because it separates the low-information contraction phase (higher uncertainty of target given $x_t$) from the equal-contribution point (target starts to dominate). Maximizing $\Delta(a)$ over $a\in(0,1]$ by solving $\Delta'(a)=0$ gives us the unique solution $a^\star \in (0,1)$:
\begin{align}
\varphi = \frac{1+\sqrt{5}}{2},\quad a^\star=\varphi - \sqrt{\varphi} \approx 0.346
\end{align}
In practice we choose \emph{$a=1/e\approx 0.368$}, which is close to the maximizer of the separation gap $\Delta(a)$ while yielding a particularly simple time-sampling parameter $m=\log a=-1$ for logit-normal sampling. Moreover, $a=1/e$ admits a clean geometric interpretation: let $\mathrm{Area}(r)$ denote the $(N\!-\!1)$-dimensional surface area of the radius-$r$ hypersphere $S^{N-1}(r)$, we have $\mathrm{Area}(r)\propto r^{N-1}$. Then the log surface-area expansion from $aR$ to $R$ equals $\log\frac{\mathrm{Area}(R)}{\mathrm{Area}(aR)}=-(N-1)\log a = N-1$ \textit{nats}, i.e., approximately $1$ nat per dimension.

\subsection{Training loss}
The model predicts a unit transport direction (ray) $\hat{r}\in\mathbb{S}^{N-1}(1)$. We train with an angular alignment loss between target and predicted unit transport directions defined by cosine similarity:
\begin{align}
L_{\mathrm{ORF}}
\;=\;
1 - \text{cos}\!\left(\hat{r},\, r^\star\right)
\label{eq:ORF_loss}
\end{align}

\subsection{Adaptive Step-size Inference via High-Dimensional Radius Locking}

Eq.~\eqref{eq:xt_norm_approx} shows that the radius of $x_t$ is approximately determined by $t$ alone. This property allows us to adaptively decide the step size during inference-time ODE integration via \emph{high-dimensional radius locking}. The main idea is to find the proper step size $\Delta_t$ such that the radius of each $x_t$ accurately aligns with a \emph{radius schedule} $\rho(t) \;=\; R\sqrt{a^2(1-t)^2 + t^2}$ in Eq.~\eqref{eq:xt_norm_approx}, under which the training-inference mismatch with respect to the radius of $x_t$ and $t$ can be minimized. We design the following inference procedure:

\paragraph{Initialization.}
Sample $x_{t_0}$ at $t_0=0$ as
\begin{align}
x_{t_0} \sim \mathrm{Unif}\big(\mathbb{S}^{N-1}(aR)\big)
\end{align}

\paragraph{Radially matched update.}
Given the estimated transport field $\hat{r}_{t_k}$, we choose a step size $\Delta_{t_k} > 0$ such that the next state matches the target radius:
\begin{align}
\|x_{t_k} + \Delta_{t_k} \hat{r}_{t_k}\|_2 = \rho(t_{k+1})
\label{eq:radial_match_condition}
\end{align}
Since $\|\hat{r}_{t_k}\|_2=1$, Eq.~\eqref{eq:radial_match_condition} yields a scalar quadratic equation:
\begin{align}
\|x_{t_k}\|_2^2 + 2\Delta_{t_k} \langle x_{t_k}, \hat{r}_{t_k}\rangle + \Delta_{t_k}^2 = \rho(t_{k+1})^2
\end{align}
Since $\|x_{t_k}\|_2^2 = \rho(t_k)^2$, simplifying the equation leads to
\begin{align}
\Delta_{t_k}
=
-\langle x_{t_k}, \hat{r}_{t_k}\rangle
\pm
\sqrt{
\langle x_{t_k}, \hat{r}_{t_k}\rangle^2
+
\rho(t_{k+1})^2
-
\rho(t_k)^2
}
\label{eq:delta_solution}
\end{align}
Let $c_k=\langle x_{t_k},\hat r_{t_k}\rangle$ and $\Delta\rho_k^2=\rho(t_{k+1})^2-\rho(t_k)^2$, then the two roots are
$\Delta_{t_k}=-c_k\pm\sqrt{c_k^2+\Delta\rho_k^2}$, whose product satisfies $\Delta_{t_k}^{(+)}\Delta_{t_k}^{(-)}=-\Delta\rho_k^2$. Therefore, in the \emph{expansion} regime where $\Delta\rho_k^2>0$, the two roots have opposite signs and the physically consistent update is the positive one. In the \emph{contraction} regime where $\Delta\rho_k^2<0$, there are two circumstances: 
\begin{enumerate}
    \item If $c_k^2+\Delta\rho_k^2 < 0$,  there is no real-valued root for the equation, and we set $\Delta_{t_k}=-c_k$ which corresponds to the step size that leads to \emph{the smallest achievable radius}, and then re-normalize $x_{t_{k+1}}$ to match the target radius.
    \item If $c_k^2+\Delta\rho_k^2 \geq 0$, the two roots have same signs and the physically consistent update is the negative one.
\end{enumerate}

We can thus write a unified update rule:
\begin{align}
\Delta_{t_k}
=
-c_k+\mathrm{sign}(\Delta\rho_k^2) \sqrt{\max (0, c_k^2+\Delta\rho_k^2}), \quad x_{t_{k+1}}^* = x_{t_k} + \Delta_{t_k}\hat{r}_{t_k}, \quad x_{t_{k+1}} = \rho(t_{k+1})\frac{x_{t_{k+1}}^*}{\|x_{t_{k+1}}^*\|_2}
\end{align}

\paragraph{Classifier-free guidance.}
When CFG is enabled, we first apply guidance to the unit ray $\hat r_{t_k}$ and then compute the step size via radial matching. Since the model predicts unit-norm directions, we perform guidance on the hypersphere using a geodesic update (spherical CFG) rather than Euclidean linear interpolation. Concretely, given the unconditional and conditional rays $\hat r_{\varnothing},\hat r_c\in\mathbb{S}^{N-1}(1)$, we define
\begin{align}
\hat r_{\mathrm{cfg}}
&=
\mathrm{Exp}_{\hat r_{\varnothing}}\!\Big(w_{\mathrm{cfg}}\;\mathrm{Log}_{\hat r_{\varnothing}}(\hat r_c)\Big)
\label{eq:spherical_cfg}
\end{align}
where $\mathrm{Log}$ and $\mathrm{Exp}$ denote the Riemannian logarithm and exponential maps on the unit sphere. This construction preserves unit norm by definition and naturally supports extrapolation for $w_{\mathrm{cfg}}>1$. For $w_{\mathrm{cfg}}\in[0,1]$, Eq.~\eqref{eq:spherical_cfg} reduces to standard spherical linear interpolation (slerp).
For $w_{\mathrm{cfg}}>1$, it performs geodesic extrapolation beyond the conditional ray, and we clamp the extrapolation component by limiting the angular norm of $(w_{\mathrm{cfg}}-1)\,\mathrm{Log}_{\hat r_{\varnothing}}(\hat r_c)$ to be at most $\theta_{\max}(t)$ at time $t$ (equivalently, we set $w(t)\leftarrow 1+\min\{w_{\mathrm{cfg}}-1,\ \theta_{\max}(t)/(\|\mathrm{Log}_{\hat r_{\varnothing}}(\hat r_c)\|_2+\varepsilon)\}$), so that the additional deviation beyond $\hat r_c$ is bounded.

\subsection{Discussion: Standard Rectified Flow on High-dimensional Spheres}
\label{sec:orf_discussion_magnitude_shrinkage}

\subsubsection{$v$-Pred Magnitude Shrinkage from Bearing-Angle Decoupling}
\label{sec:analysis_mse_shrinkage}

We show that in $v$-pred loss (e.g., MSE), any persistent angular error implies a systematic underestimation of the velocity magnitude despite the token dimension $N$. Fix an input $(x_t,t,c)$ and suppose the model predicts a unit direction $\hat r$. Consider the restricted family of predictors of the form
\begin{equation}
\hat v(s) \;=\; s\,\hat r,\quad s\in\mathbb{R}
\end{equation}
The MSE-optimal scalar $s^\star$ is obtained by solving
\begin{equation}
s^\star \;=\; \arg\min_{s\in\mathbb{R}} \|s\hat r - v^\star\|_2^2
\end{equation}
Expanding the quadratic and differentiating yields
\begin{equation}
s^\star \;=\; \|v^\star\|_2 \cos\theta
\label{eq:s_star_cos}
\end{equation}
where $\theta$ is the angular error, $\cos\theta=\langle \hat r, r^\star\rangle$, and $r^\star = v^\star/\|v^\star\|_2$. This shows that angular error is converted directly into magnitude shrinkage under MSE $v$-pred loss, as any $\theta > 0$ lead to $s^\star < \|v^\star\|_2$. As it is typically always true for a learned predictor to exhibit a nonzero angular error distribution, thus we have
\begin{equation}
\mathbb{E}\big[s^\star\big]
=
\|v^\star\|_2\,\mathbb{E}[\cos\theta]
<
\|v^\star\|_2
\quad\text{whenever}\quad \mathbb{P}(\theta\neq 0)>0.
\label{eq:mse_shrinkage_expected_subsec}
\end{equation}
which results in a systematic underestimation of the velocity magnitude. As a result, ODE integrators (e.g., Euler) is highly likely to suffer from shrinkage of displacement-per-step and may require more steps or stronger CFG guidance weights to reach the target region (thin shell). As Eq.~\eqref{eq:chi2_moments_subsec} shows that the relative thickness $O(1/\sqrt{N})$ vanishes as $N\to\infty$, the latent distribution becomes increasingly concentrated on the thin shell when $N$ is sufficiently large. This concentration has a direct implication for token decoding: in VAE-style tokenizers, the decoder is trained almost exclusively on latents sampled from the aggregated posterior, which in high dimensions also concentrates on the same thin shell. Consequently, the systematic magnitude shrinkage can cause the predicted final tokens to fall inside the hypersphere's interior—a region far from the decoder's training support. When evaluated on such out-of-distribution inputs, the decoder may fail to reconstruct reliably, leading to severe quality degradation.

\subsubsection{Conditional Ambiguity and the $a=1$ Coincidence}
The standard rectified flow setup with $N(0, 1)$ initialized $x_0$ statistically matches ORF with the $a=1$ configuration, i.e., $x_0$ reside almost always on the same sphere $\mathbb{S}^{N-1}(R)$ as $x_1$. This causes the equal-contribution point $t^*=0.5$ to coincide with the minimum-norm point $t_{\min}=0.5$, and the interpolation path lies entirely inside the sphere (i.e., $\|x_t\|_2 < R$ for $t \in (0,1)$). Consequently, an observed point $x_t$ with a given norm $r_t < R$ can be reached by a vast multitude of independent pairs $(x_0, x_1)$ on the sphere. This makes the conditional distribution $p(x_0, x_1 \mid x_t)$ broad and ill-concentrated, resulting in a high-variance learning target for the marginal vector field $u_t(x_t) = \mathbb{E}_{p(x_0,x_1 \mid x_t)}[v^*]$. In contrast, when we set $a < 1$ in ORF, $x_t$ satisfies $\|x_t\|_2 > aR$ after a short initial phase $t > a^2$, where the interior points ``emerged'' from the inner sphere of $x_0$. This ``outward'' phase dramatically reduces the \emph{ambiguity in the conditional vector field}: an $x_t$ with $\|x_t\|_2 > aR$ can only belong to those pairs $(x_0, x_1)$ for which $x_0$ lies in a restricted spherical cap (determined by solving $\|x_t - t x_1\|_2 = (1-t)aR$). This sharp reduction in conditional ambiguity is a key factor that makes the vector field in ORF with $a < 1$ significantly easier to learn and more stable than its $a = 1$ counterpart, as we will demonstrate empirically.

==> sections_old/spoon_flow.tex <==
\section{A Two-Phase Direction-only Flow Matching Framework}
\label{sec:spoon_flow}

We propose a two-stage flow-matching framework for conditional token generation on $\mathbb{S}^{N-1}(R)$. The central idea is to decompose the overall transport into two stages with complementary roles, so that each stage can be modeled and sampled in a way that is well matched to the spherical token geometry. This staged construction yields a stable conditional sampling procedure and avoids failure modes that can arise when a single flow-matching formulation is used across the entire time horizon. Moreover, using the aforementioned thin-shell concentration property, we perform \emph{direction-only} velocity field modeling in which the actual speed is unnecessary throughout training and inference.

This section is organized as follows. We begin by analyzing why standard rectified flow with $v$-prediction can underestimate effective step sizes under angular errors, which is particularly harmful in hyperspherical token spaces. We then present spherical flow matching as a natural on-shell baseline and discuss its robustness to radial drift as well as its potential conditioning-collapse failure mode. Next, we introduce Outward Ray Flow (ORF), which predicts only a unit transport direction and enforces a dimension-stable inference step-size schedule via \emph{radius locking}, and we highlight the ill-defined ``contraction regime problem'' that motivates a two-phase design. Finally, we propose \textbf{Spoon Flow}, a two-phase spherical transport that uses SFM with \emph{radian locking inference} in the early-time regime and ORF with \emph{radius locking inference} in the late-time expansion regime, combining the strengths of both frameworks in different time intervals.

\subsection{Rectified Flow with $v$-Prediction: Step-Size Underestimation under Angular Errors}
\label{subsec:rf_vpred}

We first recall a standard rectified-flow (RF) training setup. Let $x_1\in\mathbb{S}^{N-1}(R)$ denote a target token and let $x_0$ be a source sample. A linear bridge is defined by
\begin{equation}
x_t = (1-t)x_0 + t x_1,\qquad t\in[0,1],
\end{equation}
with the corresponding constant transport vector
\begin{equation}
v^\star = x_1 - x_0.
\end{equation}
Standard RF trains a network $\hat v(x_t,t,c)$ (optionally conditioned on $c$) by minimizing an $\ell_2$ regression loss $\|\hat v - v^\star\|_2^2$.

\paragraph{$v$-pred magnitude shrinkage under directional mismatch.}
We analyze a purely geometric property of $\ell_2$ regression: if the predicted direction is mismatched with the target direction, then the optimal predicted magnitude is reduced. Decompose the prediction into a unit direction and a scalar magnitude:
\begin{equation}
\hat v \;=\; \hat s\,\hat r,\qquad \hat r\in\mathbb{S}^{N-1}(1),\ \hat s\ge 0,
\end{equation}
and similarly write the ground-truth transport as
\begin{equation}
v^\star \;=\; s^\star r^\star,\qquad r^\star=\mathrm{Norm}_1(v^\star)\in\mathbb{S}^{N-1}(1),\ s^\star=\|v^\star\|_2.
\end{equation}
Let $\theta=\angle(\hat r,r^\star)$ denote the angular mismatch, so that $\langle \hat r,r^\star\rangle=\cos\theta$.
Conditioned on a fixed direction $\hat r$, the $\ell_2$ objective is a convex quadratic in $\hat s$:
\begin{align}
\|\hat v - v^\star\|_2^2
&=\|\hat s\hat r - s^\star r^\star\|_2^2 \nonumber\\
&=\hat s^2 + (s^\star)^2 - 2\hat s s^\star \langle \hat r,r^\star\rangle \nonumber\\
&=\hat s^2 + (s^\star)^2 - 2\hat s s^\star \cos\theta.
\label{eq:vpred_quadratic}
\end{align}
Minimizing \eqref{eq:vpred_quadratic} over $\hat s$ yields
\begin{equation}
\hat s_{\mathrm{opt}} \;=\; s^\star \cos\theta,
\label{eq:vpred_shrinkage}
\end{equation}
i.e., the optimal magnitude is scaled by the cosine of the directional mismatch. Equivalently, the component of $\hat v$ along the true transport direction satisfies
\begin{equation}
\langle \hat v, r^\star\rangle
=
\hat s_{\mathrm{opt}}\langle \hat r,r^\star\rangle
=
s^\star \cos^2\theta.
\end{equation}

\paragraph{Implication for iterative sampling.}
In iterative integration, this shrinkage translates into smaller-than-intended step sizes and can accumulate over multiple steps, yielding a biased trajectory that fails to reach the intended radius. In high-dimensional token spaces, such radius drift is particularly harmful because the decoder (no matter standard VAEs or out spherical token) is trained on a thin shell or a hypersphere and is sensitive to off-shell samples. Moreover, step size shrinkage may also make intermediate output statistics (e.g., $\|x_t\|_2$) biased from their training-time counterparts, further leads to training-inference mismatch.


\subsection{Direction-only Rectified Flow (DRF) with Explicit Radius Control}
\label{subsec:orf}

We now introduce Direction-only Rectified Flow (DRF), a direction-only transport scheme with explicitly controls on the radius of intermediate outputs during inference. The key idea is to predict only a unit \emph{ray} (bearing) and to recover the step size by enforcing a prescribed \emph{radius schedule}.

\subsubsection{Inner-to-Outer Bridge and Direction-only Supervision}
\label{sec:orf_bridge}

We term our method \textbf{Outward Ray Flow (ORF)} because it exploits a simple geometric identifiability property of \emph{inner-to-outer} linear mappings: when the source lies on an inner sphere ($a<1$) and the target lies on the outer token sphere, the endpoint on the outer sphere is uniquely determined by an outward ray from the source. Unlike high-dimensional SFM which requires the thin-shell concentration property for direction-only modeling, such property naturally supports direction-only parameterization in a linear bridge.

\paragraph{Definition.}
Let the source distribution be uniform on an \emph{inner} sphere:
\begin{equation}
x_0 \sim \mathrm{Unif}\big(\mathbb{S}^{N-1}(aR)\big),\qquad a\in(0,1),
\end{equation}
and let $x_1\in\mathbb{S}^{N-1}(R)$ be the target. We use the linear bridge
\begin{equation}
x_t=(1-t)x_0+t x_1,\qquad t\in[0,1],
\label{eq:orf_lerp_bridge}
\end{equation}
with constant transport vector $v^\star=x_1-x_0$. ORF trains a network to predict the \emph{unit transport ray}
\begin{equation}
r^\star = \mathrm{Norm}_1(x_1-x_0)\in\mathbb{S}^{N-1}(1),
\end{equation}
using a angular loss on the estimated and target rays
\begin{equation}
L_{\mathrm{ORF}} = 1-\cos\big(\hat r(x_t,t,c),\,r^\star\big).
\end{equation}

\paragraph{Uniqueness of the outer-sphere intersection.}
Consider the ray starting at $x_0$ in direction $r\in\mathbb{S}^{N-1}(1)$:
\begin{equation}
\ell(\Delta)=x_0+\Delta r,\qquad \Delta\ge 0.
\end{equation}
The intersection(s) with the outer sphere satisfy $\|\ell(\Delta)\|_2=R$, i.e.,
\begin{equation}
\|x_0+\Delta r\|_2^2 = a^2R^2 + \Delta^2 + 2\Delta\langle x_0,r\rangle = R^2.
\label{eq:ray_sphere_intersection}
\end{equation}
When $a<1$ and we restrict to the \emph{outward} branch $\Delta\ge 0$, the ray yields a unique physically valid intersection on $\mathbb{S}^{N-1}(R)$ (the first hit of the outer sphere along the outward direction). This makes it meaningful to learn only the ray direction.

\paragraph{Why the standard thin-shell RF setting is ambiguous.}
In the standard RF setup, the source is typically sampled from an isotropic Gaussian,
\begin{equation}
x_0 \sim \mathcal N(0,I_N),
\end{equation}
which concentrates on a thin shell of radius $\|x_0\|_2\approx \sqrt{N}$ in high dimensions. Likewise, in common latent-variable tokenizers (e.g., VAEs with an isotropic Gaussian prior), both the target and intermediate states also concentrate on a thin shell (up to a scale factor), e.g.,
\begin{equation}
x_1 \approx \sigma\sqrt{N}\cdot u,\qquad u\sim \mathrm{Unif}(\mathbb S^{N-1}(1)).
\end{equation}
As a consequence, the RF transport direction $r^\star \propto (x_1-x_0)$ is not guaranteed to be \emph{outward} with respect to the shell: depending on the relative radii and the random orientation, the velocity can point from a point on (or near) the shell toward the interior (i.e., it can have a negative radial component with respect to $x_0$). In this regime, a direction-only parameterization becomes ill-posed: knowing only a unit direction $r$ from a point $x_0$ on a thin shell does not uniquely identify the intended endpoint $x_1$ on (approximately) the same shell, because the line $x_0+\Delta r$ intersects the shell at (typically) two locations and the physically correct choice depends on the (unknown) step size/magnitude. 

\subsubsection{Dimension-stable Radius Schedule and Contraction/Expansion Phases}
\label{sec:orf_radius_schedule}

A central ingredient of ORF is a deterministic radius schedule $\rho(t)$ that approximates $\|x_t\|_2$ in high dimensions. Expanding \eqref{eq:orf_lerp_bridge} and using the thin-shell concentration property gives
\begin{align}
\|x_t\|_2^2
&=\|(1-t)x_0+t x_1\|_2^2 \nonumber\\
&=(1-t)^2\|x_0\|_2^2+t^2\|x_1\|_2^2+2t(1-t)\langle x_0,x_1\rangle\\
&\approx R^2\big(a^2(1-t)^2+t^2\big)\;\triangleq\;\rho(t)^2.
\label{eq:xt_norm_exact}
\end{align}
The schedule $\rho(t)$ is \emph{non-monotone}: it first shrinks and then expands. It is easy to see that the minimum-radius time is
\begin{equation}
t_{\min}=\frac{a^2}{1+a^2},
\label{eq:tmin}
\end{equation}
so we call $t\in[0,t_{\min}]$ the \emph{contraction phase} and $t\in[t_{\min},1]$ the \emph{expansion phase}.

\subsubsection{Radius Locking Inference for ORF}
\label{sec:orf_step}

Unlike standard RF or SFM inference-phase samplers, which typically rely on a pre-specified step-size schedule schedule on the constant-speed velocity field to advance the state, ORF does \emph{not} assume an explicit step-size schedule. Instead, ORF uses a time schedule $t_0<t_1<\cdots<t_K$ together with the \emph{radius schedule $\rho(t)$} (Sec.~\ref{sec:orf_radius_schedule}) to \emph{dynamically compute} the step size at each iteration. Concretely, at step $k$ we choose the scalar step size $\Delta_{t_k}$ so that the updated state lands exactly on the target radius prescribed by $\rho(t_{k+1})$. This systematically mitigates the step-size underestimation problem in standard $v$-prediction RF framework.

Let $x_{t_k}$ denote the current state at time $t_k$ and let $\hat r_{t_k}=\hat r(x_{t_k},t_k,c)\in\mathbb{S}^{N-1}(1)$ be the predicted ray. We update
\begin{equation}
x_{t_{k+1}} = x_{t_k} + \Delta_{t_k}\,\hat r_{t_k},
\label{eq:orf_update}
\end{equation}
and enforce the radius-locking constraint
\begin{equation}
\|x_{t_{k+1}}\|_2 = \rho(t_{k+1}).
\label{eq:radius_lock}
\end{equation}
Squaring \eqref{eq:radius_lock} and expanding yields a quadratic equation in $\Delta_{t_k}$:
\begin{align}
\|x_{t_k}+\Delta_{t_k}\hat r_{t_k}\|_2^2
&=\|x_{t_k}\|_2^2+\Delta_{t_k}^2+2\Delta_{t_k}\langle x_{t_k},\hat r_{t_k}\rangle \nonumber\\
&=\rho(t_{k+1})^2,
\end{align}
i.e.,
\begin{equation}
\Delta_{t_k}^2 + 2\langle x_{t_k},\hat r_{t_k}\rangle\,\Delta_{t_k}
+ \big(\|x_{t_k}\|_2^2-\rho(t_{k+1})^2\big)=0.
\label{eq:delta_quadratic}
\end{equation}

Let $c_k=\langle x_{t_k},\hat r_{t_k}\rangle$ and define the target radius increment
\begin{equation}
\Delta\rho_k^2 \;=\; \rho(t_{k+1})^2-\rho(t_k)^2.
\end{equation}
since $\|x_{t_k}\|_2=\rho(t_k)$ under the radius schedule, we obtain the two roots of \eqref{eq:delta_quadratic}
\begin{equation}
\Delta_{t_k} = -c_k \pm \sqrt{c_k^2+\Delta\rho_k^2}.
\label{eq:orf_two_roots}
\end{equation}

\subsubsection{Ill-defined Contraction Regime and Training-Inference Mismatch}
\label{sec:orf_ill_defined}

During the expansion phase, $c_k^2+\Delta\rho_k^2$ is always positive and the valid root becomes $\Delta_{t_k} = -c_k + \sqrt{c_k^2+\Delta\rho_k^2}$. However, the contraction phase of the radius schedule is intrinsically problematic for ray-based radius locking: $c_k^2+\Delta\rho_k^2$ is not guaranteed to be nonnegative, and the resulting fallback introduces a biased update that is not reflected in the training distribution:
\begin{enumerate}
\item \textbf{Feasible contraction ($c_k^2+\Delta\rho_k^2\ge 0$).}
There exist two real roots, both having the same sign. The physically consistent update is the negative root (moving against the radial component of $\hat r_{t_k}$):
\begin{equation}
\Delta_{t_k} = -c_k - \sqrt{c_k^2+\Delta\rho_k^2}.
\end{equation}

\item \textbf{Infeasible contraction ($c_k^2+\Delta\rho_k^2<0$).}
No real step size can reach the target smaller radius along the straight-ray update
$x_{t_{k+1}}=x_{t_k}+\Delta_{t_k}\hat r_{t_k}$.
Geometrically, along a fixed ray direction $\hat r_{t_k}$ the \emph{minimal achievable radius} is attained at
\begin{equation}
\Delta_{t_k}^{\min}=-c_k,\qquad c_k=\langle x_{t_k},\hat r_{t_k}\rangle,
\end{equation}
which yields the closest point to the origin on the ray,
\begin{equation}
x_{t_{k+1}}^\ast = x_{t_k}+\Delta_{t_k}^{\min}\hat r_{t_k},
\qquad
\langle x_{t_{k+1}}^\ast,\hat r_{t_k}\rangle=0.
\end{equation}
When $c_k^2+\Delta\rho_k^2<0$, the target radius $\rho(t_{k+1})$ is smaller than $\|x_{t_{k+1}}^\ast\|_2$, hence the radius-locking constraint is infeasible along the ray and a \emph{retraction} operator is required to map $x_{t_{k+1}}^\ast$ to the target radius. A natural idea is to retract $x_{t_{k+1}}^\ast$ to the target radius by moving along some auxiliary direction $q_{t_k}\in\mathbb{S}^{N-1}(1)$ (e.g., a correction direction). This would take the form
\begin{equation}
x_{t_{k+1}} = x_{t_{k+1}}^\ast + \lambda_{t_k}\,q_{t_k},
\qquad
\|x_{t_{k+1}}\|_2=\rho(t_{k+1}).
\label{eq:orf_aux_retract_form}
\end{equation}
However, \eqref{eq:orf_aux_retract_form} is itself not always solvable for the same reason as \eqref{eq:delta_quadratic}. Therefore, replacing the ray update by an auxiliary direction does not theoretically eliminate infeasibility; it merely shifts the feasibility condition to a different direction. To define a universally feasible retraction operator for \emph{all} nonzero $x_{t_{k+1}}^\ast$, we can simply take the radial normalization operator:
\begin{equation}
R^{\mathrm{ORF}}_{\rho'}(x_{t_{k+1}})
=
\rho(t_{k+1})\mathrm{Norm}_1(x_{t_{k+1}}^\ast).
\label{eq:orf_radial_retract}
\end{equation}
This mapping is always well-defined and enforces $\|x_{t_{k+1}}\|_2=\rho(t_{k+1})$ by construction. Crucially, in the infeasible contraction case the retraction direction defined by the radial normalization operator is \emph{necessarily orthogonal} to the predicted ray. Indeed, by definition of $x_{t_{k+1}}^\ast$ we have $\langle x_{t_{k+1}}^\ast,\hat r_{t_k}\rangle=0$, hence
\begin{equation}
\left\langle \frac{x_{t_{k+1}}^\ast}{\|x_{t_{k+1}}^\ast\|_2},\ \hat r_{t_k}\right\rangle = 0,
\qquad\Rightarrow\qquad
\angle\!\left(\frac{x_{t_{k+1}}^\ast}{\|x_{t_{k+1}}^\ast\|_2},\hat r_{t_k}\right)=\frac{\pi}{2}.
\label{eq:orf_retract_orthogonal}
\end{equation}
That is, whenever the radius-locking equation is infeasible and we fall back to the closest point $x_{t_{k+1}}^\ast$ followed by radial normalization, the retraction introduces an update component that is \emph{maximally misaligned} with the model-predicted ray. This geometric mismatch is intrinsic to the infeasible contraction regime: it does not depend on the particular choice of model or training objective, but follows directly from the ray geometry and the requirement to hit a smaller target radius.

This issue is particularly severe in settings where a single network predicts rays for multiple inputs $\{\hat r_{t_k}\}_{k=0}^{K-1}$: within the same forward pass, some inputs may satisfy $c_k^2+\Delta\rho_k^2\ge 0$ (unbiased, exact radius-locking), while others satisfy $c_k^2+\Delta\rho_k^2<0$ (biased, retracted update). This creates a sharp training--inference mismatch: during training, the model is supervised on oracle bridge states $x_{t_k}$ constructed from the ground-truth pair $(x_0,x_1)$, so every $x_{t_k}$ lies exactly on the intended bridge distribution. At inference time, however, the sampler produces states that are a mixture of (i) exact updates and (ii) biased retracted updates, and the latter can move the trajectory off the oracle bridge in a time-dependent manner. Since later predictions $\hat r_{t_{k'}}$ are conditioned on these perturbed states, the mismatch compounds across steps and can be strongly amplified in the subsequent expansion phase.
\end{enumerate}

\subsection{Spoon Flow: Two-Phase Spherical Transport}
\label{subsec:spoon_flow}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.9\textwidth]{figs/flow.pdf}
    \caption{Illustration for the bridges in (A) Spherical flow matching, (B) Outward ray flow, and (C) Spoon flow.}
    \label{fig:flows}
\end{figure}

The above analysis suggests that SFM and ORF fail in complementary time regimes. ORF is well-behaved in the large-$t$ expansion regime where radius locking is always feasible, but becomes ill-defined and biased in the small-$t$ contraction regime due to infeasible radius-locking and retraction-induced distortion (Sec.~\ref{sec:orf_ill_defined}). In contrast, SFM has no ``step-size infeasibility'' issue at small $t$ because it evolves on a fixed-radius sphere, but it is prone to a self-bootstrapping shortcut at large $t$ (Sec.~\ref{subsec:sfm_baseline}). A natural idea is therefore to \emph{use different flows in different time intervals}: we use SFM in the early-time regime and ORF in the late-time regime. The resulting trajectory first follows an arc on the inner sphere and then follows an outward ray toward the outer sphere, forming a spoon-like shape; we call this two-phase flow \textbf{Spoon Flow}.

\subsubsection{Phase Boundary from the Non-expanding Interval and the SNR-balanced Point}
\label{sec:spoon_boundary}

Recall the ORF radius schedule $\rho(t)$ attains its minimum at $t_{\min}=\frac{a^2}{1+a^2}$. We define the \emph{non-expanding interval} as
\begin{equation}
t\in[0,\,2t_{\min}],
\end{equation}
since $\rho(t)$ decreases on $[0,t_{\min}]$ and increases on $[t_{\min},2t_{\min}]$, and moreover
\begin{equation}
\rho(2t_{\min})=\rho(0)=aR.
\end{equation}
Hence the bridge state at $t=2t_{\min}$ lies again on the inner sphere radius $aR$ (in expectation / concentration), making it a natural switching point: SFM maps $x_0$ to $x_{2t_{\min}}$ on the inner-sphere through a slerp bridge, and ORF expands $x_{2t_{\min}}$ to $x_1$ through a lerp bridge. Since $x_{2t_{\min}}$ may not be strictly located on the inner-sphere, we project it to the inner-sphere for a well-defined SFM formulation
\begin{equation}
\bar x_{2t_{\min}} = \mathrm{Norm}_{\mathrm{aR}}(x_{2t_{\min}}).
\end{equation}

To decide a proper choice of $a$ under this problem formulation, we define a signal-to-noise (SNR) proxy by comparing the target contribution $t\|x_1\|_2$ to the source contribution $(1-t)\|x_0\|_2$:
\begin{equation}
\mathrm{SNR}(t)\;\triangleq\;\log\frac{t\|x_1\|_2}{(1-t)\|x_0\|_2}
=\log\frac{t}{a(1-t)}.
\end{equation}
The equal-contribution (SNR-balanced) time is defined by $\mathrm{SNR}(t_{\mathrm{eq}})=0$, which leads to
\begin{equation}
t_{\mathrm{eq}} \;\triangleq\; \frac{a}{1+a}.
\label{eq:teq_def}
\end{equation}

We set the phase switching point to be the time where \emph{$x_1$ starts to dominate}, so the late-time dynamics should be driven primarily by the target direction. This requires
\begin{equation}
t_{\mathrm{eq}} = 2t_{\min},
\end{equation}
which yields a closed-form choice of the inner radius ratio:
\begin{equation}
\frac{a}{1+a}=\frac{2a^2}{1+a^2}
\quad\Longrightarrow\quad
a=\sqrt{2}-1.
\label{eq:a_spoon}
\end{equation}

\subsubsection{Radian Locking Inference for SFM}
\label{sec:sfm_radian_locking}

We show that a \emph{radian locking} inference can also be designed for the SFM phase similar to the radius locking inference in ORF, which allows us to also perform direction-only parameterization during SFM training. We first characterize the typical angular distance between $x_0$ and the phase boundary $\bar x_{2t_{\min}}=\bar x_{t_{\mathrm{eq}}}$. Since radial projection preserves direction, the SFM endpoint angle
\begin{equation}
\omega \;\triangleq\; \angle(x_0,\bar x_{t_{\mathrm{eq}}})
\end{equation}
satisfies
\begin{equation}
\cos\omega
=
\frac{\langle x_0,\bar x_{t_{\mathrm{eq}}}\rangle}{\|x_0\|_2\,\|\bar x_{t_{\mathrm{eq}}}\|_2}
=
\frac{\langle x_0,x_{t_{\mathrm{eq}}}\rangle}{\|x_0\|_2\,\|x_{t_{\mathrm{eq}}}\|_2}.
\end{equation}
Under the thin-shell concentration property, we obtain
\begin{align}
\langle x_0,x_{t_{\mathrm{eq}}}\rangle
&=
\langle x_0,(1-t_{\mathrm{eq}})x_0+t_{\mathrm{eq}}x_1\rangle
\approx (1-t_{\mathrm{eq}})\|x_0\|_2^2
=(1-t_{\mathrm{eq}})a^2R^2,
\\
\|x_{t_{\mathrm{eq}}}\|_2^2
&=
\|(1-t_{\mathrm{eq}})x_0+t_{\mathrm{eq}}x_1\|_2^2
\approx (1-t_{\mathrm{eq}})^2\|x_0\|_2^2+t_{\mathrm{eq}}^2\|x_1\|_2^2
=R^2\big(a^2(1-t_{\mathrm{eq}})^2+t_{\mathrm{eq}}^2\big).
\end{align}
Substituting $t_{\mathrm{eq}}=\frac{a}{1+a}$ yields
\begin{equation}
\cos\omega \approx \frac{\frac{a}{1+a}}{\frac{a\sqrt{2}}{1+a}} = \frac{1}{\sqrt2},
\qquad
\Rightarrow\quad
\omega_{\mathrm{typ}}\approx \frac{\pi}{4}.
\label{eq:sfm_omega_typ}
\end{equation}
Thus the total SFM phase geodesic arc-length $L=(aR)\omega$ is approximately constant across samples. We can thus parameterize SFM training and inference in a same way as ORF: we predict only a unit tangent direction and recover the step size by enforcing a scalar \emph{radian schedule}, analogous to ORF's radius schedule.

\paragraph{Direction-constrained radian locking.}
With \eqref{eq:sfm_omega_typ}, we prescribe the deterministic radian schedule
\begin{equation}
\alpha(t)=t\,\omega_{\mathrm{tot}},
\qquad \omega_{\mathrm{tot}}=\omega_{\mathrm{typ}}\approx \frac{\pi}{4}.
\label{eq:sfm_alpha_schedule}
\end{equation}

Let $0=t_0<t_1<\cdots<t_{K_1}=1$ be the SFM phase time grid and denote $\alpha_k=\alpha(t_k)$. At step $k$, the model predicts a unit tangent direction
$\hat u_k \in T_{x_k}\mathbb{S}^{N-1}(aR)$, and we choose an angular step $\eta_k\ge 0$ along $\hat u_k$ and update by the exponential map on $\mathbb{S}^{N-1}(aR)$:
\begin{equation}
x_{k+1}=x_k(\eta_k,\,\hat u_k)
\triangleq
\mathrm{Exp}_{x_k}\!\big((aR)\eta_k\,\hat u_k\big)
=
\cos\eta_k\,x_k+\sin\eta_k\,(aR)\hat u_k,
\label{eq:sfm_exp_update_eta}
\end{equation}
where $\eta_k$ is an \emph{angular} step (radians) and the corresponding arc-length is $(aR)\eta_k$.
Radian locking enforces the progress constraint
\begin{equation}
\angle\big(x_k(\eta_k,\,\hat u_k),x_0\big)=\alpha_{k+1}
\quad\Longleftrightarrow\quad
\frac{\langle x_k(\eta_k,\,\hat u_k),x_0\rangle}{(aR)^2}=\cos\alpha_{k+1}.
\label{eq:sfm_angle_lock_constraint}
\end{equation}
Define the scalars
\begin{equation}
A_k=\frac{\langle x_k,x_0\rangle}{(aR)^2}=\cos\alpha_k,
\qquad
B_k=\frac{\langle \hat u_k,x_0\rangle}{aR}.
\end{equation}
Substituting \eqref{eq:sfm_exp_update_eta} into \eqref{eq:sfm_angle_lock_constraint} yields a 1D trigonometric equation for $\eta_k$:
\begin{equation}
A_k\cos\eta_k + B_k\sin\eta_k = \cos\alpha_{k+1}.
\label{eq:sfm_eta_equation}
\end{equation}
Let $R_k=\sqrt{A_k^2+B_k^2}$, $\phi_k=\mathrm{atan2}(B_k,A_k)$ and $\gamma_k=\arccos(\frac{\cos\alpha_{k+1}}{R_k})$. Since
$A_k\cos\eta + B_k\sin\eta = R_k\cos(\eta-\phi_k)$, the two solution branches of \eqref{eq:sfm_eta_equation} are
\begin{equation}
\eta_k^{(\pm)}=\phi_k \pm \gamma_k.
\label{eq:sfm_two_branches}
\end{equation}

Eq.~\eqref{eq:sfm_eta_equation} is feasible iff $
|\cos\alpha_{k+1}|\le R_k$. Similar to ORF, we thus need to discuss the update and retraction operators in feasible and infeasible updates, respectively:
\begin{enumerate}
\item \textbf{Feasible radian locking ($|\cos\alpha_{k+1}|\le R_k$).}
In this case, \eqref{eq:sfm_eta_equation} admits real solutions. The two candidates \eqref{eq:sfm_two_branches} correspond to the two intersections of the geodesic ray (parameterized by $\eta_k$) with the target latitude constraint. We select the \emph{smallest forward rotation} (the minimal nonnegative angular step) to avoid unnecessary wrap-around:
\begin{equation}
\bar\eta_k^{(\pm)}=\mathrm{wrap}_{[0,2\pi)}\!\big(\eta_k^{(\pm)}\big),
\qquad
\eta_k=\min\{\bar\eta_k^{(+)},\bar\eta_k^{(-)}\},
\label{eq:sfm_eta_select}
\end{equation}
where $\mathrm{wrap}_{[0,2\pi)}(\theta)=\theta-2\pi\left\lfloor \theta/(2\pi)\right\rfloor$.
We then update by:
\begin{equation}
\tilde x_{k+1}=x_k(\eta_k,\,\hat u_k)=\mathrm{Exp}_{x_k}\!\big((aR)\eta_k\,\hat u_k\big),
\qquad
x_{k+1}=\tilde x_{k+1}.
\label{eq:sfm_feasible_update}
\end{equation}

\item \textbf{Infeasible radian locking ($|\cos\alpha_{k+1}|> R_k$).}
In this case, the target latitude cannot be reached by moving along the single predicted direction $\hat u_k$. Following the same logic as ORF' retraction operator, we first take the step size that achieves the maximal progress attainable along $\hat u_k$, i.e., the smallest achievable inner product with $x_0$:
\begin{equation}
\eta_k^{\max}=\phi_k+\pi,
\qquad
\hat x_{k+1}=x_k(\eta_k^{\max},\,\hat u_k)
=\mathrm{Exp}_{x_k}\!\big((aR)\eta_k^{\max}\hat u_k\big),
\label{eq:sfm_extremal_step}
\end{equation}
which yields
\begin{equation}
A_k\cos\eta_k^{\max}+B_k\sin\eta_k^{\max}
=
R_k\cos(\eta_k^{\max}-\phi_k)
=
R_k\cos\pi
=
-R_k.
\end{equation}
We then apply an always-feasible \emph{radian retraction operator}, similar to the radius retraction operator in ORF, to enforce the target progress angle:
\begin{equation}
\tilde x_{k+1}=\mathcal R^{\mathrm{SFM}}_{\alpha_{k+1}}(\hat x_{k+1})
\;\triangleq\;
(aR)\Big(\cos\alpha_{k+1}\,\hat x_0+\sin\alpha_{k+1}\,\hat p\Big),
\label{eq:sfm_infeasible_retract}
\end{equation}
where $\hat x_0=\mathrm{Norm}_\mathrm{1}(x_0)$, $\hat z_{k+1}=\mathrm{Norm}_\mathrm{1}(\hat x_{k+1})$, and $\hat p=\mathrm{Norm}_\mathrm{1}(\hat z_{k+1}-\langle \hat z_{k+1},\hat x_0\rangle \hat x_0)$.

Recall that the ORF retraction operator $\mathcal R^{\mathrm{ORF}}_{\rho}(\cdot)$ defines a correction direction that is \emph{strictly orthogonal to the actual ray $\hat r$}. In SFM, $\mathcal R^{\mathrm{SFM}}_{\alpha}$ induces a correction direction of
\begin{equation}
d_{\mathrm{ret}}^{\mathrm{SFM}}
\;\triangleq\;
\tilde x_{k+1}-\hat x_{k+1},
\label{eq:sfm_ret_dir_def}
\end{equation}
Since $\hat u_k$ is a tangent direction at $x_k$ instead of $\hat x_{k+1}$ or $\tilde x_{k+1}$, there is no geometric constraint forcing $d_{\mathrm{ret}}^{\mathrm{SFM}}$ to be orthogonal to $\hat u_k$. Therefore, unlike ORF where infeasible-step retraction introduces a strictly orthogonal correction, the SFM latitude retraction is \emph{not} forced to be orthogonal to the predicted direction and is typically a much milder correction.
\end{enumerate}

\subsubsection{Bridge Construction for the Two Phases}
\label{sec:spoon_training}

Spoon flow uses the same final target token $x_1\in\mathbb{S}^{N-1}(R)$ in both phases, but defines \emph{different} start/endpoints and bridges for the SFM phase and the ORF phase. Here we specifies the training distributions and the corresponding bridge constructions.

\begin{enumerate}
\item \textbf{Phase I (SFM): start/endpoints and slerp bridge on the inner sphere}

We sample the SFM starting point on the inner sphere
\begin{equation}
x_0 \sim \mathrm{Unif}\big(\mathbb{S}^{N-1}(aR)\big),
\qquad a=\sqrt{2}-1.
\end{equation}

With $\bar x_{t_{\mathrm{eq}}}\triangleq\mathrm{Norm}_\mathrm{aR}(x_{t_{\mathrm{eq}}})$ as the end point, we define the phase I slerp bridge as 
\begin{equation}
x_t^{\mathrm{sfm}}
\;=\;
\mathrm{slerp}\!\left(x_0,\bar x_{t_{\mathrm{eq}}};t\right),
\qquad t\in[0,1],
\label{eq:spoon_sfm_bridge}
\end{equation}
and trains a direction-only tangent ray field.

\item \textbf{Phase II (ORF): start/endpoints and lerp bridge in the expansion regime}

To reduce training--inference mismatch at the phase boundary, we sample the ORF starting point from the same geometric locus produced by phase I radian locking schedule. We already know that during inference, radian locking schedule in phase I SFM enforces $\angle(x_{1}^{\mathrm{sfm}},x_0)\approx \omega_{\mathrm{tot}}=\frac{\pi}{4}$, so we sample $x_0^{\mathrm{orf}}$ on the latitude which is $\omega_{\mathrm{tot}}$ away from $x_0$:
\begin{equation}
\mathcal C_{\omega}(x_0)
=
\Big\{z\in\mathbb{S}^{N-1}(aR):\ \angle(z,x_0)=\omega_{\mathrm{tot}}\Big\}.
\end{equation} 
The latitude can be parameterized as:
\begin{equation}
\hat z(\psi)
=
\cos\omega_{\mathrm{tot}}\,\frac{x_0}{aR}
+
\sin\omega_{\mathrm{tot}}\big(\cos\psi\,e+\sin\psi\,w\big),
\qquad
x_0^{\mathrm{orf}}(\psi)=aR\hat z(\psi).
\label{eq:latitude_param}
\end{equation}
where $e$ is the unit tangent direction at $x_0$ pointing toward $\bar x_{t_{\mathrm{eq}}}$ and $w\in T_{x_0}\mathbb{S}^{N-1}(1)$ is a random unit vector such that $w\perp e$.

Moreover, along the phase I slerp geometry between $x_0$ and $\bar x_{t_{\mathrm{eq}}}$, the geodesic midpoint corresponds to equal progress from both endpoints. We further restrict the ORF starting point to the target-side half by requiring
\begin{equation}
\angle(x_0^{\mathrm{orf}},\bar x_{t_{\mathrm{eq}}}) \le \angle(x_0^{\mathrm{orf}},x_0)=\omega_{\mathrm{tot}},
\label{eq:target_side_constraint}
\end{equation}
i.e., $x_0^{\mathrm{orf}}$ is at least as close to $\bar x_{t_{\mathrm{eq}}}$ as it is to $x_0$. 
This constraint is equivalent to a simple bound on $\psi$: writing $\bar x_{t_{\mathrm{eq}}}=(aR)\big(\cos\omega_{\mathrm{tot}}\, \frac{x_0}{aR}+\sin\omega_{\mathrm{tot}}\,e\big)$ and using $w\perp \bar x_{t_{\mathrm{eq}}}$, we obtain
\begin{equation}
\langle x_0^{\mathrm{orf}}(\psi),\bar x_{t_{\mathrm{eq}}}\rangle
=
(aR)^2\big(\cos^2\omega_{\mathrm{tot}}+\sin^2\omega_{\mathrm{tot}}\cos\psi\big).
\end{equation}
Thus $\angle(x_0^{\mathrm{orf}},\bar x_{t_{\mathrm{eq}}})\le \omega_{\mathrm{tot}}$ is equivalent to
\begin{equation}
\cos^2\omega_{\mathrm{tot}}+\sin^2\omega_{\mathrm{tot}}\cos\psi \geq \cos\omega_{\mathrm{tot}}
\end{equation}
which can be simplified to
\begin{equation}
\cos\psi \ge \frac{\cos\omega_{\mathrm{tot}}\,(1-\cos\omega_{\mathrm{tot}})}{\sin^2\omega_{\mathrm{tot}}}=\frac{\cos\omega_{\mathrm{tot}}}{1+\cos\omega_{\mathrm{tot}}}.
\label{eq:psi_tau}
\end{equation}
With $\omega_{\mathrm{tot}}\approx \frac{\pi}{4}$, we further simplify it into a sample-independent estimation
\begin{equation}
\cos\psi \geq \frac{1/\sqrt2}{1+1/\sqrt2}=\frac{1}{\sqrt2+1}=\sqrt2-1=a,
\end{equation}
where we find it coincides with the inner-sphere radius $a$. The sampling of $x_0^{\mathrm{orf}}$ can thus be summarized as
\begin{equation}
\psi \sim \mathrm{Unif}(0,\arccos(a)),
\qquad
x_0^{\mathrm{orf}}
=
\cos\omega_{\mathrm{tot}}\,x_0
+
aR\sin\omega_{\mathrm{tot}}\big(\cos\psi\,e+\sin\psi\,w\big).
\label{eq:psi_sampling}
\end{equation}
\end{enumerate}

The overall training and inference procedure is summarized in Algorithm~\ref{alg:spoon_flow}.

\begin{algorithm}[!ht]
\caption{Spoon Flow: training and inference}
\label{alg:spoon_flow}
\DontPrintSemicolon
\KwIn{Token dimension $N$, conditioning $c$, radius schedule $\rho(t)$, radian schedule $\alpha(t)$, $R=\sqrt{N}$, $a=\sqrt2-1$, $t_{\mathrm{eq}}=\frac{a}{1+a}$, $\omega_{\mathrm{tot}}=\pi/4$}
\KwOut{final token $x_{t=1}\in\mathbb{S}^{N-1}(R)$}

\BlankLine
\textbf{Training}\;
\Indp
Sample target token $x_1\in\mathbb{S}^{N-1}(R)$\;
Sample $x_0\sim\mathrm{Unif}(\mathbb{S}^{N-1}(aR))$\;
Compute $x_{t_{\mathrm{eq}}}=(1-t_{\mathrm{eq}})x_0+t_{\mathrm{eq}}x_1$ and $\bar x_{t_{\mathrm{eq}}}=\mathrm{Norm}_\mathrm{aR}(x_{t_{\mathrm{eq}}})$\;

\BlankLine
\textit{Phase I (SFM)}\;
\Indp
Sample $t\sim\mathrm{Unif}(0,1)$ and set $x_t^{\mathrm{sfm}}=\mathrm{slerp}(x_0,\bar x_{t_{\mathrm{eq}}};t)$\;
Set target ray $v_t^\star=\mathrm{Norm}_1(\mathrm{Log}_{x_t^{\mathrm{sfm}}}(\bar x_{t_{\mathrm{eq}}}))$\;
Predict $\hat v_t=\mathrm{Norm}_1(\hat v(x_t^{\mathrm{sfm}},t,c))\in T_{x_t^{\mathrm{sfm}}}\mathbb{S}^{N-1}(aR)$\;
Backpropagate by minimizing
$L_{\mathrm{SFM}}=1-\cos(\hat v_t,v_t^\star)$\;
\Indm

\BlankLine
\textit{Phase II (ORF)}\;
\Indp
Calculate $e$ as the unit tangent direction at $x_0$ pointing toward $\bar x_{t_{\mathrm{eq}}}$\;
Sample $\psi\sim\mathrm{Unif}(0,\arccos(a))$ and sample $w\in T_{ x_0}\mathbb{S}^{N-1}(1)$ with $w\perp e$\;
Set ORF start $x_0^{\mathrm{orf}}=\cos\omega_{\mathrm{tot}}\,x_0+aR\sin\omega_{\mathrm{tot}}\big(\cos\psi\,e+\sin\psi\,w\big)\Big)$\;
Sample $s\sim\mathrm{Unif}(0,1)$ and set $x_s^{\mathrm{orf}}=(1-s)x_0^{\mathrm{orf}}+sx_1$\;
Set target ray $r^\star=\mathrm{Norm}_1(x_1-x_0^{\mathrm{orf}})$\;
Predict $\hat r_s=\mathrm{Norm}_1(\hat r(x_s^{\mathrm{orf}},s,c)$)\;
Backpropagate by minimizing $L_{\mathrm{ORF}}=1-\cos(\hat r_s,r^\star)$\;
\Indm
\Indm

\BlankLine
\textbf{Inference}\;
\Indp
Sample $x_0\sim\mathrm{Unif}(\mathbb{S}^{N-1}(aR))$\;

\BlankLine
\textit{Phase I (SFM sampling)}\;
\Indp
Choose a time grid $0=t_0<t_1<\cdots<t_{K_1}=1$\;
Sample $x_{t_0} \sim \mathrm{Unif}(\mathbb{S}^{N-1}(aR))$\;
\For{$k\leftarrow 0$ \KwTo $K_1-1$}{
  Predict unconditional and conditional rays
  $\hat v_{\varnothing}\leftarrow \hat v(x_{t_k},t_k,\varnothing)$,
  $\hat v_c\leftarrow \hat v(x_{t_k},t_k,c)$\;
  Apply CFG on rays and normalize:
  $\hat v_{\mathrm{cfg}}\leftarrow \mathrm{Norm}_1(\hat v_{\varnothing}+w_{\mathrm{cfg}}^{\mathrm{sfm}}(\hat v_c-\hat v_{\varnothing}))$\;
  Compute $\eta_{t_k}$ for radian $\alpha(s_{k+1})$ \;
  Update and (optionally) retract:
  $x_{t_{k+1}}\leftarrow R^{\mathrm{SFM}}_{\alpha_{k+1}}(x_{t_k}(\eta_{t_k},\,\hat v_{\mathrm{cfg}}))$\;
}
\Indm

\BlankLine
\textit{Phase II (ORF sampling)}\;
\Indp
Choose a time grid $0=s_0<s_1<\cdots<s_{K_2}=1$\;
Set $x_{s_0} = x_{t_{K_1}}$\;
\For{$k\leftarrow 0$ \KwTo $K_2-1$}{
  Predict unconditional and conditional rays
  $\hat r_{\varnothing}\leftarrow \hat r(x_{s_k},s_k,\varnothing)$,
  $\hat r_c\leftarrow \hat r(x_{s_k},s_k,c)$\;
  Apply CFG on rays and normalize:
  $\bar r_{\mathrm{cfg}}\leftarrow \mathrm{Norm}_1(\hat r_{\varnothing}+w_{\mathrm{cfg}}^{\mathrm{orf}}(\hat r_c-\hat r_{\varnothing}))$\;
  Compute $\Delta_{s_k}$ for radius $\rho(s_{k+1})$ \;
  Update: $x_{s_{k+1}} = x_{s_k} + \Delta_{s_k}\hat r_{\mathrm{cfg}}$\;
}
\Indm

\Return{$x_{t=1}$}\;
\Indm
\end{algorithm}

\subsection{Discussion: Basin Overlap and Posterior Broadening at the Mixture Endpoint}
\label{subsec:spoon_discussion}

We provide a quantitative explanation for why phase I SFM in Spoon Flow is less prone to self-bootstrapping than a single-stage SFM model targeting a data-token endpoint. The key mechanism is \emph{posterior broadening}: at the SNR-balanced mixture endpoint, decoder basins corresponding to different data tokens necessarily overlap under mild regularity assumptions, so basin membership no longer identifies a unique final token.

Recall that in Sec.~\ref{subsec:sfm_baseline} we defined the basin of a data token as $\mathcal{B}_\epsilon(x_1)
\;\triangleq\;
\Big\{z\in\mathbb{S}^{N-1}(R):\ d_\phi\big(D(z),D(x_1)\big)\le \epsilon\Big\}$ (Eq.~\ref{eq:basin_def}). We assume:
\begin{enumerate}
\item \textbf{(Local Lipschitz)} There exists $L>0$ such that for all $u,v$ in the neighborhood of interest,
\begin{equation}
d_\phi(D(u),D(v))\le L\|u-v\|_2.
\label{eq:lip_disc}
\end{equation}
\item \textbf{(Data-token separation)} There exists $\Delta_{\min}>0$ such that for any two distinct data tokens $x_1\neq x_1'$ on the outer shell,
\begin{equation}
d_\phi(D(x_1),D(x_1'))\ge \Delta_{\min}.
\label{eq:sep_disc}
\end{equation}
\end{enumerate}
Both quantities can be estimated empirically (e.g., by finite differences for $L$ and by a low quantile of pairwise distances for $\Delta_{\min}$). If $\epsilon<\Delta_{\min}/2$, then for any $x_1\neq x_1'$,
\begin{equation}
\mathcal B_\epsilon(x_1)\cap \mathcal B_\epsilon(x_1')=\emptyset.
\label{eq:disjoint_disc}
\end{equation}
Indeed, if $z$ belonged to both basins, then by the triangle inequality,
$d_\phi(D(x_1),D(x_1'))\le d_\phi(D(x_1),D(z))+d_\phi(D(z),D(x_1'))\le 2\epsilon<\Delta_{\min}$, contradicting \eqref{eq:sep_disc}.
Thus, once a trajectory enters $\mathcal B_\epsilon(x_1)$, the endpoint is effectively identified, enabling the self-bootstrapping shortcut in single-stage SFM.

In the phase I SFM in Spoon flow, we fix a start point $x_0$ and consider the SNR-balanced mixture map $G_{x_0}(x_1)\;\triangleq\;(1-t_{\mathrm{eq}})x_0+t_{\mathrm{eq}}x_1$. For any two data tokens $x_1,x_1'$,
\begin{equation}
\|G_{x_0}(x_1)-G_{x_0}(x_1')\|_2
=
t_{\mathrm{eq}}\|x_1-x_1'\|_2.
\label{eq:mix_contract_disc}
\end{equation}
Thus, distinct endpoints on the outer shell are mapped to much closer points at the mixture time. By the Lipschitz assumption \eqref{eq:lip_disc}, the Euclidean ball of radius $r=\epsilon/L$ around any point is contained in its basin:
\begin{equation}
\|z-y\|_2\le \frac{\epsilon}{L}
\quad\Longrightarrow\quad
z\in\mathcal B_\epsilon(y).
\label{eq:ball_in_basin_disc}
\end{equation}
Now let $y=G_{x_0}(x_1)$ and $y'=G_{x_0}(x_1')$. If $\|y-y'\|_2\le 2r$, then the two balls $B(y,r)$ and $B(y',r)$ intersect, hence
\begin{equation}
\mathcal B_\epsilon(y)\cap \mathcal B_\epsilon(y')\ \supseteq\ B(y,r)\cap B(y',r)\ \neq\ \emptyset.
\label{eq:overlap_nonempty_disc}
\end{equation}
Using \eqref{eq:mix_contract_disc}, a sufficient condition for nonempty overlap is
\begin{equation}
t_{\mathrm{eq}}\|x_1-x_1'\|_2 \le \frac{2\epsilon}{L}.
\label{eq:overlap_condition_disc}
\end{equation}
Moreover, when \eqref{eq:overlap_condition_disc} holds, the intersection contains a ball centered at the midpoint $(y+y')/2$ with radius at least
\begin{equation}
r_{\cap}\ \ge\ r-\frac{\|y-y'\|_2}{2}
\ =\ \frac{\epsilon}{L}-\frac{t_{\mathrm{eq}}}{2}\|x_1-x_1'\|_2.
\label{eq:overlap_radius_disc}
\end{equation}
Therefore, unlike the data-token case \eqref{eq:disjoint_disc}, mixture endpoints corresponding to different data tokens can have \emph{overlapping} basins for the same $\epsilon$.

\paragraph{Implication.} Basin overlap implies that membership in $\mathcal B_\epsilon(G_{x_0}(x_1))$ does not uniquely identify $x_1$: there exist states $z$ that are simultaneously $\epsilon$-close (in decoded semantics) to multiple mixture endpoints. Consequently, the conditional distribution over final data tokens given an intermediate state remains broader, and the model has a stronger incentive to use the conditioning signal $c$ to resolve ambiguity. his reduces the self-bootstrapping shortcut that arises when the endpoint basins are disjoint and sharply identify a unique $x_1$.

==> sections_old/tokenizer.tex <==
\section{Hierarchical Spherical Tokenization}
\label{sec:tokenizer}

We present a tokenizer design built around a simple geometric principle: in a high-dimensional continuous token space, the most natural representation geometry is spherical, and once the radial degree of freedom is removed, useful structure should be encoded through \emph{direction} together with a \emph{controlled hierarchy of group-wise energies}. This leads to a token space that is simultaneously reconstruction-oriented, generative-friendly, and geometrically aligned with a spherical denoising bridge.

The section is organized as follows. We first motivate fixed-norm spherical tokens from high-dimensional concentration and normalized embedding geometry. We then introduce a group-wise energy hierarchy on the token sphere and show how it creates an explicit distinction between random spherical states and structured data tokens. Based on this structure, we analyze how spherical perturbations affect different groups, and show that the resulting perturbation hierarchy naturally induces an importance-ordered decomposition of information. We next explain why the reconstruction-stable region that should be learned by the tokenizer decoder should be shaped by a \emph{hierarchy-preserving} perturbation model, and derive a product-sphere noise construction that preserves the predefined group energies while perturbing only the group-wise directions. Finally, we instantiate the resulting tokenizer with a minimalist cross-modal architecture.

\subsection{From High-Dimensional Latents to Fixed-Norm Spherical Tokens}
\label{subsec:tok_sphere_motivation}

Let $z\in\mathbb R^N$ denote a continuous token. A standard starting point for continuous latent modeling is the isotropic Gaussian distribution
\begin{equation}
z \sim \mathcal N(0,\sigma^2 I_N).
\end{equation}
In high dimension, such a distribution is already concentrated near a sphere. Indeed,
\begin{equation}
\frac{\|z\|_2^2}{\sigma^2} \sim \chi^2_N,
\end{equation}
hence
\begin{equation}
\mathbb E[\|z\|_2^2] = N\sigma^2,
\qquad
\mathrm{Var}(\|z\|_2^2)=2N\sigma^4.
\end{equation}
Therefore the relative fluctuation of the squared norm is
\begin{equation}
\frac{\sqrt{\mathrm{Var}(\|z\|_2^2)}}{\mathbb E[\|z\|_2^2]}
=
\sqrt{\frac{2}{N}},
\end{equation}
which vanishes as $N\to\infty$. Equivalently, the norm itself concentrates sharply around
\begin{equation}
\|z\|_2 \approx \sigma\sqrt N.
\end{equation}
Thus, in high dimension, an isotropic Gaussian latent already behaves like a \emph{thin-shell spherical latent}: most of its probability mass lies near a sphere of essentially fixed radius.

This observation motivates removing the radial degree of freedom explicitly and representing each token directly on a hypersphere. Throughout this section, we set the token radius to
\begin{equation}
R = \sqrt N
\end{equation}
and constrain every token to lie on
\begin{equation}
\mathbb S^{N-1}(R)
=
\{z\in\mathbb R^N:\|z\|_2=R\}.
\end{equation}
Accordingly, the tokenizer encoder $E$ maps an input signal $x$ to
\begin{equation}
z = E(x)\in \mathbb S^{N-1}(R).
\end{equation}

This choice has two direct advantages. First, it matches the effective geometry already induced by high-dimensional Gaussian latents. Second, it aligns naturally with normalized representation spaces widely used in modern embedding models, where angular structure is the primary similarity geometry. Once the radius is fixed, the geometry of the token space is governed entirely by direction:
\begin{equation}
\cos(z_1,z_2)
=
\frac{\langle z_1,z_2\rangle}{R^2},
\qquad
z_1,z_2\in\mathbb S^{N-1}(R).
\end{equation}
This makes spherical interpolation, angular perturbation, and geodesic transport the canonical operations in the token space.

\subsection{Why a Spherical Token Should Not Be Energy-Uniform}
\label{subsec:tok_hierarchy_motivation}

A fixed-norm spherical token removes global magnitude, but does not by itself distinguish a structured data token from a random spherical vector. To make the token space useful for generation, the data manifold should differ from a random spherical state not only in direction, but also in its \emph{internal organization}. We achieve this by imposing a group-wise energy hierarchy.

\paragraph{Group partition.}
We partition the $N$ token dimensions into $G$ disjoint groups of equal size
\begin{equation}
N = GH,
\end{equation}
where $H$ is the dimensionality of each group. Writing
\begin{equation}
z = [z_1,\dots,z_G],
\qquad
z_g\in\mathbb R^H,
\end{equation}
we define the group energy by
\begin{equation}
\|z_g\|_2 = r_g.
\end{equation}
Since the whole token lies on $\mathbb S^{N-1}(R)$ with $R=\sqrt N$, the group energies must satisfy
\begin{equation}
\sum_{g=1}^G r_g^2 = N.
\label{eq:group_energy_budget}
\end{equation}

\paragraph{Random spherical states are energy-equalized.}
The role of the group hierarchy is best understood by comparing a data token with a random spherical vector. Let
\begin{equation}
u \sim \mathrm{Unif}\big(\mathbb S^{N-1}(R)\big).
\end{equation}
By rotational symmetry, each group carries the same expected energy:
\begin{equation}
\mathbb E[\|u_g\|_2^2] = \frac{H}{N}R^2 = H.
\label{eq:random_group_energy_mean}
\end{equation}
Moreover, concentration implies that in high dimension the fluctuations around this value are small. One convenient way to see this is to represent
\begin{equation}
u = R \frac{\xi}{\|\xi\|_2},
\qquad
\xi\sim\mathcal N(0,I_N).
\end{equation}
Then
\begin{equation}
\|u_g\|_2^2
=
R^2\frac{\|\xi_g\|_2^2}{\|\xi\|_2^2},
\end{equation}
where $\|\xi_g\|_2^2\sim\chi^2_H$ and $\|\xi\|_2^2\sim\chi^2_N$. Since both concentrate around their means $H$ and $N$, respectively, we obtain the high-dimensional approximation
\begin{equation}
\|u_g\|_2^2 \approx H
\qquad
\text{for all } g.
\label{eq:random_group_energy_concentrate}
\end{equation}
Therefore a random spherical state is characterized, at the level of group energies, by an \emph{approximately equalized energy profile}. This equalized state is also the maximum-entropy configuration compatible with the global norm constraint and the chosen group partition.

The data token should not collapse to this random-like configuration. Instead, it should exhibit a structured, non-uniform group-energy profile. Intuitively, such a profile makes the data manifold distinguishable from a random spherical source state, so that a denoising bridge can be interpreted not merely as a change in direction, but as a progressive transition from a more random, energy-equalized state to a more structured, hierarchically organized state.

\subsection{A Fixed Group-Energy Hierarchy}
\label{subsec:tok_fixed_hierarchy}

We now impose an explicit group-wise energy hierarchy on every token. The groups are ordered from high to low energy, and their energies are prescribed in closed form.

\paragraph{Design requirements.}
The group-energy sequence $\{r_g^2\}_{g=1}^G$ is designed to satisfy three properties:
\begin{enumerate}[leftmargin=2em,label=(\roman*)]
\item the total energy is fixed:
\begin{equation}
\sum_{g=1}^G r_g^2 = N;
\end{equation}
\item the energies decay monotonically with group index;
\item the decay is linear in dB scale, so that the hierarchy is multiplicative rather than additive.
\end{enumerate}

Let
\begin{equation}
r_g^2 = A q^{g-1},
\qquad
g=1,\dots,G,
\label{eq:geom_energy_form}
\end{equation}
with $0<q\le 1$. Then
\begin{equation}
10\log_{10}(r_g^2)
=
10\log_{10}A + 10(g-1)\log_{10}q,
\end{equation}
which is linear in the group index on the dB scale.

To determine the decay uniquely from the group count, we set the ratio between the largest and smallest group energies to
\begin{equation}
\frac{r_1^2}{r_G^2} = G^2.
\label{eq:max_min_energy_ratio}
\end{equation}
Equivalently, the largest and smallest group norms differ by a factor of $G$:
\begin{equation}
\frac{r_1}{r_G}=G.
\end{equation}
This choice yields a hierarchy whose total dynamic range grows with the number of groups while remaining fully determined by $G$. In dB scale, the total range becomes
\begin{equation}
10\log_{10}\frac{r_1^2}{r_G^2}
=
20\log_{10}G.
\end{equation}

Combining \eqref{eq:geom_energy_form} and \eqref{eq:max_min_energy_ratio}, we obtain
\begin{equation}
q^{-(G-1)} = G^2
\qquad\Longrightarrow\qquad
q = G^{-2/(G-1)}.
\label{eq:q_closed_form}
\end{equation}
The total energy constraint \eqref{eq:group_energy_budget} then gives
\begin{equation}
A \sum_{g=0}^{G-1} q^g = N
\qquad\Longrightarrow\qquad
A = N\frac{1-q}{1-q^G}.
\label{eq:A_closed_form}
\end{equation}
Hence the group-energy hierarchy is
\begin{equation}
\boxed{
r_g^2
=
N\frac{1-q}{1-q^G}\,q^{g-1},
\qquad
q = G^{-2/(G-1)}.
}
\label{eq:rg_closed_form}
\end{equation}

This hierarchy provides a fixed energy scaffold for the token space. A token is still a point on the full sphere $\mathbb S^{N-1}(\sqrt N)$, but its energy is not free to distribute arbitrarily across dimensions: it is organized across groups according to the prescribed profile \eqref{eq:rg_closed_form}. Consequently, the data manifold becomes a product-of-spheres structure embedded inside the ambient sphere:
\begin{equation}
z_g \in \mathbb S^{H-1}(r_g),
\qquad
g=1,\dots,G.
\end{equation}
The encoder is thus encouraged to allocate information across a hierarchy of groups with different prescribed stabilities and capacities.

\subsection{How Spherical Perturbations Act on the Group Hierarchy}
\label{subsec:tok_rotation_effect}

The group-energy hierarchy is meaningful only if spherical perturbations affect different groups differently. This is exactly what happens under high-dimensional spherical rotation.

Let $z\in\mathbb S^{N-1}(\sqrt N)$ be a token with group energies $\|z_g\|_2=r_g$. A full-dimensional spherical perturbation of angle $\theta$ is given by
\begin{equation}
\tilde z
=
\cos\theta\, z
+
\sqrt N \sin\theta\, u,
\label{eq:full_sphere_perturb}
\end{equation}
where
\begin{equation}
u \in T_z \mathbb S^{N-1}(\sqrt N),
\qquad
\|u\|_2=1.
\end{equation}
By construction, $\tilde z$ remains on the sphere and satisfies
\begin{equation}
\angle(z,\tilde z)=\theta.
\end{equation}

Writing the perturbation group-wise,
\begin{equation}
\tilde z_g
=
\cos\theta\, z_g
+
\sqrt N \sin\theta\, u_g,
\end{equation}
we can quantify how strongly each group is perturbed.

\paragraph{Expected group energy after rotation.}
Expanding the squared norm gives
\begin{equation}
\|\tilde z_g\|_2^2
=
\cos^2\theta\,\|z_g\|_2^2
+
N\sin^2\theta\,\|u_g\|_2^2
+
2\sqrt N\sin\theta\cos\theta\,\langle z_g,u_g\rangle.
\end{equation}
In high dimension, tangent-space isotropy implies
\begin{equation}
\mathbb E\|u_g\|_2^2 \approx \frac{H}{N},
\qquad
\mathbb E\langle z_g,u_g\rangle \approx 0,
\end{equation}
hence
\begin{equation}
\boxed{
\mathbb E\|\tilde z_g\|_2^2
\approx
r_g^2\cos^2\theta + H\sin^2\theta.
}
\label{eq:rotated_group_energy_general}
\end{equation}
This formula shows that spherical rotation gradually pulls each group energy toward the random-spherical equilibrium value $H$. In particular, for $\theta=\pi/4$,
\begin{equation}
\mathbb E\|\tilde z_g\|_2^2
\approx
\frac{r_g^2+H}{2},
\label{eq:rotated_group_energy_45}
\end{equation}
so a $45^\circ$ perturbation moves every group halfway toward energy equalization. Therefore, spherical randomization can be interpreted as an entropy-increasing operation that progressively erases the hierarchical energy pattern of the data token.

\paragraph{Effective local perturbation angle in each group.}
The same full-dimensional rotation angle does not affect all groups equally. To quantify this, we compare the perturbation energy injected into each group with its clean group norm. Since
\begin{equation}
\sqrt N \sin\theta\, \|u_g\|_2
\approx
\sqrt H \sin\theta
\end{equation}
in high dimension, the effective local perturbation angle $\phi_g$ in group $g$ satisfies
\begin{equation}
\tan \phi_g
\approx
\frac{\sqrt H \sin\theta}{r_g \cos\theta}
=
\frac{\sqrt H}{r_g}\tan\theta.
\end{equation}
Equivalently,
\begin{equation}
\boxed{
\phi_g(\theta)
=
\arctan\!\left(\frac{\sqrt H}{r_g}\tan\theta\right).
}
\label{eq:phi_g_from_theta}
\end{equation}
Thus, for a fixed full-dimensional perturbation angle $\theta$, groups with larger energy $r_g$ experience smaller effective local rotation angles. This induces a natural perturbation hierarchy:
\begin{itemize}
\item high-energy groups are perturbed mildly and remain relatively stable;
\item low-energy groups are perturbed more strongly and are therefore less stable.
\end{itemize}

This property is central. Once reconstruction training is performed under spherical perturbation, the encoder-decoder pair is encouraged to place information unevenly across groups: components that matter more for reconstruction are more efficiently stored in groups whose effective perturbation angles are smaller, while less critical details can be assigned to more strongly perturbed groups. In this way, the group-energy hierarchy induces an automatic decomposition of information according to reconstruction importance.

\subsection{Why the Tokenizer Noise Should Preserve the Group Energies}
\label{subsec:tok_product_sphere_noise_motivation}

The preceding analysis shows that a full-dimensional spherical rotation simultaneously changes two things:
\begin{enumerate}[leftmargin=2em,label=(\arabic*)]
\item the \emph{direction} inside each group;
\item the \emph{energy profile} across groups.
\end{enumerate}
For a tokenizer, these two effects play very different roles.

The decoder should be robust to local directional inconsistencies around a token, because such inconsistencies naturally arise from imperfect generation. However, requiring the decoder to remain equally robust under large group-energy drift is unnecessary and undesirable. The reason is geometric: if the decoder is explicitly trained to reconstruct from tokens whose group energies have already been pulled substantially toward the random-spherical equilibrium, then the resulting reconstruction-stable region around each token becomes too large in the ambient sphere. Under a spherical denoising bridge, this makes a long final segment of the trajectory effectively reconstruction-trivial, since many nearby bridge states already fall inside the same stable region.

For the tokenizer, the desired notion of local robustness is therefore the following:
\begin{quote}
\emph{The decoder should be robust to local directional perturbations around a token while preserving the predefined group-energy hierarchy.}
\end{quote}
This leads naturally to a product-sphere perturbation model.

\subsection{Hierarchy-Preserving Product-Sphere Noise}
\label{subsec:tok_product_sphere_noise}

We now construct a perturbation process that preserves the group energies exactly and perturbs only the group-wise directions. Let
\begin{equation}
z = [z_1,\dots,z_G],
\qquad
z_g\in \mathbb S^{H-1}(r_g).
\end{equation}
For each group, we sample a unit tangent vector
\begin{equation}
u_g \in T_{z_g}\mathbb S^{H-1}(r_g),
\qquad
\|u_g\|_2 = 1,
\end{equation}
and apply a geodesic rotation of angle $\phi_g$:
\begin{equation}
\tilde z_g
=
\cos\phi_g\, z_g
+
r_g \sin\phi_g\, u_g.
\label{eq:group_sphere_noise}
\end{equation}
Since $u_g\perp z_g$, this preserves the group norm exactly:
\begin{equation}
\|\tilde z_g\|_2 = r_g.
\end{equation}
Applying this independently to all groups yields a perturbed token
\begin{equation}
\tilde z = [\tilde z_1,\dots,\tilde z_G]
\end{equation}
that remains on the product manifold
\begin{equation}
\tilde z_g \in \mathbb S^{H-1}(r_g),
\qquad
g=1,\dots,G.
\end{equation}

\paragraph{Choosing the group-wise angles.}
The local angles should respect the hierarchy induced by the full-dimensional spherical geometry. Equation~\eqref{eq:phi_g_from_theta} shows how a full-dimensional perturbation of angle $\theta$ would be perceived in each group. This suggests a natural transfer principle: the tokenizer perturbation should preserve the same \emph{relative} cross-group perturbation ordering as full-dimensional rotation, but should do so while keeping the group energies fixed.

A convenient way to parameterize this is to choose a maximum perturbation angle for the lowest-energy group, denoted by $\phi_G^{\max}$, and derive the other groups by preserving the scaling of local perturbation strength. Since local perturbation strength is proportional to $\tan\phi_g$, and from \eqref{eq:phi_g_from_theta} we have $\tan\phi_g\propto 1/r_g$, we set
\begin{equation}
\tan\phi_g
=
\frac{r_G}{r_g}\tan\phi_G.
\end{equation}
Equivalently,
\begin{equation}
\boxed{
\phi_g
=
\arctan\!\left(\frac{r_G}{r_g}\tan\phi_G\right).
}
\label{eq:phi_g_from_phiG}
\end{equation}
This ensures that lower-energy groups are perturbed more strongly and higher-energy groups more mildly, while preserving every group norm exactly.

\paragraph{Why the maximum angle is set at \(45^\circ\).}
We use
\begin{equation}
\phi_G^{\max} = \frac{\pi}{4}.
\end{equation}
This choice has two geometric interpretations. First, in high dimension, adding a standard Gaussian perturbation to a vector typically induces an angular deviation of roughly $45^\circ$ after normalization, making $\pi/4$ a natural reference scale for substantial but not destructive perturbation. Second, two unrelated high-dimensional spherical vectors are concentrated near $90^\circ$ apart. If one wishes the reconstruction-stable regions associated with the most important group not to overlap substantially across unrelated tokens, then a natural upper limit for the local stable radius is half of this typical unrelated angle, namely $90^\circ/2=45^\circ$.

To bias training toward moderate perturbations while still occasionally exposing the decoder to near-maximal perturbations, we sample
\begin{equation}
\phi_G
=
\frac{\pi}{4}\cdot \mathrm{Beta}(1,2),
\label{eq:phiG_sampling}
\end{equation}
and then determine the remaining group angles through \eqref{eq:phi_g_from_phiG}. Since $\mathrm{Beta}(1,2)$ concentrates near zero, most perturbations remain local, while the tail still provides meaningful coverage of the intended stability region.

\subsection{Tokenizer Objective and Representation Parameterization}
\label{subsec:tok_objective_and_param}

The tokenizer encoder first produces a free hidden representation
\begin{equation}
h = [h_1,\dots,h_G],
\qquad
h_g\in\mathbb R^H.
\end{equation}
Each group is normalized to unit direction and then scaled to the predefined group norm:
\begin{equation}
u_g = \frac{h_g}{\|h_g\|_2+\varepsilon},
\qquad
z_g = r_g\,u_g.
\label{eq:group_token_param}
\end{equation}
By construction,
\begin{equation}
\|z_g\|_2 = r_g,
\qquad
\sum_{g=1}^G \|z_g\|_2^2 = \sum_{g=1}^G r_g^2 = N,
\end{equation}
so the full token automatically lies on $\mathbb S^{N-1}(\sqrt N)$ while also satisfying the prescribed product-sphere structure.

Given a perturbed token $\tilde z$ sampled via \eqref{eq:group_sphere_noise}, the decoder $D$ reconstructs the input:
\begin{equation}
\hat x = D(\tilde z).
\end{equation}
The tokenizer is then trained with a reconstruction objective
\begin{equation}
L_{\mathrm{tok}} = L_{\mathrm{rec}}(x,\hat x) + \lambda_{\mathrm{GAN}}L_{\mathrm{GAN}},
\end{equation}
where the adversarial term is optional and used only as a perceptual realism prior. The essential part of the tokenizer design is not the choice of the signal-space reconstruction loss itself, but the geometry of the perturbation process under which the decoder is required to reconstruct reliably.

\subsection{Interpretation: Automatic Importance-Ordered Decomposition}
\label{subsec:tok_interpretation}

The resulting tokenizer has a clear geometric interpretation.

\paragraph{Structured data manifold versus random spherical state.}
A random spherical vector has, in expectation and with high probability, approximately equalized group energies \eqref{eq:random_group_energy_concentrate}. By contrast, a data token produced by the tokenizer has a predefined non-uniform group-energy hierarchy \eqref{eq:rg_closed_form}. Therefore the data manifold is separated from a random-like spherical state not only by direction, but also by internal energy organization.

\paragraph{Reconstruction importance is aligned with perturbation stability.}
Since higher-energy groups undergo smaller effective local perturbations under the spherical geometry, the encoder is encouraged to place reconstruction-critical information in those groups. Conversely, details that can tolerate stronger perturbation may be assigned to lower-energy groups. This produces an importance-ordered decomposition of information inside the token.

\paragraph{A coarse-to-fine structure is built into the token space.}
The hierarchy induces a natural ordering from stable, high-energy groups to unstable, low-energy groups. In many continuous signal domains, low-frequency or coarse structure contributes more to signal energy and to reconstruction quality than high-frequency detail. The proposed token space does not hard-code any particular frequency assignment, but it provides exactly the geometric bias needed for such a decomposition to emerge automatically under reconstruction training.

\subsection{A Minimalist Cross-Modal Architecture}
\label{subsec:tok_architecture}

The geometric construction above is compatible with a wide range of architectures. For concreteness and cross-modal consistency, we adopt a minimalist tokenizer design that separates local signal compression from global token-space reconstruction.

\paragraph{Encoder.}
Given an input signal $x$ (e.g., a 1D waveform segment, a 2D image, or a higher-dimensional continuous tensor), the encoder first extracts local features on the native signal grid and compresses them into a low-rate token tensor:
\begin{equation}
h = f_{\mathrm{enc}}^{\mathrm{conv}}(x),
\qquad
\bar h = \mathrm{Linear}_{\downarrow}(h).
\end{equation}
The compressed representation is then reshaped into token groups and converted into a product-sphere token via \eqref{eq:group_token_param}.

\paragraph{Decoder.}
The decoder takes either a clean token or a hierarchy-preserving perturbed token $\tilde z$, first mixes information across tokens, and then maps the representation back to the native signal domain:
\begin{equation}
\tilde h = g_{\mathrm{dec}}^{\mathrm{mix}}(\tilde z),
\qquad
\bar x = \mathrm{Linear}_{\uparrow}(\tilde h),
\qquad
\hat x = f_{\mathrm{dec}}^{\mathrm{conv}}(\bar x).
\end{equation}
The role of $g_{\mathrm{dec}}^{\mathrm{mix}}$ is particularly important: because the decoder is trained under group-wise directional perturbations, this module learns to reconcile local token inconsistencies before signal-level reconstruction.

\paragraph{Optional separable transform front-end.}
For continuous signals with strong local frequency structure, a separable $N$-D transform front-end such as MDCT may be applied before the neural encoder. This provides a structured local coefficient grid and can improve the inductive bias of the tokenizer. The geometric formulation of the token space, however, is independent of whether such a front-end is used.

\subsection{Summary}
\label{subsec:tok_summary}

The tokenizer introduced in this section is defined by three coupled design choices:
\begin{enumerate}[leftmargin=2em,label=(\arabic*)]
\item \textbf{Fixed-norm spherical tokens:}
the token space is a high-dimensional sphere, reflecting the thin-shell geometry of high-dimensional continuous latents.

\item \textbf{A predefined group-energy hierarchy:}
the token is partitioned into equal-dimensional groups with closed-form energies \eqref{eq:rg_closed_form}, making the data manifold structurally distinct from a random spherical state.

\item \textbf{Hierarchy-preserving product-sphere perturbation:}
tokenizer robustness is trained by rotating each group on its own sphere according to \eqref{eq:group_sphere_noise} and \eqref{eq:phi_g_from_phiG}, so that the decoder learns directional robustness without collapsing the group-energy hierarchy.
\end{enumerate}

Together, these ingredients create a token space in which information is organized along a stability hierarchy, random spherical states are geometrically distinguishable from structured data tokens, and the induced coarse-to-fine structure is naturally aligned with spherical denoising bridges used by the generative model.

==> sections_old/tokenizer_old.tex <==
\section{Spherical Tokenizer}
\label{sec:tokenizer}

We propose a spherical tokenizer that maps each input instance (e.g., an image or an audio segment) into a set of fixed-norm continuous tokens lying on a hypersphere \cite{davidson2018hyperspherical, ke2025hyperspherical}. By constraining each token to have a fixed radius, the representation geometry is governed by \emph{direction} rather than \emph{magnitude}. Beyond introducing a hyperspherical latent space, we train the tokenizer to be \emph{generative-friendly}: the decoder should remain stable under structured perturbations that resemble typical generation errors, and the token space should be regular and traversable rather than brittle or folded. To this end, we combine geometry-respecting geodesic noise injection in both the high-dimensional token space and an auxiliary low-dimensional spherical manifold with explicit manifold-shaping constraints. In particular, we introduce a low-dimensional spherical projection together with a learnable lift, and train this pathway with a spherical commitment objective and a conformal regularizer to promote a well-structured high-dimensional token space. Finally, we present a minimalist design paradigm that is shared across modalities.

\subsection{Spherical Latent Space}
Let $N$ denote the token dimensionality and let $R=\sqrt{N}$. We constrain each token to lie on the $(N-1)$-sphere of radius $R$:
\begin{align}
\mathbb{S}^{N-1}(R) \;=\; \{ z \in \mathbb{R}^N : \|z\|_2 = R \}.
\end{align}
Given an input $x$, the encoder $E(\cdot)$ produces spherical tokens
\begin{align}
z = E(x) \in \mathbb{S}^{N-1}(R),
\end{align}
and a decoder $D(\cdot)$ maps (possibly perturbed) tokens back to the input domain, yielding a reconstruction $\hat{x}=D(z)$.

\paragraph{Angular similarity.}
For $z_1,z_2\in\mathbb{S}^{N-1}(R)$, cosine similarity reduces to a scaled inner product:
\begin{align}
\cos(z_1,z_2) \;=\; \frac{\langle z_1,z_2\rangle}{\|z_1\|_2\|z_2\|_2}
\;=\; \frac{\langle z_1,z_2\rangle}{R^2}.
\end{align}
We use cosine similarity (equivalently angular distance) as the primary geometric primitive throughout the tokenizer objectives.

\subsection{Encoder-Side Low-Dimensional Spherical Manifold Regularizer}
\label{sec:method_ld_sphere_regularizer}
While each high-dimensional token lies on a hypersphere, the geometry of the \emph{token distribution} can still be highly underdetermined. We therefore introduce an explicit low-dimensional spherical manifold that acts as an information bottleneck and a geometric regularizer to the high-dimensional token space.

\subsubsection{Fixed Random Spherical Projection and Learnable Lift}

We introduce a low-dimensional spherical space of dimension $d\ll N$ with radius $R_d=\sqrt{d}$. To connect this space to the high-dimensional token sphere, we use a random spherical projection $P$ together with a nonlinear lift $Q$:
\begin{equation}
P\in\mathbb{R}^{d\times N},\qquad Q:\mathbb{R}^{d}\rightarrow\mathbb{R}^{N},
\end{equation}
where $P$ is a \emph{fixed} row-orthonormal random projection (i.e., $PP^\top=I_d$) and $Q$ is a small \emph{learnable} MLP. Such random row-orthonormal projections are known to act as near-isometries on finite sets and low-dimensional subspaces with high probability under the Johnson--Lindenstrauss lemma \cite{larsen2017optimality}, approximately preserving pairwise distances and inner products.

Given a high-dimensional token $z$, we first compute its low-dimensional spherical code by
\begin{equation}
y \;=\; \mathrm{Norm}_{R_d}(Pz)
\;\triangleq\;
R_d\,\frac{Pz}{\|Pz\|_2}
\;\in\;
\mathbb{S}^{d-1}(R_d),
\label{eq:ld_code}
\end{equation}
and then lift it back to the high-dimensional sphere by
\begin{equation}
\hat z \;=\; \mathrm{Norm}_{R}\!\big(Q(y)\big)
\;\in\;
\mathbb{S}^{N-1}(R).
\label{eq:hd_recon_from_ld}
\end{equation}

\paragraph{\textbf{Spherical commitment.}}
To encourage $z$ to remain close to the low-dimensional manifold while keeping the lift learnable, we use a VQ-VAE-style bidirectional commitment objective on the sphere \cite{van2017neural}:
\begin{equation}
L_{\mathrm{commit}}
=
\big(1-\cos(z,\mathrm{stopgrad}(\hat z))\big)
+
\big(1-\cos(\mathrm{stopgrad}(z),\hat z)\big),
\label{eq:commit_spherical}
\end{equation}
where $\mathrm{stopgrad}(\cdot)$ blocks gradients. 

\paragraph{\textbf{Conformal regularization for geometry transfer.}}
\label{sec:conformal}
The low-dimensional manifold is useful as a geometric prior only if its local neighborhood structure is preserved after lifting. To encourage this, we impose a local conformality constraint on the lift $Q$, so that nearby points on the low-dimensional sphere remain nearby in the lifted high-dimensional space rather than being folded or distorted. For a low-dimensional token $y$, we sample two local perturbations $y_1,y_2$ via a geodesic noise injection mechanism (which will be described in Sec.~\ref{sec:noise_inject}). We then define $\tilde z_i = Q(y_i),\, i\in\{1,2\}$ and penalize angular distortion:
\begin{equation}
L_{\mathrm{conf}}
=
\Big|
\mathrm{stopgrad}\big(\cos(y_1,y_2)\big)
-
\cos(\tilde z_1,\tilde z_2)
\Big|_1.
\label{eq:conf_loss}
\end{equation}
We backpropagate this loss only through $Q$, without directly updating the tokenizer encoder.

This design allows the low-dimensional sphere to act as a geometric reference for the lifted high-dimensional manifold. Since $L_{\mathrm{conf}}$ encourages local angular relations in the low-dimensional space to be preserved by $Q$, the lifted tokens $\hat z$ are encouraged to inherit the local neighborhood structure of their low-dimensional codes $y$. The commitment objective in Eq.~\eqref{eq:commit_spherical} then provides the optimization path that transfers this structure to the encoder tokens themselves: because the encoder output $z$ is trained to remain close to its lifted reconstruction $\hat z$, the high-dimensional token space is gradually pulled toward a liftable geometry whose local neighborhoods are consistent with those of the low-dimensional spherical manifold. In this way, the low-dimensional manifold serves not merely as a compressed coordinate system, but as an explicit geometric scaffold that shapes the organization of the high-dimensional token space.

\subsubsection{Low-Dimensional Spherical Noise and Reconstruction Training}

We further regularize the low-dimensional manifold by injecting \emph{strong} geodesic noise in the low-dimensional spherical space, thereby creating an information bottleneck. Similar in spirit to the variational posterior noise and the strengthened KL regularization in $\beta$-VAEs \cite{higgins2017betavae}, this perturbation increases overlap between nearby codes and discourages the model from encoding brittle, high-frequency information in $y$. As a result, the low-dimensional manifold is encouraged to become more ``semantic'', ``clustered'', and ``traversable''. This yields a perturbed low-dimensional code $\tilde y$, which is then lifted and decoded:
\begin{equation}
\tilde z_{\mathrm{ld}} = \mathrm{Norm}_{R}(Q\tilde y)\in\mathbb{S}^{N-1}(R), \quad \hat x_{\mathrm{ld}} = D(\tilde z_{\mathrm{ld}}).
\end{equation}

\subsection{Riemannian Noise Injection via Tangent-Space Sampling}
\label{sec:noise_inject}
The perturbations introduced above should respect the geodesic geometry of the hyperspherical token space. A natural way is to perform noise injection by sampling in the tangent space and mapping back to the sphere via the exponential map. For $z\in\mathbb{S}^{N-1}(R)$, the tangent space is
\begin{align}
T_z\mathbb{S}^{N-1}(R) \;=\; \{ u\in\mathbb{R}^N : \langle u,z\rangle = 0 \}.
\end{align}
We sample a random unit tangent direction $u$ such that $\|u\|_2=1$ and $u\perp z$. Given a rotation angle $\theta\in[0,\theta_{\max}]$, we define the perturbed token by exponential map (geodesic rotation):
\begin{align}
\tilde{z} \;=\; \mathrm{Exp}_z(R\theta\,u)
\;=\; \cos(\theta)\,z \;+\; R\sin(\theta)\,u.
\label{eq:exp_map}
\end{align}
By construction, $\|\tilde{z}\|_2=R$ and the geodesic angle satisfies $\angle(z,\tilde{z})=\theta$. 

\paragraph{\textbf{Noise injection in high-dimensional and low-dimensional spaces.}} Noise injection in the high-dimensional and low-dimensional spherical spaces serves different purposes, and the corresponding strength and sampling distributions should therefore differ. In the high-dimensional token space, noise injection is mainly used to improve decoder robustness against generator-typical errors and to create local \emph{reconstruction-stable basins} around each token. In the low-dimensional spherical space, by contrast, noise injection acts primarily as an information bottleneck that shapes the manifold itself. Together with the lift-only conformal regularization and the spherical commitment objective introduced in Sec.~\ref{sec:method_ld_sphere_regularizer}, strong low-dimensional perturbations encourage nearby codes to overlap, suppress brittle local encoding patterns, and induce a smoother and more clustered geometry. Through the lift $Q$ and the commitment path from $\hat z$ back to the encoder token $z$, this low-dimensional neighborhood structure is gradually transferred to the high-dimensional token space.

These two effects should not dominate each other. The low-dimensional branch is intended to define the semantic geometry, while the high-dimensional branch should only train local decoder robustness around that geometry. If the high-dimensional perturbation is made too strong, the model can instead respond by separating tokens more aggressively on the high-dimensional sphere in order to maintain reconstruction stability under large perturbations. Since the low-dimensional manifold is simultaneously encouraged to remain locally compact and traversable, overly strong high-dimensional perturbations would counteract the geometry-smoothing effect induced by the low-dimensional branch. To this end, we use different sampling strategies in the two spaces:
\begin{itemize}
    \item \textbf{Low-dimensional space.} We use a large maximum perturbation angle while biasing perturbations toward small rotations:
    \begin{align}
    \theta_{\mathrm{LD}} \;=\; \frac{\pi}{2}\cdot \mathrm{Beta}(1,2).
    \label{eq:theta_ld}
    \end{align}
    Since $\pi/2$ corresponds to the angle of uncorrelated codes, we use it as the largest perturbation radius that still avoids pushing the noisy code beyond the regime of nonnegative correlation with the clean one. This allows the low-dimensional branch to impose the strongest possible bottleneck without making optimization unnecessarily unstable. At the same time, the $\mathrm{Beta}(1,2)$ distribution concentrates more mass near small angles, so most perturbations remain local while occasional larger perturbations still encourage substantial neighborhood overlap and manifold smoothing. Under this choice, the average low-dimensional perturbation angle is
    \begin{align}
    \mathbb{E}[\theta_{\mathrm{LD}}]
    \;=\;
    \frac{\pi}{2}\cdot \frac{1}{1+2}
    \;=\;
    \frac{\pi}{6}.
    \end{align}
    We treat this average angle heuristically as the \emph{radius of a low-dimensional semantic basin}: after training with such perturbations, information within this angular scale is encouraged to remain semantically similar and locally traversable on the low-dimensional spherical manifold.

    \item \textbf{High-dimensional space.} In the high-dimensional token space, we define the perturbation range relative to this low-dimensional semantic scale. Specifically, we use a mild maximum perturbation angle and sample uniformly within this range:
    \begin{align}
    \theta_{\mathrm{HD}} \;=\; \frac{\pi}{6}\cdot \mathcal{U}(0,1).
    \label{eq:theta_hd}
    \end{align}
    This choice defines a local \emph{reconstruction-stable basin}: the decoder is trained to remain approximately uniformly robust to perturbations throughout the entire angular range $[0,\pi/6]$ around each token. By matching the maximum high-dimensional perturbation angle to the characteristic radius of the low-dimensional semantic basin, we keep the high-dimensional robustness objective local relative to the geometry imposed by the low-dimensional manifold. In this way, the high-dimensional branch trains decoder tolerance around the geometry defined by the low-dimensional branch, rather than competing with it by encouraging unnecessarily large token separations or excessive overlap between neighboring semantic basins.
\end{itemize}

When tokens form a set (e.g., a grid of tokens), sampling $\theta$ independently for each token causes the \emph{sample-level} average perturbation strength to concentrate tightly due to averaging across many tokens. To expose the decoder to a broader range of sample-level perturbation radii while keeping the \emph{marginal} per-token angle distribution unchanged, we use a mixture of independent-angle and shared-angle perturbations. Specifically, for each input instance we sample $s\sim\mathrm{Bernoulli}(p_{\mathrm{share}})$ (by default $p_{\mathrm{share}}=0.5$). If $s=1$, we sample a single angle and apply it to all tokens; if $s=0$, we sample angles independently for each token from the same distribution. In both cases, tangent directions $u$ are sampled independently for each token. This increases the diversity of sample-level perturbation strengths without changing the marginal angle distribution at the token level.

\subsection{Overall Tokenizer Objective}
\label{sec:tok_objective}

We train the tokenizer with a weighted sum of objectives, grouped into a high-dimensional (HD) part and a low-dimensional (LD) part:
\begin{equation}
\label{eq:tok_loss_full_grouped}
\begin{aligned}
L_{\mathrm{tok}}
=&\;\lambda_{\mathrm{rec}}^{\mathrm{hd}}L_{\mathrm{rec}}\!\big(x,D(\tilde z)\big)
&&\hfill \text{\footnotesize// HD: decoder robustness and spread-out control}
\\
&+\lambda_{\mathrm{rec}}^{\mathrm{ld}}L_{\mathrm{rec}}\!\big(x,D(\tilde z_{\mathrm{ld}})\big)
+\lambda_{\mathrm{conf}}L_{\mathrm{conf}}+\lambda_{\mathrm{commit}}L_{\mathrm{commit}}
&&\hfill \text{\footnotesize// LD: token-space shaping}
\\
&+\lambda_{\mathrm{GAN}}L_{\mathrm{GAN}}
&&\hfill \text{\footnotesize// Aux: perceptual realism enhancement}
\end{aligned}
\end{equation}

These terms play complementary roles:
\begin{itemize}
\item \textbf{HD group (}$L_{\mathrm{rec}}^{\mathrm{hd}}$\textbf{):}
enforces reconstruction-stable basins and improves decoder robustness to token perturbations.

\item \textbf{LD group (}$L_{\mathrm{rec}}^{\mathrm{ld}} + L_{\mathrm{commit}} + L_{\mathrm{conf}}$\textbf{):}
shapes the high-dimensional token space by constructing a liftable, generative-friendly low-dimensional spherical coordinate system with a strong information bottleneck.

\item \textbf{Auxiliary (}$L_{\mathrm{GAN}}$\textbf{):}
acts as a perceptual realism prior that complements pointwise reconstruction metrics.
\end{itemize}

\subsection{A Minimalist Model Architecture Design Paradigm}
\label{sec:tok_arch}

While the tokenizer objectives introduced above can be applied to a wide range of existing architectures, we also present a minimalist, modality-agnostic design paradigm for completeness and self-consistency. More importantly, this design illustrates that a tokenizer can achieve sufficiently strong reconstruction fidelity while remaining generation-friendly using only simple architectural components.

We adopt a simple asymmetric tokenizer architecture that separates local signal processing on the native grid from token-space decompression on the compressed representation. The encoder maps the input to a low-rate token tensor through a convolutional backbone followed by a single-step downsampling operator, while the decoder first performs token-space mixing and then maps the representation back to the native grid.

\paragraph{\textbf{Encoder.}}
The encoder consists of a convolutional backbone followed by a single-step downsampling operator:
\begin{equation}
h = f_{\mathrm{enc}}^{\mathrm{conv}}(x),
\qquad
\bar u = \text{Linear}_{\downarrow}(h),
\qquad
z=\mathrm{Norm}_{R}(\bar u)\in\mathbb{S}^{N-1}(R)^{\mathcal I},
\label{eq:enc_template}
\end{equation}
where $\mathcal I$ denotes the token index set (a sequence or a grid) and $N$ is the token dimensionality. Here $f_{\mathrm{enc}}^{\mathrm{conv}}$ first performs local and meso-scale feature extraction on the native signal grid, and $\text{Linear}_{\downarrow}(\cdot)$ then enforces the token budget by compressing the signal into a low-rate token representation.

\paragraph{\textbf{Decoder.}}
The decoder maps tokens back to the native signal grid by first reconciling token-level inconsistencies and then applying upsampling and convolutional refinement:
\begin{equation}
\tilde z = g_{\mathrm{dec}}^{\mathrm{mix}}(z_{\mathrm{in}}),
\qquad
\tilde h = \text{Linear}_{\uparrow}(\tilde z),
\qquad
\hat x = f_{\mathrm{dec}}^{\mathrm{conv}}(\tilde h),
\label{eq:dec_template}
\end{equation}
where $z_{\mathrm{in}}$ denotes either clean tokens or perturbed tokens (e.g., Sec.~\ref{sec:noise_inject}). Because token-level spherical perturbations are injected during tokenizer training, the role of $g_{\mathrm{dec}}^{\mathrm{mix}}$ is to improve noise-robust decompression by reconciling small token inconsistencies before convolutional refinement. Finally, $f_{\mathrm{dec}}^{\mathrm{conv}}$ maps the upsampled features back to the input domain.

\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\textwidth]{figs/tokenizer.pdf}
    \caption{Caption Tokenizer}
    \label{fig:tokenizer_design}
\end{figure}

\paragraph{\textbf{Example Instantiations Across Modalities.}}

We provide concrete architecture instantiations to illustrate how the above design principles can be realized in practice. Figure~\ref{fig:tokenizer_design} shows a modality-shared core pipeline together with representative instantiations for 1D and 2D signals.

For an $N$-dimensional continuous signal, we first map the raw input to a structured coefficient grid using a \emph{separable $N$-D modified discrete cosine transform (MDCT)}, implemented by applying 1-D MDCT along each axis. We use MDCT as a common front-end because DCT-style transform is a standard signal representation in practical continuous-signal compression systems (e.g., standard audio and image codecs \cite{rfc6716, wallace1991jpeg}), and because it provides a useful signal-level inductive bias before neural tokenization. In particular, the default 50\% overlap gives smooth transitions across neighboring windows or patches, while the frequency decomposition itself provides a structured local representation that is often easier to model than raw samples or pixels directly. The MDCT window/kernel size determines the native coefficient-grid resolution seen by the tokenizer: with kernel size $k$, the corresponding stride is $k/2$ along each axis. Different boundary padding schemes can also be applied for different modalities and tasks: for streaming-oriented settings such as audio, we use zero padding; for image generation where a single image is typically modeled non-autoregressively within the spatial extent, we use circular padding.

Since MDCT coefficients can exhibit substantially different magnitudes across frequency bands, with high-frequency components often having much lower energy than low-frequency ones, we further apply a simple signed dynamic-range compression before feeding the coefficients into the encoder:
\begin{equation}
x \;\leftarrow\; \operatorname{sign}(x)\,|x|^{1/3}.
\label{eq:mdct_compress}
\end{equation}
This transformation preserves coefficient sign while compressing amplitude range, reducing the tendency of the model to over-emphasize low-frequency components and underfit high-frequency details that are important for faithful reconstruction.

On top of this MDCT coefficient grid, we use a deliberately minimalist architecture in which all modules are instantiated as $N$-D ConvNeXt blocks \cite{liu2022convnet} and all rate-changing operators are implemented as linear projections. Concretely, the encoder processes the MDCT coefficient grid with an $N$-D ConvNeXt backbone, and then applies a linear downsampling layer to compress the resulting features into low-rate latent tokens, followed by fixed-norm spherical normalization. The decoder starts from clean or perturbed tokens, applies a decoder-side token mixing module implemented by the same ConvNeXt family, maps the representation back to the native coefficient-grid resolution through a linear upsampling layer, and finally refines it with an $N$-D ConvNeXt decoder backbone. This keeps the entire tokenizer highly uniform: encoder aggregation, decoder refinement, and decoder-side token reconciliation are all built from the same basic block, with only dimensionality and optionally causality constraints varying across modalities. Moreover, instead of directly regressing reconstructed MDCT coefficients, the decoder output layer predicts two tensors corresponding to a magnitude branch and a sign branch, and combines them as
\begin{equation}
\widehat{\mathrm{coef}}
\;=\;
\exp\!\big(h_{\mathrm{mag}}\big)\cdot \tanh\!\big(h_{\mathrm{sign}}\big).
\label{eq:coef_param}
\end{equation}
Here $h_{\mathrm{mag}}$ controls a nonnegative amplitude term and $h_{\mathrm{sign}}$ controls a bounded signed factor. The estimated coefficients $\widehat{\mathrm{coef}}$ are then passed through the inverse separable $N$-D MDCT to reconstruct the signal in the original domain.

\subsection{Discussion: Connecting Standard VAEs with Spherical Tokens}
\label{sec:disc_vae_coverage}

\subsubsection{Thin-Shell Concentration of High-Dimensional Gaussians}
\label{sec:analysis_thin_shell}
Let $x\in\mathbb{R}^N$ be a Gaussian vector
\begin{equation}
x \sim \mathcal{N}(0,\sigma^2 I_N).
\end{equation}
Then
\begin{equation}
\frac{\|x\|_2^2}{\sigma^2}=\sum_{i=1}^N \left(\frac{x_i}{\sigma}\right)^2 \sim \chi^2_N,
\end{equation}
so
\begin{equation}
\mathbb{E}\big[\|x\|_2^2\big]=N\sigma^2,
\quad
\mathrm{Var}\big(\|x\|_2^2\big)=2N\sigma^4.
\label{eq:chi2_moments_subsec}
\end{equation}
In particular, the relative standard deviation of $\|x\|_2^2$ scales as $\sqrt{2/N}$ and vanishes as $N\to\infty$. Thus, in high dimensions, a Gaussian distribution places almost all its mass on a thin spherical shell of radius $\approx \sigma\sqrt{N}$ with relative thickness $O(1/\sqrt{N})$.

\subsubsection{Euclidean VAE Noise Implies Limited Angular Support}
Consider a standard VAE-style tokenizer in a high-dimensional latent space, where the encoder produces a mean vector $z\in\mathbb{R}^N$ and sampling is implemented by the reparameterization trick with a fixed isotropic noise scale,
\begin{equation}
\tilde z = z + \varepsilon,\quad \varepsilon\sim\mathcal N(0,\sigma^2 I_N).
\label{eq:vae_reparam_fixed_sigma}
\end{equation}
Using the thin-shell concentration property, we can relate the strength of $\sigma$ to angular coverage on the sphere. We can fix the token direction $u=z/\|z\|_2$ and write $\|z\|_2=R$ and decompose the noise into components parallel and orthogonal to $u$,
\begin{equation}
\varepsilon = \varepsilon_\parallel u + \varepsilon_\perp,\quad \langle \varepsilon_\perp,u\rangle=0,
\end{equation}
so that
\begin{equation}
\tilde z = (R+\varepsilon_\parallel)u + \varepsilon_\perp.
\end{equation}
The induced rotation angle $\theta=\angle(z,\tilde z)$ satisfies the exact identity
\begin{equation}
\tan\theta = \frac{\|\varepsilon_\perp\|_2}{R+\varepsilon_\parallel}.
\label{eq:tan_theta}
\end{equation}
Since $\varepsilon$ is isotropic, $\varepsilon_\parallel\sim\mathcal N(0,\sigma^2)$ and $\|\varepsilon_\perp\|_2^2/\sigma^2\sim\chi^2_{N-1}$, hence $\|\varepsilon_\perp\|_2\approx \sigma\sqrt{N-1}$ for large $N$ while $\varepsilon_\parallel=O_p(\sigma)$. When the latent norm scales as $R=\Theta(\sqrt{N})$ (as implied by the KL loss in VAE training together with thin-shell concentration property), the denominator in Eq.~\eqref{eq:tan_theta} is dominated by $R$ and we obtain the high-dimensional approximation
\begin{equation}
\theta \approx \arctan\!\left(\frac{\sigma\sqrt{N-1}}{R}\right).
\label{eq:theta_typical}
\end{equation}
In particular, under the common normalization $R\approx \sqrt{N}$, the typical angular perturbation becomes approximately
\begin{equation}
\theta \approx \arctan(\sigma),
\end{equation}
which is essentially \emph{dimension-independent}. This implies that, for a fixed $\sigma$, the VAE perturbation corresponds to a roughly constant angular radius on the hypersphere even as $N$ grows.

However, the \emph{relative} coverage of a fixed angular neighborhood shrinks rapidly with dimension. Let $X$ be uniformly distributed on the unit sphere $\mathbb{S}^{N-1}(1)$ and let $u$ be a fixed unit vector. The probability mass of a spherical cap of half-angle $\theta$ is
\begin{equation}
F_N(\theta)
=
\mathbb{P}\big(\angle(X,u)\le \theta\big)
=
\mathbb{P}\big(\langle X,u\rangle \ge \cos\theta\big).
\end{equation}
For large $N$, $\langle X,u\rangle \approx \mathcal N(0,1/N)$, hence for any fixed $\theta<\pi/2$ (so $\cos\theta>0$),
\begin{equation}
F_N(\theta)
\approx
1-\Phi\!\big(\sqrt{N}\cos\theta\big),
\end{equation}
which decays super-polynomially (indeed exponentially in $N$) as $N\to\infty$. In other words, a fixed Euclidean noise scale $\sigma$ induces an angular neighborhood whose \emph{absolute} radius is stable, but whose \emph{relative} hyperspherical coverage vanishes in high dimensions. This provides a geometric perspective on why Euclidean Gaussian perturbations can be poorly matched to hyperspherical token spaces at large $N$: the induced angular support occupies an exponentially small fraction of the sphere, so the model is trained on a very thin neighborhood around the data directions. In contrast, our perturbation scheme is specified directly in angular terms on the sphere, with dimension-independent maximum angles in both the high-dimensional and low-dimensional spaces, making the effective neighborhood geometry explicit and directly controllable.

\subsection{A Group-wise Energy Hierarchy for Coarse-to-Fine Token Geometry}
\label{sec:group_energy_hierarchy}

The analysis above suggests that what we truly want to preserve in token space is not a strict frequency-to-dimension correspondence, but rather a \emph{coarse-to-fine geometric hierarchy}: some token subspaces should be more stable under spherical perturbations and become target-dominant earlier along the generative bridge, while other subspaces should behave as progressively finer and more fragile residual channels. This motivates a simpler design than explicit band-wise dimension allocation. Instead of requiring each input subband to compress into a dedicated token block, we let the encoder consume the full MDCT coefficient tensor and only impose a structured \emph{energy hierarchy} on the output token dimensions.

\paragraph{Group partition and fixed group radii.}
Let the token dimensionality be $N$, and partition the token into $G$ groups of equal size
\begin{equation}
H = \frac{N}{G},
\qquad
z = [\,z^{(1)}, z^{(2)}, \dots, z^{(G)}\,],
\qquad
z^{(g)} \in \mathbb{R}^{H}.
\end{equation}
We let the encoder produce a full-dimensional hidden vector
\begin{equation}
h = [\,h^{(1)}, h^{(2)}, \dots, h^{(G)}\,], \qquad h^{(g)} \in \mathbb{R}^{H},
\end{equation}
and normalize each group independently:
\begin{equation}
u^{(g)} = \frac{h^{(g)}}{\|h^{(g)}\|_2+\varepsilon}.
\end{equation}
We then assign a fixed target energy $r_g^2$ to each group and form the final token by
\begin{equation}
z^{(g)} = r_g\,u^{(g)}, 
\qquad
z = [\,z^{(1)},\dots,z^{(G)}\,].
\label{eq:group_energy_token}
\end{equation}
By construction, if the group energies satisfy
\begin{equation}
\sum_{g=1}^{G} r_g^2 = N,
\label{eq:group_energy_sum_constraint}
\end{equation}
then the resulting token already lies on the hypersphere $\|z\|_2=\sqrt{N}$ up to the small numerical effect of $\varepsilon$, so no further global normalization is needed.

\paragraph{Why energy hierarchy instead of explicit band allocation?}
A strict band-to-band compression scheme becomes impractical when the transform has many frequency bins. For example, with a large 1D MDCT kernel, each frequency band may receive only a very small number of token dimensions under a fixed total token budget, making faithful reconstruction difficult. More importantly, in separable $N$-D MDCT, grouping neighboring coefficients into larger hand-crafted frequency bands is no longer well grounded physically. Our goal is therefore weaker and more practical: we do not require token dimensions to correspond exactly to transform coefficients; rather, we require token subspaces to exhibit a stable \emph{importance ordering} that the encoder can exploit automatically.

\paragraph{Energy hierarchy from a geometric progression.}
We choose the group energies as a geometric progression
\begin{equation}
r_g^2 = A q^{g-1}, \qquad g=1,\dots,G,
\label{eq:rg2_geom}
\end{equation}
where $g=1$ denotes the highest-energy group and $g=G$ the lowest-energy group. This makes the energy profile linear on the dB scale:
\begin{equation}
10\log_{10} r_g^2
=
10\log_{10} A
+
10(g-1)\log_{10} q.
\end{equation}
To remove any extra shape hyperparameter, we use a simple closed-form rule:
\begin{equation}
\frac{r_1}{r_G} = G.
\label{eq:energy_ratio_G}
\end{equation}
Since $r_1^2/r_G^2 = q^{-(G-1)}$, Eq.~\eqref{eq:energy_ratio_G} gives
\begin{equation}
q = G^{-2/(G-1)}.
\label{eq:q_from_G}
\end{equation}
Applying the total-energy constraint \eqref{eq:group_energy_sum_constraint},
\begin{equation}
\sum_{g=1}^{G} r_g^2
=
A\sum_{g=0}^{G-1} q^g
=
A\frac{1-q^G}{1-q}
=
N,
\end{equation}
yields the closed-form normalization constant
\begin{equation}
A = N\,\frac{1-q}{1-q^G}.
\label{eq:A_closed_form}
\end{equation}
Substituting Eq.~\eqref{eq:q_from_G} into Eq.~\eqref{eq:A_closed_form}, the final group energy schedule becomes
\begin{equation}
\boxed{
r_g^2
=
N\,\frac{1-q}{1-q^G}\,q^{g-1},
\qquad
q = G^{-2/(G-1)}.
}
\label{eq:rg2_final}
\end{equation}
This design has several desirable properties. First, it is fully closed-form and depends only on the number of groups $G$. Second, the total dynamic range is
\begin{equation}
10\log_{10}\frac{r_1^2}{r_G^2}
=
20\log_{10} G \;\text{dB},
\end{equation}
so the hierarchy becomes broader as more groups are used, but only logarithmically, avoiding overly aggressive decay. Third, when $G=1$ or, more generally, in the limiting case $q\to 1$, Eq.~\eqref{eq:rg2_final} reduces to the uniform-energy baseline $r_g^2=H$. Fourth, it assigns the norm of $r_1$ to $G$ times $r_G$, which linearly scales with $G$.

\paragraph{Local effect under a global spherical perturbation.}
Consider the standard spherical perturbation used in our tokenizer training,
\begin{equation}
\tilde z = \cos\theta\, z + \sqrt{N}\sin\theta\,u,
\qquad
u \perp z,\ \|u\|_2=1,
\end{equation}
and in particular the reference maximum angle $\theta=45^\circ$. Since each group has dimension $H$, the perturbation energy carried by group $g$ is approximately $\sqrt{H}\sin\theta$ in the high-dimensional regime, while the clean group norm is $r_g$. Therefore, the local effective perturbation angle inside group $g$ satisfies
\begin{equation}
\tan\phi_g
\approx
\frac{\sqrt{H}}{r_g}\tan\theta.
\end{equation}
Under $\theta=45^\circ$, this simplifies to
\begin{equation}
\tan\phi_g \approx \frac{\sqrt{H}}{r_g}.
\label{eq:phi_g_45}
\end{equation}
Thus, higher-energy groups experience smaller local rotation angles and are more stable under the same global perturbation, while lower-energy groups behave as finer and more fragile residual channels. Importantly, the \emph{global} perturbation angle remains exactly $45^\circ$; the hierarchy only changes the \emph{local} effective perturbation geometry seen by different token groups.

\paragraph{Implication for rectified-flow bridges.}
The same hierarchy also induces a coarse-to-fine progression under the standard rectified-flow bridge
\begin{equation}
x_t = (1-t)x_0 + tx_1,
\qquad
x_0 \sim \mathcal N(0,I_N),
\end{equation}
when analyzed group-wise. Since the source contributes expected group energy
\begin{equation}
\mathbb E\|x_0^{(g)}\|_2^2 = H,
\end{equation}
while the target contributes
\begin{equation}
\|x_1^{(g)}\|_2^2 = r_g^2,
\end{equation}
the expected group-wise signal-to-noise ratio is
\begin{equation}
\mathrm{SNR}_g(t)
=
\frac{t^2 r_g^2}{(1-t)^2 H},
\label{eq:group_snr}
\end{equation}
or equivalently
\begin{equation}
\log \mathrm{SNR}_g(t)
=
2\log\frac{t}{1-t}
+
\log\frac{r_g^2}{H}.
\label{eq:group_logsnr}
\end{equation}
Hence all groups share the same temporal slope, but their trajectories are vertically shifted by $\log(r_g^2/H)$. Higher-energy groups become target-dominant earlier in time, while lower-energy groups remain source-dominant longer. In this sense, the proposed energy hierarchy not only regularizes the tokenizer geometry, but also directly shapes the \emph{coarse-to-fine prediction order} induced by the generative bridge.
